High order geometric methods with splines: an analysis of discrete Hodge--star operators

A new kind of spline geometric method approach is presented. Its main ingredient is the use of well established spline spaces forming a discrete de Rham complex to construct a primal sequence $\{X^k_h\}^n_{k=0}$, starting from splines of degree $p$, and a dual sequence $\{\tilde{X}^k_h\}_{k=0}^n$, starting from splines of degree $p-1$. By imposing homogeneous boundary conditions to the spaces of the primal sequence, the two sequences can be isomorphically mapped into one another. Within this setup, many familiar second order partial differential equations can be finally accommodated by explicitly constructing appropriate discrete versions of constitutive relations, called Hodge--star operators. Several alternatives based on both global and local projection operators between spline spaces will be proposed. The appeal of the approach with respect to similar published methods is twofold: firstly, it exhibits high order convergence. Secondly, it does not rely on the geometric realization of any (topologically) dual mesh. Several numerical examples in various space dimensions will be employed to validate the central ideas of the proposed approach and compare its features with the standard Galerkin approach in Isogeometric Analysis.

==> application.tex <==
In this final section, we apply the hierarchical B-spline complex to the numerical solution of two canonical problems of interest, one stemming from electromagnetics and the other from creeping flow.  For both problems, we examine the convergence properties of the hierarchical B-spline complex and its suitability for adaptive methods, and we further examine the accuracy gains hierarchical B-splines provide as compared with uniform B-splines.

\subsection{Application to Electromagnetics: The Curved L-shaped Domain}
As a first test problem, we solve the Maxwell eigenvalue problem, given in variational form by \eqref{eq:maxwell}, over the curved L-shaped domain.  This is a challenging problem as the first few eigenfunctions exhibit a strong singularity at the reentrant corner.  The problem details are adopted from Monique Dauge's webpage of benchmark computations for Maxwell equations \cite{BMAX}. The domain, shown in Figure~\ref{fig:curvedL}, is represented by three patches, and for the computations we start with a zero level mesh of $8\times 8$ element on each patch. Then, at each refinement step we refine on each patch one quarter of the (parametric) domain near the reentrant corner, to obtain a better approximation of the singularity. The meshes obtained with this refinement procedure, as the one represented in Figure~\ref{fig:curvedL} for six levels, satisfy both Assumptions~\ref{ass:support} and~\ref{ass:overlap}.

\begin{figure}[b!]
\begin{subfigure}[Mesh with six levels]
{\includegraphics[width=0.4\textwidth,trim=3cm 2.5cm 2cm 1.8cm, clip]{curved_Lshaped_mesh_6levels} \label{fig:curvedL}}
\end{subfigure}
\begin{subfigure}[Convergence of the first eigenvalue]
{\includegraphics[width=0.58\textwidth,trim=4cm 1cm 4cm 1cm, clip]{curvedL_errors} \label{fig:curvedL-results} }
% \includegraphics[width=0.48\textwidth,trim=5cm 2cm 4cm 1cm, clip]{curvedL_errors_radical}
\end{subfigure}
\caption{Curved L-shaped domain: Hierarchical B\'{e}zier mesh and convergence results.} 
\end{figure}

\begin{table}[b!]
\caption{Comparison of the first five computed eigenvalues of the curved L-shaped domain, for uniform tensor-product B-splines and hierarchical B-splines.} \label{tab:curvedL}
\centering
\begin{tabular}{|c||c|c|c|c|}
\hline
 & \multicolumn{2}{|c|}{$p_1 = p_2 = 3$} & \multicolumn{2}{|c|}{$p_1 = p_2 = 4$} \\
\cline{2-5}
Exact & Uniform & HB-splines & Uniform & HB-splines \\
\hline
1.818571152 & 1.818555761 & 1.818555754 & 1.818561623 & 1.818561620 \\
3.490576233 & 3.490576123 & 3.490576132 & 3.490576165 & 3.490576165 \\
10.06560150 & 10.06560150 & 10.06560272 & 10.06560150 & 10.06560150 \\
10.11188623 & 10.11188494 & 10.11188615 & 10.11188543 & 10.11188544 \\
12.43553725 & 12.43550823 & 12.43550992 & 12.43551928 & 12.43551928 \\
\hline
d.o.f. & 400416 & 2040 & 403522 & 2170 \\
\hline
\end{tabular}
\end{table}

We compare in Figure~\ref{fig:curvedL-results} the convergence results for the approximation of the first eigenvalue using hierarchical B-splines and tensor-product B-splines with uniform refinement, for degrees three and four. The associated eigenfunction only belongs to $H^{2/3-\epsilon}$ for any $\epsilon > 0$, which determines the convergence rate in the case of uniform B-splines. The results show much better approximation results for hierarchical B-splines, although the asymptotic regime is not reached after ten refinement steps. We also present, in Table~\ref{tab:curvedL}, the first five computed eigenvalues for the mesh of level six, and a comparison with the exact\footnote{The eigenvalues are taken from \cite{BMAX} and are correct up to 11 digits.} eigenvalues. The results are almost identical, but hierarchical B-splines require 200 times fewer degrees of freedom to obtain the same accuracy.

\begin{remark}
The results for tensor-product B-splines can be improved by generating a radical graded mesh, see \cite{Beirao_Cho_Sangalli} and \cite[Section~6]{BBSV-acta}. However, in this case the condition number strongly deteriorates due to the presence of anisotropic elements.
\end{remark}


\subsection{Application to Creeping Flow: Lid-Driven Cavity Flow}
As a second test problem, we solve the creeping lid-driven cavity flow problem.  Creeping flow is governed by the Stokes equations, given in variational form by \eqref{eq:stokes}, and the setup for the lid-driven cavity flow problem is elaborated in Figure \ref{f:lidcavitysetup}.  The left, right, and bottom sides of the cavity are fixed no-slip walls while the top side of the cavity is a wall which slides to the right with velocity magnitude $U$.  For the computations here, $H$ and $U$ are set to one.  Like the curved L-shaped domain problem described previously, the pressure and stress fields associated with the lid-driven cavity flow problem experience corner singularities which impede the convergence of numerical methods and expose unstable velocity/pressure pairs.  The velocity field is further characterized by a primary vortex near the center of the cavity and an infinite sequence of Moffatt eddies of decreasing size and intensity in the lower left and right corners of the cavity.  We demonstrate here that a discretization based on the hierarchical B-spline complex is able to both resolve the corner singularities as well as a select number of Moffatt eddies with a properly chosen adaptive strategy.

\begin{figure}[b!]
	\centering
	\includegraphics[height=3.25in]{Figures/Stokes_Cavity_Setup.pdf}
	\caption{Problem setup for creeping lid-driven cavity flow.}
	\label{f:lidcavitysetup}
\end{figure}

We have computed approximations of lid-driven cavity flow using both hierarchical B-splines and tensor-product B-splines with varying mesh size and polynomial degrees two, three, and four.  For the case of tensor-product B-splines, we employed uniform refinement to resolve the features of the flow.  The computed streamlines for $h = 1/32$ and $h = 1/128$ with $p_1 = p_2 = 2$ are shown in Figure~\ref{f:tensorprodstreamlines}. Note that while the first Moffatt eddy is apparent in the $h = 1/32$ mesh, it is highly distorted.  The second Moffatt eddy does appear in the $h = 1/128$ mesh, but the third cannot be calculated using tensor-product B-splines until a mesh resolution of $h = 1/1024$.  For the case of hierarchical B-splines, we began with a uniform tensor-product B-spline mesh and applied three levels of hierarchical refinement in each of the corners of the domain as illustrated in Figure~\ref{f:lidcavityhierarchicalmesh}.  The computed streamlines for $h = 1/32$ and $h = 1/128$ with $p_1 = p_2 = 2$ are shown in Figure~\ref{f:hierarchicalstreamlines}, where $h$ indicates the element size for the initial tensor-product B-spline mesh and hence is the maximal element size for the hierarchical mesh.  Note that both the first and second Moffatt eddies are well-resolved for the $h = 1/32$ mesh, and the third Moffatt eddy can also be observed for the $h = 1/128$ mesh.  Consequently, while 3,153,925 degrees of freedom are necessary to capture the third Moffatt eddy with uniform tensor-product B-splines, one can capture the eddy with hierarchical B-splines using only $93,381$ degrees of freedom.  This is more than a thirty-fold reduction in total number of degrees of freedom.  It should be noted that the fourth Moffatt eddy cannot be obtained with double precision floating point arithmetic as the magnitudes of the velocities of the eddies are simply too small (below $1e{-12}$).

\begin{figure}[t]
	\centering
	\includegraphics[height=2.75in]{stokes_lid_driven/Lid_Driven_3_Level_Refine_Corners_Elem32.png}
	\caption{Hierarchical refinement strategy for the creeping lid-driven cavity flow problem.  The displayed hierarchical B\'{e}ziermesh corresponds to $h = 1/32$ where $h$ is the element size for the initial tensor-product B-spline mesh.}
	\label{f:lidcavityhierarchicalmesh}
\end{figure}

%
% Figure of stream functions for tensor product mesh of lid-driven cavity flow for k' = 1
\begin{figure}[t]
	\centering

	\subfigure[{$[0,1] \times [0,1]$, $h = 1/32$}]{\includegraphics[height=2.3in]{stokes_lid_driven/Lid_Driven_Streamlines_p2_elem32_tensorprod.png}\label{f:tensorprodstreamlinesh32}}
	\qquad
	\subfigure[{$[0,0.0073] \times [0,0.0073]$, $h = 1/32$}]{\includegraphics[height=2.3in]{stokes_lid_driven/Lid_Driven_Streamlines_p2_elem32_tensorprod_Zoom.png}\label{f:tensorprodstreamlinesh32zoom}}
	
	\subfigure[{$[0,1] \times [0,1]$, $h = 1/128$}]{\includegraphics[height=2.3in]{stokes_lid_driven/Lid_Driven_Streamlines_p2_elem128_tensorprod.png}\label{f:tensorprodstreamlinesh128}}
	\qquad
	\subfigure[{$[0,0.0073] \times [0,0.0073]$, $h = 1/128$}]{\includegraphics[height=2.3in]{stokes_lid_driven/Lid_Driven_Streamlines_p2_elem128_tensorprod_Zoom.png}\label{f:tensorprodstreamlinesh128zoom}}

	\caption{Streamlines for the creeping lid-driven cavity problem obtained from tensor-product B-splines with $p_1 = p_2 = 2$. The first Moffatt eddies can be seen in the corners of the domain, while a second Moffatt eddy is shown by zooming in to the lower-left corner of the domain.}
	\label{f:tensorprodstreamlines}
\end{figure}

%
% Figure of stream functions for hierarchical mesh of lid-driven cavity flow for k' = 1
\begin{figure}[t]
	\centering

	\subfigure[{$[0,1] \times [0,1]$, $h = 1/32$}]{\includegraphics[height=2.3in]{stokes_lid_driven/Lid_Driven_Streamlines_p2_elem32_locref3.png}\label{f:hierarchicalstreamlinesh32}}
	\qquad
	\subfigure[{$[0,0.0073] \times [0,0.0073]$, $h = 1/32$}]{\includegraphics[height=2.3in]{stokes_lid_driven/Lid_Driven_Streamlines_p2_elem32_locref3_Zoom.png}\label{f:hierarchicalstreamlinesh32zoom}}
	
	\subfigure[{$[0,1] \times [0,1]$, $h = 1/128$}]{\includegraphics[height=2.3in]{stokes_lid_driven/Lid_Driven_Streamlines_p2_elem128_locref3.png}\label{f:hierarchicalstreamlinesh128}}
	\qquad
	\subfigure[{$[0,0.0073] \times [0,0.0073]$, $h = 1/128$}]{\includegraphics[height=2.3in]{stokes_lid_driven/Lid_Driven_Streamlines_p2_elem128_locref3_Zoom.png}\label{f:hierarchicalstreamlinesh128zoom}}

	\caption{Streamlines for the creeping lid-driven cavity problem obtained from thrice-refined hierarchical B-splines with $p_1 = p_2 = 2$ (see Figure~\ref{f:lidcavityhierarchicalmesh}). The first Moffatt eddies can be seen in the corners of the domain, while a second and a third Moffatt eddy are shown by zooming in to the lower-left corner of the domain.}
	\label{f:hierarchicalstreamlines}
\end{figure}

To examine how well hierarchical B-splines and tensor-product B-splines resolve the corner singularities in the lid-driven cavity flow problem, we also compared the vorticity solution $(\omega = \textnormal{curl} \hspace{3pt} \mathbf{u}_{h})$ obtained by these approaches near the upper right corner of the cavity with the highly accurate pseudospectral results obtained in \cite{BoPe98}.  The results of this study are shown in Table~\ref{t:StokesLidDriven}.  From these results, it is apparent that hierarchical B-splines are much more effective in capturing the corner singularities than tensor-product B-splines.  For example, when $h = 1/256$ and $p_1 = p_2 = 4$, the hierarchical B-spline results match the pseudospectral results up to six significant digits.  This is particularly impressive when taking into consideration that the pseudospectral results were obtained using a subtraction of the leading terms of the asymptotic solution of the Stokes equations in order to exactly represent the corner singularities.


%
% Table of Lid-driven cavity flow
\begin{table}
\caption{Vorticity values at the point $\mathbf{x} = (0,0.95)$ and computational expense associated with tensor-product B-splines and hierarchical B-splines as applied to the creeping lid-driven cavity flow problem.}\label{t:StokesLidDriven}
\centering
Polynomial Degree $p_1 = p_2 = 2$ \\
\begin{tabular}{ l c c c}
\hline
Method  & $\omega$ & No. Elements & No. Unknowns \\
\hline
Tensor product B-splines, $h = 1/32$	 & 18.07580 & 1,024	 & 3,333 \\
Tensor product B-splines, $h = 1/64$ 	 & 19.18682 & 4,096	 & 12,805\\
Tensor product B-splines, $h = 1/128$ & 23.47947 & 16,384 & 50,181\\
Tensor product B-splines, $h = 1/256$ & 25.42558 & 65,536 & 198,661\\
\hline
Hierarchical B-splines, $h = 1/32$ 	& 23.59458 & 1,924 	& 6,033 \\
Hierarchical B-splines, $h = 1/64$ 	& 25.47702 & 7,696 	& 23,605 \\
Hierarchical B-splines, $h = 1/128$ 	& 26.38816 & 30,784 & 93,381 \\
Hierarchical B-splines, $h = 1/256$ 	& 26.83601 & 123,136 & 371,461 \\
\hline
Pseudospectral (Ref. \cite{BoPe98}) & 27.27901 & --- & --- \\
\hline
\end{tabular}

\vspace{12pt}
Polynomial Degree $p_1 = p_2 = 3$ \\
\begin{tabular}{ l c c c}
\hline
Method  & $\omega$ & No. Elements & No. Unknowns \\
\hline
Tensor product B-splines, $h = 1/32$	 & 33.27731 & 1,024	 & 3,536 \\
Tensor product B-splines, $h = 1/64$ 	 & 35.01708 & 4,096	 & 13,200 \\
Tensor product B-splines, $h = 1/128$ & 25.84879 & 16,384 & 50,960 \\
Tensor product B-splines, $h = 1/256$ & 27.34235 & 65,536 & 200,208\\
\hline
Hierarchical B-splines, $h = 1/32$ 	& 27.54476 & 1,924 	& 6,236 \\
Hierarchical B-splines, $h = 1/64$ 	& 27.33604 & 7,696 	& 24,000\\
Hierarchical B-splines, $h = 1/128$ 	& 27.29035 & 30,784 & 94,160\\
Hierarchical B-splines, $h = 1/256$ 	& 27.28284 & 123,136 & 373,008\\
\hline
Pseudospectral (Ref. \cite{BoPe98}) & 27.27901 & --- & --- \\
\hline
\end{tabular}

\vspace{12pt}
Polynomial Degree $p_1 = p_2 = 4$ \\
\begin{tabular}{ l c c c}
\hline
Method  & $\omega$ & No. Elements & No. Unknowns \\
\hline
Tensor product B-splines, $h = 1/32$	 & 22.52289 & 1,024	 & 3,745 \\
Tensor product B-splines, $h = 1/64$ 	 & 30.29182 & 4,096	 & 13,601 \\
Tensor product B-splines, $h = 1/128$ & 29.32455 & 16,384 & 51,745 \\
Tensor product B-splines, $h = 1/256$ & 27.64269 & 65,536 & 201,761 \\
\hline
Hierarchical B-splines, $h = 1/32$ 	& 27.25594 & 1,924 	& 6,445\\
Hierarchical B-splines, $h = 1/64$ 	& 27.28393 & 7,696 	& 24,401\\
Hierarchical B-splines, $h = 1/128$ 	& 27.27935 & 30,784 & 94,945\\
Hierarchical B-splines, $h = 1/256$ 	& 27.27905 & 123,136 & 374,561\\
\hline
Pseudospectral (Ref. \cite{BoPe98}) & 27.27901 & --- & --- \\
\hline
\end{tabular}

\end{table}


==> exactness.tex <==
In this section, we begin the analysis of the hierarchical B-spline complex, and in particular, we study under which conditions the complex is exact. For our analysis, we make use of some powerful tools from abstract cohomology theory that we present at the beginning of the section. These results are then applied to the particular case of the hierarchical B-spline complex, from which we obtain a sufficient and necessary condition for exactness, given in Theorem~\ref{th:exact}. Since the proof is based on abstract cohomology theory, the condition we obtain is valid in a very general setting: it is dimension independent and can be also applied to other hierarchical spaces constructed with the algorithm in Definition~\ref{def:hierarchical}, including hierarchical T-splines \cite{Evans15}. We also give an interpretation of the derived condition based on Greville subgrids. 

The drawback of the aforementioned condition is that is not easily computable. For this reason, we introduce a local condition related to the support of the basis functions on the hierarchical B\'ezier mesh which is local and easier to implement. The last part of this section is devoted to proving this is a sufficient condition for exactness for the two-dimensional case. Some of the proofs in this section are rather technical, hence we will relegate the details to the appendix.

% In this section we start the analysis of the hierarchical spline complex, and in particular develop a condition for the exactness, with a proof based on abstract cohomology theory. We begin the section presenting the necessary results in cohomology, and then apply them to the particular case of the hierarchical spline complex. Coming from an abstract theory, the condition we obtain is valid in a very general setting. Indeed, the result works for the construction of a hierarchical spline complex in any dimension, and it can also be applied to other hierarchical spaces constructed with the algorithm in Definition~\ref{def:hierarchical}, such as hierarchical T-splines \cite{Evans15}. In the last part of the section we show that the local condition presented in Section~\ref{} {\Rd FIX} is a sufficient condition for exactness. Some of the proofs in this section are rather technical, hence we will relegate the details to the appendix.

\subsection{Background Results from Cohomology Theory}\label{sec:homology}
%% To present the abstract setting of cohomology we mainly follow \cite[Section~3]{AFW-2}. We define a Hilbert complex $(V,d)$ as a sequence of Hilbert spaces $V^i$, which are the domain of definition of the linear maps $d^i$
%% \begin{equation} \label{eq:sequence}
%% \begin{CD}
%% 0 @>>> V^0 @>d^0>> V^1 @>d^1>> V^2 @>d^2>> \ldots @>d^{n-1}>> V^n @>>> 0,
%% \end{CD}
%% \end{equation}
%% with $d^i \circ d^{i-1} = 0$. The elements of the kernel of $d^i$ are called closed forms, and denoted by $Z^i(V) \equiv Z^i(V,d)$. %:= \{u^i \in V^i : d^i u^i = 0 \}$. 
%% The elements of the range of $d^{i-1}$ are called exact forms, and denoted by $B^i(V) \equiv B^i(V,d)$. % := \{ u^i \in V^i : u^i = d^{i-1} u^{i-1}, u^{i-1} \in V^{i-1} \}$. 
%% The $i$th {\bf \emph{cohomology group}} is given by the quotient space $H^i(V) \equiv H^i(V,d) = Z^i(V) / B^i(V)$. When the cohomology groups are all trivial, we say that the sequence is {\bf \emph{exact}}.

%% We say that $(V_h,d)$ is a {\bf \emph{subcomplex}} of $(V,d)$ if $V_h^k \subset V^k$, and $d^k(V_h^k) \subset V_h^{k+1}$. We notice that what we have denoted Hilbert complex is called the domain subcomplex in \cite{AFW-2}, {\Rd but for the theory developed in this paper we don't need the missing ``supercomplex''}. We will make use of the following result about subcomplexes.

\begin{lemma}\label{lemma:cupcap_derham}
Let $(V_h,d)$ and $(W_h,d)$ be two subcomplexes of $(V,d)$. Then $(V_h \cap W_h,d)$ and $(V_h + W_h, d)$ are also subcomplexes.
\end{lemma}
\begin{proof}
The result is trivial, since $V^k_h \cap W^k_h \subset V^k$ and $V^k_h + W^k_h \subset V^k$, and moreover we also have $d^k(V_h^k \cap W_h^k) \subset V_h^{k+1} \cap W_h^{k+1}$ and $d^k(V_h^k + W_h^k) \subset V_h^{k+1} + W_h^{k+1}$.
\end{proof}

Let $(V,d_V)$ and $(W,d_W)$ be two Hilbert complexes, and let $f^k : V^k \rightarrow W^k$ be a set of linear maps satisfying $d_W^k f^k = f^{k+1} d_V^k$. Following \cite{AFW-2} we call this a cochain map, and we denote by $f^*$ its induced map in the cohomology groups. The map induced in cohomology by a composition of cochain maps takes the form $(f \circ g)^* = f^* \circ g^*$. Given a Hilbert complex $(V,d)$ and any subcomplex $(V_h,d)$, the inclusion map $j:V_h \rightarrow V$ is a cochain map which induces a map between the cohomology spaces, $j^* : H^k(V_h) \longrightarrow H^k(V)$.

\begin{lemma}\label{lemma:MV}
Let $(V_h, tion*}
\begin{CD}
\ldots \rightarrow H^k(V_h \cap W_h) @>\varphi^*>> H^k(V_h) \oplus H^k(W_h)  @>\psi^*>> H^k(V_h + W_h) @>d^*>> H^{k+1}(V_h \cap W_h) \rightarrow \ldots
\end{CD}
\end{equation*}
\end{lemma}
\begin{proof}
From Lemma~\ref{lemma:cupcap_derham}, both $(V_h \cap W_h,d)$ and $(V_h + W_h,d)$ are subcomplexes. We define the inclusion maps $i_{V_h}$ and $i_{W_h}$ from $V_h \cap W_h$ into $V_h$ and $W_h$, respectively, and also the inclusion maps $j_{V_h}$ and $j_{W_h}$ into $V_h + W_h$, from $V_h$ and $W_h$, respectively. It is trivial to prove that the following sequence is exact
\begin{equation} \label{eq:short}
\begin{CD}
0 @>>> V_h \cap W_h @>\varphi>> V_h \oplus W_h  @>\psi>> V_h + W_h @>>> 0,
\end{CD}
\end{equation}
where $\varphi(u) = (u,u) \equiv (i_{V_h} u, i_{W_h} u)$, and $\psi (v,w) = v-w \equiv j_{V_h}v - j_{W_h}w$. This induces a Mayer-Vietoris sequence of the form (see Chapters~2 and~3 in \cite{Hatcher})
\begin{equation*}
\begin{CD}
\ldots \rightarrow H^k(V_h \cap W_h) @>\varphi^*>> H^k(V_h) \oplus H^k(W_h)  @>\psi^*>> H^k(V_h + W_h) @>d^*>> H^{k+1}(V_h \cap W_h) \rightarrow \ldots
\end{CD}
\end{equation*}
The map $d^*$ is defined in the following way: given a closed form  $u \in Z(V_h + W_h)$, from the exactness of \eqref{eq:short} there exist $v \in V_h$ and $w \in W_h$ such that $u = \psi (v,w) = v-w$, and since it is a closed form $du = dv - dw = 0$. Thus in the cohomology groups we can define $d^*[u] = [dv] = [dw]$, where the brackets represent the equivalence class in the cohomology groups.
\end{proof}

\begin{theorem}\label{th:exactness}
Let $(V_h,d)$ and $(W_h,d)$ be two subcomplexes of the Hilbert complex $(V,d)$. Then the map induced by the inclusion, $i_{W_h}^*: H^k(V_h \cap W_h) \rightarrow H^k(W_h)$, is an isomorphism if and only if $j_{V_h}^*: H^k(V_h) \rightarrow H^k(V_h + W_h)$ is also an isomorphism.
\end{theorem}
\begin{proof}
We will only prove that if $i_{W_h}^*$ is an isomorphism, then $j_{V_h}^*$ is also an isomorphism. The second implication is proved similarly.

If $i_{W_h}^*$ is an isomorphism, then $\varphi^*$ is injective. Thus, the Mayer-Vietoris sequence can be split into the short exact sequences
\begin{equation*}
\begin{CD}
0 @>>> H^k(V_h \cap W_h) @>\varphi^*>> H^k(V_h) \oplus H^k(W_h)  @>\psi^*>> H^k(V_h + W_h) @>>> 0,
\end{CD}
\end{equation*}
which in particular implies that $\psi^*$ is surjective.

To prove that $j_{V_h}^*$ is an isomorphism, first we prove that it is injective. Assume that $v \in V_h$ is such that $j_{V_h}^*[v] = 0$. Then the pair $([v],0) \in \ker \psi^* = {\rm Im} \, \varphi^*$, that is, $\varphi^* [u] = ([v],0)$ for some $u \in V_h \cap W_h$. Since $\varphi^* = (i_{V_h}^*, i_{W_h}^*)$ and $i_{W_h}^*$ is injective, we get $[u] = 0$ and therefore $[v] = i_{V_h}^*[u] = 0$.

To prove the surjectivity of $j_{V_h}^*$ we use that $\psi^*$ is surjective. That is, given $z \in V_h+W_h$ there exist $v \in V_h$ and $w \in W_h$ such that $\psi^*([v],[w]) = j^*_{V_h} [v] - j^*_{W_h} [w] = [z]$. Since $i_{W_h}^*$ is surjective, there exists $u \in V_h \cap W_h$ such that $i_{W_h}^*[u] = [w]$, and by the exactness of the sequence $\varphi^*[u] = (i^*_{V_h}[u], [w]) \in \ker \psi^*$. As a consequence, $\psi^* ([v], [w]) - \psi^* (i^*_{V_h}[u], [w]) = j^*_{V_h}([v] - i^*_{V_h}[u]) = [z]$, which proves that $j_{V_h}^*$ is surjective.
\end{proof}

\begin{corollary}
Let $(V_h,d)$ an exact subcomplex of the Hilbert complex $(V,d)$, and $(W_h,d)$ another subcomplex not necessarily exact. Then the subcomplex $(V_h + W_h, d)$ is exact if and only if $i^*_{W_h} : H^k(V_h \cap W_h) \rightarrow H^k(W_h)$ is an isomorphism.
\end{corollary}

%% \begin{remark}
%% We notice that our Mayer-Vietoris sequence is not ordered like the standard Mayer-Vietoris sequence in cohomology, but rather like the Mayer-Vietoris sequence for cohomology with compact support, see \cite[Lemma~3.36]{Hatcher}.
%% \end{remark}

\subsection{A Necessary and Sufficient Condition for Exactness} \label{sec:nec-suff}
By applying the previous results to hierarchical B-splines, we obtain a necessary and sufficient condition for the exactness of the hierarchical B-spline complex. We first present the result, and then we explain how it can be applied in practice with the help of the Greville subgrids.

\begin{theorem} \label{th:exact}
The hierarchical B-spline complex $(\What_{\ell+1},d)$ is exact for $\ell = 0, \ldots, N-1$ if and only if the inclusion $j: \Xhat^k_{\ell, {\ell+1}} \rightarrow \Xhat^k_{\ell+1, {\ell+1}}$ induces an isomorphism between the cohomology groups $H^k(\Xhat_{\ell, {\ell+1}})$ and $H^k(\Xhat_{\ell+1,{\ell+1}})$ for $k = 1, \ldots, n$.
\end{theorem}
\begin{proof}
We proceed by induction. The exactness of the sequence holds for $\ell =0$ since $\What^k_0 = \hat X^k_{0,h}$ are tensor-product spline spaces, and the exactness of the tensor-product spline sequence~\eqref{eq:spline_complex} is known from \cite{BRSV11}. Assume now that the sequence $(\What_\ell,d)$ is exact. The result is immediately proved for level $\ell+1$ by applying Theorem~\ref{th:exactness} with $V_h^k = \What^k_\ell$ and $W_h^k = \Xhat^k_{\ell+1,{\ell+1}}$, using the relations given in Lemma~\ref{lemma:cupcap}.
\end{proof}

\noindent In simple words, the above condition tells us that, at each step of the recursive algorithm in Definition~\ref{def:hierarchical}, the spaces spanned by the basis functions to be removed and by the basis functions to be added should have the {\bf \emph{same topological properties}}, and these should be preserved by the inclusion operator indicated in Theorem \ref{th:exact}.

\subsubsection{An interpretation of the exactness condition using Greville subgrids}
The condition in Theorem~\ref{th:exact} may not be easy to understand for practitioners, as it requires a basic knowledge of homology theory. We give now an intuitive interpretation of this condition with the help of Greville subgrids. 

As we have seen in Section~\ref{sec:submesh}, there exist isomorphisms that define a commutative diagram between the spline subcomplex $(\Xhat_{\ell,\ell+1},d)$ (respectively, $(\Xhat_{\ell+1,\ell+1},d)$) and the low-order finite element complex $(\hat Z_{\ell,\ell+1},d)$ (resp. $(\hat Z_{\ell+1,\ell+1}, d)$) defined on the Greville subgrid. As a consequence, the topological properties of the spline subcomplex are identical to those of the finite element complex on the Greville subgrid. One can, indeed, consider the Greville subgrids associated to the basis functions to be added and removed and check that they have the same topological properties, that is, the same number of connected components, the same number of holes and, in the three-dimensional case, the same number of cavities.  If the Greville subgrids do not have the same topological properties for every $\ell = 0, \ldots, N-1$, then the condition in Theorem~\ref{th:exact} is not met and the hierarchical B-spline complex is not exact.

\begin{figure}[t]
\includegraphics[width=0.32\textwidth,trim=2cm 1.2cm 2cm 0cm, clip]{refined_1x1}
\includegraphics[width=0.32\textwidth,trim=2cm 1.2cm 2cm 0cm, clip]{remove_1x1}
\includegraphics[width=0.32\textwidth,trim=2cm 1.2cm 2cm 0cm, clip]{add_1x1}
\caption{An example of a maximally continuous hierarchical B-spline complex which is exact for $p_1=p_2=3$. On the left, the hierarchical B\'{e}zier mesh is depicted, with the refined region $\Omega_1$ colored in green. In the center and on the right, the vertices, edges, and faces on the Greville subgrids $\MG_{0,1}$ and $\MG_{1,1}$ are depicted, related to the spaces $\Xhat^k_{0,1}$ and $\Xhat^k_{1,1}$, respectively.}
\label{fig:remove-add-1x1}
\end{figure}

\begin{figure}[t!]
\includegraphics[width=0.32\textwidth,trim=2cm 1.2cm 2cm 0cm, clip]{refined_2x2}
\includegraphics[width=0.32\textwidth,trim=2cm 1.2cm 2cm 0cm, clip]{remove_2x2}
\includegraphics[width=0.32\textwidth,trim=2cm 1.2cm 2cm 0cm, clip]{add_2x2}
\caption{An example of a maximally continuous hierarchical B-spline complex which is not exact for $p_1=p_2=3$. On the left, the hierarchical B\'{e}zier mesh is depicted, with the refined region $\Omega_1$ colored in red. In the center and on the right, the vertices, edges, and faces on the Greville subgrids $\MG_{0,1}$ and $\MG_{1,1}$ are depicted, related to the spaces $\Xhat^k_{0,1}$ and $\Xhat^k_{1,1}$, respectively.}
\label{fig:remove-add-2x2}
\end{figure}

Two examples are shown in Figures~\ref{fig:remove-add-1x1} and~\ref{fig:remove-add-2x2} for maximally continuous bicubic splines. The hierarchical B-spline complex associated to the mesh in Figure~\ref{fig:remove-add-1x1} is exact, because the two Greville subgrids associated to the spaces $\Xhat^k_{0,1}$ and $\Xhat^k_{1,1}$ each consist of two connected components without holes and thus have the same topology. Instead, the hierarchical B-spline complex of the example in Figure~\ref{fig:remove-add-2x2}, which is the same as that presented in Figure~\ref{fig:2x2}, does not provide an exact sequence because the number of connected components for the two Greville subgrids is different and changes from two to one.

%\end{document}
\subsection{A Local and Sufficient Condition for Exactness} \label{sec:local}
Despite its generality, the condition for the exactness provided in Theorem~\ref{th:exact} is not easy to check in practice. In fact, in real three-dimensional applications, the Greville subgrids may become very intricate objects\footnote{For instance, the region to be refined could consist of several (topological) knots with links.}, and computation of the cohomology groups is not a simple task, requiring tools from computational (co)homology. Moreover, the comparison of the cohomology groups must be done through the map induced by the inclusion, because even if the cohomology groups of the two Greville subgrids are isomorphic, it may happen that the map induced by the inclusion is not an isomorphism, which would give a non-exact sequence. Finally, for the development of adaptive methods, the refined region $\Omega_\ell$ is chosen with respect to the B\'ezier mesh, and one would like to obtain a condition in this mesh that guarantees the exactness of the sequence. We will now introduce a \textbf{\emph{local and sufficient}} condition for the exactness of the hierarchical B-spline complex. Apart from being local, the advantage of this condition is that it is easier to check because it is defined directly with respect to the B\'ezier submeshes and not with respect to the Greville subgrids.

From now on, we will restrict ourselves to the two-dimensional case, that is, $n=2$. 
%We recall that we are always working with spaces with homogeneous boundary conditions, but we have removed the zero subindex to simplify the notation. JOHN: This was already mentioned at the beginning of the section.
We start by introducing a mild assumption about the choice of the refined subdomains (see equation (11) in \cite{Vuong_giannelli_juttler_simeon}):
\begin{assumption}\label{ass:support}
The subdomain $\Omega_{\ell+1}$ is given as the union of supports of basis functions in the previous level, that is, for $\ell = 0, \ldots, N-1$
\begin{equation}
\Omega_{\ell+1} = \bigcup_{\beta \in S} \supp (\beta), \text{ with } S \subset {\cal B}^n_\ell.  \label{eq:supports}
\end{equation}
As a consequence, (the closure of) the subdomain $\Omega_{\ell+1}$ is given as (the closure of) the union of elements of level $\ell$.
\end{assumption}
The second assumption is closely related to the one introduced in \cite{Mokris2014}, where the authors prove that hierarchical B-splines span the space of piecewise polynomials in the corresponding hierarchical B\'{e}zier mesh. Let us first define, for each level $\ell = 0, \ldots, N-1$, the \textbf{\emph{open}} complementary region
\begin{equation*}
\Omega_{\ell+1}^c = \Omega_0 \setminus \overline \Omega_{\ell+1}.
\end{equation*}
\begin{assumption}\label{ass:overlap}
For each level $\ell = 0, \ldots, N-1$, and for any basis function $\beta^k \in {\cal B}^k_\ell$ of the tensor-product spaces $\Xhatlh{k}$, with $k = 0, 1, 2$, the overlap 
\begin{equation*}
{\rm overlap} (\beta^k) := \supp (\beta^k) \cap \Omega_{\ell+1}^c
\end{equation*}
is connected and simply connected.
\end{assumption}

\begin{figure}[t!]
\begin{subfigure}[]
{\includegraphics[width=0.3\textwidth,trim=2cm 2cm 2cm 1cm, clip]{mesh_not_assumption1} \label{fig:not-assumption1}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width=0.3\textwidth,trim=2cm 2cm 2cm 1cm, clip]{mesh_not_assumption2} \label{fig:not-assumption2}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width=0.3\textwidth,trim=2cm 2cm 2cm 1cm, clip]{mesh_assumptions_1_2} \label{fig:assumption12}}
\end{subfigure}
\caption{Different hierarchical B\'{e}zier mesh configurations for maximally continuous B-splines and $p_1=p_2=3$. The first mesh does not satisfy Assumption~\ref{ass:support}, nor Assumption~\ref{ass:overlap}, because for the function highlighted with the red square, the overlap (given by the purple colored elements) is not connected. The second mesh does not satisfy Assumption~\ref{ass:overlap}, because the overlap of the highlighted function is also not connected. The third mesh satisfies both Assumptions.}
\label{fig:assumptions-1-2}
\end{figure}

The main result of this section is the following theorem, that for $\ell = N$ gives the exactness of the hierarchical B-spline complex.
\begin{theorem} \label{th:local}
If Assumptions~\ref{ass:support} and~\ref{ass:overlap} hold, then the complex 
\begin{equation}
\begin{CD}
0 @>>> \What^0_{\ell} @>\grad>> \What^1_{\ell} @>\curl>> \What^2_{\ell} @>>> \mathbb{R} @>>> 0
\end{CD}
\end{equation}
is exact, for $\ell = 0, \ldots, N$.
\end{theorem}

The constraints posed by the two assumptions are better understood using the simple examples depicted in Figure~\ref{fig:assumptions-1-2}. For maximally continuous B-splines and $p_1=p_2=3$, the hierarchical B\'{e}zier mesh in Figure~\ref{fig:not-assumption1} violates Assumption~\ref{ass:support}, because the refined region does not contain the support of any basis function of level zero. It also violates Assumption~\ref{ass:overlap}, because there exists one function of level zero, whose support is highlighted in red in the figure, that violates the condition in the assumption. Indeed, the intersection of the support with the non-refined region $\Omega^c_1$, which is represented by the eight purple elements, is not connected. The hierarchical B\'{e}zier mesh in Figure~\ref{fig:not-assumption2} satisfies Assumption~\ref{ass:support}, but it does not satisfy Assumption~\ref{ass:overlap}, because the same function violates the overlap condition in the assumption. Finally, the hierarchical B\'{e}zier mesh in Figure~\ref{fig:assumption12} satisfies both assumptions. More examples are given later in Section~\ref{sec:stability}.

The remainder of this section is devoted to the proof of Theorem~\ref{th:local}. We recall that, as stated in Theorem~\ref{th:exact}, the condition for the exactness is given by the relation between the spaces spanned by the functions to remove, $\Xhat^k_{\ell,\ell+1} = {\rm span} \{ {\cal B}^k_{\ell,\ell+1} \}$, and the functions to add, $\Xhat^k_{\ell+1,\ell+1} = {\rm span} \{ {\cal B}^k_{\ell+1,\ell+1} \}$. We will prove the result with the help of the Greville subgrids corresponding to these spaces, that using the same notation of Section~\ref{sec:submesh} we denote by $\MG_{\ell,\ell+1}$ and $\MG_{\ell+1,\ell+1}$, respectively. With the same abuse of notation in Section~\ref{sec:submesh}, we denote in the same manner the two subdomains covered by the Greville subgrids, that we recall that are different from $\Omega_{\ell+1}$, and also different between them.

The proof follows in three steps. First, we show that the three involved subdomains, that is, the subdomain $\Omega_{\ell+1}$ and the two Greville subgrids, are manifolds with boundary and share the same homological properties. Second, using the relations in Section~\ref{sec:submesh} between spline subspaces and finite element spaces defined in the Greville subgrids, we construct a family of commutative projectors for the subspaces restricted to a subgrid. Finally, joining the above results gives the exactness of the sequence.

\begin{remark}
The analogous condition to Assumption~\ref{ass:overlap} in the three-dimensional setting is that the overlaps are connected, simply connected, and with connected boundary.
\end{remark}
\begin{remark}
In two dimensions, Assumption~\ref{ass:support} implies that the overlaps are simply connected, so this condition could be dropped in Assumption~\ref{ass:overlap}, in this case obtaining exactly the same assumption that is used in \cite{Mokris2014} to characterize hierarchical B-splines in terms of piecewise polynomials. We have preferred to maintain the simply connected condition to make more evident that topology is playing a major role in our construction. The results of this section can actually be proved without using Assumption~\ref{ass:support}, but the proofs become more tedious.
\end{remark}

\subsubsection{First Part of the Proof: Topology of the Grids}

\begin{lemma}\label{lemma:omwb}
If Assumptions~\ref{ass:support} and~\ref{ass:overlap} hold, then the subdomain $\Omega_{\ell+1}$ is a manifold with boundary, for $\ell = 0,\ldots, N-1$.
\end{lemma}
\begin{proof}
In the two-dimensional case, the only configuration for which $\Omega_{\ell+1}$ is not a manifold with boundary is the one in Figure~\ref{fig:not-manifold} (see also Figure~3 in \cite{Berdinsky201486}), in which two connected components of $\Omega_{\ell+1}$ meet in a corner. From Assumption~\ref{ass:support}, every cell in $\Omega_{\ell+1}$ belongs to the support of a basis function as in \eqref{eq:supports}. That is, in the case of maximum continuity, we have a rectangle of size $p_{1,\ell} \times p_{2,\ell}$ elements contained in $\Omega_{\ell+1}$. Therefore, we can obviously choose a basis function in ${\cal B}^0_\ell$ such that its support contains the two white elements of $\Omega^c_{\ell+1}$ in Figure~\ref{fig:not-manifold} and the overlap is not connected, which contradicts Assumption~\ref{ass:overlap}.
\end{proof}

\begin{figure}[t!]
\centerline{\includegraphics[width=0.40\textwidth]{not-manifold}}
\caption{Configuration for which a subdomain is not a manifold with boundary. The colored elements belong to the subdomain, whereas the white elements do not.}\label{fig:not-manifold}
\end{figure}

\begin{lemma} \label{lemma:mwb}
If Assumptions~\ref{ass:support} and~\ref{ass:overlap} hold, then the regions of the Greville subgrids $\MG_{\ell,{\ell+1}}$ and $\MG_{\ell+1,{\ell+1}}$ are manifolds with boundary, for $\ell = 0,\ldots, N-1$.
\end{lemma}
\begin{proof}
Similar to the previous proof, the only configuration for which a Greville subgrid is not a manifold with boundary is the one in Figure~\ref{fig:not-manifold}, where now the elements correspond to the Greville cells. If $\MG_{\ell,{\ell+1}}$ is not a manifold with boundary, i.e., it is as in Figure~\ref{fig:not-manifold}, the support of the basis functions in ${\cal B}^2_\ell$ associated to the colored cells is completely contained in $\Omega_{\ell+1}$, and the support of the basis functions associated to the white cells is not. As a consequence, the overlap of the basis function in ${\cal B}^0_\ell$ corresponding to the middle Greville point is not connected, which contradicts Assumption~\ref{ass:overlap}.

If $\MG_{\ell+1,{\ell+1}}$ is as in Figure~\ref{fig:not-manifold} the support of the basis functions associated to the colored cells, which are now in ${\cal B}^2_{\ell+1}$, is contained in $\Omega_{\ell+1}$, and from Assumption~\ref{ass:support} each one of the cells is contained in a rectangle of $p_{1,\ell} \times p_{2,\ell}$ cells of level $\ell$ contained in $\Omega_{\ell+1}$. Since the support of the basis functions associated to the white cells is not contained in $\Omega_{\ell+1}$, analogously to the proof of Lemma~\ref{lemma:omwb} there exists a function in ${\cal B}^0_\ell$ such that its overlap is not connected, which contradicts Assumption~\ref{ass:overlap}.
\end{proof}


\begin{theorem}\label{th:homology}
If Assumptions~\ref{ass:support} and~\ref{ass:overlap} hold, then the homology groups of $\Omega_{\ell+1}$, $\MG_{\ell,{\ell+1}}$ and $\MG_{\ell+1,{\ell+1}}$ are isomorphic, that is, $H_k(\Omega_{\ell+1}) \cong H_k(\MG_{\ell,\ell+1}) \cong H_k(\MG_{\ell+1,\ell+1})$ for $k = 0, 1, 2$.
\end{theorem}
\begin{proof}
The proof of this result is presented in Appendix~\ref{sec:appendix}.
\end{proof}

\begin{corollary} \label{corol:cohomology}
If Assumptions~\ref{ass:support} and~\ref{ass:overlap} hold, then $H^k(\Xhat_{\ell,\ell+1}) \cong H^k(\Xhat_{\ell+1,\ell+1})$, for $k = 0,1,2$.
\end{corollary}
\begin{proof}
Using the definitions from Section~\ref{sec:submesh}, the spline subspaces $\Xhat_{\ell,{\ell+1}}$ and $\Xhat_{\ell+1,{\ell+1}}$ are isomorphic to the finite element spaces (with boundary conditions) defined on the Greville subgrids $\MG_{\ell,\ell+1}$ and $\MG_{\ell+1,\ell+1}$, respectively, and that we denote by $\hat Z_{\ell,\ell+1}$ and $\hat Z_{\ell+1,\ell+1}$. As it is known, the cohomology groups of finite element spaces with homogeneous boundary conditions are isomorphic to the relative cohomology groups of the domain, where the boundary plays the role of the subspace in relative cohomology. We do not need any details here, and refer the interested reader to \cite[Chapter~3]{Hatcher} for a deeper understanding of relative cohomology, and to \cite{GK} for its use in finite elements. In our case, the cohomology groups of the finite element spaces are isomorphic to the relative cohomology groups of the subdomains $\MG_{\ell,{\ell+1}}$ and $\MG_{\ell+1,{\ell+1}}$. From Lemma~\ref{lemma:mwb} they are both manifolds with boundary, and we can use the classical Lefschetz duality theorem (see \cite[Theorem~3.43]{Hatcher}), to obtain
\begin{equation*}
H^k(\Xhat_{\ell,{\ell+1}}) \cong H^k(\hat Z_{\ell,{\ell+1}})
\cong H^{k}(\MG_{\ell,\ell+1},\partial \MG_{\ell,\ell+1})
\cong H_{n-k} (\MG_{\ell,\ell+1}),
\end{equation*}
and
\begin{equation*}
H^k(\Xhat_{{\ell+1},{\ell+1}}) \cong H^k(\hat Z_{\ell+1,{\ell+1}})
\cong H^{k}(\MG_{\ell+1,\ell+1},\partial \MG_{\ell+1,\ell+1})
\cong H_{n-k} (\MG_{\ell+1,\ell+1}),
\end{equation*}
where $H^k(A,B)$ denotes relative cohomology groups. Moreover, from Theorem~\ref{th:homology} we have
\begin{equation*}
H_{n-k} (\MG_{\ell,{\ell+1}}) \cong H_{n-k} (\MG_{\ell+1,{\ell+1}}) \cong H_{n-k}(\Omega_{\ell+1}),
\end{equation*}
which implies that $H^k(\Xhat_{\ell,{\ell+1}}) \cong H^k(\Xhat_{\ell+1,{\ell+1}})$, that is, the cohomology groups are isomorphic.
\end{proof}

\subsubsection{Second Part of the Proof: Commutative Projectors}

The second step is to prove that the inclusion induces an isomorphism, as required by Theorem~\ref{th:exact}. In order to do so, we will construct a set of commutative projectors for the spline spaces, using the relation between the spline spaces $\Xhat^k_{\ell,\ell+1}$ and the low-order finite element spaces $\hat Z^k_{\ell,\ell+1}$. Before defining the projectors, we have to construct a set of generators of the cohomology groups for the finite element and the spline spaces. We explain the construction for $\hat Z_{\ell,\ell+1}$, since the construction for $\hat Z_{\ell+1,\ell+1}$ is completely analogous.

We recall that the dimension of $H^2(\hat Z_{\ell,\ell+1})$ is the number of connected components of $\MG_{\ell,\ell+1}$ minus one, that we denote by $\nc-1$. To build a generating set of $H^2(\hat Z_{\ell,\ell+1})$ we choose on each connected component (except one) of $\MG_{\ell,\ell+1}$ one Greville cell, and the associated piecewise constant basis function $z^2_j$, for $j=1, \ldots, \nc - 1$. The generating set of $H^2(\hat Z_{\ell+1,\ell+1})$ is built in an analogous way.

The dimension of $H^1(\hat Z_{\ell,\ell+1})$ is equal to the number of ``holes'' of $\MG_{\ell,\ell+1}$, $\nh$, that in the case of a planar manifold with boundary is the number of connected components of the boundary $\partial \MG_{\ell,\ell+1}$ minus the number of connected components of $\MG_{\ell,\ell+1}$. To construct a generating set of the cohomology group we first choose a reference boundary on each connected component of $\MG_{\ell,\ell+1}$, and then we pick the remaining connected components of the boundary in such a way that we have a set of boundaries $\Gamma^\MG_j$, for $j = 1, \ldots, \nh$. For each index $j$ we consider the nodal finite element function with degrees of freedom equal to one on $\Gamma^\MG_j$ and zero elsewhere, and then take the function ${\bf z}^1_j$ as its gradient, see Figure~\ref{fig:harmonic} for a graphical explanation. For a discussion on the construction of a basis of harmonic forms see Section~1.4 and Appendix~A.4 in \cite{AV-book}, and references therein.

The generators of the cohomology groups for spline spaces $H^k(\Xhat_{\ell,\ell+1})$ are constructed from the finite element ones, applying the isomorphisms \eqref{eq:cd-iga-fem}, and will be denoted by ${\boldsymbol \zeta}^1_j := \hat{I}^1_h ({\bf z}^1_j)$ and $\zeta^2_j := \hat{I}^2_h(z^2_j)$.
\begin{figure}[t!]
\includegraphics[width=0.32\textwidth]{harmonic_bezier}
\includegraphics[width=0.32\textwidth]{harmonic_greville_vertices}
\includegraphics[width=0.32\textwidth]{harmonic_greville_edges}
\caption{Construction of the harmonic function for $\MG_{0,1}$ corresponding to the hierarchical B\'ezier mesh on the left. In the middle, we choose the degrees of freedom associated to $\Gamma^\MG_2$ to be equal to one and all the others equal to zero. On the right, the gradient of that function expressed in terms of the degrees of freedom of $\hat Z^1_{\ell,\ell+1}$, with coefficients equal to one or minus one depending on the arrow orientation, gives ${\bf z}^1_j$.} \label{fig:harmonic}
\end{figure}

\begin{remark} \label{rem:orthogonal}
The functions ${\bf z}^1_j$ are generators of the cohomology group for finite elements, but are not \emph{harmonic forms}, in the sense that they are not orthogonal to the exact forms. In order to obtain the harmonic forms, one could take the gradients of the functions that solve the problem
\begin{equation*}
\left \{
\begin{array}{rl}
\displaystyle 
\int_{\MG_{\ell,\ell+1}} \grad \phi_j \cdot \grad \psi = 0 & \forall \psi \in \hat Z^0_{\ell,\ell+1}, \\
\phi_j = 1 & \text{\rm  on } \Gamma^\MG_j, \\
\phi_j = 0 & \text{\rm  on } \partial \MG_{\ell,\ell+1} \setminus \Gamma^\MG_j.
\end{array}
\right.
\end{equation*}
However, orthogonality is lost when applying the isomorphism $\hat I_h^1$ to construct the spline functions ${\boldsymbol \zeta}_j^1$.
\end{remark}

\begin{lemma} \label{lemma:curves}
Under Assumptions~\ref{ass:support} and~\ref{ass:overlap}, the following statements hold.
\begin{enumerate}[i)]
\item Given a spline closed form $\psi \in Z^2(\Xhat_{\ell,\ell+1})$ (respectively, $\psi \in Z^2(\Xhat_{\ell+1,\ell+1})$), its equivalence class in $H^2(\Xhat_{\ell,\ell+1})$ (resp. $H^2(\Xhat_{\ell+1,\ell+1})$) is uniquely determined by
\begin{equation*}
\int_{\omega_j} \psi \, dx \quad \text{\rm for } j = 1, \ldots, \nc-1,
\end{equation*}
with $\omega_j \subset \Omega_{\ell+1}$ denoting the connected components of $\Omega_{\ell+1}$.
\item There exists a set of curves $\gamma_j$ in $\Omega_{\ell+1}$, with $j = 1, \ldots, \nh$, such  that given a closed form $\bv \in Z^1(\Xhat_{\ell,\ell+1})$ (respectively $\bv \in Z^1(\Xhat_{\ell+1,\ell+1})$), its equivalence class in $H^1(\Xhat_{\ell,\ell+1})$ (resp. $H^1(\Xhat_{\ell+1,\ell+1})$) is uniquely determined by
\begin{equation*}
\int_{\gamma_j} \bv \cdot d{\bf s} \quad \text{\rm for } j = 1, \ldots, \nh.
\end{equation*}
\end{enumerate}
\end{lemma}
\begin{proof}
Noting that the support of a B-spline function associated to a Greville cell of $\MG_{\ell,\ell+1}$ is contained in a connected component of $\Omega_{\ell+1}$, point i) is an immediate consequence of the definition of the forms $\zeta^2_j$, and the fact that there is a one-to-one correspondence between the connected components of $\MG_{\ell,\ell+1}$ and $\Omega_{\ell+1}$, as stated in Theorem~\ref{th:homology}, and more specifically in Proposition~\ref{prop:cc}. It is then clear that $\int_{\omega_j} \zeta^2_i$ form a non-singular diagonal matrix.

Point ii) requires a more technical proof, which is detailed in Appendix~\ref{sec:appendixb}.
\end{proof}


\begin{lemma} \label{lemma:projectors}
If Assumptions~\ref{ass:support} and~\ref{ass:overlap} hold, then it is possible to define a set of cochain projectors $\hat \Pi^k: \Xhat^k_{\ell+1,\ell+1} \rightarrow \Xhat^k_{\ell,\ell+1}$. That is, for every $\phi^k \in \Xhat^k_{\ell,\ell+1}$ it holds $\hat \Pi^k(\phi^k) = \phi^k$, and the following diagram commutes:
\begin{equation*}
\begin{CD}
0 @>>> \Xhat^0_{\ell+1,\ell+1} @>\grad>> \Xhat^1_{\ell+1,\ell+1} @>\curls>> \Xhat^2_{\ell+1,\ell+1} @>>> \mathbb{R} @>>> 0 \\
@. @V\hat \Pi^0VV @V\hat \Pi^1VV @V\hat \Pi^2VV  \\
0 @>>> \Xhat^0_{\ell,\ell+1} @>\grad>> \Xhat^1_{\ell,\ell+1} @>\curls>> \Xhat^2_{\ell,\ell+1} @>>> \mathbb{R} @>>> 0.
\end{CD}
\end{equation*}
\end{lemma}
\begin{proof}
The construction of these commutative projectors is inspired by \cite{DB05}. We recall that we are always considering spaces with homogeneous boundary conditions.

Given $q \in \Xhat^0_{\ell+1,\ell+1}$, we define $\hat \Pi^0 q \in \Xhat^0_{\ell,\ell+1}$ as the unique solution to
\begin{align*}
(\grad \hat \Pi^0 q, \grad \phi) = (\grad q, \grad \phi) \quad \forall \phi \in \Xhat^0_{\ell,\ell+1}.
\end{align*}

Given $\bv \in \Xhat^1_{\ell+1,\ell+1}$, we define $\hat \Pi^1 \bv \in \Xhat^1_{\ell,\ell+1}$ as the unique solution to 
\begin{align*}
(\curls \hat \Pi^1 \bv, \curls \bw) = (\curls \bv, \curls \bw) &\quad \forall \bw \in \Xhat^1_{\ell,\ell+1}, \\
(\hat \Pi^1 \bv, \grad \phi) = (\bv, \grad \phi) & \quad \forall \phi \in \Xhat^0_{\ell,\ell+1}, \\
\int_{\gamma_j} \hat \Pi^1 \bv \cdot d{\bf s} = \int_{\gamma_j} \bv \cdot d{\bf s} & \quad \text{ for } j = 1, \ldots, \nh,
\end{align*}
where the curves $\gamma_j$ are defined as in Lemma~\ref{lemma:curves}.

Given $\psi \in \Xhat^2_{\ell+1,\ell+1}$ we define $\hat \Pi^2 \psi \in \Xhat^2_{\ell,\ell+1}$ as the unique solution to 
\begin{align*}
(\hat \Pi^2 \psi, \curls \bw) = (\psi, \curls \bw) &\quad \forall \bw \in \Xhat^1_{\ell,\ell+1}, \\
\int_{\omega_j} \hat \Pi^2 \psi \, dx = \int_{\omega_j} \psi \, dx &\quad \text{ for } j = 1, \ldots, \nc,
\end{align*}
where $\omega_j \subset \Omega_{\ell+1}$ are the connected components of $\Omega_{\ell+1}$.

The correct definition of the projectors is a consequence of Lemma~\ref{lemma:curves}, and the fact that we are working with spaces with boundary conditions. The commutativity of the diagram comes trivially from the definition of the projectors.
\end{proof}

\subsubsection{Final Part of the Proof: The Main Result}

We can finally prove the main result of this section.
\begin{proof}[Proof of Theorem~\ref{th:local}]
The theorem is proved by an induction argument. The case of $\ell = 0$ corresponds to standard tensor-product B-splines, and the result holds from \cite{BRSV11}. Assuming that the sequence is exact for $\ell$, and using Theorem~\ref{th:exact}, in order to prove the exactness for $\ell+1$ we have to show that the inclusion $j: \Xhat_{\ell,{\ell+1}} \longrightarrow \Xhat_{\ell+1,{\ell+1}}$ induces an isomorphism between the cohomology groups $H^k(\Xhat_{\ell,{\ell+1}})$ and $H^k(\Xhat_{\ell+1,{\ell+1}})$.

From Corollary~\ref{corol:cohomology} we have $H^k(\Xhat_{\ell,{\ell+1}}) \cong H^k(\Xhat_{\ell+1,{\ell+1}})$, and since the spaces are finite-dimensional, it is enough to prove that $j^*:H^k(\Xhat^k_{\ell,\ell+1}) \rightarrow H^k(\Xhat^k_{\ell+1,\ell+1})$ is injective. This is proved using the cochain projectors in Lemma~\ref{lemma:projectors}. Since $\hat \Pi^k \circ j = {\rm Id}$, we have that $(\hat \Pi^k \circ j)^* = (\hat \Pi^k)^* \circ j^* = {\rm Id}^*$, which is the identity in cohomology. As a consequence $j^*$ is injective (and ($\hat \Pi^k)^*$ is surjective), which ends the proof.
\end{proof}

\begin{remark}
The exactness of the sequence might be also proved using the characterization of hierarchical B-splines in terms of piecewise polynomials of \cite{Mokris2014}, invoking the same arguments already used for T-splines in \cite{BSV14} and for LR-splines in \cite{Johannessen15}.
\end{remark}


==> hierarchicalcomplex.tex <==
In this section, we finally present the hierarchical B-spline complex of isogeometric discrete differential forms.  We start with a short introduction of hierarchical B-splines, where we follow the construction in \cite{Kraft} and \cite{Vuong_giannelli_juttler_simeon}, and we present an auxiliary lemma that will be useful for further study of the hierarchical B-spline complex. We then introduce a simple definition of the hierarchical B-spline complex, and we provide a counterexample showing that the complex is not always exact.  We next introduce the concept of Greville subgrids which will prove useful for the analysis of exactness in Section~\ref{sec:exactness}. We end the section with an explanation on how to construct the complex in the physical domain as well as for multi-patch domains.

For the sake of simplicity, from now on we only use spaces with homogeneous boundary conditions. The zero subindex corresponding to these spaces is removed to alleviate notation. For ease of reading, a given level of the multi-level mesh associated with a hierarchical B-spline basis is indicated by the subindex $\ell$, while the position in the complex for $k$-forms is indicated by the superindex $k$. %We will also often refer to hierarchical B-splines as simply hierarchical splines.



\subsection{Hierarchical B-splines} \label{sec:HB-splines}

Recall that the parametric domain is given by $\hat \Omega = (0,1)^n$. Let us assume that we have a sequence of tensor-product spline spaces of 0-forms
\begin{equation}\label{eq:subspaces}
\Xhat_{0,h} \subset \Xhat_{1,h} \subset \ldots \subset \Xhat_{N,h}.
\end{equation}
More precisely, for each {\bf\emph{level}} $\ell = 0, \ldots, N$, the $n$-variate tensor product spline space $\Xhat_{\ell,h} \subset H^1(\hat \Omega)$ is defined as the tensor product of univariate spline spaces $S_{p_{j,\ell}}(\Xi_{j,\ell})$, each of degree $p_{j,\ell}$ and built using a knot vector $\Xi_{j,\ell}$.  That is, $\Xhat_{\ell,h} = \otimes_{j=1}^n S_{p_{j,\ell}}(\Xi_{j,\ell})$. We denote the set of B-spline basis functions for each level by ${\cal B}_\ell$, and we denote by $\M_\ell$ the corresponding B\'ezier mesh, that is, the Cartesian grid generated by the knot vectors without repetitions. 
Let moreover
\begin{equation}\label{eq:subdomains}
\hat \Omega = \Omega_0 \supset \Omega_1 \supset \ldots \supset \Omega_{N} \supset \Omega_{N+1} = \emptyset
\end{equation}
denote a sequence of nested subdomains, where we assume that (the closure of) each subdomain $\Omega_\ell$ is (the closure of) a union of elements of $\M_{\ell-1}$ for $\ell = 1, \ldots, N$. This is the same condition as the {\bf \emph{strong condition}} in \cite{Vuong_giannelli_juttler_simeon}.  With the above notation, \textbf{\textit{hierarchical B-splines}} are defined in a recursive manner as follows.

\begin{definition} \label{def:hierarchical}
We define the space of hierarchical splines $\What_N = {\rm span} \{{\cal H}_N\}$, with ${\cal H}_N$ the hierarchical basis constructed with the following recursive algorithm \cite{Kraft}:
\begin{enumerate}
\item Initialization: ${\cal H}_0 = {\cal B}_0$.
\item Recursively construct ${\cal H}_{\ell+1}$ from ${\cal H}_{\ell}$ by setting
\begin{equation*}
{\cal H}_{\ell+1} = {\cal H}_{\ell+1,c} \cup {\cal H}_{\ell+1,f}, \text{ for } \ell = 0, \ldots N-1,
\end{equation*}
with 
\begin{equation*}
\begin{array}{l}
{\cal H}_{\ell+1,c} = \{\beta \in {\cal H}_{\ell} : \supp(\beta) \not \subset \Omega_{\ell+1}\}, \\
{\cal H}_{\ell+1,f} = \{\beta \in {\cal B}_{\ell+1} : \supp(\beta) \subset \Omega_{\ell+1}\}.
\end{array}
\end{equation*}
%\item ${\cal H} = {\cal H}_{N}$.
\end{enumerate}
\end{definition}
\noindent That is, at step $\ell$ of the recursive algorithm we add the basis functions of level $\ell+1$ completely supported in $\Omega_{\ell+1}$ to the basis and remove the functions of previous levels completely supported in $\Omega_{\ell+1}$ from the basis. B-spline basis functions which are included in ${\cal H}_N$ are referred to as \textbf{\textit{active}} basis functions, and in particular, ${\cal H}_N \cap {\cal B}_\ell$ is the set of active basis functions of level $\ell$, for an integer $0 \leq \ell \leq N$.

Associated with the space of hierarchical splines $\What_N$ is a \textit{\textbf{hierarchical B\'{e}zier mesh}}
\begin{equation}
\mathcal{M}_\mathcal{H} := \bigcup_{\ell=0}^N \{Q \in {\cal M}_\ell \, \text{ such that } \, Q \subset \Omega_\ell \, \text{ and } \, Q \not \subset \Omega_{\ell+1} \}.
\end{equation}
The elements of the hierarchical B\'{e}zier mesh are precisely those included in a formation and assembly routine for isogeometric analysis \cite{Hennig16, Garau16}. An example of a two-dimensional hierarchical B\'ezier mesh, for a simple configuration with only two levels, is depicted in Figure~\ref{fig:hierarchical_bezier}. We have identified the Greville points (see Subsection~\ref{sec:geometric_interpretation}) associated with the active basis functions for both levels in Figure~\ref{fig:0forms_two_levels} assuming the basis functions are maximally continuous and of degree $p_1 = p_2 = 2$.

\begin{figure}
\centerline{\includegraphics[width=0.4\textwidth, trim = 11cm 2cm 11cm 2cm, clip]{Figures/hmsh_2levels_bezier.pdf}}
\caption{Example of a hierarchical B\'ezier mesh with two levels.}
\label{fig:hierarchical_bezier}
\end{figure}

\begin{figure}
\centerline{\includegraphics[width=0.4\textwidth, trim = 11cm 2cm 11cm 1cm, clip]{Figures/hmsh_2levels_0forms_level1.pdf}
\includegraphics[width=0.4\textwidth, trim = 11cm 2cm 11cm 1cm, clip]{Figures/hmsh_2levels_0forms_level2.pdf}}
\caption{Greville points associated with the active basis functions for levels $\ell = 0$ (left) and $\ell = 1$ (right) in the hierarchical B\'ezier mesh depicted in Figure~\ref{fig:hierarchical_bezier} assuming the basis functions are maximally continuous and of degree $p_1 = p_2 = 2$.}
\label{fig:0forms_two_levels}
\end{figure}

It is useful to define, for $0 \le \ell \le \ell' \le N$, the set of basis functions of level $\ell$ with support contained in $\Omega_{\ell'}$, that is 
\begin{equation} \label{eq:B_lk}
{\cal B}_{\ell,\Omega_{\ell'}} \equiv {\cal B}_{\ell,\ell'} := \{ \beta \in {\cal B}_\ell : \supp (\beta) \subset \Omega_{\ell'} \}.
\end{equation}
Notice that, in Definition \ref{def:hierarchical}, we have ${\cal H}_{\ell+1,f} = {\cal B}_{\ell+1, {\ell+1}}$. We will also make use of the following auxiliary spaces, which are closely related to the recursive construction of the hierarchical spline space.
\begin{definition} \label{def:X_ell}
For $0 \le \ell \le \ell' \le N$, we define the spaces:
\begin{align*}
& \What_\ell := {\rm span} \{ {\cal H}_\ell \}, \\
& \Xhat_{\ell,\Omega_{\ell'}} \equiv \Xhat_{\ell,\ell'} := {\rm span} \{ {\cal B}_{\ell,\ell'} \} = \{ \beta \in \hat X_{\ell,h} : \supp (\beta) \subset \Omega_{\ell'} \},
\end{align*}
where the equality holds thanks to the local linear independence of B-splines.
\end{definition}
\noindent Note that we are using the $\Xhat$ notation for spaces spanned by basis functions of one single level, and we are using $\What$ for spaces spanned by functions of multiple levels. In particular, in the previous definition, the space $\What_\ell$ represents the space of hierarchical splines when applying the recursive algorithm up to level $\ell$. The set of auxiliary spaces denoted with the $\Xhat$ notation is helpful to represent the spaces spanned by the basis functions that have to be added ($\Xhat_{\ell+1,{\ell+1}}$) and removed ($\Xhat_{\ell,{\ell+1}}$) at each level in the recursive algorithm, as stated in the following lemma.

\begin{lemma} \label{lemma:cupcap}
For $0 \le \ell \le N-1$ it holds that
\begin{enumerate}[i)]
\item $\What_{\ell+1} = \What_{\ell} + \Xhat_{\ell+1,{\ell+1}} := \{u = v + w: v \in \What_\ell, \, w \in \Xhat_{\ell, {\ell+1}} \}$.
\item $\What_\ell \cap \Xhat_{\ell+1, {\ell+1}} = \Xhat_{\ell, {\ell+1}}$.
\end{enumerate}
\end{lemma}
\begin{proof}
To prove the result, we show that inclusions in both directions hold. The first inclusion in i), that is, $\What_{\ell+1} \subset \What_{\ell} + \Xhat_{\ell+1,{\ell+1}}$, follows from Definitions~\ref{def:hierarchical} and~\ref{def:X_ell} since ${\cal H}_{\ell+1} = {\cal H}_{\ell+1,c} \cup {\cal H}_{\ell+1,f} \subset {\cal H}_\ell \cup {\cal H}_{\ell+1,f}$ and $\Xhat_{\ell+1,{\ell+1}} = {\rm span}\{{\cal H}_{\ell+1,f}\}$. For the second inclusion, it is obvious that $\Xhat_{\ell+1,{\ell+1}} \subset \What_{\ell+1}$, and $\What_\ell \subset \What_{\ell+1}$ is a consequence of their definition and the nestedness provided by~\eqref{eq:subspaces}.

For the first inclusion in ii), we have that $u \in \What_\ell = {\rm span}\{{\cal H}_\ell\} \subset {\rm span\{\cal B}_\ell\}$, and moreover $u \in \Xhat_{\ell+1,{\ell+1}}$ implies that $\supp (u) \subset \Omega_{\ell+1}$, which along with the local linear independence of \mbox{B-splines} yields $u \in \Xhat_{\ell, {\ell+1}}$. For the second inclusion we first use the nestedness of the subdomains given by~\eqref{eq:subdomains} and then the result from i) to obtain $\Xhat_{\ell,{\ell+1}} \subset \Xhat_{\ell,\ell} \subset \What_\ell$. Then, the nestedness of the spline spaces~\eqref{eq:subspaces}, together with the local linear independence of B-splines, immediately gives $\Xhat_{\ell, {\ell+1}} \subset \Xhat_{\ell+1, {\ell+1}}$, which completes the proof.
\end{proof}

\subsection{The Hierarchical B-spline Complex}
The construction of the hierarchical B-spline complex is based on a simple idea: given a multi-level mesh, construct a sequence of hierarchical B-splines of mixed degree, using for each level the B-spline complex in Section~\ref{sec:spline-complex}. We will see, however, that this construction does not, in general, yield an exact complex of hierarchical B-splines.  As was done for the tensor-product B-spline complex, we first define the hierarchical B-spline complex in the parametric domain before mapping it onto the physical domain.

Assume we are given a sequence of nested tensor-product spline spaces
\begin{equation*}
\Xhat_{0,h} \subset \Xhat_{1,h} \subset \ldots \subset \Xhat_{N,h},
\end{equation*}
as in~\eqref{eq:subspaces} and a sequence of nested subdomains as in~\eqref{eq:subdomains}. For each level $\ell = 0, \ldots, N$, we select $\Xhatlh{0} = \Xhat_{\ell,h}$ as the discrete space of 0-forms, and we construct a discrete de Rham complex using tensor-product splines of mixed degree as explained in Section~\ref{sec:spline-complex}. This forms a complex $(\Xhatlh{},d)$ for each level:
\begin{equation} \label{eq:spline_complex}
\begin{CD}
\Xhatlh{0} @>d^0>> \Xhatlh{1} @>d^1>> \ldots @>d^{n-1}>> \Xhatlh{n} .
\end{CD}
\end{equation}
Moreover, with each space of the sequence, $\Xhatlh{k}$, we associate the same set of basis functions introduced in Section~\ref{sec:spline-complex}, and we denote this set of basis functions by ${\cal B}^k_\ell$. Recall that we can define isomorphisms from our B-spline complex to the low-order finite element complex defined on the Greville grid using these bases.

Now, for each $k =0, \ldots, n$, we can construct the hierarchical B-splines bases ${\cal H}^k_N$ and the corresponding hierarchical spline spaces $\What^k_N = {\rm span} \{ {\cal H}^k_N \}$ following the same procedure as in Definition~\ref{def:hierarchical}.  In practice, for spaces of vector-valued splines, the hierarchical B-spline basis can be determined using the recursive algorithm for each component. Adopting the notation introduced in Section \ref{sec:derham} for Hilbert complexes, the \textbf{\textit{hierarchical B-spline complex}} is then simply $\left(\What_N,d\right)$.  As an example, let us recall consider a maximally continuous hierarchical B-spline complex with $p_1 = p_2 = 3$ defined on the hierarchical B\'ezier mesh depicted in Figure~\ref{fig:hierarchical_bezier}.  The Greville nodes associated with active basis functions for $0$-forms are displayed in Figure~\ref{fig:0forms_two_levels}.  All 0-form basis functions are biquadratic, that is, of degree $(2,2)$.  The Greville edges associated with active 1-form basis functions are displayed in Figure~\ref{fig:1forms_two_levels}, where the horizontal arrows correspond to rightward oriented basis functions of degree $(1,2)$ and the vertical arrows to upward oriented basis functions of degree $(2,1)$.  The Greville cells associated with active 2-form basis functions are displayed in Figure~\ref{fig:2forms_two_levels}.  All 2-form basis functions are bilinear, that is, of degree $(1,1)$.

As in \eqref{eq:B_lk}, it will be useful to define, for $0 \le \ell \le \ell' \le N$ and $0 \le k \le n$, the set of basis functions of level $\ell$ that are completely contained in $\Omega_{\ell'}$, that is
\begin{equation} \label{eq:Bik}
{\cal B}^k_{\ell,\Omega_{\ell'}} \equiv {\cal B}^k_{\ell,\ell'} := \{ \beta^k \in {\cal B}^k_\ell : \supp (\beta^k) \subset \Omega_{\ell'} \}.
\end{equation}
Moreover, we can also apply Definition~\ref{def:X_ell} for each $k$ to define
\begin{align}
& \What^k_\ell := {\rm span}\{{\cal H}^k_\ell\}, \\
& \Xhat^k_{\ell,\Omega_{\ell'}} \equiv \Xhat^k_{\ell,\ell'} := {\rm span} \{{\cal B}^k_{\ell,\ell'}\} =  \{ \beta^k \in \Xhatlh{k}  : \supp (\beta^k) \subset \Omega_{\ell'} \},
\end{align}
and the results of Lemma~\ref{lemma:cupcap} also hold. These spaces also form spline complexes, as proved in the next lemma.

\begin{figure}
\centerline{\includegraphics[width=0.4\textwidth, trim = 11cm 2cm 11cm 1cm, clip]{Figures/hmsh_2levels_1forms_level1.pdf}
\includegraphics[width=0.4\textwidth, trim = 11cm 2cm 11cm 1cm, clip]{Figures/hmsh_2levels_1forms_level2.pdf}}
\caption{Greville edges associated with the active 1-form basis functions for levels $\ell = 0$ (left) and $\ell = 1$ (right) in the hierarchical B\'ezier mesh depicted in Figure~\ref{fig:hierarchical_bezier} assuming the 0-form basis functions are maximally continuous and of degree $p_1 = p_2 = 2$.}
\label{fig:1forms_two_levels}
\end{figure}

\begin{figure}[t!]
\centerline{\includegraphics[width=0.4\textwidth, trim = 11cm 2cm 11cm 1cm, clip]{Figures/hmsh_2levels_2forms_level1.pdf}
\includegraphics[width=0.4\textwidth, trim = 11cm 2cm 11cm 1cm, clip]{Figures/hmsh_2levels_2forms_level2.pdf}}
\caption{Greville faces associated with the active 2-form basis functions for levels $\ell = 0$ (left) and $\ell = 1$ (right) in the hierarchical B\'ezier mesh depicted in Figure~\ref{fig:hierarchical_bezier} assuming the 0-form basis functions are maximally continuous and of degree $p_1 = p_2 = 2$.}
\label{fig:2forms_two_levels}
\end{figure}

\begin{lemma}\label{lemma:subcomplex}
For $0 \le \ell \le \ell' \le N$, $(\Xhat_{\ell,\ell'},d)$ and $(\What_\ell,d)$ are Hilbert complexes, not necessarily exact.
\end{lemma}
\begin{proof}
The result for $\Xhat^k_{\ell,\ell'}$ is trivial, because clearly $d^k(\Xhat^k_{\ell,\ell'}) \subset \Xhat^{k+1}_{\ell,\ell'}$ and $(\Xhat_{\ell,\ell'},d)$ is a subcomplex of $(\Xhat_{\ell,h},d)$. For $\What^k_\ell$, since the spaces are contained in $\Xhatlh{k}$, the differential operators $d^k$ are well defined, and to prove the result we proceed by induction. The result is true for $\ell =0$, since $\What^k_0 = \hat X^k_{0,h}$ are the tensor-product spline spaces in Section~\ref{sec:spline-complex}. Assuming that $(\What_\ell,d)$ forms a Hilbert complex, the result holds for $(\What_{\ell+1},d)$, because $\What^k_{\ell+1} = \What^k_{\ell} + \Xhat^k_{\ell+1,{\ell+1}}$ by Lemma~\ref{lemma:cupcap}, and it is immediate to see that $d^k (\What^k_{\ell} + \Xhat^k_{\ell+1,{\ell+1}}) \subset (\What^{k+1}_{\ell} + \Xhat^{k+1}_{\ell+1,{\ell+1}})$.
% and {\Rd Lemma~\ref{lemma:cupcap_derham}}, because $\What^i_{\ell+1} = \What^i_{\ell} \cup \What^i_{\ell+1,\Omega_{\ell+1}}$.
\end{proof}


%\subsection{A Counterexample of the Exactness}
The result of Lemma~\ref{lemma:subcomplex} for $\ell = N$ guarantees that the hierarchical spline spaces $\What^k_N$ form a Hilbert complex, but in general the complex {\bf \emph{may not be exact}}. Actually, it is relatively easy to find counterexamples where the hierarchical spline spaces do not form an exact sequence. For instance, in the two-dimensional case a necessary (but not sufficient) condition for exactness is
\begin{equation*}
\dim (\What^0_N) + \dim (\What^2_N) = \dim (\What^1_N) + 1.
\end{equation*}
We can see that the condition is not fulfilled for the maximally continuous hierarchical B-spline complex with $p_1 = p_2 = 3$ defined on the hierarchical B\'{e}zier mesh depicted in Figure~\ref{fig:2x2}. In this case, a simple computation gives that the dimensions of the hierarchical spaces with boundary conditions are $\dim (\What^0_N) = 147$, $\dim (\What^1_N) = 328$, $\dim(\What^2_N) = 181$, which violates the previous condition.

\begin{figure}[t]
\centerline{\includegraphics[width=0.45\textwidth]{refined_2x2}}
\caption{A hierarchical B\'{e}zier mesh for which the sequence is not exact for $p_1 = p_2 = 3$.}
\label{fig:2x2}
\end{figure}

Exactness of the hierarchical B-spline complex is crucial for the correct behavior of discretization schemes based on the complex, as we will see later in the examples of Section~\ref{sec:stability}. In Section~\ref{sec:exactness}, we develop conditions guaranteeing exactness of the complex based on an analysis of the spaces $\Xhat^k_{\ell,\ell}$ and $\Xhat^k_{\ell,\ell+1}$ appearing in the construction of the hierarchical B-spline complex. In this analysis, we invoke the concept of a Greville subgrid which we now describe in detail.

\begin{remark}
In the two-dimensional setting, a \textbf{rotated hierarchical B-spline complex} may easily be constructed by rotating the orientation of the discrete 1-forms by $\pi/2$ in parametric space, just as was the case for tensor-product B-splines.
\end{remark}

\subsection{The Spline Complex Restricted to a Submesh and the Greville Subgrid}\label{sec:submesh}
Consider a particular level $\ell$, and consider a subdomain $\Omega_{\ell'}$ with $0 \le \ell \le \ell' \le N-1$. From the strong condition in Section~\ref{sec:HB-splines}, we know that $\Omega_{\ell'}$ is a union of elements in $\M_\ell$ for $\ell' \in \{\ell,\ell+1\}$. %We recall that we defined ${\cal B}^k_{\ell, \ell'}$ in \eqref{eq:Bik} as the basis of tensor product $k$-forms completely contained in $\Omega_{\ell'}$, and $\Xhat^k_{\ell,\ell'}$ is the space they span. 
As we already proved in Lemma~\ref{lemma:subcomplex}, the spaces $\Xhat^k_{\ell,\ell'}$ form the complex $(\Xhat_{\ell,\ell'},d)$, but the sequence they form is not necessarily exact.

Employing the geometrical entities in the Greville grid $\MG_\ell$ associated with the basis functions in ${\cal B}^k_{\ell,\ell'}$, we build a {\bf \emph{Greville subgrid}} that we denote by $\MG_{\ell,\ell'} \subset \MG_\ell$. With some abuse of notation, we will also denote by $\MG_{\ell,\ell'}$ (the interior of the closure of) the union of the cells in $\MG_{\ell,\ell'}$. In Figure~\ref{fig:submeshes} we have included, for the same spaces of tensor-product B-splines depicted in Figure~\ref{fig:meshes}, an example of a subdomain $\Omega_{\ell'}$ and the corresponding Greville subgrid. We notice that, in general, the subdomain defined by $\MG_{\ell,\ell'}$ is different from $\Omega_{\ell'}$, and in fact it will depend on the degree of the spline space. We also notice that, since the support of the B-spline basis functions is reduced with the degree, the basis functions associated to the entities on the boundary of $\MG_{\ell,\ell'}$ do not belong to ${\cal B}^k_{\ell,\ell'}$.

\begin{figure}[tp]
\begin{subfigure}[The subdomain $\Omega_{\ell'}$ as a B\'ezier submesh of $\M_\ell$]{
\centering
\includegraphics[width=3.0in]{Bezier_submesh.pdf}
\label{fig:subbezier}
}
\end{subfigure}
\begin{subfigure}[The corresponding Greville subgrid $\MG_{\ell,\ell'}$]{
\includegraphics[width=3.0in]{Greville_submesh.pdf}
\label{fig:subgreville}
}
\end{subfigure}
\caption{Construction of the Greville subgrid $\MG_{\ell,\ell'}$. Considering the same degrees and knot vectors as in Figure~\ref{fig:meshes} to represent $\M_\ell$ and $\MG_\ell$, we choose the subdomain  $\Omega_{\ell'} = (1/6,5/6) \times (1/5,4/5)$ in (a). The Greville subgrid $\MG_{\ell,\ell'}$ is formed by the darkened elements in (b), while the geometric entities corresponding to basis functions in ${\cal B}^k_{\ell,\ell'}$ are marked by blue dots (0-forms), red arrows (1-forms) and green squares (2-forms).}
\label{fig:submeshes}
\end{figure}

Finally, for each level $\ell$, we can define isomorphisms as in the diagram \eqref{eq:cd-iga-fem} that relate the B-spline complex to the low-order finite element complex defined on the Greville grid. Considering the subdomain $\Omega_{\ell'}$, the same isomorphisms relate the spline subspaces $\Xhat^k_{\ell,\ell'}$ to the spaces of the finite element complex defined on the Greville subgrid, which we henceforth denote by $\hat{Z}^k_{\ell,\ell'}$, and a commutative diagram can also be defined for these subspaces.

\begin{remark}
Since we are assuming homogeneous boundary conditions on $\partial \Omega$, the finite element spaces $\hat{Z}^k_{\ell,\ell'}$ have homogeneous boundary conditions on $\partial \MG_{\ell,\ell'}$. Removing this assumption would cause the finite element spaces to have homogeneous boundary conditions on $\partial \MG_{\ell,\ell'} \setminus (\partial \MG_{\ell,\ell'} \cap \partial \hat \Omega)$. The results of the paper can be easily applied to this case, but writing it in detail would only add more complexity without giving more insight.
\end{remark}

\subsection{Extension to the Physical Domain and Multi-patch Geometries}

The hierarchical B-spline complex in the physical domain is built in exactly the same manner as the B-spline complex. Namely, assuming that we have a parametrization ${\bf F}: \hat \Omega \rightarrow \Omega$, we simply use the pullback operators defined in Subsection \ref{subsec:pullback}, yielding:
\begin{equation*}
W_\ell^k\left(\Omega\right) := \left\{ \omega \in X^k\left(\Omega\right) : \iota^k(\omega) \in \What^k_\ell \right\}
\end{equation*}
for all integers $0 \leq k \leq n$ and $0 \leq \ell \leq N$.

To define hierarchical differential forms in a multi-patch domain, one must take into account the presence of non-conforming meshes between patches \cite{Scott2014222}. This can be easily done following the approach used in \cite{Buchegger2016159} for 0-forms. We start by defining a multi-patch B-spline complex for each level, exactly as in Section~\ref{sec:multipatch}. Then, we apply the hierarchical algorithm of Definition~\ref{def:hierarchical} to the multi-patch spaces of the complex, taking into account that the supports of interface functions overlap two or more patches. 
%With this procedure, the check of the support and the orientation assignment for each basis function can be done at the tensor-product level.  JOHN: I found this possibly confusing for the reader.
We show an example of the construction for a multi-patch, maximally continuous hierarchical B-spline complex with $p_1 = p_2 = 2$ defined on the hierarchical B\'{e}zier mesh in Figure~\ref{fig:multipatch}, where the thick line represents the interface between both interfaces. The set of active basis functions for 0-forms is represented in the Greville grid in Figure~\ref{fig:multi_0forms}, for levels 0 and 1. We note the presence of an active basis function at level 0 on the interface that would not appear on the left patch when considering the patches separately. This is due to the fact that the basis function is supported on both patches. Similarly, some functions of level 1 on the interface are not active but would be active on the left patch if we considered the patches separately. A similar behavior is also encountered for the 1-forms depicted in Figure~\ref{fig:multi_1forms}.

\begin{figure}[t]
\centerline{\includegraphics[width=0.6\textwidth, trim=5cm 4cm 4cm 3cm, clip]{multipatch_bezier}}
\caption{A hierarchical B\'{e}zier mesh for a simple multi-patch geometry with $p_1 = p_2 = 2$.}\label{fig:multipatch}
\end{figure}

\begin{figure}[t]
\begin{subfigure}[Active basis functions of level 0]{
\includegraphics[width=0.49\textwidth, trim=5cm 4cm 4cm 3cm, clip]{multipatch_0forms_level1}
\label{fig:multi_0forms_1lev}
}
\end{subfigure}
\begin{subfigure}[Active basis functions of level 1]{
\includegraphics[width=0.49\textwidth, trim=5cm 4cm 4cm 3cm, clip]{multipatch_0forms_level2}
\label{fig:multi_0forms_2lev}
}
\end{subfigure}
\caption{Geometric entities in the Greville grids associated with active basis functions for 0-forms corresponding to the multi-patch example in Figure~\ref{fig:multipatch}.}
\label{fig:multi_0forms}
\end{figure}

\begin{figure}[h!]
\begin{subfigure}[Active basis functions of level $\ell = 0$]{
\includegraphics[width=0.49\textwidth, trim=5cm 4cm 4cm 3cm, clip]{multipatch_1forms_level1}
\label{fig:multi_1forms_1lev}
}
\end{subfigure}
\begin{subfigure}[Active basis functions of level $\ell = 1$]{
\includegraphics[width=0.49\textwidth, trim=5cm 4cm 4cm 3cm, clip]{multipatch_1forms_level2}
\label{fig:multi_1forms_2lev}
}
\end{subfigure}
\caption{Geometric entities in the Greville grids associated with active basis functions for 1-forms corresponding to the multi-patch example in Figure~\ref{fig:multipatch}.}
\label{fig:multi_1forms}
\end{figure}

%% \subsection{The Spline Complex Restricted to a Submesh}\label{sec:submesh}
%% For the construction of a de Rham complex with hierarchical splines, we need to define suitable spline complexes in the subdomains $\Omega_\ell$. We recall that we assume (the closure of) each subdomain $\Omega_\ell$ to be (the closure of) the union of the union of B\'ezier elements in $\M$. {\Rd We will denote by $\M_{\Omega_\ell}$ the {\bf \emph{B\'ezier submesh}}, that is, the restriction of the B\'ezier mesh $\M$ to the subdomain~$\Omega_\ell$.}

%% We now construct the B-spline complexes restricted to the subdomain $\Omega_\ell$. Let us first define, in an analogous way to \eqref{eq:B_lk}
%%  the set of basis functions
%% \begin{equation} %\label{eq:Bik}
%% {\cal B}^k_{\Omega_\ell} := \{\beta \in {\cal B}^k : \supp (\beta^k) \subset \Omega_\ell \},
%% \end{equation}
%% and the space spanned by them
%% \begin{equation*}
%% \XhatOm{k}{\ell} := {\rm span} ({\cal B}^k_{\Omega_\ell}) = \{ u \in \Xhath{k} : \supp (u) \subset \Omega_\ell \},
%% \end{equation*}
%% where the equality holds thanks to the local linear independence of B-splines. It is easily shown that $d^k (\XhatOm{k}{\ell}) \subset \XhatOm{k+1}{\ell}$, so we have the following complex:
%% \begin{equation*}
%% \begin{CD}
%% \XhatOm{0}{\ell} @>d^0>> \XhatOm{1}{\ell} @>d^1>> \ldots @>d^{n-1}>> \XhatOm{n}{\ell}.
%% \end{CD}
%% \end{equation*}
%% However, the complex is {\bf \emph{not}} necessarily {\bf \emph{exact}}. {\Rd REDUCED COHOMOLOGY}

%% Selecting for the basis functions in ${\cal B}^k_{\Omega_\ell}$ their associated geometrical entities in the Greville grid $\MG$, we build a {\bf \emph{Greville subgrid}} $\MG_{\Omega_\ell} \equiv \MG_{\ell} \subset \MG$. With some abuse of notation, we will also denote by $\MG_{\ell}$ (the interior of the closure of) the union of the cells in $\MG_{\ell}$. In Figure~\ref{fig:submeshes} we have included an example of a B\'ezier submesh, and the corresponding Greville subgrid when considering the same spaces of B-splines of Figure~\ref{fig:meshes}. We notice that, in general, the subdomain defined by $\MG_{\ell}$ is different from $\Omega_\ell$, and in fact it will depend on the degree of the spline space. We also notice that, since the support of the spline basis functions is reduced with the degree, the basis functions associated to the entities on the boundary of $\MG_{\ell}$ do not belong to ${\cal B}^k_{\Omega_\ell}$.
%% \begin{figure}[tp]
%% \begin{subfigure}[A B\'ezier submesh]{
%% \centering
%% \includegraphics[width=3.0in]{Bezier_submesh.pdf}
%% }
%% \end{subfigure}
%% \begin{subfigure}[The corresponding Greville subgrid]{
%% \includegraphics[width=3.0in]{Greville_submesh.pdf}
%% }
%% \end{subfigure}
%% \caption{B-spline submeshes associated with polynomial degrees $p_1 = 2$ and $p_2 = 2$, knot vectors $\Xi_1 = [0,0,0,1/6,2/6,3/6,4/6,5/6,1,1,1]$ and $\Xi_2 = [0,0,0,1/5,2/5,3/5,4/5,1,1,1]$, and the subdomain $\Omega_\ell = (1/6,5/6) \times (1/5,4/5)$. The Greville subgrid $\MG_\ell$ is formed by the darkened elements in (b), while the the functions in ${\cal B}^k_{\Omega_\ell}$ are marked by blue dots (0-forms), red arrows (1-forms) and green squares (2-forms).}
%% \label{fig:submeshes}
%% \end{figure}

%% We can restrict the isomorphisms $\hat I^k_h$ to the subspaces $\XhatOm{k}{\ell}$, and define the finite element spaces $\ZhatOm{k}{\ell} := \hat I^k_h (\XhatOm{k}{\ell})$. The isomorphisms also relate the topological structure of the spline subspaces $\XhatOm{k}{\ell}$ to that of the finite element spaces $\ZhatOm{k}{\ell}$, and we have the following commutative diagram:
%% {\Rd IS THIS NECESSARY?}
%% \begin{equation} \label{eq:subcd-iga-fem}
%% \begin{CD}
%% %\mathbb{R} @>>> 
%% \XhatOm{0}{\ell} @>d^0>> \XhatOm{1}{\ell} @>d^1>> \ldots @>d^{n-1}>> \XhatOm{n}{\ell} \\
%% @V\hat I^0_hVV @V\hat I^1_hVV @. @V\hat I^n_hVV \\
%% %\mathbb{R} @>>> 
%% \ZhatOm{0}{\ell} @>d^0>> \ZhatOm{1}{\ell} @>d^1>> \ldots @>d^{n-1}>> \ZhatOm{n}{\ell}.
%% \end{CD}
%% \end{equation}
%% Notice that, since we are assuming homogeneous boundary conditions on $\partial \Omega$, the spaces $\ZhatOm{k}{\ell}$ are in fact the lowest-order finite element spaces defined in the Greville subgrids, with homogenous boundary conditions on $\partial \MG_{\ell}$. Working on spaces without boundary conditions would cause the finite-element spaces $\ZhatOm{k}{\ell}$ to have homogeneous boundary conditions on $\partial \MG_{\ell} \setminus (\partial \MG_{\ell} \cap \partial \hat \Omega)$, that is, on the boundaries of the subgrid $\MG_{\ell}$ that do not belong to the boundary of the domain. We have preferred to work with spaces with boundary conditions to avoid precising the boundary of each subdomain, but the results work also without boundary conditions with minor changes.






%% Finally, we can also define suitable projectors $\hat \Pi^k_{\Omega_\ell} \equiv \hat \Pi^k_\ell$ to obtain a commutative diagram similar to \eqref{eq:cd-iga-pi} (or \eqref{eq:cd-iga-pi}) for the spaces of the subcomplex. In practice, the projectors $\hat \Pi^k$ in \eqref{eq:cd-iga-pi} are defined from a dual basis, see \cite{BRSV11}, thus it is enough to restrict the definition to the dual functionals associated to the basis functions in ${\cal B}^k_\ell$ to obtain $\hat \Pi^k_\ell$. By doing so we obtain the commutative diagram {\Rd BOUNDARY CONDITIONS}

%% {\Rd REMOVE THE PROJECTORS, IF NOT NEEDED}
%% \begin{equation} \label{eq:subcd-iga-pi}
%% \begin{CD}
%% \Xhat^0(\Omega_\ell) @>d^0>> \Xhat^1(\Omega_\ell) @>d^1>> \ldots @>d^{n-1}>> \Xhat^n(\Omega_\ell) \\
%% @V\hat \Pi_\ell^0 VV @V\hat \Pi_\ell^1 VV @. @V\hat \Pi_\ell^n VV\\
%% \XhatOm{0}{\ell} @>d^0>> \XhatOm{1}{\ell} @>d^1>> \ldots @>d^{n-1}>> \XhatOm{n}{\ell} .
%% \end{CD}
%% \end{equation}
%% It is worth to note that, although the projectors are local and stable and the diagram commutes, the subspaces $\XhatOm{k}{\ell}$ do not guarantee optimal approximation properties in $\Omega_\ell$. Indeed, since the spaces $\XhatOm{k}{\ell}$ only contain the functions of $\Xhath{k}$ that are completely contained in $\Omega_\ell$, they do not reproduce global polynomials in $\Omega_\ell$, because this requires functions that are not completely supported in the subdomain.

%% After introducing all the machinery, we are now in a position to define the spline complex with hierarchical B-splines.

%% \subsection{The Hierarchical Spline Complex in the Parametric Domain}
%% The construction of the hierarchical spline complex is based on a simple idea: given a multi-level mesh, construct a sequence of hierarchical splines of mixed degree, using for each level the de Rham complex of tensor product B-splines in Section~\ref{sec:spline-complex}. We will see, however, that in general this construction does not give an exact complex of hierarchical splines.

%% Assume we are given a sequence of nested spline spaces
%% \begin{equation*}
%% \Xhat_{0,h} \subset \Xhat_{1,h} \subset \ldots \subset \Xhat_{N,h},
%% \end{equation*}
%% as in~\eqref{eq:subspaces}, and a sequence of nested subdomains as in~\eqref{eq:subdomains}. For each level $\ell = 0, \ldots, N$ we select $\Xhatlh{0} = \Xhat_{\ell,h}$, and construct a discrete de Rham complex using tensor-product splines of mixed degree, as explained in Section~\ref{sec:spline-complex}. This forms a complex $(\Xhatlh{},d)$ for each level:
%% \begin{equation} \label{eq:spline_complex}
%% \begin{CD}
%% \Xhatlh{0} @>d^0>> \Xhatlh{1} @>d^1>> \ldots @>d^{n-1}>> \Xhatlh{n} .
%% \end{CD}
%% \end{equation}
%% Moreover, for each space of the sequence we use the same set of basis functions explained in Section~\ref{sec:spline-complex}, and denote it by ${\cal B}^k_\ell$. We recall that using these bases we can define isomorphisms from our spline complex to the low-order finite element complex defined on the Greville grid.

%% Now, for each $k =0, \ldots, n$ we can construct the hierarchical spline bases ${\cal H}^k_N$ and the corresponding hierarchical spline space $\What^k_N = {\rm span} \{ {\cal H}^k_N \}$ following the same procedure as in Definition~\ref{def:hierarchical}. {\Rd In practice, for spaces of vector-valued splines, the hierarchical spline space can be computed using the recursive algorithm for each component}.

%% As in \eqref{eq:B_lk} and \eqref{eq:Bik}, it will be useful to define for $0 \le \ell \le \ell' \le N$, and for $0 \le k \le n$ the set of basis functions of level $\ell$ that are completely contained in $\Omega_{\ell'}$, that is
%% \begin{equation*}
%% {\cal B}^k_{\ell,\Omega_{\ell'}} \equiv {\cal B}^k_{\ell,\ell'} := \{ \beta^k \in {\cal B}^k_\ell : \supp (\beta^k) \subset \Omega_{\ell'} \}.
%% \end{equation*}
%% Moreover, we can also apply Definition~\ref{def:X_ell} for each $k$ to define
%% \begin{align}
%% & \What^k_\ell := {\rm span}\{{\cal H}^k_\ell\}, \\
%% & \Xhat^k_{\ell,\Omega_{\ell'}} \equiv \Xhat^k_{\ell,\ell'} := {\rm span} \{{\cal B}^k_{\ell,\ell'}\} =  \{ u^k \in \Xhatlh{k}  : \supp (u^k) \subset \Omega_{\ell'} \},
%% \end{align}
%% and the results of Lemma~\ref{lemma:cupcap} also hold. These spaces also form spline complexes, as it is proved in the next lemma.

%% \begin{lemma}
%% For $0 \le \ell \le \ell' \le N$, $(\Xhat_{\ell,\ell'},d)$ and $(\What_\ell,d)$ are two de Rham sequences, not necessarily exact.
%% \end{lemma}
%% \begin{proof}
%% The result for $\Xhat^k_{\ell,\ell'}$ holds from Section~\ref{sec:submesh}. For $\What^k_\ell$, since the spaces are contained in $\Xhatlh{k}$, the differential operators $d^k$ are well defined, and to prove the result we proceed by induction. The result is true for $\ell =0$, since $\What^k_0 = \hat X^k_{0,h}$ are the tensor-product spline spaces in Section~\ref{sec:spline-complex}. Assuming that $(\What_\ell,d)$ forms a de Rham sequence, the result holds for $(\What_{\ell+1},d)$, because by Lemma~\ref{lemma:cupcap} $\What^k_{\ell+1} = \What^k_{\ell} + \Xhat^k_{\ell+1,{\ell+1}}$, and it is immediate to see that $d^k (\What^k_{\ell} + \Xhat^k_{\ell+1,{\ell+1}}) \subset (\What^{k+1}_{\ell} + \Xhat^{k+1}_{\ell+1,{\ell+1}})$.
%% % and {\Rd Lemma~\ref{lemma:cupcap_derham}}, because $\What^i_{\ell+1} = \What^i_{\ell} \cup \What^i_{\ell+1,\Omega_{\ell+1}}$.
%% \end{proof}

%% In particular, for $\ell = N$ the lemma guarantees that the hierarchical spline spaces $\What^i_N$ form a de Rham complex, but the complex {\bf \emph{may not be exact}}.{\Rd REDUCED COHOMOLOGY} Actually, it is relatively easy to find counterexamples where the hierarchical spline spaces do not form an exact sequence. For instance, in the two-dimensional case a necessary (but not sufficient) condition for exactness is
%% \begin{equation*}
%% \dim (\What^0_N) + \dim (\What^2_N) = \dim (\What^1_N) + 1.
%% \end{equation*}
%% We can see that the condition is not fulfilled in the example of Figure~\ref{fig:2x2} for degree $p=3$ and maximum continuity. In this case, a simple computation gives that the dimension of the hierarchical spaces with boundary conditions is $\dim (\What^0_N) = 147$, $\dim (\What^1_N) = 328$, $\dim(\What^2_N) = 181$, which violates the previous condition.

%% \begin{figure}[ht]
%% \centerline{\includegraphics[width=0.45\textwidth]{refined_2x2}}
%% \caption{A hierarchical mesh for which the sequence is not exact, for $p=3$.}
%% \label{fig:2x2}
%% \end{figure}

%% The exactness of the sequence is crucial for the correct behavior of discretization schemes based on this discrete complex. {\Rd REWRITE For instance, if the spaces of the complex are to be used for the solution of mixed problems, working with a non-exact sequence may deteriorate the inf-sup stability constant at each refinement step}. Losing the exactness of the sequence may also lead to spurious solutions, as we will see in the examples of Section~\ref{sec:tests} for the solution of Maxwell eigenvalue problem.

%% In the next sections we provide conditions to guarantee that the hierarchical spline spaces form an exact de Rham complex.

%% \subsection{The Hierarchical Spline Complex in the Physical Domain}
%% The hierarchical spline complex in the physical domain is built in exactly the same manner as the B-spline complex.  Namely, we simply use the pullback operators defined in Subsection \ref{subsec:pullback}, yielding:
%% \begin{equation*}
%% W_\ell^k := \left\{ \omega : \iota^k(\omega) \in \Xhath{k} \right\}
%% \end{equation*}
%% for all integers $0 \leq k \leq n$ and $0 \leq \ell \leq N$.

%% \subsection{Extension to Multi-patch Geometries}
%% {\color{blue} \textbf{Remarks (John):} This is not the worst ever, but it may be pretty confusing for the new reader.  Though at this point, I am not sure I care so much about the new reader =).}\\

%% {\Rd I DON'T LIKE THIS SECTION, BUT IT IS A STARTING POINT}

%% {\Rd WE SHOULD DISCUSS ABOUT THE FIGURES.}

%% Most geometries of scientific and engineering interest cannot be represented as the image of the unit domain. For complex geometries we invoke the multi-patch concept. We assume that there exist $n_p$ smooth parametrizations of the form
%% \[
%% {\bf F}^{(j)} : (0,1)^n \rightarrow \Omega^{(j)} \subset \mathbb{R}^n, \quad j = 1, \ldots, n_p,
%% \]
%% such that the patches $\Omega^{(j)}$ do not overlap, then the domain is defined as the union of the $n_p$ patches
%% \[
%% \overline \Omega = \bigcup_{j=1}^{n_p} \overline {\Omega^{(j)}}.
%% \]
%% The construction of multi-patch spaces for tensor-product B-splines and conforming meshes is standard: assuming that the meshes of two adjacent patches are conforming on the interface, that is, the restriction of the parametrization and the knot vectors on the interface are the same, then $C^0$ functions for 0-forms are constructed as an equivalence of basis functions from the adjacent patches, see \cite[Section~3.5]{IGA-book}, and \cite[Section~3.2]{BBSV-acta} for the assumptions on the interface. Under the same assumptions, differential forms for B-splines on multi-patch domains can be also defined \cite[Section~5.4]{BBSV-acta}. Denoting by $(X_h^{(j)},d)$ the B-spline complex in the patch $\Omega^{(j)}$, the multi-patch spaces are given by 
%% \begin{equation} \label{eq:spline_complex_multipatch}
%% X^k_h = \{ u \in X^k : u|_{\Omega^{(j)}} \in X_h^{k,(j)} \},
%% \end{equation}
%% while in practice the basis functions are again constructed as an equivalence of basis functions between adjacent patches, plus an {\bf \emph{orientation}} for the functions associated to edges and faces of the Greville grid. The orientation of these functions can be directly associated to the entities of the Greville grid, and it works exactly as in the finite element case.

%% To define hierarchical differential forms in a multi-patch domain, one must take into account the presence of non-conforming meshes between patches \cite{Scott2014222}. This can be easily done following the approach used in \cite{Buchegger2016159} for 0-forms: we start defining a multi-patch spline complex for each level, using only tensor-product B-splines on each patch as in \eqref{eq:spline_complex_multipatch}; then we apply the hierarchical algorithm of Definition~\ref{def:hierarchical} to the multi-patch spaces of the complex, taking into account that the support of interface functions overlaps two or more patches. With this procedure, the check of the support and the orientation assignment can be done at the tensor-product level. We show an example of the construction for the mesh in Figure~\ref{fig:multipatch}, where the thick line represents the interface between both interfaces. The set of active basis functions for 0-forms is given in Figure~\ref{fig:multi_0forms}, for levels zero and one. We note the presence at level zero of an active basis function on the interface, that would not appear on the left patch when considering the patches separately. Similarly, some functions of level one on the interface are not active, but would be active on the left patch if we considered the patches separately. A similar behavior is also encountered for the 1-forms of Figure~\ref{fig:multi_1forms}.

%% \begin{figure}
%% \centerline{\includegraphics[width=0.8\textwidth, trim=5cm 4cm 4cm 3cm, clip]{multipatch_bezier}}
%% \caption{B\'ezier mesh for a simple multi-patch geometry}\label{fig:multipatch}
%% \end{figure}

%% \begin{figure}[ht]
%% \begin{subfigure}[Active basis functions of level 0]{
%% \includegraphics[width=0.49\textwidth, trim=5cm 4cm 4cm 3cm, clip]{multipatch_0forms_level1}
%% \label{fig:multi_0forms_1lev}
%% }
%% \end{subfigure}
%% \begin{subfigure}[Active basis functions of level 1]{
%% \includegraphics[width=0.49\textwidth, trim=5cm 4cm 4cm 3cm, clip]{multipatch_0forms_level2}
%% \label{fig:multi_0forms_2lev}
%% }
%% \end{subfigure}
%% \caption{Active basis functions for 0-forms, corresponding to the multi-patch example in Figure~\ref{fig:multipatch}}
%% \label{fig:multi_0forms}
%% \end{figure}

%% \begin{figure}[ht]
%% \begin{subfigure}[Active basis functions of level 0]{
%% \includegraphics[width=0.49\textwidth, trim=5cm 4cm 4cm 3cm, clip]{multipatch_1forms_level1}
%% \label{fig:multi_1forms_1lev}
%% }
%% \end{subfigure}
%% \begin{subfigure}[Active basis functions of level 1]{
%% \includegraphics[width=0.49\textwidth, trim=5cm 4cm 4cm 3cm, clip]{multipatch_1forms_level2}
%% \label{fig:multi_1forms_2lev}
%% }
%% \end{subfigure}
%% \caption{Active basis functions for 1-forms, corresponding to the multi-patch example in Figure~\ref{fig:multipatch}}
%% \label{fig:multi_1forms}
%% \end{figure}



==> paper_1/application.tex <==
In this final section, we apply the hierarchical B-spline complex to the numerical solution of two canonical problems of interest, one stemming from electromagnetics and the other from creeping flow.  For both problems, we examine the convergence properties of the hierarchical B-spline complex and its suitability for adaptive methods, and we further examine the accuracy gains hierarchical B-splines provide as compared with uniform B-splines.

\subsection{Application to Electromagnetics: The Curved L-shaped Domain}
As a first test problem, we solve the Maxwell eigenvalue problem, given in variational form by \eqref{eq:maxwell}, over the curved L-shaped domain.  This is a challenging problem as the first few eigenfunctions exhibit a strong singularity at the reentrant corner.  The problem details are adopted from Monique Dauge's webpage of benchmark computations for Maxwell equations \cite{BMAX}. The domain, shown in Figure~\ref{fig:curvedL}, is represented by three patches, and for the computations we start with a zero level mesh of $8\times 8$ element on each patch. Then, at each refinement step we refine on each patch one quarter of the (parametric) domain near the reentrant corner, to obtain a better approximation of the singularity. The meshes obtained with this refinement procedure, as the one represented in Figure~\ref{fig:curvedL} for six levels, satisfy both Assumptions~\ref{ass:support} and~\ref{ass:overlap}.

\begin{figure}[b!]
\begin{subfigure}[Mesh with six levels]
{\includegraphics[width=0.4\textwidth,trim=3cm 2.5cm 2cm 1.8cm, clip]{curved_Lshaped_mesh_6levels} \label{fig:curvedL}}
\end{subfigure}
\begin{subfigure}[Convergence of the first eigenvalue]
{\includegraphics[width=0.58\textwidth,trim=4cm 1cm 4cm 1cm, clip]{curvedL_errors} \label{fig:curvedL-results} }
% \includegraphics[width=0.48\textwidth,trim=5cm 2cm 4cm 1cm, clip]{curvedL_errors_radical}
\end{subfigure}
\caption{Curved L-shaped domain: Hierarchical B\'{e}zier mesh and convergence results.} 
\end{figure}

\begin{table}[b!]
\caption{Comparison of the first five computed eigenvalues of the curved L-shaped domain, for uniform tensor-product B-splines and hierarchical B-splines.} \label{tab:curvedL}
\centering
\begin{tabular}{|c||c|c|c|c|}
\hline
 & \multicolumn{2}{|c|}{$p_1 = p_2 = 3$} & \multicolumn{2}{|c|}{$p_1 = p_2 = 4$} \\
\cline{2-5}
Exact & Uniform & HB-splines & Uniform & HB-splines \\
\hline
1.818571152 & 1.818555761 & 1.818555754 & 1.818561623 & 1.818561620 \\
3.490576233 & 3.490576123 & 3.490576132 & 3.490576165 & 3.490576165 \\
10.06560150 & 10.06560150 & 10.06560272 & 10.06560150 & 10.06560150 \\
10.11188623 & 10.11188494 & 10.11188615 & 10.11188543 & 10.11188544 \\
12.43553725 & 12.43550823 & 12.43550992 & 12.43551928 & 12.43551928 \\
\hline
d.o.f. & 400416 & 2040 & 403522 & 2170 \\
\hline
\end{tabular}
\end{table}

We compare in Figure~\ref{fig:curvedL-results} the convergence results for the approximation of the first eigenvalue using hierarchical B-splines and tensor-product B-splines with uniform refinement, for degrees three and four. The associated eigenfunction only belongs to $H^{2/3-\epsilon}$ for any $\epsilon > 0$, which determines the convergence rate in the case of uniform B-splines. The results show much better approximation results for hierarchical B-splines, although the asymptotic regime is not reached after ten refinement steps. We also present, in Table~\ref{tab:curvedL}, the first five computed eigenvalues for the mesh of level six, and a comparison with the exact\footnote{The eigenvalues are taken from \cite{BMAX} and are correct up to 11 digits.} eigenvalues. The results are almost identical, but hierarchical B-splines require 200 times fewer degrees of freedom to obtain the same accuracy.

\begin{remark}
The results for tensor-product B-splines can be improved by generating a radical graded mesh, see \cite{Beirao_Cho_Sangalli} and \cite[Section~6]{BBSV-acta}. However, in this case the condition number strongly deteriorates due to the presence of anisotropic elements.
\end{remark}


\subsection{Application to Creeping Flow: Lid-Driven Cavity Flow}
As a second test problem, we solve the creeping lid-driven cavity flow problem.  Creeping flow is governed by the Stokes equations, given in variational form by \eqref{eq:stokes}, and the setup for the lid-driven cavity flow problem is elaborated in Figure \ref{f:lidcavitysetup}.  The left, right, and bottom sides of the cavity are fixed no-slip walls while the top side of the cavity is a wall which slides to the right with velocity magnitude $U$.  For the computations here, $H$ and $U$ are set to one.  Like the curved L-shaped domain problem described previously, the pressure and stress fields associated with the lid-driven cavity flow problem experience corner singularities which impede the convergence of numerical methods and expose unstable velocity/pressure pairs.  The velocity field is further characterized by a primary vortex near the center of the cavity and an infinite sequence of Moffatt eddies of decreasing size and intensity in the lower left and right corners of the cavity.  We demonstrate here that a discretization based on the hierarchical B-spline complex is able to both resolve the corner singularities as well as a select number of Moffatt eddies with a properly chosen adaptive strategy.

\begin{figure}[b!]
	\centering
	\includegraphics[height=3.25in]{Figures/Stokes_Cavity_Setup.pdf}
	\caption{Problem setup for creeping lid-driven cavity flow.}
	\label{f:lidcavitysetup}
\end{figure}

We have computed approximations of lid-driven cavity flow using both hierarchical B-splines and tensor-product B-splines with varying mesh size and polynomial degrees two, three, and four.  For the case of tensor-product B-splines, we employed uniform refinement to resolve the features of the flow.  The computed streamlines for $h = 1/32$ and $h = 1/128$ with $p_1 = p_2 = 2$ are shown in Figure~\ref{f:tensorprodstreamlines}. Note that while the first Moffatt eddy is apparent in the $h = 1/32$ mesh, it is highly distorted.  The second Moffatt eddy does appear in the $h = 1/128$ mesh, but the third cannot be calculated using tensor-product B-splines until a mesh resolution of $h = 1/1024$.  For the case of hierarchical B-splines, we began with a uniform tensor-product B-spline mesh and applied three levels of hierarchical refinement in each of the corners of the domain as illustrated in Figure~\ref{f:lidcavityhierarchicalmesh}.  The computed streamlines for $h = 1/32$ and $h = 1/128$ with $p_1 = p_2 = 2$ are shown in Figure~\ref{f:hierarchicalstreamlines}, where $h$ indicates the element size for the initial tensor-product B-spline mesh and hence is the maximal element size for the hierarchical mesh.  Note that both the first and second Moffatt eddies are well-resolved for the $h = 1/32$ mesh, and the third Moffatt eddy can also be observed for the $h = 1/128$ mesh.  Consequently, while 3,153,925 degrees of freedom are necessary to capture the third Moffatt eddy with uniform tensor-product B-splines, one can capture the eddy with hierarchical B-splines using only $93,381$ degrees of freedom.  This is more than a thirty-fold reduction in total number of degrees of freedom.  It should be noted that the fourth Moffatt eddy cannot be obtained with double precision floating point arithmetic as the magnitudes of the velocities of the eddies are simply too small (below $1e{-12}$).

\begin{figure}[t]
	\centering
	\includegraphics[height=2.75in]{stokes_lid_driven/Lid_Driven_3_Level_Refine_Corners_Elem32.png}
	\caption{Hierarchical refinement strategy for the creeping lid-driven cavity flow problem.  The displayed hierarchical B\'{e}ziermesh corresponds to $h = 1/32$ where $h$ is the element size for the initial tensor-product B-spline mesh.}
	\label{f:lidcavityhierarchicalmesh}
\end{figure}

%
% Figure of stream functions for tensor product mesh of lid-driven cavity flow for k' = 1
\begin{figure}[t]
	\centering

	\subfigure[{$[0,1] \times [0,1]$, $h = 1/32$}]{\includegraphics[height=2.3in]{stokes_lid_driven/Lid_Driven_Streamlines_p2_elem32_tensorprod.png}\label{f:tensorprodstreamlinesh32}}
	\qquad
	\subfigure[{$[0,0.0073] \times [0,0.0073]$, $h = 1/32$}]{\includegraphics[height=2.3in]{stokes_lid_driven/Lid_Driven_Streamlines_p2_elem32_tensorprod_Zoom.png}\label{f:tensorprodstreamlinesh32zoom}}
	
	\subfigure[{$[0,1] \times [0,1]$, $h = 1/128$}]{\includegraphics[height=2.3in]{stokes_lid_driven/Lid_Driven_Streamlines_p2_elem128_tensorprod.png}\label{f:tensorprodstreamlinesh128}}
	\qquad
	\subfigure[{$[0,0.0073] \times [0,0.0073]$, $h = 1/128$}]{\includegraphics[height=2.3in]{stokes_lid_driven/Lid_Driven_Streamlines_p2_elem128_tensorprod_Zoom.png}\label{f:tensorprodstreamlinesh128zoom}}

	\caption{Streamlines for the creeping lid-driven cavity problem obtained from tensor-product B-splines with $p_1 = p_2 = 2$. The first Moffatt eddies can be seen in the corners of the domain, while a second Moffatt eddy is shown by zooming in to the lower-left corner of the domain.}
	\label{f:tensorprodstreamlines}
\end{figure}

%
% Figure of stream functions for hierarchical mesh of lid-driven cavity flow for k' = 1
\begin{figure}[t]
	\centering

	\subfigure[{$[0,1] \times [0,1]$, $h = 1/32$}]{\includegraphics[height=2.3in]{stokes_lid_driven/Lid_Driven_Streamlines_p2_elem32_locref3.png}\label{f:hierarchicalstreamlinesh32}}
	\qquad
	\subfigure[{$[0,0.0073] \times [0,0.0073]$, $h = 1/32$}]{\includegraphics[height=2.3in]{stokes_lid_driven/Lid_Driven_Streamlines_p2_elem32_locref3_Zoom.png}\label{f:hierarchicalstreamlinesh32zoom}}
	
	\subfigure[{$[0,1] \times [0,1]$, $h = 1/128$}]{\includegraphics[height=2.3in]{stokes_lid_driven/Lid_Driven_Streamlines_p2_elem128_locref3.png}\label{f:hierarchicalstreamlinesh128}}
	\qquad
	\subfigure[{$[0,0.0073] \times [0,0.0073]$, $h = 1/128$}]{\includegraphics[height=2.3in]{stokes_lid_driven/Lid_Driven_Streamlines_p2_elem128_locref3_Zoom.png}\label{f:hierarchicalstreamlinesh128zoom}}

	\caption{Streamlines for the creeping lid-driven cavity problem obtained from thrice-refined hierarchical B-splines with $p_1 = p_2 = 2$ (see Figure~\ref{f:lidcavityhierarchicalmesh}). The first Moffatt eddies can be seen in the corners of the domain, while a second and a third Moffatt eddy are shown by zooming in to the lower-left corner of the domain.}
	\label{f:hierarchicalstreamlines}
\end{figure}

To examine how well hierarchical B-splines and tensor-product B-splines resolve the corner singularities in the lid-driven cavity flow problem, we also compared the vorticity solution $(\omega = \textnormal{curl} \hspace{3pt} \mathbf{u}_{h})$ obtained by these approaches near the upper right corner of the cavity with the highly accurate pseudospectral results obtained in \cite{BoPe98}.  The results of this study are shown in Table~\ref{t:StokesLidDriven}.  From these results, it is apparent that hierarchical B-splines are much more effective in capturing the corner singularities than tensor-product B-splines.  For example, when $h = 1/256$ and $p_1 = p_2 = 4$, the hierarchical B-spline results match the pseudospectral results up to six significant digits.  This is particularly impressive when taking into consideration that the pseudospectral results were obtained using a subtraction of the leading terms of the asymptotic solution of the Stokes equations in order to exactly represent the corner singularities.


%
% Table of Lid-driven cavity flow
\begin{table}
\caption{Vorticity values at the point $\mathbf{x} = (0,0.95)$ and computational expense associated with tensor-product B-splines and hierarchical B-splines as applied to the creeping lid-driven cavity flow problem.}\label{t:StokesLidDriven}
\centering
Polynomial Degree $p_1 = p_2 = 2$ \\
\begin{tabular}{ l c c c}
\hline
Method  & $\omega$ & No. Elements & No. Unknowns \\
\hline
Tensor product B-splines, $h = 1/32$	 & 18.07580 & 1,024	 & 3,333 \\
Tensor product B-splines, $h = 1/64$ 	 & 19.18682 & 4,096	 & 12,805\\
Tensor product B-splines, $h = 1/128$ & 23.47947 & 16,384 & 50,181\\
Tensor product B-splines, $h = 1/256$ & 25.42558 & 65,536 & 198,661\\
\hline
Hierarchical B-splines, $h = 1/32$ 	& 23.59458 & 1,924 	& 6,033 \\
Hierarchical B-splines, $h = 1/64$ 	& 25.47702 & 7,696 	& 23,605 \\
Hierarchical B-splines, $h = 1/128$ 	& 26.38816 & 30,784 & 93,381 \\
Hierarchical B-splines, $h = 1/256$ 	& 26.83601 & 123,136 & 371,461 \\
\hline
Pseudospectral (Ref. \cite{BoPe98}) & 27.27901 & --- & --- \\
\hline
\end{tabular}

\vspace{12pt}
Polynomial Degree $p_1 = p_2 = 3$ \\
\begin{tabular}{ l c c c}
\hline
Method  & $\omega$ & No. Elements & No. Unknowns \\
\hline
Tensor product B-splines, $h = 1/32$	 & 33.27731 & 1,024	 & 3,536 \\
Tensor product B-splines, $h = 1/64$ 	 & 35.01708 & 4,096	 & 13,200 \\
Tensor product B-splines, $h = 1/128$ & 25.84879 & 16,384 & 50,960 \\
Tensor product B-splines, $h = 1/256$ & 27.34235 & 65,536 & 200,208\\
\hline
Hierarchical B-splines, $h = 1/32$ 	& 27.54476 & 1,924 	& 6,236 \\
Hierarchical B-splines, $h = 1/64$ 	& 27.33604 & 7,696 	& 24,000\\
Hierarchical B-splines, $h = 1/128$ 	& 27.29035 & 30,784 & 94,160\\
Hierarchical B-splines, $h = 1/256$ 	& 27.28284 & 123,136 & 373,008\\
\hline
Pseudospectral (Ref. \cite{BoPe98}) & 27.27901 & --- & --- \\
\hline
\end{tabular}

\vspace{12pt}
Polynomial Degree $p_1 = p_2 = 4$ \\
\begin{tabular}{ l c c c}
\hline
Method  & $\omega$ & No. Elements & No. Unknowns \\
\hline
Tensor product B-splines, $h = 1/32$	 & 22.52289 & 1,024	 & 3,745 \\
Tensor product B-splines, $h = 1/64$ 	 & 30.29182 & 4,096	 & 13,601 \\
Tensor product B-splines, $h = 1/128$ & 29.32455 & 16,384 & 51,745 \\
Tensor product B-splines, $h = 1/256$ & 27.64269 & 65,536 & 201,761 \\
\hline
Hierarchical B-splines, $h = 1/32$ 	& 27.25594 & 1,924 	& 6,445\\
Hierarchical B-splines, $h = 1/64$ 	& 27.28393 & 7,696 	& 24,401\\
Hierarchical B-splines, $h = 1/128$ 	& 27.27935 & 30,784 & 94,945\\
Hierarchical B-splines, $h = 1/256$ 	& 27.27905 & 123,136 & 374,561\\
\hline
Pseudospectral (Ref. \cite{BoPe98}) & 27.27901 & --- & --- \\
\hline
\end{tabular}

\end{table}


==> paper_1/conclusion.tex <==
In this paper, we introduced the hierarchical B-spline complex of isogeometric discrete differential forms for arbitrary spatial dimension.
By appealing to abstract cohomology theory, we derived a sufficient and necessary condition guaranteeing exactness of the hierarchical B-spline complex for arbitrary spatial dimension, and we presented an intuitive interpretation of this condition based on the topologies of the Greville grids associated with various levels of a hierarchical B-spline discretization.  We further derived a set of local, easy-to-compute, and sufficient exactness conditions for the two-dimensional setting, and we demonstrated via example that the hierarchical B-spline complex yields stable approximations of both the Maxwell eigenproblem and Stokes problem provided these local exactness conditions are satisfied.  We concluded by providing numerical results in the context of electromagnetics and creeping flow.

In future work, we plan to continue the analysis of the hierarchical B-spline complex.  First, we plan to extend our local, easy-to-compute, and sufficient exactness conditions to the three-dimensional setting.  We anticipate that this will be an exceptionally technical exercise if we follow the method of proof employed in this paper.  However, we expect that a more intelligent use of cohomology theory may yield a much simpler proof that also extends to arbitrary spatial dimension.  Second, we seek to construct commuting projection operators which make the spaces of hierarchical B-spline complex conform to a commutative de Rham diagram.  It is expected that not all hierarchical B-spline complexes will admit such commuting projection operators, though based on the results presented here, we believe that hierarchical B-spline complexes satisfying the local exactness conditions presented in this paper will.  This belief is further strengthened by the fact that hierarchical B-spline spaces satisfying our local exactness conditions are complete in that they contain all piecewise polynomial functions on the hierarchical grid with the smoothness specified by the grid and underlying polynomial degree \cite{Mokris2014}.

We also plan to further explore application of the hierarchical B-spline complex in the adaptive isogeometric solution of vector field problems such as those arising in electromagnetics and incompressible fluid flow.  In this direction, we first seek to develop refinement algorithms which yield hierarchical B-spline complexes satisfying the local exactness conditions presented in this paper with a minimal level of added degrees of freedom.   We additionally seek to develop appropriate error estimators for use in vector field problems, drawing inspiration from finite element exterior calculus \cite{Demlow14}.

==> paper_1/conclusion_modified.tex <==
We have introduced a new discrete method based on spline spaces satisfying a de Rham complex. Thanks to the high continuity of splines, the dual complex is defined with a simple change of degree, and without explicitly constructing a dual mesh. Since B-splines are defined by tensor-product, the method works in arbitrary dimensions and exterior derivatives are always given by incidence matrices of a Cartesian mesh, even for curved domains. The method is completed by discrete Hodge--star operators linking the primal and the dual complex. We have introduced three different such operators: two global ones, and a third local one, with an improved sparsity pattern. We have analyzed the discretization error and the order of the method applied to an elliptic problem, for the three different choices, following a variational approach. We have proved that, with the first choice, the method is equivalent to the standard Galerkin method used in IGA, whose same order of convergence is attained. For the other two choices the expected order of convergence is attained, lower by one due to the lower degree of splines in the dual complex. 

% In a forthcoming paper we will analyze the method for the solution of the time domain Maxwell's equations. So far, the method is restricted to the case of a single patch, i.e., the domain is the image of the parametric domain through a given parameterization. 
\textcolor{magenta}{In a forthcoming paper, we will build on the present work heavily to devise schemes for the geometric integration of hyperbolic systems of equations.
More generally in future work we aim to extend it to geometries formed by multiple patches and domains comprising different materials. The difficulty lies there in the regularity across patches, which is usually $C^0$. In such cases it is not clear how the dual complex can be constructed by a simple change of degree.}
% The same issue arises when the domain is formed by multiple materials, and we expect that the necessary modifications will be the same for both cases.


==> paper_1/derham.tex <==
%\noindent {\color{blue} \textbf{Assigned Author(s):} Evans, Thomas, and Vazquez}\\

%\noindent {\color{blue} \textbf{Synopsis:} Provide background on the de Rham complex and present basic mathematical notation.  In addition, discuss how physical vector quantities (e.g., magnetic field, electric field, velocity field, pressure field) belong to the various Sobolev spaces in the complex.  For now, we can be brief as we are targeting a more mathematical audience, but we also do not want to completely lose the general isogeometric community (yet).}

In this section, we introduce the de Rham complex of differential forms and present basic mathematical notation.
%In addition, we demonstrate how physical vector quantities arising in continuum mechanics (e.g., magnetic fields, electric fields, velocity fields, and pressure fields) belong to various spaces appearing in the de Rham complex.  As such, the de Rham complex provides a natural mathematical setting for the discretization of vector fields.
Before explicitly defining the de Rham complex, we first introduce the more general concept of a Hilbert complex.  Our presentation largely follows \cite[Sections~3 and 4]{AFW-2}, so the interested reader is referred to that work for a more thorough introduction.

\subsection{Hilbert Complexes and Subcomplexes}

A {\bf \emph{Hilbert complex}} $\left( V, d \right)$ is a sequence of Hilbert spaces $\left\{V^k\right\}_{k=0}^n$ connected by a set of closed linear maps $d^k: V^k \rightarrow V^{k+1}$ such that the composition of any two consecutive maps is zero (that is, $d^k \circ d^{k-1} = 0$ for $k = 0, \ldots, n-1$).  A Hilbert complex is typically written as
\begin{equation} \label{eq:complex}
\begin{CD}
V^0 @>d^0>> V^1 @>d^1>> V^2 @>d^2>> \ldots @>d^{n-1}>> V^n.
\end{CD}
\end{equation}
%Note that the first and last spaces in the above sequence are {\bf \emph{trivial}} in that they only contain zero.
The elements of the kernel of $d^k$ are called {\bf \emph{closed forms}}, and we denote $Z^k(V) \equiv Z^k(V,d) = \ker\left(d^k\right)$.  The elements of the range of $d^{k-1}$ are called {\bf \emph{exact forms}}, and we denote $B^k(V) \equiv B^k(V,d) = \Ima\left(d^{k-1}\right)$.  
%It is implied that the space $Z^n(V) = V^n$ and the space $B^0(V)$ is trivial (that is, the only member of $B^0(V)$ is zero).  
The $k^{\textup{th}}$ {\bf \emph{cohomology group}} is given by the quotient space $H^k(V) \equiv H^k(V,d) = Z^k(V)/B^k(V)$.  When the cohomology groups are all trivial, we say that the sequence is {\bf \emph{exact}}.  We will deal with exact Hilbert complexes extensively in this work.

A Hilbert complex is said to be {\bf \emph{bounded}} if, for each $k$, $d^k$ is a bounded operator from $V^k$ to $V^{k+1}$, and a Hilbert complex is said to be {\bf \emph{closed}} if, for each $k$, the range of $d^k$ is closed in $V^{k+1}$.  Finite-dimensional Hilbert complexes are bounded and closed by construction, but infinite-dimensional Hilbert complexes are generally neither closed nor bounded.  Most of the Hilbert complexes presented in this paper, including the de Rham complex, are bounded and closed.

Utilizing the inner product structure of the Hilbert space $V^k$, we define the space of {\bf \emph{harmonic forms}} as $\mathfrak{h}^k(V) = Z^k(V) \cap \left(B^k(V)\right)^\perp$ where $\left(B^k(V)\right)^\perp$ is the {\bf \emph{orthogonal complement}} to $B^k(V)$ with respect to the inner-product defined on $V^k$.  For a closed Hilbert complex, the space of harmonic forms $\mathfrak{h}^k(V)$ is isomorphic to the cohomology group $H^k(V)$, and we have the {\bf \emph{Hodge decomposition}}:
\begin{equation*}
V^k = B^k(V) \oplus \left(Z^k(V)\right)^\perp \oplus \mathfrak{h}^k(V).
\end{equation*}
As most of the Hilbert complexes presented in this paper are closed, we will employ cohomology groups and harmonic forms interchangeably in our mathematical analysis.

We finish here by defining the notion of a Hilbert {\bf \emph{subcomplex}}.  We say that $(V_h,d)$ is a subcomplex of $(V,d)$ if $V_h^k \subset V^k$ for $k = 0, \ldots, n$ and $d^k(V_h^k) \subset V_h^{k+1}$ for $k = 0, \ldots, n-1$.  An important fact to note is that a subcomplex of a given Hilbert complex may not share its cohomology structure.  More specifically, the cohomology groups of the subcomplex may not be equal to the cohomology groups of the parent Hilbert complex, and in fact, the cohomology groups of the subcomplex may not even be isomorphic to the cohomology groups of the parent Hilbert complex.  Consequently, a subcomplex of an exact Hilbert complex may not be exact.

\subsection{The de Rham Complex of Differential Forms}

We are now in a position to define the {\bf \emph{de Rham complex}} of {\bf \emph{differential forms}}.  As previously mentioned, the de Rham complex is an example of a bounded and closed Hilbert complex, and to distinguish between the de Rham complex and the more general notion of a Hilbert complex, we employ the notation $\left(X(D), d\right)$ where $D$ is a domain of interest.

Before proceeding, let us briefly review the concepts of {\bf \emph{differential $\textbf{k}$-forms}} and {\bf \emph{exterior derivative operators}}.  We restrict our discussion to the Euclidean setting, but the foundational ideas also extend to the setting of smooth manifolds (see \cite[Section~4.1]{AFW-2} for more details).  With this in mind, let $D \subset \mathbb{R}^n$ be a given open domain.  For such a domain, a differential $0$-form is simply a function $\omega: D \rightarrow \mathbb{R}$, and a differential $1$-form is a function
\begin{equation*}
\omega = \sum_{\alpha=1}^{n} \omega_{\alpha} dx_{\alpha},
\end{equation*}
where $\omega_{\alpha}: D \rightarrow \mathbb{R}$ for $\alpha = 1, \ldots, n$ and $dx_{\alpha}: \mathbb{R}^n \rightarrow \mathbb{R}$ is the linear form which associates to a vector its $\alpha^{\textup{th}}$ coordinate.  Note that we may also view $dx_{\alpha}$ as a differential length element or, more specifically, the differential change in the $\alpha^{\textup{th}}$ spatial coordinate.  With this in mind, we can also define differential surface elements $dx_{\alpha_1} \wedge dx_{\alpha_2}$ and differential volume elements $dx_{\alpha_1} \wedge dx_{\alpha_2} \wedge dx_{\alpha_3}$ where it is assumed that $\alpha_1 < \alpha_2 < \alpha_3$\footnote{It should be noted that under the assumption that $\alpha_1 < \alpha_2$, the differential surface elements $dx_{\alpha_1} \wedge dx_{\alpha_2}$ may not be positively oriented for the standard orientation on $\mathbb{R}^n$, and this is also true for general $k$-forms $dx_{\alpha_1} \wedge dx_{\alpha_2} \wedge \cdots \wedge dx_{\alpha_k}$ with $\alpha_1 < \alpha_2 < \ldots < \alpha_k$.  For instance in the three-dimensional setting, $dx_1 \wedge dx_2$ and $dx_2 \wedge dx_3$ are positively oriented while $dx_1 \wedge dx_3$ is negatively oriented.  That being said, the assumption of ordered multi-indices dramatically simplifies our later presentation.}, and these elements comprise a basis for differential $2$-forms and differential $3$-forms respectively.  Generally, for $k > 1$, a differential $k$-form is a function
\begin{equation*}
\omega = \sum_{\boldsymbol \alpha \in \mathcal{I}_k} \omega_{\boldsymbol \alpha} dx_{\alpha_1} \wedge dx_{\alpha_2} \wedge \cdots \wedge dx_{\alpha_k},
\end{equation*}
where $\omega_{\boldsymbol \alpha}: D \rightarrow \mathbb{R}$, $\boldsymbol \alpha = (\alpha_1, \alpha_2, \ldots, \alpha_k)$ is a multi-index, and $\mathcal{I}_k$ is the set of ordered multi-indices
\begin{equation*}
\mathcal{I}_k = \left\{ \boldsymbol \alpha = (\alpha_1, \alpha_2, \ldots, \alpha_k): 1 \leq \alpha_1 < \alpha_2 < \ldots < \alpha_k \leq n \right\}.
\end{equation*}
Up to this point, we have assumed that $\alpha_1 < \alpha_2 < \ldots < \alpha_k$ when defining the differential basis $k$-form $dx_{\alpha_1} \wedge dx_{\alpha_2} \wedge \cdots \wedge dx_{\alpha_k}$.  However, we may break this assumption if we define
\begin{equation*}
dx_{\alpha_1} \wedge dx_{\alpha_2} \wedge \cdots \wedge dx_{\alpha_k} = \textup{sgn}(\sigma) dx_{\sigma(\alpha_1)} \wedge dx_{\sigma(\alpha_2)} \wedge \ldots \wedge dx_{\sigma(\alpha_k)},
\end{equation*}
where $\sigma: \left\{\alpha_1, \alpha_2, \ldots, \alpha_k\right\} \rightarrow \left\{\alpha_1, \alpha_2, \ldots, \alpha_k\right\}$ is an arbitrary permutation of the set $\left\{\alpha_1, \alpha_2, \ldots, \alpha_k\right\}$ and $\textup{sgn}(\sigma)$ is its sign (+1 if there is an even number of pairs $\alpha_i < \alpha_j$ such that $\sigma(\alpha_i) > \sigma(\alpha_j)$ and -1 otherwise).  Note that this implies
\begin{equation*}
dx_{\alpha_1} \wedge dx_{\alpha_2} \wedge \cdots \wedge dx_{\alpha_k} = 0
\end{equation*}
if $\alpha_i = \alpha_j$ for some $i \neq j$.  With these conventions in mind, we define the {\bf \emph{wedge product}} between a differential $k$-form and a differential $l$-form as
\begin{equation*}
\omega \wedge \eta = \sum_{\boldsymbol \alpha \in \mathcal{I}_k} \sum_{\boldsymbol \beta \in \mathcal{I}_l} \omega_{\boldsymbol \alpha} \eta_{\boldsymbol \beta} dx_{\alpha_1} \wedge \ldots \wedge dx_{\alpha_k} \wedge dx_{\beta_1} \wedge \ldots \wedge dx_{\beta_l},
\end{equation*}
and the result is a differential $(k+l)$-form. We note that the wedge product generalizes the notion of cross product to arbitrary dimension. %, and indeed we note that:
%\begin{equation*}
%\omega \wedge \eta = \sum_{1 \leq \alpha < \beta \leq n} \left( \omega_{\alpha} \eta_{\beta} - \omega_{\beta} \eta_{\alpha} \right) dx_{\alpha} \wedge dx_{\beta}
%\end{equation*}
%for two differential $1$-forms $\omega = \sum_{\alpha=1}^{n} \omega_{\alpha} dx_{\alpha}$ and $\eta = \sum_{\beta=1}^{n} \eta_{\beta} dx_{\beta}$.  Further note that the wedge product between a differential $k$-form and a differential $l$-form yields a differential $(k+l)$-form.
We are now finally ready to define the exterior derivative operator for a differential $k$-form.  The exterior derivative of a differential $0$-form, which is also referred to as the {\bf \emph{differential}}, is defined as
\begin{equation*}
d\omega = \sum_{\alpha=1}^n \frac{\partial \omega}{\partial x_{\alpha}} dx_\alpha,
\end{equation*}
while the exterior derivative of a differential $k$-form for $k > 0$ is defined as
\begin{equation*}
d^k \omega = \sum_{\boldsymbol \alpha \in \mathcal{I}_k} d\omega_{\boldsymbol \alpha} \wedge dx_{\alpha_1} \wedge dx_{\alpha_2} \wedge \cdots \wedge dx_{\alpha_k},
\end{equation*}
where we note $d\omega_{\boldsymbol \alpha}$ is the differential of the differential $0$-form $\omega_{\boldsymbol \alpha}$.  For ease of notation, we interchangeably write the exterior derivative of a differential $k$-form $\omega$ as $d\omega$ and $d^k\omega$.  Note that, by construction, the exterior derivative of a differential $k$-form is a differential $(k+1)$-form, and we also have that the composition of two exterior derivatives is identically zero (i.e, $d^k \circ d^{k-1} = 0$).  

To construct the de Rham complex, we need to endow differential $k$-forms with Hilbert space structure.  To do so, we first define the space of {\bf \emph{smooth}} differential $k$-forms as $\Lambda^k(D)$, and we define an $L^2$-inner product between two smooth differential $k$-forms as
\begin{equation*}
\left( \omega, \eta \right)_{L^2 \Lambda^k(D)} =  \sum_{\boldsymbol \alpha \in \mathcal{I}_k} \int_D \omega_{\boldsymbol \alpha} \eta_{\boldsymbol \alpha} dD.
\end{equation*}
If we take the completion of $\Lambda^k(D)$ with respect to the above inner-product, we obtain a Hilbert space which we denote as $L^2 \Lambda^k(D)$.  Now, let us define
\begin{equation*}
X^k(D) = \left\{ \omega \in L^2\Lambda^k(D) : d^k \omega \in L^2\Lambda^{k+1}(D) \right\},
\end{equation*}
which is a Hilbert space equipped with the inner-product
\begin{equation*}
\left( \omega, \eta \right)_{X^k(D)} = \left( \omega, \eta \right)_{L^2 \Lambda^k(D)} + \left( d^k \omega, d^k \eta \right)_{L^2 \Lambda^{k+1}(D)}.
\end{equation*}
With the above notation established, we see that we have arrived at a bounded and closed Hilbert complex of the form:
\begin{equation} \label{eq:derhamcomplex}
\begin{CD}
X^0(D) @>d^0>> X^1(D) @>d^1>> X^2(D) @>d^2>> \ldots @>d^{n-1}>> X^n(D).
\end{CD}
\end{equation}
We refer to the above as the $L^2$ de Rham complex of differential forms or simply the de Rham complex for short.

The meaning of the de Rham complex is most evident in the two- and three-dimensional settings.  Here, all differential $k$-forms may be viewed as either scalar or vector {\bf \emph{proxy}} fields  (see \cite[Section~4.2]{AFW-2} for more details).  Via proxy fields, the exterior derivatives coincide with standard differential operators of calculus.  For a three-dimensional domain $D \subset \mathbb{R}^3$, we find that
\begin{equation*}
d^0 = \grad, \hspace{15pt} d^1 = \curl, \hspace{15pt} d^2 = \div,
\end{equation*}
and the de Rham complex becomes:
\begin{equation} \label{eq:derhamcomplex_3D}
\begin{CD}
H^1(D) @>\grad>> {\bf H}(\curl, D) @>\curl>> {\bf H}(\div, D) @>\div>> L^2(D).
\end{CD}
\end{equation}
For a two-dimensional domain $D \subset \mathbb{R}^2$, we find that
\begin{equation*}
d^0 = \grad, \hspace{15pt} d^1 = \curls,
\end{equation*}
and the de Rham complex becomes:
\begin{equation} \label{eq:derhamcomplex_2D}
\begin{CD}
H^1(D) @>\grad>> {\bf H}(\curls, D) @>\curls>> L^2(D).
\end{CD}
\end{equation}
Consequently, the de Rham complex provides an algebraic framework for vector calculus in the two- and three-dimensional settings.  We will often work with proxy fields in the paper as they are both easier to intuit and to visualize.

In the two-dimensional setting, one can also consider the {\bf \emph{rotated de Rham complex}}, that is, the standard de Rham complex rotated by $\pi/2$, that takes the form:
\begin{equation} \label{eq:stokescomplex_2D}
\begin{CD}
H^1(D) @>\rot>> {\bf H}(\div,D) @>\div>> L^2(D),
\end{CD}
\end{equation}
where $\rot$ is the {\bf \emph{rotor}} or {\bf \emph{perpendicular gradient}} operator.  The rotated de Rham complex is particularly useful in the development of discretization methodologies for the mixed form of the Laplacian operator, and as we will later see, it also provides a natural framework for incompressible fluid flow.

In this work, we will primarily work with de Rham complexes of differential forms subject to {\bf \emph{homogeneous}} or {\bf \emph{vanishing boundary conditions}}.  Such complexes are built from spaces of differential $k$-forms with {\bf \emph{compact support}} in exactly the same manner as that above.  We denote de Rham complexes with vanishing boundary boundary conditions by $(X_0(D),d)$, and we write:
\begin{equation} \label{eq:derhamcomplex_homogeneous}
\begin{CD}
X^0_0(D) @>d^0>> X^1_0(D) @>d^1>> X^2_0(D) @>d^2>> \ldots @>d^{n-1}>> X^n_0(D).
\end{CD}
\end{equation}
Through the use of proxy fields, the de Rham complex $(X_0(D), d)$ is comprised of the spaces
\begin{equation*}
X^0_0(D) = H^1_0(D), \; X^1_0(D) = {\bf H}_0(\curls, D), \; X^2_0(D) = L^2(D),
\end{equation*}
for a two-dimensional domain $D \subset \mathbb{R}^2$, and
\begin{equation*}
X^0_0(D) = H^1_0(D), \; X^1_0(D) = {\bf H}_0(\curl, D), \; X^2_0(D) = {\bf H}_0(\div, D), \; X^3_0(D) = L^2(D),
\end{equation*}
for a three-dimensional domain $D \subset \mathbb{R}^3$.

In the setting when the domain $D$ is {\bf \emph{contractible}}, the de Rham complexes presented above have special structure.  Specifically, when the domain $D$ is contractible, the {\bf \emph{extended de Rham complexes}}
\begin{equation*}
\begin{CD}
0 @>>> \mathbb{R} @>\subset>> X^0(D) @>d^0>> X^1(D) @>d^1>> X^2(D) @>d^2>> \ldots @>d^{n-1}>> X^n(D) @>>> 0,
\end{CD}
\end{equation*}
and
\begin{equation*}
\begin{CD}
0 @>>> X^0_0(D) @>d^0>> X^1_0(D) @>d^1>> X^2_0(D) @>d^2>> \ldots @>d^{n-1}>> X^n_0(D) @>\int>> \mathbb{R} @>>> 0
\end{CD}
\end{equation*}
are exact.  Consequently, in this setting, all of the cohomology groups of the de Rham complex $(X(D),d)$ are trivial except for $H^0(X(D)) = \mathbb{R}$, and all of cohomology groups of the de Rham complex $(X_0(D),d)$ are trivial except for $H^n(X_0(D)) = \mathbb{R}$.  When the domain $D$ is not contractible, the extended de Rham complexes presented above are no longer exact.  However, the structure of the cohomology groups is well-understood in this more general setting.  Namely, $\dim H^k(X(D)) = \dim H^{n-k}(X_0(D)) = \beta_k$, where $\beta_k$ is the $k^{\textup{th}}$ {\bf \emph{Betti number}} for the domain $D$.  Recall the zeroth Betti number is the number of connected components in the domain, the first Betti number is the number of one-dimensional or ``circular'' holes in the domain, and the second Betti number is the number of two-dimensional ``voids'' or ``cavities'' in the domain.  Betti numbers exist for more general  topological spaces including graphs, and the topological meaning of the Betti number will be implicitly exploited throughout this paper in establishing theoretical results for discrete spaces of differential forms.

\subsection{The Parametric Domain, The Physical Domain, and Pullback Operators}
\label{subsec:pullback}
Throughout this paper, we will work with a particular open domain, $\hat \Omega = (0,1)^n$, which we refer to as the {\bf \emph{parametric domain}}.  It is most natural in the isogeometric setting to first define discretizations over the parametric domain $\hat \Omega$ and then map these to a {\bf \emph{physical domain}} $\Omega \subset \mathbb{R}^n$ using a parametric mapping $\textbf{F}: \hat \Omega \rightarrow \Omega$.  Given the frequency with which we will work with the parametric domain, we will denote the de Rham complex corresponding to the parametric domain by $(\hat{X}(\hat \Omega),d)$ or simply $(\hat{X},d)$.

We relate differential $k$-forms in the parametric domain to differential $k$-forms in the physical domain using a set of {\bf \emph{pullback operators}} $\iota^k: X^k(\Omega) \rightarrow \hat{X}^k(\hat{\Omega})$.  The pullback operator for differential $0$-forms takes the form $\iota^0(\omega) = \omega \circ \textbf{F}$ for all $\omega \in X^0(\Omega)$, while the pullback operator for differential $n$-forms takes the form $\iota^n(\omega) = \det(D\textbf{F}) \left(\omega \circ \textbf{F}\right)$ for all $\omega \in X^n(\Omega)$ where $D\textbf{F}$ is the Jacobian matrix of the mapping $\textbf{F}$.  The exact form of the pullback operator for other differential $k$-forms is more involved, and the interested reader is referred to \cite[Section~2]{AFW06} for more details.  The pullback operators are commutative in the sense that $d^k \circ \iota^k = \iota^{k+1} \circ d^k$.  Consequently, the following commutative de Rham diagram is satisfied:
\begin{equation}
\begin{CD}
\Xhat^0(\hat \Omega) @>d^0>> \Xhat^1(\hat \Omega) @>d^1>> \ldots @>d^{n-1}>> \Xhat^n(\hat \Omega) \\
@A\iota^0AA @A\iota^1AA @. @A\iota^nAA  \\
X^0(\Omega) @>d^0>> X^1(\Omega) @>d^1>> \ldots @>d^{n-1}>> X^n(\Omega).
\end{CD}
\end{equation}
The commutative property of the pullback operators will be exploited when defining the spline complex of discrete differential forms in the physical domain.

\subsection{Application of the de Rham Complex in Electromagnetics and the Stokes Complex for Incompressible Fluid Mechanics}
The most prominent application of differential forms in numerical analysis is in computational electromagnetism. Bossavit formulated Maxwell's equations in terms of differential forms in \cite{BOS88}, and he established a link between {\bf\emph{Whitney forms}}, developed in the computational geometry community, and low-order finite element methods used in computational electromagnetics. Specifically, he showed the electric and magnetic field intensities may be represented as differential 1-forms which can be further approximated through edge finite elements, while the magnetic induction and the electric displacement may be represented as differential 2-forms which can be approximated with face finite elements. The computational electromagnetics community has further developed this connection, and it is now common to introduce finite element schemes as discrete differential forms (see \cite{AFW-2,HIP02a} and the references therein). Coincidentally, preservation of the structure of the de Rham complex at the discrete level is crucial for the development of stable and convergent approximation schemes in computational electromagnetics, and in particular for the solution of Maxwell's eigenproblem \cite{Boffi01} as we will see later in this paper.

%The scalar and vector fields appearing in electromagnetics are often represented as differential forms.  Specifically, the electric and magnetic field intensities are commonly represented as differential one-forms while the magnetic flux and electric current densities are commonly represented as differential two-forms.  Coincidentally, preservation of the structure of the de Rham complex at the discrete level is vital to the development of stable and convergent approximations of Maxwell's eigenproblem \cite{Boffi01} as we will see later in this paper.


The scalar and vector fields appearing in incompressible fluid mechanics may also be represented as differential forms, although additional smoothness is required in the context of viscous flow.  The {\bf \emph{Stokes complex}} naturally accommodates such smoothness requirements \cite{Buffa_deFalco_Sangalli,EvHu12,EvHu12-2,EvHu12-3}.  For a two-dimensional domain $D \subset \mathbb{R}^2$, the Stokes complex is a subcomplex of the rotated de Rham complex and takes the form:
\begin{equation} \label{eq:stokescomplex_2D_regular}
\begin{CD}
H^2(D) @>\rot>> {\bf H}^1(D) @>\div>> L^2(D),
\end{CD}
\end{equation}
where
\begin{equation*}
{\bf H}^1(D) = \left(H^1(D)\right)^n.
\end{equation*}
For a three-dimensional domain $D \subset \mathbb{R}^3$, the Stokes complex is a subcomplex of the standard de Rham complex and takes the form:
\begin{equation} \label{eq:stokescomplex}
\begin{CD}
H^1(D) @>\grad>> \boldsymbol{\Phi}(D) @>\curl>> {\bf H}^1(D) @>\div>> L^2(D),
\end{CD}
\end{equation}
where
\begin{equation*}
\boldsymbol{\Phi}(D) = \left\{ \boldsymbol{\phi} \in {\bf H}(\curl, D): \curl \boldsymbol{\phi} \in {\bf H}^1(D) \right\}.
\end{equation*}
The last two spaces of the Stokes complex, namely ${\bf H}^1(D)$ and $L^2(D)$, are natural spaces for the velocity and pressure fields in incompressible fluid mechanics.  Preservation of the Stokes complex at the discrete level yields stable finite element methods which return point-wise divergence-free velocity fields, a property which is highly desirable in multi-physics applications such as coupled flow-transport \cite{Matthies_Tobiska07} and fluid-structure interaction \cite{Kamensky17}.


%\subsection{Application of the de Rham Complex in Continuum Mechanics}
%{\color{blue} \textbf{Remarks (John):} I am not entirely happy with this section (and with our ultimate dual presentation of differential forms as forms and vectors), but I need to stop stressing about that.}\\
%
%The scalar and vector fields commonly appearing in continuum mechanics may be conveniently represented as differential forms.  For example, in electromagnetics, the electric and magnetic field intensities $\textbf{E}$ and $\textbf{H}$ are commonly represented as differential one-forms $\mathcal{E}$ and $\mathcal{H}$ while the magnetic flux and electric current densities $\textbf{B}$ and $\textbf{J}$ are commonly represented as differential two-forms $\mathcal{B}$ and $\mathcal{J}$.  With this in mind, the Dirichlet Maxwell eigenvalue problem for the electric field intensity may be written either in terms of vector fields as: Find $\textbf{E} \in {\bf H}_0(\curls, D)$ and $\omega \in \mathbb{R}^+$ such that
%\begin{equation}
%\int_D \curl \textbf{E} \cdot \curl \widetilde{\textbf{E}} \hspace{2pt} dD = \omega^2 \int_D \textbf{E} \cdot \widetilde{\textbf{E}} \hspace{2pt} dD \hspace{15pt} \forall \widetilde{\textbf{E}} \in {\bf H}_0(\curls, D),
%\end{equation}
%or in terms of differential forms as: Find $\mathcal{E} \in X^1_0(D)$ and $\omega \in \mathbb{R}^+$ such that
%\begin{equation}
%\left( d\mathcal{E}, d\widetilde{\mathcal{E}} \right)_{L^2\Lambda^2(D)} = \omega^2 \left( \mathcal{E}, \widetilde{\mathcal{E}} \right)_{L^2\Lambda^1(D)} \hspace{15pt} \forall \widetilde{\mathcal{E}} \in X^1_0(D).
%\end{equation}
%Coincidentally, preservation of the structure of the de Rham complex at the discrete level is vital to the development of stable and convergent approximations of Maxwell's eigenproblem \cite{Boffi01}.
%
%The scalar and vector fields appearing in incompressible fluid mechanics may also be represented as differential forms, although additional smoothness is required in the context of viscous flow \cite{EvHu12,EvHu12-2,EvHu12-3}.  For instance, in the three-dimensional setting, the velocity field $\textbf{u}$ may be represented as a differential two-form belonging to the subspace $\textbf{H}^1(D) = \left( H^1(D) \right)^3 \subset X^2(D)$ while the pressure field $p$ may be represented as a standard differential three-form.  While preservation of the structure of the de Rham complex at the discrete level is not required for the construction of stable finite element methods for incompressible flow, it does yield methods which return point-wise divergence-free velocity fields, a property which is highly desirable in multi-physics applications such as coupled flow-transport \cite{Matthies_Tobiska07} and fluid-structure interaction \cite{Kamensky17}.

%\subsection{Remarks on Notation}
%{\color{blue} \textbf{Remarks (John):} Fix once the rest of the paper is finished, as notation will then be finalized!}\\
%
%We explain some of the conventions we will follow in our notation throughout the paper. For Hilbert complexes and cohomology spaces, the position of the space in the sequence will be denoted by the $i$ superindex. For multi-level hierarchical splines, we will refer to the level with the $\ell$ subindex. Finally, bases and spline spaces that are defined from a certain subdomain $\Omega_k$ will be denoted with a subindex $\Omega_k$, like in $X_{\Omega_k}$, or, when this does not lead to confusion, only with the subindex $k$, like in $X_k$. The subindex of the level will always precede the subindex of the subdomain.


==> paper_1/dsplinecomplex.tex <==
As already mentioned in the introduction, we look for a method based on two de Rham complexes of splines. 
%The primal complex in our case is constructed as already outlined in the previous section. 
This section deals therefore with constructing the dual sequence and contextually how to connect the sequences to make the final system solvable.

\subsection{The dual spline complex}
Relying on the high continuity of splines, we will define a dual complex without introducing a dual mesh. We will first explain the construction in the one-dimensional case, and then extend it to arbitrary dimensions (in principle) by tensorization. The idea of construction of a dual complex with spline spaces appeared first in \cite{hiemstra_isogeometric_2011} and was also suggested in \cite{BSV14}. It was then used in \cite{Buffa_2020aa,kapidani2021treecotree} to define a Lagrange multiplier for mortar gluing.

\subsubsection{The one-dimensional dual complex}
From here on we assume that the degree is greater than one and that the 0--forms of the primal complex are at least $C^1$ continuous.
We start on the unit interval, where the exterior derivative amounts to the full derivative and the maximum order non-trivial differential forms we can define are therefore 1--forms. For the primal complex, we have the discrete spaces of 0--forms and 1--forms given by
\[
\Xhath{0} = S_{p}(\Xi), \quad \Xhath{1} = \{\hat \omega^h dx : \hat \omega^h \in S_{p-1}(\Xi')\},
%\Xhath{0} = S_{p+1}(\Xi), \quad \Xhath{1} = \{\hat \omega^h dx : \hat \omega^h \in S_{p}(\Xi')\},
\]
and the one-dimensional primal sequence
\begin{equation*}
    \begin{CD}
    \Xhathb{0} @>d^0>> \Xhathb{1},
    \end{CD}
    \label{eq:cd-iga-1d}
\end{equation*}
where the zero subscript denotes homogeneous boundary conditions as in \eqref{eq:cd-iga-tp-bc}.

In principle, functions in the primal space of discrete 1--forms $\Xhath{1}$ are only required to be in the $L^2$ space. But since we assume that functions in $\Xhath{0}$ are $C^1$ continuous, the functions in $\Xhath{1}$ are at least continuous. We can thus construct a new sequence starting in which the spline space $S_{p-1}(\Xi')$ is the space of 0--forms. We define
\[
\XhathT{0} = S_{p-1}(\Xi'), \quad \XhathT{1} = \{\hat \omega^h dx : \hat \omega^h \in S_{p-2}(\Xi'')\},
%\XhathT{0} = S_{p}(\Xi'), \quad \XhathT{1} = \{\hat \omega^h dx : \hat \omega^h \in S_{p-1}(\Xi'')\},
\]
and we have the one-dimensional dual sequence
\begin{equation*}
    \begin{CD}
    \XhathT{0} @>d^0>> \XhathT{1},
    \end{CD}
    \label{eq:cd-iga-1d-dual}
\end{equation*}
where now vanishing boundary conditions are not included anymore. In practice, the definition of this dual complex is not different from the one we have already seen in \eqref{eq:cd-iga-tp-bc}.
By construction, there is a trivial isomorphism between $\Xhathb{1}$ and $\XhathT{0}$. Indeed, in the unit interval their corresponding spaces of proxy fields are identical, as they are both $S_{p-1}(\Xi')$. Moreover, due to the vanishing boundary conditions, the algebraic dimension of the spaces $\Xhathb{0}$ and $\XhathT{1}$  also matches making the definition of an isomorphism in the finite dimensional setting possible. However, its optimal explicit construction in terms of a discrete Hodge--star operator, which will occupy Section~\ref{sec:discrete_hodge}, is not immediate. Note also that if there is a nontrivial metric on the physical domain, i.e. on a one-dimensional manifold, the push-forward makes also the spaces $X_{h,0}^1$ and $\XhT{0}$, defined in the physical domain, different.

\subsubsection{The tensor-product dual complex}
The construction for dimension $n>1$ proceeds by tensorization of the one-dimensional case. As before, we first define the primal space of 0--forms as $\Xhath{0} = S_{\mathbf{p}}(\boldsymbol{\Xi})$, which gives the primal sequence as in \eqref{eq:cd-iga-tp-bc},
\begin{equation*}
    \begin{CD}
   \Xhathb{0}   @>d^0>>  \Xhathb{1}  @>d^1>> \dots @>d^{n-2}>>  \Xhathb{n-1} @>d^{n-1}>> \Xhathb{n}.
    \end{CD}
\end{equation*}
Assuming that the spline functions in $\Xhath{0}$ are $C^1$ continuous, the functions defining the space of $n$--forms are at least continuous. Hence, as in the one dimensional case, we can use the same spline space appearing in primal $n$--forms to define the dual space of 0--forms, and to start a second sequence. Therefore, with obvious notation, we define the dual space of 0--forms as 
\[
\XhathT{0} = \otimes_{\ell=1}^n S_{p_\ell-1}(\Xi'_\ell) = S_{\mathbf{p-1}}(\boldsymbol{\Xi}'),
\]
from which we have the dual complex
\begin{equation*}
    \begin{CD}
   \XhathT{0}   @>d^0>>  \XhathT{1}  @>d^1>> \dots @>d^{n-2}>>  \XhathT{n-1} @>d^{n-1}>> \XhathT{n}. \\
    \end{CD}
\end{equation*}
The same arguments that we used in the one-dimensional case apply via tensorization: each parametric direction for which the univariate splines in the definition $\Xhathb{k}$ have degree $p$ corresponds to the parametric direction for which univariate splines in  $\XhathT{n-k}$ have degree $p-2$, while all remaining directions are of equal degree $p-1$. 
This is easily seen again taking the vector proxy field example in three dimensions, lowering all degrees by one and comparing the appropriate $(n-k,k)$ pairs. Consequently, the space $\Xhathb{k}$ and its ``dual'' $\XhathT{n-k}$ have the same dimension.

In practice, the construction of this dual complex does not differ from the one already explained in Section~\ref{sec:psplinecomplex}, as we are simply defining a spline sequence of one degree lower than the primal one, using the same knot vector. Consequently, the explanations therein are also valid for the dual complex. In particular, we can map discrete spaces of differential forms to the physical domain $\Omega$, to define the spaces $\XhT{k}$ which form the dual complex in $\Omega$. Moreover, the exterior derivative across all the dual complex is well defined, and given by incidence matrices on another auxiliary control mesh. To distinguish them from the operators of the primal complex, we denote them with $\widetilde{\mathbf{D}}^k$.

\begin{remark}
All spaces in the two sequences are defined on the same mesh (given by the knot vector), and there is no need to explicitly construct a dual mesh. 
This achievement is thanks to the high continuity of the spline spaces in the primal complex, and it is not reproducible in standard FEM approaches.
It is also worth to remark that the construction works for any degree, any regularity, and for non-uniform knot vectors, as long as the starting space in the primal sequence is $C^1$ continuous.
\end{remark}

\subsubsection{Pairing matrices}
Following \cite{HIP99c}, we can define pairing matrices between the spaces of primal differential $k$--forms $X^k_{h,0}$ and dual differential $(n-k)$--forms $\XhT{n-k}$. 
Let $\omega_h^k \in X^k_{h,0}$ and $\eta_h^{n-k} \in \XhT{n-k}$ be respectively represented by the vectors of degrees of freedom $\boldsymbol{\omega}$ and $\boldsymbol{\eta}$. The square pairing matrices ${\bf K}_k^{n-k}$ and $\tilde{\bf K}^k_{n-k}$, are respectively determined by
\begin{align*}
\boldsymbol{\eta}^\top {\bf K}_k^{n-k} \boldsymbol{\omega} = \int_\Omega \eta_h^{n-k} \wedge \omega_h^k,  \quad \text{ for all } \omega_h^k \in X^k_{h,0}, \eta_h^{n-k} \in \XhT{n-k} , \\
\boldsymbol{\omega}^\top \tilde{\bf K}^k_{n-k} \boldsymbol{\eta} = \int_\Omega \omega_h^{k} \wedge \eta_h^{n-k}, \quad \text{ for all } \omega_h^k \in X^k_{h,0}, \eta_h^{n-k} \in \XhT{n-k}, 
\end{align*}
and from the properties of the wedge product, a fundamental property linking them (see~\cite{HIP99c}) immediately follows:
\begin{equation} \label{eq:pairing_transpose}
    \tilde{\bf K}^k_{n-k} = (-1)^{k (n-k)} ({\bf K}_k^{n-k})^\top.
\end{equation}
Moreover, because the pairing $(X^k_{h,0}, \XhT{n-k})$ is stable, as proved in the framework of mortar methods in \cite{Buffa_2020aa}, all the pairing matrices are invertible.
There is an intimate connection between pairing matrices and discrete exterior derivatives: recalling the assumption of vanishing boundary conditions for all spaces of forms in the primal sequence, from the definition of the pairing matrices and the incidence matrices representing the exterior derivatives, it then holds   %{\Rd CHECK SIGN.}
\begin{equation*}
    ({\bf D}^{k-1})^\top \tilde{\bf K}^k_{n-k} = (-1)^{k} \tilde{\bf K}^{k-1}_{n-k+1} \tilde{\bf D}^{n-k},
\end{equation*}
for any $k$ and conversely, using \eqref{eq:pairing_transpose} it holds
\begin{equation*}
    (\tilde{\bf D}^{n-k})^\top {\bf K}^{n-k+1}_{k-1} = (-1)^{n-k+1} {\bf K}^{n-k}_{k} {\bf D}^{k-1},
\end{equation*}
which both represent the discrete counterpart of the integration by parts formula in \eqref{eq:int_by_parts}. We remark that as such, no metric property is yet involved in these properties.

\subsection{Discrete Hodge--star operators} \label{sec:discrete_hodge}
We will hereafter introduce three different choices of the discrete Hodge--star operator which preserve the high order nature of the spline based discretization. The first two are in some sense natural.
They are induced by the properties of the Hodge--star operator in Section~\ref{sec:derham-hodge}, and adapt to our setting the discrete Hodge operators as presented in \cite{HIP99c}. Their main drawback is that they are global operators. The third choice we present is instead based on local projection operations from \cite{LLM01}.

\subsubsection{Global discrete Hodge operators}
Let $\omega_h^k \in X^k_{h,0}$, and let us denote in general $u_h^{n-k} = \star_{{h,\gamma}}^k \omega_h^k$, with the discrete Hodge--star operator $\star_{{h,\gamma}}^k:X^k_{h,0} \rightarrow \XhT{n-k}$ yet undefined. The first discrete operator, mimicking the definition of the continuous Hodge--star operator in \eqref{eq:def_hodge_diff}, is uniquely determined by
%$$\int_\Omega \star_{{\alpha}}^k \omega_h^k \wedge \eta^k = (\omega_h^k, \eta^k)_{L_{{\alpha}}^2\Lambda^k(\Omega)}, \quad \forall \eta^k \in X_h^{k},$$
\begin{equation} \label{eq:def_hodge_discrete1}
    \int_\Omega \eta_h^k \wedge \star_{h,\gamma}^k \omega_h^k = \left( \eta_h^k, \omega_h^k \right)_{L_\gamma^2 \Lambda^k(\Omega)} ,
    \quad \forall \eta^k \in X_{h,0}^k,
\end{equation}
\noindent which in matrix form, using boldface symbols for vectors of degrees of freedom, reads
$$\boldsymbol{\eta}^\top \tilde{\bf K}^k_{n-k} {\bf u} = \boldsymbol{\eta}^\top  {\bf M}^k_\gamma \boldsymbol \omega.$$
\noindent where ${\bf M}^k_\gamma$ is the standard mass matrix for $X^k_{h,0}$ and $\tilde{\bf K}^k_{n-k}$ is the pairing matrix between $X^k_{h,0}$ and $\XhT{n-k}$, which we recall being square and invertible. Our first discrete Hodge--star operator is hence written in matrix form as 
\begin{equation*}
    {\bf H}_\gamma^k = (\tilde{\bf K}^k_{n-k})^{-1}  {\bf M}^k_\gamma,
\end{equation*}
\noindent whereas, for the definition of the second discrete Hodge--star operator, we mimic property \eqref{eq:def_hodge_diff_inv} from the continuous setting: the operator is this time uniquely determined by
\begin{equation}\label{eq:def_hodge_discrete2}
(\eta_h^{n-k},\star_{h,\gamma}^k \omega_h^k)_{L^2_{1/\gamma}\Lambda^{n-k}(\Omega)} = (-1)^{k(n-k)} \int_\Omega \eta_h^{n-k} \wedge \omega_h^k, \quad \forall \eta_h^{n-k} \in \XhT{n-k},
\end{equation}
\noindent from which it ensues, in matrix form again,
$$\boldsymbol{\eta}^\top\tilde{\bf M}^{n-k}_{1/\gamma} {\bf u} = (-1)^{k(n-k)} \boldsymbol{\eta}^\top {\bf K}_k^{n-k} \boldsymbol \omega,$$
\noindent from which, in turn, we deduce its matrix representation as 
\begin{equation*}
    {\bf H}_\gamma^k = (-1)^{k(n-k)} (\tilde {\bf M}^{n-k}_{1/\gamma})^{-1} {\bf K}_k^{n-k},
\end{equation*}
\noindent where, similarly to above $\tilde {\bf M}^{n-k}_{1/\gamma}$ is the mass matrix for the space $\XhT{n-k}$ and ${\bf K}_k^{n-k}$ is the pairing matrix.

\subsubsection{A local discrete Hodge operator} \label{sec:LLM}
%The two previous operators are global as previously anticipated. 
The global nature of the two above choices is somehow unfortunate since methods based on dual grids use sparse, sometimes even diagonal, Hodge operators. We propose a third version of the discrete Hodge operator which partially mends this drawback.
By glancing at the second proposed choice for the operator, it is easy to see that
\[
\star_{{h,\gamma}}^k \omega_h^k = \tilde \Pi^{n-k}_{L^2} (\star^k_\gamma \omega^k_h),
\]
i.e., the discrete Hodge operator is a standard $L^2$--projection composed with the continuous Hodge--star operator.%, which we recall leaves vector proxies unchanged.

The idea is then to use another projector, which has approximation properties proven to be equivalent to the $L^2$--projection, but exhibiting a local nature. We here use a quasi-interpolant projector for splines, which we label $\tilde \Pi^{n-k}_{\text{\tiny LLM}}$, part of the family of quasi-interpolants defined in \cite{LLM01}.
The projector is best described as an algorithm in three steps, which for $\star_{{h,\gamma}}^k$ acts on the basis of the target space $\XhT{n-k}$ as follows:

\begin{enumerate}
\item[i)] For each basis function $\lambda_{i}$ of the space $\XhT{n-k}$, choose $Q_i \subset \mathrm{supp} \lambda_{i}$.
\item[ii)] Project locally on $Q_i$, more precisely on $\XhT{n-k}|_{Q_i}$ (in our case again with an $L^2$--projection $\tilde \Pi^{Q_i}_{L^2} (\star^k_\gamma \omega^k_h|_{Q_i})$).
\item[iii)] Choose the coefficients of the local projection associated to $\lambda_{i}$. This will be the coefficient in the final matrix representation of the global projection.
\end{enumerate}

Steps i) and ii) entail some liberty in the choice of a specific subset of the support of basis functions and on the choice of projection, respectively. We choose local $L^2$--projections in step ii) instead of point interpolation used for the examples in \cite{LLM01}, because it suits better the approximation of general $k$--forms and the definition of the Hodge--star operator, as point evaluation is only meaningful for $0$--forms. For the choice of $Q_i$ in step i), we choose the barycentric element in the support of the univariate B-spline for each specific parametric direction. The $n$-dimensional support $Q_i$ for the local projection will then be the Cartesian product of the one-dimensional supports, mapped to the physical domain, where the projection is finally computed taking into account the Jacobian of the mapping of $\Omega$ (differently from \cite{LLM01}, where the projection is performed on the parametric domain).
We try to take the smallest possible support centered around the maximum of each target basis spline.
If the number of mesh elements in a specific direction is even, e.g. if the degree of the splines is odd or we have repeated knots, we choose the two elements containing the barycentric knot of the support, which tends to reduce the sparsity of the operator.
A matrix representation of the discrete Hodge--star operator is also possible in this case, although an explicit expression is not as simple as for the previous two operators. However, the advantage is that since the operator is local, the resulting matrix is expected to be sparser.

\begin{figure}
    \centering
    \begin{tikzpicture}[]
        \begin{axis}[width=0.5\columnwidth, 
            major tick length = 14pt,
%            xmajorgrids=false, 
            xtick = {                   0,
            0.200000000000000,
            0.400000000000000,
            0.600000000000000,
            0.800000000000000,
            1.000000000000000}, 
            xtick pos = bottom,
            ytick = {0,0.5,1.0},
            height=0.45\columnwidth, ylabel={},xlabel={},  
            ymin=-0.15, ymax=1.15, ylabel near ticks, tick label style={font=\footnotesize},  legend style={font=\footnotesize, }, label style={font=\footnotesize}, every x tick scale label/.style={at={(1,0)}, anchor=north, yshift=-5pt,inner sep=0pt},legend pos= south east]
        \addplot [red, domain=0:1, range=-0.2:1] table [x index=0, y index=4, col sep=comma] {figures/bsplines_p2r1.csv};
        \addplot [dotted, black, domain=0:1] table [x index=0, y index=1, col sep=comma] {figures/bsplines_p2r1.csv};
        \addplot [dotted, black, domain=0:1] table [x index=0, y index=2, col sep=comma] {figures/bsplines_p2r1.csv};
        \addplot [dashed, blue, domain=0:1] table [x index=0, y index=3, col sep=comma] {figures/bsplines_p2r1.csv};
        \addplot [dashed, blue, domain=0:1] table [x index=0, y index=5, col sep=comma] {figures/bsplines_p2r1.csv};
        \addplot [dotted, black, domain=0:1] table [x index=0, y index=6, col sep=comma] {figures/bsplines_p2r1.csv};
        \addplot [dotted, black, domain=0:1] table [x index=0, y index=7, col sep=comma] {figures/bsplines_p2r1.csv};
        \draw[red,decorate,decoration={calligraphic brace,amplitude=3pt},thick] (axis cs:0.6,-0.01) -- (axis cs:0.4,-0.01);
        \node[] at (axis cs:0.5, 0.9)   (a) {$\tilde{X}_h^1,\;p-2=2$};
        \node[] at (axis cs:0.5, -0.1)   (q) {$Q_i$};
        % \addplot [dotted, black, domain=0:1] table [x index=0, y index=8, col sep=comma] {figures/bsplines_p2r1.csv};
        % \addplot [dotted, black, domain=0:1] table [x index=0, y index=9, col sep=comma] {figures/bsplines_p2r1.csv};
        % \addplot [dotted, black, domain=0:1] table [x index=0, y index=10, col sep=comma] {figures/bsplines_p2r1.csv};
        % \addplot [dotted, black, domain=0:1] table [x index=0, y index=11, col sep=comma] {figures/bsplines_p2r1.csv};
        % \addplot [red, mark=*, mark options={solid}] table [x index=0, y index=1, col sep=comma] {figures/laplace_results_mappedsquare_p3r2_l2.csv};
        % \addplot [green, mark=square*, mark options={solid}] table [x index=0, y index=1, col sep=comma] {figures/laplace_results_mappedsquare_p3r2_llm.csv};
        % \addplot [magenta, mark=diamond*, mark options={solid}] table [x index=0, y index=1, col sep=comma] {figures/laplace_results_mappedsquare_p3r2_standard_iga.csv};
        % \node[] at (axis cs:10^-1.6, 10^-1.8)   (a) {$p=3,\;r=2$};
        % \draw (axis cs:10^-1.8,10^-4.5)--(axis cs:10^-1.6,10^-4.5/10^0.1)--(axis cs:10^-1.6,10^-4.5) node[pos=0.5,anchor=west] {\footnotesize$2$}--cyclenode[pos=0.5,anchor=north] {\footnotesize$1$};
        % \legend{$L^2$ inverse proj. \\$L^2$ proj. \\Local proj. \\Standard IGA\\}
        \end{axis}
    \end{tikzpicture}
\qquad
    \begin{tikzpicture}[]
    \begin{axis}[width=0.5\columnwidth, 
        major tick length = 14pt,
%        xmajorgrids=false, 
        xtick = {                   0,
        0.200000000000000,
        0.400000000000000,
        0.600000000000000,
        0.800000000000000,
        1.000000000000000},
        xtick pos = bottom,
        ytick = {0,0.5,1.0},
        height=0.45\columnwidth, ylabel={},xlabel={}, xrange=0:1, 
        ymin=-0.15, ymax=1.15, ylabel near ticks,tick label style={font=\footnotesize},  legend style={font=\footnotesize, }, label style={font=\footnotesize}, every x tick scale label/.style={at={(1,0)}, anchor=north, yshift=-5pt,inner sep=0pt},legend pos= south east]
%    \addplot [dotted, black, domain=0:1] table [x index=0, y index=1, col sep=comma] {figures/bsplines_p4r3.csv};
    \addplot [dotted, black, domain=0:1] table [x index=0, y index=2, col sep=comma] {figures/bsplines_p4r3.csv};
    \addplot [red, domain=0:1] table [x index=0, y index=3, col sep=comma] {figures/bsplines_p4r3.csv};
    \addplot [red, domain=0:1] table [x index=0, y index=4, col sep=comma] {figures/bsplines_p4r3.csv};
    \addplot [red, domain=0:1] table [x index=0, y index=5, col sep=comma] {figures/bsplines_p4r3.csv};
    \addplot [red, domain=0:1] table [x index=0, y index=6, col sep=comma] {figures/bsplines_p4r3.csv};
    \addplot [red, domain=0:1] table [x index=0, y index=7, col sep=comma] {figures/bsplines_p4r3.csv};
    \addplot [dotted, black, domain=0:1] table [x index=0, y index=8, col sep=comma] {figures/bsplines_p4r3.csv};
%    \addplot [dotted, black, domain=0:1] table [x index=0, y index=9, col sep=comma] {figures/bsplines_p4r3.csv};
    \draw[red,decorate,decoration={calligraphic brace,amplitude=3pt},thick] (axis cs:0.6,-0.01) -- (axis cs:0.4,-0.01);
    \node[] at (axis cs:0.5, 0.9)   (a) {${X}_{h,0}^0,\;p=4$};
    \node[] at (axis cs:0.5, -0.1)   (q) {$Q_i$};
    % \addplot [dotted, black, domain=0:1] table [x index=0, y index=10, col sep=comma] {figures/bsplines_p2r1.csv};
    % \addplot [dotted, black, domain=0:1] table [x index=0, y index=11, col sep=comma] {figures/bsplines_p2r1.csv};
    % \addplot [red, mark=*, mark options={solid}] table [x index=0, y index=1, col sep=comma] {figures/laplace_results_mappedsquare_p3r2_l2.csv};
    % \addplot [green, mark=square*, mark options={solid}] table [x index=0, y index=1, col sep=comma] {figures/laplace_results_mappedsquare_p3r2_llm.csv};
    % \addplot [magenta, mark=diamond*, mark options={solid}] table [x index=0, y index=1, col sep=comma] {figures/laplace_results_mappedsquare_p3r2_standard_iga.csv};
    % \node[] at (axis cs:10^-1.6, 10^-1.8)   (a) {$p=3,\;r=2$};
    % \draw (axis cs:10^-1.8,10^-4.5)--(axis cs:10^-1.6,10^-4.5/10^0.1)--(axis cs:10^-1.6,10^-4.5) node[pos=0.5,anchor=west] {\footnotesize$2$}--cyclenode[pos=0.5,anchor=north] {\footnotesize$1$};
    % \legend{$L^2$ inverse proj. \\$L^2$ proj. \\Local proj. \\Standard IGA\\}
    \end{axis}
    \end{tikzpicture}
\caption{Choice of the support of integration for the local projector in the case of a discrete Hodge--star operator $\star_h^0 : {X}_{h,0}^0\mapsto\XhT{1}$, from splines of degree four to splines of degree two. For the solid red B-spline 1--form $\lambda_i \in \XhT{1}$ highlighted in the left panel, $Q_i$ is the central element. Blue dashed B-splines contribute to the matrix involved in the local $L^2$ projection operation. Solid red B-splines in the starting space $X_{h,0}^0$ on the right panel are the basis functions that do not vanish in $Q_i$, and may have a nonzero contribution from $\lambda_i$ after applying the Hodge--star operator. The rest of the basis functions in both panels are shown dotted in black.}
    \label{fig:bsplines}
\end{figure} 

To better understand the sparsity of this local Hodge operator, let us consider the one-dimensional case with the maximum allowed smoothness, and assume we construct a Hodge--star operator $\star_{h,\gamma}^0: X_{h,0}^0\mapsto \XhT{1}$, from the space of primal $0$--forms of degree $p$ to the space of dual $1$--forms of degree $p-2$. Each basis function $\lambda_i$ of $S_{p-2}(\Xi'')$ is supported on $p-1$ knot intervals, therefore we choose $Q_i$ as the central knot interval if $p$ is even, see Fig.~\ref{fig:bsplines}, or as the union of two central knot intervals if $p$ is odd. Near the endpoints of the knot vector the choice has to be adapted due to the reduced support of the basis functions. 
Considering that each element is contained in the support of $p+1$ functions of $X_{h,0}^0$, and $p-1$ functions of $\XhT{1}$, in the worst case of choosing two elements each local $L^2$ projection requires solving a $p \times p$ system of equations, with a multi-column right-hand side of size at most $p+2$ columns. Each system can be solved concurrently, and the resulting coefficients associated with $\lambda_i$ will contribute to $p+2$ nonzero entries in each row of the final matrix representation of the projector. In higher dimensional cases, the accurate computation of the sparsity is given by tensor product arguments on univariate spaces, noting that for $k$--forms with $0<k<n$, the presence of a non-diagonal Jacobian matrix will reduce sparsity by mixing up forms with different multi-index $\boldsymbol{\alpha}$ (i.e. the components of proxy fields).

\subsection{The discrete method}
%With the dual complex and the discrete Hodge--star operators in place, our numerical method can now be defined. 
The discrete version of the continuous problem \eqref{eq:continuousproblem} is given by the problem of finding $\omega_h \in X^k_{h,0}$ such that 
\begin{equation} \label{eq:discreteproblem}
(-1)^{k+1} d^{n-k-1} \star_{h,\gamma}^{k+1} (d^k \omega_h) + \star^k_{h,\beta} \omega_h = \star^k_h f,
\end{equation}
where the discrete Hodge--star operators can follow any of the three constructions given above. Using the matrix representation of the exterior derivatives and the discrete Hodge--star operators, the problem can also be written in matrix form as
\begin{equation}  \label{eq:problem_matrix}
(-1)^{k+1} \tilde{{\bf D}}^{n-k-1} {\bf H}_\gamma^{k+1} ({\bf D}^k \boldsymbol{\omega}_h) + {\bf H}^k_\beta \boldsymbol{\omega}_h = {\bf H}^k \boldsymbol{f}_h,
\end{equation}
where we remark that the resulting system matrix is square even though the approximation is not performed in Galerkin fashion, due to the dimension of the spaces of the dual complex. With a completely analogous procedure, we obtain the discrete version of the eigenvalue problem \eqref{eq:evp_with_forms}.

Finally, we note that the right-hand side in \eqref{eq:discreteproblem} must be a discrete differential form in $\XhT{n-k}$. Although we have written the equation applying the same kind of discrete Hodge--star operator, nothing prevents us to use, for instance, an $L^2$ projection into $\XhT{n-k}$.
Both choices provide a consistent right-hand side.


==> paper_1/error_analysis.tex <==
In this section we perform the error analysis of the solution of the discrete problem \eqref{eq:discreteproblem}. Unlike \cite{HIP99c}, for the analysis of the problem we leverage standard variational techniques. We will see that the first Hodge operator is in fact equivalent to a standard Galerkin discretization, while the other two yield new methods with a reduced order of convergence. For the sake of simplicity, in this section we will consider the same starting degree in every direction, i.e., $p_\ell = p$ for $\ell = 1, \ldots, n$.

We first multiply (using the wedge product) the equation of the continuous problem \eqref{eq:continuousproblem} by a test function, and integrate on $\Omega$, to obtain the variational formulation
\begin{equation} \label{eq:problem_continuous}
a(\omega, \eta) = {\cal F}(\eta) \quad \text{ for all } \eta \in H_0 \Lambda^k (\Omega),
\end{equation}
where, using \eqref{eq:int_by_parts} and \eqref{eq:def_hodge_diff}, we get three equivalent expressions for the bilinear form $a(\cdot, \cdot)$, namely:%\redmod{CHECK THE SIGNS, and eventually simplify (remove) the red part}
\begin{align} \label{eq:definition_a}
a(\omega, \eta) := & (-1)^{(k+1)} \int_\Omega \eta \wedge d^{n-k-1} \star^{k+1}_\gamma (d^k \omega)  + \int_\Omega  \eta \wedge \star^k_\beta \omega \notag \\
 = & %{\Rd (-1)^{(k+1)^2}}
 \int_\Omega  d^k \eta \wedge \star^{k+1}_\gamma (d^k \omega) + \int_\Omega \eta \wedge \star^k_\beta \omega \\
 = & \left(d^k \omega, d^k \eta \right)_{L^2_\gamma \Lambda^{k+1}(\Omega)} + \Big( \omega, \eta \Big)_{L^2_\beta\Lambda^k(\Omega)}, \notag
\end{align}
while the linear form ${\cal F}$ is defined as
\[
{\cal F}(\eta) := \int_\Omega \eta \wedge \star^k f = (f, \eta)_{L^2\Lambda^k(\Omega)}.
\]
\magentamod{The discrete Hodge operators define analogous bilinear forms and linear forms which we will respectively denote by $a_h$ and ${\cal F}_h$ in all cases.} 
Since the exterior derivative is well defined for spline spaces of the two sequences, integration by parts remains valid and they are defined by
\begin{align}
 a_h(\omega_h, \eta_h) := & (-1)^{(k+1)} \int_\Omega \eta_h \wedge d^{n-k-1} \star^{k+1}_{h,\gamma} (d^k \omega_h) + \int_\Omega \eta_h \wedge \star^k_{h,\beta} \omega_h \notag \\
 = & \int_\Omega d^k \eta_h \wedge \star^{k+1}_{h,\gamma} (d^k \omega_h) + \int_\Omega \eta_h \wedge \star^k_{h,\beta} \omega_h  \label{eq:definition_ah} \\
 {\cal F}_h(\eta_h) := & \int_\Omega \eta_h \wedge \star^k_h f , \notag
\end{align}
and the discrete problem \eqref{eq:discreteproblem} is then equivalent to find $\omega_h \in X^k_{h,0}$ such that
\begin{equation} \label{eq:discreteproblem_weak}
a_h(\omega_h, \eta_h) = {\cal F}_h (\eta_h) \quad \forall \eta_h \in X^k_{h,0}.
\end{equation}

Clearly, the bilinear form $a(\cdot,\cdot)$ is symmetric, continuous and coercive in $H_0\Lambda^k(\Omega)$, and the linear form ${\cal F}$ is continuous. The analysis is then based on first Strang's lemma \cite[Thm.~5.5.1]{Quarteroni-Valli-1994}, that we restate here for convenience.
\begin{lemma}
Assuming that the bilinear form $a_h(\cdot, \cdot)$ is uniformly coercive over $X^k_{h,0}$, then there exists $\omega_h \in X^k_{h,0}$ a unique solution to \eqref{eq:discreteproblem_weak}, and it holds that
\begin{align*}
\| \omega - \omega_h \|_{H\Lambda^k(\Omega)} & \le 
C_1 \sup_{\lambda_h \in X^k_{h,0} \setminus\{0\}} \frac{|{\cal F}(\lambda_h) - {\cal F}_h(\lambda_h)|}{\|\lambda_h\|_{H\Lambda^k(\Omega)}}\\
& +\inf_{\eta_h \in X^k_{h,0}}\!\left[ C_2 \| \omega - \eta_h \|_{H\Lambda^k(\Omega)} + C_3\! \sup_{\lambda_h \in X^k_{h,0} \setminus\{0\}} \!\hspace{-6pt}\frac{|a(\eta_h,\lambda_h) - a_h(\eta_h,\lambda_h)|}{\|\lambda_h\|_{H\Lambda^k(\Omega)}} \right],
\end{align*}
where the constants $C_1, C_2$ and $C_3$ depend on the coerciveness constant of $a_h(\cdot,\cdot)$, and $C_2$ also depends on the continuity constant of $a(\cdot,\cdot)$.
\end{lemma}

In all the three cases, that is, independently of the discrete Hodge--star operator, the second term of the error can be bounded using the projectors in \cite{BRSV11}, and for $0 \le s \le p$ we have
\begin{equation} \label{eq:interpolation_error}
\inf_{\eta_h \in X^k_{h,0}} \| \omega - \eta_h \|_{H\Lambda^k(\Omega)} \le C h^{\min\{p,s\}} \| \omega \|_{H^s\Lambda^k(\Omega)}, \quad \text{ for } \omega \in H_0\Lambda^k(\Omega) \cap H^s\Lambda^k(\Omega).
\end{equation}
Therefore, the error analysis reduces to the study of the consistency errors. From now on, and to simplify the analysis, we will assume that there is no consistency error in the right-hand side, i.e. ${\cal F}(\eta_h) = {\cal F}_h(\eta_h)$. 
This is a reasonable hypothesis, since $f$ is a given datum, and not a discrete function.
\begin{remark}
The correct choice of the right-hand side ${\cal F}_h(\eta_h)$, or equivalently of $f_h \equiv \star^k_h f$, may be relevant in some cases, for instance when the discrete function $f_h$ must be divergence free.
\end{remark}

The first theoretical result concerns the first Hodge-star operator, defined in \eqref{eq:def_hodge_discrete1}. In fact, for this operator there is no consistency error, and the total error behaves as the interpolation error in \eqref{eq:interpolation_error}. Therefore, as long as there is also no consistency error in the right-hand side, the solutions obtained applying this first operator or a standard Galerkin method are equivalent, although yielding different matrices.
\begin{theorem} \label{thm:first-hodge}
Let $\omega \in H_0 \Lambda^k(\Omega) \cap H^s \Lambda^k(\Omega)$ be the solution to \eqref{eq:problem_continuous}. Then, the solution $\omega_h$ of the discrete problem \eqref{eq:discreteproblem_weak}, with the discrete Hodge--star operator defined in \eqref{eq:def_hodge_discrete1}, satisfies
\[
\|\omega - \omega_h \|_{H\Lambda^k(\Omega)} \le C h^{\min\{s,p\}} \| \omega \|_{H^s\Lambda^k(\Omega)}.
\]
\end{theorem}
\begin{proof}
Using the definition of the discrete Hodge--star operator \eqref{eq:def_hodge_discrete1} in \eqref{eq:definition_ah}, it holds that
\[
a_h(\eta_h, \lambda_h) = a(\eta_h, \lambda_h) \text{ for all }\eta_h, \lambda_h \in X^k_{h,0},
\]
and the result immediately follows from first Strang's lemma.
\end{proof}

For the analysis of the second and third Hodge--star operators, we first write them as the combination of the continuous Hodge--star operator with a projection onto $\XhT{n-k}$, which we can denote in general by $\tilde{\Pi}^{n-k}$, resulting in
\begin{equation} \label{eq:hodge-projector}
\star^k_{h,\beta} \omega_h = \tilde{\Pi}^{n-k} (\star^k_\beta \omega_h),
\end{equation}
and analogously for $\star^{k+1}_{h,\gamma}$. Both operators have the approximation properties stated in the following lemma, which we present without proof. For the $L^2$-projection the result is due to the approximation properties of B-splines, while for the local operator it comes from the fact that this is nevertheless based on local $L^2$ projections, possibly with a weight due to the presence of the transformation to the physical domain.
\begin{lemma} \label{lemma:approx}
Let $\tilde \Pi^{n-k}$ denote either $\tilde \Pi^{n-k}_{L^2}$, the $L^2$-projection onto $\XhT{n-k}$, or the local projection $\tilde \Pi^{n-k}_{\text{\tiny LLM}}$ defined in Section~\ref{sec:LLM}. Then, for any $\eta \in H^s\Lambda^{n-k}(\Omega)$ with $0 \le s \le p$ it holds that
\begin{align*}
& \| \eta - \tilde \Pi^{n-k} (\eta) \|_{L^2\Lambda^{n-k}(\Omega)} \lesssim h^{\min\{s,p-1\}} \| \eta \|_{H^s \Lambda^{n-k}(\Omega)}.
\end{align*}
\end{lemma}
Note that the order of the approximation is reduced with respect to \eqref{eq:interpolation_error}, because we are projecting onto spaces of a spline sequence of one degree less. 
Before analyzing the error, we shall prove that the bilinear forms defined by these discrete Hodge--star operators are coercive.
\begin{lemma} \label{lem:coerciveness}
There exists $h_0 >0$ such that, for $h < h_0$, 
\[
a_h(\eta_h, \eta_h) \gtrsim \| \eta_h \|_{H \Lambda^{k}(\Omega)} \quad \text{ for all } \eta_h \in X^k_{h,0}.
\]
\end{lemma}
\begin{proof}
Using first the definition of $a_h(\cdot, \cdot)$ and expression \eqref{eq:hodge-projector} of the discrete Hodge--star operators, property \eqref{eq:def_hodge_diff_inv} and the fact that $\star^k_\beta \circ \star^{n-k}_{1/\beta} = (-1)^{k(n-k)}$ (and similarly for $\star^{k+1}_\gamma$), we have
\begin{align*}
& a_h(\eta_h, \eta_h) = \int_\Omega d^k \eta_h \wedge \tilde \Pi^{n-k-1} (\star^{k+1}_\gamma (d^k \eta_h)) + \int_\Omega \eta_h \wedge \tilde \Pi^{n-k} (\star^k_\beta \eta_h) \\
& = \left(\star^{k+1}_\gamma d^k \eta_h, \tilde \Pi^{n-k-1} (\star^{k+1}_\gamma (d^k \eta_h))\right)_{L^2_{1/\gamma}\Lambda^{n-k-1}(\Omega)} + 
\left(\star^k_\beta \eta_h, \tilde \Pi^{n-k} (\star^k_\beta \eta_h)\right)_{L^2_{1/\beta}\Lambda^{n-k}(\Omega)} \\
& = \left(\phi_h, \tilde \Pi^{n-k-1} (\phi_h))\right)_{L^2_{1/\gamma}\Lambda^{n-k-1}(\Omega)} + 
\left(\psi_h, \tilde \Pi^{n-k} (\psi_h)\right)_{L^2_{1/\beta}\Lambda^{n-k}(\Omega)},
\end{align*}
where we have introduced $\phi_h := \star^{k+1}_\gamma (d^k \eta_h) \in \XhT{n-k-1}$ and $\psi_h := \star^k_\beta \eta_h \in \XhT{n-k}$, to simplify notation. By adding and subtracting equal terms, applying Cauchy-Schwarz inequality, and finally by virtue of the approximation result of Lemma~\ref{lemma:approx}, which can be used due to all the spline spaces involved in the definition $X^k_{h,0}$ being at least continuous, it ensues
\begin{align*}
a_h(\eta_h, \eta_h) 
& \ge \left(\phi_h, \phi_h\right)_{L^2_{1/\gamma}\Lambda^{n-k-1}(\Omega)} - \left|\left(\phi_h, \phi_h - \tilde \Pi^{n-k-1} \phi_h)\right)_{L^2_{1/\gamma}\Lambda^{n-k-1}(\Omega)}\right| \\
& + \left(\psi_h, \psi_h \right)_{L^2_{1/\beta}\Lambda^{n-k}(\Omega)} - \left|\left(\psi_h, \psi_h - \tilde \Pi^{n-k} \psi_h \right)_{L^2_{1/\beta}\Lambda^{n-k}(\Omega)}\right| \\
%
& \gtrsim \| \phi_h \|^2_{L^2\Lambda^{n-k-1}(\Omega)} - \| \phi_h\|_{L^2\Lambda^{n-k-1}(\Omega)} \| \phi_h - \tilde \Pi^{n-k-1} \phi_h\|_{L^2\Lambda^{n-k-1}(\Omega)} \\
& + \| \psi_h \|^2_{L^2\Lambda^{n-k}(\Omega)} - \| \psi_h \|_{L^2\Lambda^{n-k}(\Omega)} \| \psi_h - \tilde \Pi^{n-k} \psi_h \|_{L^2\Lambda^{n-k}(\Omega)} \\
%
& \gtrsim \| \phi_h \|^2_{L^2\Lambda^{n-k-1}(\Omega)} + \| \psi_h \|^2_{L^2\Lambda^{n-k}(\Omega)} \\
& - C h \left( \| \phi_h \|_{L^2\Lambda^{n-k-1}(\Omega)} \| \phi_h \|_{H\Lambda^{n-k-1}(\Omega)} + \| \psi_h \|_{L^2\Lambda^{n-k}(\Omega)} \| \psi_h\|_{H\Lambda^{n-k}(\Omega)} \right),
\end{align*}
where we have also used the equivalence of the standard $L^2$ norm with the weighted norms, due to the assumptions on the material properties $\gamma$ and $\beta$. Coerciveness then holds, for $h$ sufficiently small, by recalling the definitions of $\phi_h$ and $\psi_h$, the definition of the norm $H\Lambda^k(\Omega)$, and by the continuity of the Hodge--star operators and their inverse, using again the assumptions on the material properties.
\end{proof}

\begin{theorem}\label{thm:error_bound}
Let $\omega \in H_0 \Lambda^k(\Omega) \cap H^s \Lambda^k(\Omega)$ be the solution to \eqref{eq:problem_continuous}, and let $\omega_h$ the solution of the discrete problem \eqref{eq:discreteproblem_weak}, with the discrete Hodge--star operators defined in \eqref{eq:def_hodge_discrete2} or in Section~\ref{sec:LLM}. Then, there exists $h_0 > 0$ such that, for $h < h_0$, it holds that
\begin{equation*}
\| \omega - \omega_h \|_{H\Lambda^k(\Omega)} \lesssim h^{\min\{s,p-1\}} \| \omega \|_{H^s\Lambda^k(\Omega)},
\end{equation*}
\end{theorem}
\begin{proof}
The coerciveness of the bilinear form $a_h$ was proved in Lemma~\ref{lem:coerciveness}, for $h$ sufficiently small. The result is then a consequence of Strang's lemma, where we have to analyze the consistency error. As in the proof of Lemma~\ref{lem:coerciveness}, let us introduce $\phi_h := \star^{k+1}_\gamma (d^k \eta_h)$ and $\psi_h := \star^k_\beta \eta_h$ to simplify notation. Using first the definition of the bilinear forms $a(\cdot, \cdot)$ and $a_h(\cdot, \cdot)$ in \eqref{eq:definition_a} and \eqref{eq:definition_ah}, the definition of the discrete Hodge--star operators as the composition of a projector and the continuous Hodge--star operator as in \eqref{eq:hodge-projector}, and subsequently using the property of the continuous Hodge--star operator in~\eqref{eq:def_hodge_diff_inv} (neglecting the signs, as we take absolute values), we get 
%% \begin{align*}
%% & |a(\eta_h, \lambda_h) - a_h(\eta_h, \lambda_h)| = 
%% \left| \int_\Omega  d^k \lambda_h \wedge (\star^{k+1}_\gamma (d^k \eta_h) - \star^{k+1}_{h,\gamma} (d^k \eta_h)) + \int_\Omega \lambda_h \wedge (\star^k_\beta \eta_h - \star^k_{h,\beta} \eta_h) \right| \\
%% & = \left| \int_\Omega  d^k \lambda_h \wedge \left(\star^{k+1}_\gamma (d^k \eta_h) - \tilde{\Pi}^{k+1} (\star^{k+1}_{\gamma} (d^k \eta_h))\right) + \int_\Omega \lambda_h \wedge \left(\star^k_\beta \eta_h - \tilde{\Pi}^{k}(\star^k_{\beta} \eta_h)\right) \right| \\
%% & = \left| (\star^{k+1}_\gamma d^k \lambda_h , \star^{k+1}_\gamma (d^k \eta_h) - \tilde{\Pi}^{k+1} (\star^{k+1}_{\gamma} (d^k \eta_h)))_{L^2_{1/\gamma}\Lambda^{n-k-1}(\Omega)} + \left( \star^k_\beta \lambda_h , \star^k_\beta \eta_h - \tilde{\Pi}^{k}(\star^k_{\beta} \eta_h) \right)_{L^2_\beta \Lambda^{n-k}(\Omega)} \right|.
%% \end{align*}
\begin{align*}
& |a(\eta_h, \lambda_h) - a_h(\eta_h, \lambda_h)| = 
% \left| \int_\Omega  d^k \lambda_h \wedge (\phi_h - \star^{k+1}_{h,\gamma} (d^k \eta_h)) + \int_\Omega \lambda_h \wedge (\psi_h - \star^k_{h,\beta} \eta_h) \right| \\
%& = 
\left| \int_\Omega  d^k \lambda_h \wedge \left(\phi_h - \tilde{\Pi}^{k+1} (\phi_h)\right) + \int_\Omega \lambda_h \wedge \left(\psi_h - \tilde{\Pi}^{k}(\psi_h)\right) \right| \\
& = \left| (\star^{k+1}_\gamma d^k \lambda_h , \phi_h - \tilde{\Pi}^{k+1} (\phi_h))_{L^2_{1/\gamma}\Lambda^{n-k-1}(\Omega)} + \left( \star^k_\beta \lambda_h , \psi_h - \tilde{\Pi}^{k}(\psi_h) \right)_{L^2_\beta \Lambda^{n-k}(\Omega)} \right|.
\end{align*}
Then, by Cauchy-Schwarz inequality we obtain
%% \begin{align*}
%% |a(\eta_h, \lambda_h) - a_h(\eta_h, \lambda_h)| 
%% \lesssim & \| \star^{k+1}_\gamma d^k \lambda_h \|_{L^2_{1/\gamma}\Lambda^{n-k-1}(\Omega)} \, \| \star^{k+1}_\gamma (d^k \eta_h) - \tilde{\Pi}^{k+1} (\star^{k+1}_{\gamma} (d^k \eta_h))\|_{L^2_{1/\gamma}\Lambda^{n-k-1}(\Omega)} \\
%% + & \|\star^k_\beta \lambda_h \|_{L^2_{1/\beta} \Lambda^{n-k}(\Omega)} \, \| \star^k_\beta \eta_h - \tilde{\Pi}^{k}(\star^k_{\beta} \eta_h) \|_{L^2_{1/\beta} \Lambda^{n-k}(\Omega)}.
%% \end{align*}
\begin{align*}
|a(\eta_h, \lambda_h) - a_h(\eta_h, \lambda_h)| 
\lesssim & \| \star^{k+1}_\gamma d^k \lambda_h \|_{L^2_{1/\gamma}\Lambda^{n-k-1}(\Omega)} \, \| \phi_h - \tilde{\Pi}^{k+1} (\phi_h)\|_{L^2_{1/\gamma}\Lambda^{n-k-1}(\Omega)} \\
+ & \|\star^k_\beta \lambda_h \|_{L^2_{1/\beta} \Lambda^{n-k}(\Omega)} \, \| \psi_h - \tilde{\Pi}^{k}(\psi_h) \|_{L^2_{1/\beta} \Lambda^{n-k}(\Omega)}.
\end{align*}
Recalling the definition of $\phi_h$ and $\psi_h$, the approximation properties of the projection in Lemma~\ref{lemma:approx} plus the continuity of the Hodge--star operators yield
%% \begin{align*}
%% |a(\eta_h, \lambda_h) - a_h(\eta_h, \lambda_h)| 
%% \lesssim & h^{\min\{s,p-1\}} \| \star^{k+1}_\gamma d^k \lambda_h \|_{L^2_{1/\gamma}\Lambda^{n-k-1}(\Omega)} \, \| \star^{k+1}_\gamma (d^k \eta_h)\|_{H^s \Lambda^{n-k-1}(\Omega)} \\
%% %
%% + & h^{\min\{s,p-1\}} \|\star^k_\beta \lambda_h \|_{L^2_{1/\beta} \Lambda^{n-k}(\Omega)} \, \| \star^k_\beta \eta_h \|_{H^s \Lambda^{n-k}(\Omega)} \\
%% %
%% \lesssim & h^{\min\{s,p-1\}} (\| d^k \lambda_h \|_{L^2_\gamma \Lambda^{k+1}(\Omega)} \| (d^k \eta_h)\|_{H^s \Lambda^{k+1}(\Omega)} + \| \lambda_h \|_{L^2_{\beta} \Lambda^{k}(\Omega)} \| \eta_h \|_{H^s \Lambda^{k}(\Omega)}),
%% \end{align*}
\begin{align*}
& |a(\eta_h, \lambda_h) - a_h(\eta_h, \lambda_h)| 
\lesssim  h^{\min\{s,p-1\}} \| \star^{k+1}_\gamma d^k \lambda_h \|_{L^2_{1/\gamma}\Lambda^{n-k-1}(\Omega)} \, \| \phi_h\|_{H^s \Lambda^{n-k-1}(\Omega)} \\
%
& \hspace{3.56cm} + h^{\min\{s,p-1\}} \|\star^k_\beta \lambda_h \|_{L^2_{1/\beta} \Lambda^{n-k}(\Omega)} \, \| \psi_h \|_{H^s \Lambda^{n-k}(\Omega)} \\
%
& \lesssim h^{\min\{s,p-1\}} (\| d^k \lambda_h \|_{L^2_\gamma \Lambda^{k+1}(\Omega)} \| d^k \eta_h\|_{H^s \Lambda^{k+1}(\Omega)} + \| \lambda_h \|_{L^2_{\beta} \Lambda^{k}(\Omega)} \| \eta_h \|_{H^s \Lambda^{k}(\Omega)}),
\end{align*}
and the estimate follows from the definition of the norms, the assumptions on the material properties $\gamma$ and $\beta$ given in Section~\ref{sec:derham}, and from using \eqref{eq:interpolation_error} for the other term in Strang's lemma.
\end{proof}

\begin{remark}
For the second and third Hodge--star operators we have only been able to prove coerciveness under the condition of a sufficiently fine mesh. However, all the numerical tests we have conducted so far to estimate the coerciveness constant strongly suggest the bilinear form to be uniformly coercive.
\end{remark}




==> paper_1/exactness.tex <==
In this section, we begin the analysis of the hierarchical B-spline complex, and in particular, we study under which conditions the complex is exact. For our analysis, we make use of some powerful tools from abstract cohomology theory that we present at the beginning of the section. These results are then applied to the particular case of the hierarchical B-spline complex, from which we obtain a sufficient and necessary condition for exactness, given in Theorem~\ref{th:exact}. Since the proof is based on abstract cohomology theory, the condition we obtain is valid in a very general setting: it is dimension independent and can be also applied to other hierarchical spaces constructed with the algorithm in Definition~\ref{def:hierarchical}, including hierarchical T-splines \cite{Evans15}. We also give an interpretation of the derived condition based on Greville subgrids. 

The drawback of the aforementioned condition is that is not easily computable. For this reason, we introduce a local condition related to the support of the basis functions on the hierarchical B\'ezier mesh which is local and easier to implement. The last part of this section is devoted to proving this is a sufficient condition for exactness for the two-dimensional case. Some of the proofs in this section are rather technical, hence we will relegate the details to the appendix.

% In this section we start the analysis of the hierarchical spline complex, and in particular develop a condition for the exactness, with a proof based on abstract cohomology theory. We begin the section presenting the necessary results in cohomology, and then apply them to the particular case of the hierarchical spline complex. Coming from an abstract theory, the condition we obtain is valid in a very general setting. Indeed, the result works for the construction of a hierarchical spline complex in any dimension, and it can also be applied to other hierarchical spaces constructed with the algorithm in Definition~\ref{def:hierarchical}, such as hierarchical T-splines \cite{Evans15}. In the last part of the section we show that the local condition presented in Section~\ref{} {\Rd FIX} is a sufficient condition for exactness. Some of the proofs in this section are rather technical, hence we will relegate the details to the appendix.

\subsection{Background Results from Cohomology Theory}\label{sec:homology}
%% To present the abstract setting of cohomology we mainly follow \cite[Section~3]{AFW-2}. We define a Hilbert complex $(V,d)$ as a sequence of Hilbert spaces $V^i$, which are the domain of definition of the linear maps $d^i$
%% \begin{equation} \label{eq:sequence}
%% \begin{CD}
%% 0 @>>> V^0 @>d^0>> V^1 @>d^1>> V^2 @>d^2>> \ldots @>d^{n-1}>> V^n @>>> 0,
%% \end{CD}
%% \end{equation}
%% with $d^i \circ d^{i-1} = 0$. The elements of the kernel of $d^i$ are called closed forms, and denoted by $Z^i(V) \equiv Z^i(V,d)$. %:= \{u^i \in V^i : d^i u^i = 0 \}$. 
%% The elements of the range of $d^{i-1}$ are called exact forms, and denoted by $B^i(V) \equiv B^i(V,d)$. % := \{ u^i \in V^i : u^i = d^{i-1} u^{i-1}, u^{i-1} \in V^{i-1} \}$. 
%% The $i$th {\bf \emph{cohomology group}} is given by the quotient space $H^i(V) \equiv H^i(V,d) = Z^i(V) / B^i(V)$. When the cohomology groups are all trivial, we say that the sequence is {\bf \emph{exact}}.

%% We say that $(V_h,d)$ is a {\bf \emph{subcomplex}} of $(V,d)$ if $V_h^k \subset V^k$, and $d^k(V_h^k) \subset V_h^{k+1}$. We notice that what we have denoted Hilbert complex is called the domain subcomplex in \cite{AFW-2}, {\Rd but for the theory developed in this paper we don't need the missing ``supercomplex''}. We will make use of the following result about subcomplexes.

\begin{lemma}\label{lemma:cupcap_derham}
Let $(V_h,d)$ and $(W_h,d)$ be two subcomplexes of $(V,d)$. Then $(V_h \cap W_h,d)$ and $(V_h + W_h, d)$ are also subcomplexes.
\end{lemma}
\begin{proof}
The result is trivial, since $V^k_h \cap W^k_h \subset V^k$ and $V^k_h + W^k_h \subset V^k$, and moreover we also have $d^k(V_h^k \cap W_h^k) \subset V_h^{k+1} \cap W_h^{k+1}$ and $d^k(V_h^k + W_h^k) \subset V_h^{k+1} + W_h^{k+1}$.
\end{proof}

Let $(V,d_V)$ and $(W,d_W)$ be two Hilbert complexes, and let $f^k : V^k \rightarrow W^k$ be a set of linear maps satisfying $d_W^k f^k = f^{k+1} d_V^k$. Following \cite{AFW-2} we call this a cochain map, and we denote by $f^*$ its induced map in the cohomology groups. The map induced in cohomology by a composition of cochain maps takes the form $(f \circ g)^* = f^* \circ g^*$. Given a Hilbert complex $(V,d)$ and any subcomplex $(V_h,d)$, the inclusion map $j:V_h \rightarrow V$ is a cochain map which induces a map between the cohomology spaces, $j^* : H^k(V_h) \longrightarrow H^k(V)$.

\begin{lemma}\label{lemma:MV}
Let $(V_h,d)$ and $(W_h,d)$ be two subcomplexes of the Hilbert complex $(V,d)$, with cohomology groups $H^k(V_h)$ and $H^k(W_h)$. Then we have an exact Mayer-Vietoris sequence of the form
\begin{equation*}
\begin{CD}
\ldots \rightarrow H^k(V_h \cap W_h) @>\varphi^*>> H^k(V_h) \oplus H^k(W_h)  @>\psi^*>> H^k(V_h + W_h) @>d^*>> H^{k+1}(V_h \cap W_h) \rightarrow \ldots
\end{CD}
\end{equation*}
\end{lemma}
\begin{proof}
From Lemma~\ref{lemma:cupcap_derham}, both $(V_h \cap W_h,d)$ and $(V_h + W_h,d)$ are subcomplexes. We define the inclusion maps $i_{V_h}$ and $i_{W_h}$ from $V_h \cap W_h$ into $V_h$ and $W_h$, respectively, and also the inclusion maps $j_{V_h}$ and $j_{W_h}$ into $V_h + W_h$, from $V_h$ and $W_h$, respectively. It is trivial to prove that the following sequence is exact
\begin{equation} \label{eq:short}
\begin{CD}
0 @>>> V_h \cap W_h @>\varphi>> V_h \oplus W_h  @>\psi>> V_h + W_h @>>> 0,
\end{CD}
\end{equation}
where $\varphi(u) = (u,u) \equiv (i_{V_h} u, i_{W_h} u)$, and $\psi (v,w) = v-w \equiv j_{V_h}v - j_{W_h}w$. This induces a Mayer-Vietoris sequence of the form (see Chapters~2 and~3 in \cite{Hatcher})
\begin{equation*}
\begin{CD}
\ldots \rightarrow H^k(V_h \cap W_h) @>\varphi^*>> H^k(V_h) \oplus H^k(W_h)  @>\psi^*>> H^k(V_h + W_h) @>d^*>> H^{k+1}(V_h \cap W_h) \rightarrow \ldots
\end{CD}
\end{equation*}
The map $d^*$ is defined in the following way: given a closed form  $u \in Z(V_h + W_h)$, from the exactness of \eqref{eq:short} there exist $v \in V_h$ and $w \in W_h$ such that $u = \psi (v,w) = v-w$, and since it is a closed form $du = dv - dw = 0$. Thus in the cohomology groups we can define $d^*[u] = [dv] = [dw]$, where the brackets represent the equivalence class in the cohomology groups.
\end{proof}

\begin{theorem}\label{th:exactness}
Let $(V_h,d)$ and $(W_h,d)$ be two subcomplexes of the Hilbert complex $(V,d)$. Then the map induced by the inclusion, $i_{W_h}^*: H^k(V_h \cap W_h) \rightarrow H^k(W_h)$, is an isomorphism if and only if $j_{V_h}^*: H^k(V_h) \rightarrow H^k(V_h + W_h)$ is also an isomorphism.
\end{theorem}
\begin{proof}
We will only prove that if $i_{W_h}^*$ is an isomorphism, then $j_{V_h}^*$ is also an isomorphism. The second implication is proved similarly.

If $i_{W_h}^*$ is an isomorphism, then $\varphi^*$ is injective. Thus, the Mayer-Vietoris sequence can be split into the short exact sequences
\begin{equation*}
\begin{CD}
0 @>>> H^k(V_h \cap W_h) @>\varphi^*>> H^k(V_h) \oplus H^k(W_h)  @>\psi^*>> H^k(V_h + W_h) @>>> 0,
\end{CD}
\end{equation*}
which in particular implies that $\psi^*$ is surjective.

To prove that $j_{V_h}^*$ is an isomorphism, first we prove that it is injective. Assume that $v \in V_h$ is such that $j_{V_h}^*[v] = 0$. Then the pair $([v],0) \in \ker \psi^* = {\rm Im} \, \varphi^*$, that is, $\varphi^* [u] = ([v],0)$ for some $u \in V_h \cap W_h$. Since $\varphi^* = (i_{V_h}^*, i_{W_h}^*)$ and $i_{W_h}^*$ is injective, we get $[u] = 0$ and therefore $[v] = i_{V_h}^*[u] = 0$.

To prove the surjectivity of $j_{V_h}^*$ we use that $\psi^*$ is surjective. That is, given $z \in V_h+W_h$ there exist $v \in V_h$ and $w \in W_h$ such that $\psi^*([v],[w]) = j^*_{V_h} [v] - j^*_{W_h} [w] = [z]$. Since $i_{W_h}^*$ is surjective, there exists $u \in V_h \cap W_h$ such that $i_{W_h}^*[u] = [w]$, and by the exactness of the sequence $\varphi^*[u] = (i^*_{V_h}[u], [w]) \in \ker \psi^*$. As a consequence, $\psi^* ([v], [w]) - \psi^* (i^*_{V_h}[u], [w]) = j^*_{V_h}([v] - i^*_{V_h}[u]) = [z]$, which proves that $j_{V_h}^*$ is surjective.
\end{proof}

\begin{corollary}
Let $(V_h,d)$ an exact subcomplex of the Hilbert complex $(V,d)$, and $(W_h,d)$ another subcomplex not necessarily exact. Then the subcomplex $(V_h + W_h, d)$ is exact if and only if $i^*_{W_h} : H^k(V_h \cap W_h) \rightarrow H^k(W_h)$ is an isomorphism.
\end{corollary}

%% \begin{remark}
%% We notice that our Mayer-Vietoris sequence is not ordered like the standard Mayer-Vietoris sequence in cohomology, but rather like the Mayer-Vietoris sequence for cohomology with compact support, see \cite[Lemma~3.36]{Hatcher}.
%% \end{remark}

\subsection{A Necessary and Sufficient Condition for Exactness} \label{sec:nec-suff}
By applying the previous results to hierarchical B-splines, we obtain a necessary and sufficient condition for the exactness of the hierarchical B-spline complex. We first present the result, and then we explain how it can be applied in practice with the help of the Greville subgrids.

\begin{theorem} \label{th:exact}
The hierarchical B-spline complex $(\What_{\ell+1},d)$ is exact for $\ell = 0, \ldots, N-1$ if and only if the inclusion $j: \Xhat^k_{\ell, {\ell+1}} \rightarrow \Xhat^k_{\ell+1, {\ell+1}}$ induces an isomorphism between the cohomology groups $H^k(\Xhat_{\ell, {\ell+1}})$ and $H^k(\Xhat_{\ell+1,{\ell+1}})$ for $k = 1, \ldots, n$.
\end{theorem}
\begin{proof}
We proceed by induction. The exactness of the sequence holds for $\ell =0$ since $\What^k_0 = \hat X^k_{0,h}$ are tensor-product spline spaces, and the exactness of the tensor-product spline sequence~\eqref{eq:spline_complex} is known from \cite{BRSV11}. Assume now that the sequence $(\What_\ell,d)$ is exact. The result is immediately proved for level $\ell+1$ by applying Theorem~\ref{th:exactness} with $V_h^k = \What^k_\ell$ and $W_h^k = \Xhat^k_{\ell+1,{\ell+1}}$, using the relations given in Lemma~\ref{lemma:cupcap}.
\end{proof}

\noindent In simple words, the above condition tells us that, at each step of the recursive algorithm in Definition~\ref{def:hierarchical}, the spaces spanned by the basis functions to be removed and by the basis functions to be added should have the {\bf \emph{same topological properties}}, and these should be preserved by the inclusion operator indicated in Theorem \ref{th:exact}.

\subsubsection{An interpretation of the exactness condition using Greville subgrids}
The condition in Theorem~\ref{th:exact} may not be easy to understand for practitioners, as it requires a basic knowledge of homology theory. We give now an intuitive interpretation of this condition with the help of Greville subgrids. 

As we have seen in Section~\ref{sec:submesh}, there exist isomorphisms that define a commutative diagram between the spline subcomplex $(\Xhat_{\ell,\ell+1},d)$ (respectively, $(\Xhat_{\ell+1,\ell+1},d)$) and the low-order finite element complex $(\hat Z_{\ell,\ell+1},d)$ (resp. $(\hat Z_{\ell+1,\ell+1}, d)$) defined on the Greville subgrid. As a consequence, the topological properties of the spline subcomplex are identical to those of the finite element complex on the Greville subgrid. One can, indeed, consider the Greville subgrids associated to the basis functions to be added and removed and check that they have the same topological properties, that is, the same number of connected components, the same number of holes and, in the three-dimensional case, the same number of cavities.  If the Greville subgrids do not have the same topological properties for every $\ell = 0, \ldots, N-1$, then the condition in Theorem~\ref{th:exact} is not met and the hierarchical B-spline complex is not exact.

\begin{figure}[t]
\includegraphics[width=0.32\textwidth,trim=2cm 1.2cm 2cm 0cm, clip]{refined_1x1}
\includegraphics[width=0.32\textwidth,trim=2cm 1.2cm 2cm 0cm, clip]{remove_1x1}
\includegraphics[width=0.32\textwidth,trim=2cm 1.2cm 2cm 0cm, clip]{add_1x1}
\caption{An example of a maximally continuous hierarchical B-spline complex which is exact for $p_1=p_2=3$. On the left, the hierarchical B\'{e}zier mesh is depicted, with the refined region $\Omega_1$ colored in green. In the center and on the right, the vertices, edges, and faces on the Greville subgrids $\MG_{0,1}$ and $\MG_{1,1}$ are depicted, related to the spaces $\Xhat^k_{0,1}$ and $\Xhat^k_{1,1}$, respectively.}
\label{fig:remove-add-1x1}
\end{figure}

\begin{figure}[t!]
\includegraphics[width=0.32\textwidth,trim=2cm 1.2cm 2cm 0cm, clip]{refined_2x2}
\includegraphics[width=0.32\textwidth,trim=2cm 1.2cm 2cm 0cm, clip]{remove_2x2}
\includegraphics[width=0.32\textwidth,trim=2cm 1.2cm 2cm 0cm, clip]{add_2x2}
\caption{An example of a maximally continuous hierarchical B-spline complex which is not exact for $p_1=p_2=3$. On the left, the hierarchical B\'{e}zier mesh is depicted, with the refined region $\Omega_1$ colored in red. In the center and on the right, the vertices, edges, and faces on the Greville subgrids $\MG_{0,1}$ and $\MG_{1,1}$ are depicted, related to the spaces $\Xhat^k_{0,1}$ and $\Xhat^k_{1,1}$, respectively.}
\label{fig:remove-add-2x2}
\end{figure}

Two examples are shown in Figures~\ref{fig:remove-add-1x1} and~\ref{fig:remove-add-2x2} for maximally continuous bicubic splines. The hierarchical B-spline complex associated to the mesh in Figure~\ref{fig:remove-add-1x1} is exact, because the two Greville subgrids associated to the spaces $\Xhat^k_{0,1}$ and $\Xhat^k_{1,1}$ each consist of two connected components without holes and thus have the same topology. Instead, the hierarchical B-spline complex of the example in Figure~\ref{fig:remove-add-2x2}, which is the same as that presented in Figure~\ref{fig:2x2}, does not provide an exact sequence because the number of connected components for the two Greville subgrids is different and changes from two to one.

%\end{document}
\subsection{A Local and Sufficient Condition for Exactness} \label{sec:local}
Despite its generality, the condition for the exactness provided in Theorem~\ref{th:exact} is not easy to check in practice. In fact, in real three-dimensional applications, the Greville subgrids may become very intricate objects\footnote{For instance, the region to be refined could consist of several (topological) knots with links.}, and computation of the cohomology groups is not a simple task, requiring tools from computational (co)homology. Moreover, the comparison of the cohomology groups must be done through the map induced by the inclusion, because even if the cohomology groups of the two Greville subgrids are isomorphic, it may happen that the map induced by the inclusion is not an isomorphism, which would give a non-exact sequence. Finally, for the development of adaptive methods, the refined region $\Omega_\ell$ is chosen with respect to the B\'ezier mesh, and one would like to obtain a condition in this mesh that guarantees the exactness of the sequence. We will now introduce a \textbf{\emph{local and sufficient}} condition for the exactness of the hierarchical B-spline complex. Apart from being local, the advantage of this condition is that it is easier to check because it is defined directly with respect to the B\'ezier submeshes and not with respect to the Greville subgrids.

From now on, we will restrict ourselves to the two-dimensional case, that is, $n=2$. 
%We recall that we are always working with spaces with homogeneous boundary conditions, but we have removed the zero subindex to simplify the notation. JOHN: This was already mentioned at the beginning of the section.
We start by introducing a mild assumption about the choice of the refined subdomains (see equation (11) in \cite{Vuong_giannelli_juttler_simeon}):
\begin{assumption}\label{ass:support}
The subdomain $\Omega_{\ell+1}$ is given as the union of supports of basis functions in the previous level, that is, for $\ell = 0, \ldots, N-1$
\begin{equation}
\Omega_{\ell+1} = \bigcup_{\beta \in S} \supp (\beta), \text{ with } S \subset {\cal B}^n_\ell.  \label{eq:supports}
\end{equation}
As a consequence, (the closure of) the subdomain $\Omega_{\ell+1}$ is given as (the closure of) the union of elements of level $\ell$.
\end{assumption}
The second assumption is closely related to the one introduced in \cite{Mokris2014}, where the authors prove that hierarchical B-splines span the space of piecewise polynomials in the corresponding hierarchical B\'{e}zier mesh. Let us first define, for each level $\ell = 0, \ldots, N-1$, the \textbf{\emph{open}} complementary region
\begin{equation*}
\Omega_{\ell+1}^c = \Omega_0 \setminus \overline \Omega_{\ell+1}.
\end{equation*}
\begin{assumption}\label{ass:overlap}
For each level $\ell = 0, \ldots, N-1$, and for any basis function $\beta^k \in {\cal B}^k_\ell$ of the tensor-product spaces $\Xhatlh{k}$, with $k = 0, 1, 2$, the overlap 
\begin{equation*}
{\rm overlap} (\beta^k) := \supp (\beta^k) \cap \Omega_{\ell+1}^c
\end{equation*}
is connected and simply connected.
\end{assumption}

\begin{figure}[t!]
\begin{subfigure}[]
{\includegraphics[width=0.3\textwidth,trim=2cm 2cm 2cm 1cm, clip]{mesh_not_assumption1} \label{fig:not-assumption1}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width=0.3\textwidth,trim=2cm 2cm 2cm 1cm, clip]{mesh_not_assumption2} \label{fig:not-assumption2}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width=0.3\textwidth,trim=2cm 2cm 2cm 1cm, clip]{mesh_assumptions_1_2} \label{fig:assumption12}}
\end{subfigure}
\caption{Different hierarchical B\'{e}zier mesh configurations for maximally continuous B-splines and $p_1=p_2=3$. The first mesh does not satisfy Assumption~\ref{ass:support}, nor Assumption~\ref{ass:overlap}, because for the function highlighted with the red square, the overlap (given by the purple colored elements) is not connected. The second mesh does not satisfy Assumption~\ref{ass:overlap}, because the overlap of the highlighted function is also not connected. The third mesh satisfies both Assumptions.}
\label{fig:assumptions-1-2}
\end{figure}

The main result of this section is the following theorem, that for $\ell = N$ gives the exactness of the hierarchical B-spline complex.
\begin{theorem} \label{th:local}
If Assumptions~\ref{ass:support} and~\ref{ass:overlap} hold, then the complex 
\begin{equation}
\begin{CD}
0 @>>> \What^0_{\ell} @>\grad>> \What^1_{\ell} @>\curl>> \What^2_{\ell} @>>> \mathbb{R} @>>> 0
\end{CD}
\end{equation}
is exact, for $\ell = 0, \ldots, N$.
\end{theorem}

The constraints posed by the two assumptions are better understood using the simple examples depicted in Figure~\ref{fig:assumptions-1-2}. For maximally continuous B-splines and $p_1=p_2=3$, the hierarchical B\'{e}zier mesh in Figure~\ref{fig:not-assumption1} violates Assumption~\ref{ass:support}, because the refined region does not contain the support of any basis function of level zero. It also violates Assumption~\ref{ass:overlap}, because there exists one function of level zero, whose support is highlighted in red in the figure, that violates the condition in the assumption. Indeed, the intersection of the support with the non-refined region $\Omega^c_1$, which is represented by the eight purple elements, is not connected. The hierarchical B\'{e}zier mesh in Figure~\ref{fig:not-assumption2} satisfies Assumption~\ref{ass:support}, but it does not satisfy Assumption~\ref{ass:overlap}, because the same function violates the overlap condition in the assumption. Finally, the hierarchical B\'{e}zier mesh in Figure~\ref{fig:assumption12} satisfies both assumptions. More examples are given later in Section~\ref{sec:stability}.

The remainder of this section is devoted to the proof of Theorem~\ref{th:local}. We recall that, as stated in Theorem~\ref{th:exact}, the condition for the exactness is given by the relation between the spaces spanned by the functions to remove, $\Xhat^k_{\ell,\ell+1} = {\rm span} \{ {\cal B}^k_{\ell,\ell+1} \}$, and the functions to add, $\Xhat^k_{\ell+1,\ell+1} = {\rm span} \{ {\cal B}^k_{\ell+1,\ell+1} \}$. We will prove the result with the help of the Greville subgrids corresponding to these spaces, that using the same notation of Section~\ref{sec:submesh} we denote by $\MG_{\ell,\ell+1}$ and $\MG_{\ell+1,\ell+1}$, respectively. With the same abuse of notation in Section~\ref{sec:submesh}, we denote in the same manner the two subdomains covered by the Greville subgrids, that we recall that are different from $\Omega_{\ell+1}$, and also different between them.

The proof follows in three steps. First, we show that the three involved subdomains, that is, the subdomain $\Omega_{\ell+1}$ and the two Greville subgrids, are manifolds with boundary and share the same homological properties. Second, using the relations in Section~\ref{sec:submesh} between spline subspaces and finite element spaces defined in the Greville subgrids, we construct a family of commutative projectors for the subspaces restricted to a subgrid. Finally, joining the above results gives the exactness of the sequence.

\begin{remark}
The analogous condition to Assumption~\ref{ass:overlap} in the three-dimensional setting is that the overlaps are connected, simply connected, and with connected boundary.
\end{remark}
\begin{remark}
In two dimensions, Assumption~\ref{ass:support} implies that the overlaps are simply connected, so this condition could be dropped in Assumption~\ref{ass:overlap}, in this case obtaining exactly the same assumption that is used in \cite{Mokris2014} to characterize hierarchical B-splines in terms of piecewise polynomials. We have preferred to maintain the simply connected condition to make more evident that topology is playing a major role in our construction. The results of this section can actually be proved without using Assumption~\ref{ass:support}, but the proofs become more tedious.
\end{remark}

\subsubsection{First Part of the Proof: Topology of the Grids}

\begin{lemma}\label{lemma:omwb}
If Assumptions~\ref{ass:support} and~\ref{ass:overlap} hold, then the subdomain $\Omega_{\ell+1}$ is a manifold with boundary, for $\ell = 0,\ldots, N-1$.
\end{lemma}
\begin{proof}
In the two-dimensional case, the only configuration for which $\Omega_{\ell+1}$ is not a manifold with boundary is the one in Figure~\ref{fig:not-manifold} (see also Figure~3 in \cite{Berdinsky201486}), in which two connected components of $\Omega_{\ell+1}$ meet in a corner. From Assumption~\ref{ass:support}, every cell in $\Omega_{\ell+1}$ belongs to the support of a basis function as in \eqref{eq:supports}. That is, in the case of maximum continuity, we have a rectangle of size $p_{1,\ell} \times p_{2,\ell}$ elements contained in $\Omega_{\ell+1}$. Therefore, we can obviously choose a basis function in ${\cal B}^0_\ell$ such that its support contains the two white elements of $\Omega^c_{\ell+1}$ in Figure~\ref{fig:not-manifold} and the overlap is not connected, which contradicts Assumption~\ref{ass:overlap}.
\end{proof}

\begin{figure}[t!]
\centerline{\includegraphics[width=0.40\textwidth]{not-manifold}}
\caption{Configuration for which a subdomain is not a manifold with boundary. The colored elements belong to the subdomain, whereas the white elements do not.}\label{fig:not-manifold}
\end{figure}

\begin{lemma} \label{lemma:mwb}
If Assumptions~\ref{ass:support} and~\ref{ass:overlap} hold, then the regions of the Greville subgrids $\MG_{\ell,{\ell+1}}$ and $\MG_{\ell+1,{\ell+1}}$ are manifolds with boundary, for $\ell = 0,\ldots, N-1$.
\end{lemma}
\begin{proof}
Similar to the previous proof, the only configuration for which a Greville subgrid is not a manifold with boundary is the one in Figure~\ref{fig:not-manifold}, where now the elements correspond to the Greville cells. If $\MG_{\ell,{\ell+1}}$ is not a manifold with boundary, i.e., it is as in Figure~\ref{fig:not-manifold}, the support of the basis functions in ${\cal B}^2_\ell$ associated to the colored cells is completely contained in $\Omega_{\ell+1}$, and the support of the basis functions associated to the white cells is not. As a consequence, the overlap of the basis function in ${\cal B}^0_\ell$ corresponding to the middle Greville point is not connected, which contradicts Assumption~\ref{ass:overlap}.

If $\MG_{\ell+1,{\ell+1}}$ is as in Figure~\ref{fig:not-manifold} the support of the basis functions associated to the colored cells, which are now in ${\cal B}^2_{\ell+1}$, is contained in $\Omega_{\ell+1}$, and from Assumption~\ref{ass:support} each one of the cells is contained in a rectangle of $p_{1,\ell} \times p_{2,\ell}$ cells of level $\ell$ contained in $\Omega_{\ell+1}$. Since the support of the basis functions associated to the white cells is not contained in $\Omega_{\ell+1}$, analogously to the proof of Lemma~\ref{lemma:omwb} there exists a function in ${\cal B}^0_\ell$ such that its overlap is not connected, which contradicts Assumption~\ref{ass:overlap}.
\end{proof}


\begin{theorem}\label{th:homology}
If Assumptions~\ref{ass:support} and~\ref{ass:overlap} hold, then the homology groups of $\Omega_{\ell+1}$, $\MG_{\ell,{\ell+1}}$ and $\MG_{\ell+1,{\ell+1}}$ are isomorphic, that is, $H_k(\Omega_{\ell+1}) \cong H_k(\MG_{\ell,\ell+1}) \cong H_k(\MG_{\ell+1,\ell+1})$ for $k = 0, 1, 2$.
\end{theorem}
\begin{proof}
The proof of this result is presented in Appendix~\ref{sec:appendix}.
\end{proof}

\begin{corollary} \label{corol:cohomology}
If Assumptions~\ref{ass:support} and~\ref{ass:overlap} hold, then $H^k(\Xhat_{\ell,\ell+1}) \cong H^k(\Xhat_{\ell+1,\ell+1})$, for $k = 0,1,2$.
\end{corollary}
\begin{proof}
Using the definitions from Section~\ref{sec:submesh}, the spline subspaces $\Xhat_{\ell,{\ell+1}}$ and $\Xhat_{\ell+1,{\ell+1}}$ are isomorphic to the finite element spaces (with boundary conditions) defined on the Greville subgrids $\MG_{\ell,\ell+1}$ and $\MG_{\ell+1,\ell+1}$, respectively, and that we denote by $\hat Z_{\ell,\ell+1}$ and $\hat Z_{\ell+1,\ell+1}$. As it is known, the cohomology groups of finite element spaces with homogeneous boundary conditions are isomorphic to the relative cohomology groups of the domain, where the boundary plays the role of the subspace in relative cohomology. We do not need any details here, and refer the interested reader to \cite[Chapter~3]{Hatcher} for a deeper understanding of relative cohomology, and to \cite{GK} for its use in finite elements. In our case, the cohomology groups of the finite element spaces are isomorphic to the relative cohomology groups of the subdomains $\MG_{\ell,{\ell+1}}$ and $\MG_{\ell+1,{\ell+1}}$. From Lemma~\ref{lemma:mwb} they are both manifolds with boundary, and we can use the classical Lefschetz duality theorem (see \cite[Theorem~3.43]{Hatcher}), to obtain
\begin{equation*}
H^k(\Xhat_{\ell,{\ell+1}}) \cong H^k(\hat Z_{\ell,{\ell+1}})
\cong H^{k}(\MG_{\ell,\ell+1},\partial \MG_{\ell,\ell+1})
\cong H_{n-k} (\MG_{\ell,\ell+1}),
\end{equation*}
and
\begin{equation*}
H^k(\Xhat_{{\ell+1},{\ell+1}}) \cong H^k(\hat Z_{\ell+1,{\ell+1}})
\cong H^{k}(\MG_{\ell+1,\ell+1},\partial \MG_{\ell+1,\ell+1})
\cong H_{n-k} (\MG_{\ell+1,\ell+1}),
\end{equation*}
where $H^k(A,B)$ denotes relative cohomology groups. Moreover, from Theorem~\ref{th:homology} we have
\begin{equation*}
H_{n-k} (\MG_{\ell,{\ell+1}}) \cong H_{n-k} (\MG_{\ell+1,{\ell+1}}) \cong H_{n-k}(\Omega_{\ell+1}),
\end{equation*}
which implies that $H^k(\Xhat_{\ell,{\ell+1}}) \cong H^k(\Xhat_{\ell+1,{\ell+1}})$, that is, the cohomology groups are isomorphic.
\end{proof}

\subsubsection{Second Part of the Proof: Commutative Projectors}

The second step is to prove that the inclusion induces an isomorphism, as required by Theorem~\ref{th:exact}. In order to do so, we will construct a set of commutative projectors for the spline spaces, using the relation between the spline spaces $\Xhat^k_{\ell,\ell+1}$ and the low-order finite element spaces $\hat Z^k_{\ell,\ell+1}$. Before defining the projectors, we have to construct a set of generators of the cohomology groups for the finite element and the spline spaces. We explain the construction for $\hat Z_{\ell,\ell+1}$, since the construction for $\hat Z_{\ell+1,\ell+1}$ is completely analogous.

We recall that the dimension of $H^2(\hat Z_{\ell,\ell+1})$ is the number of connected components of $\MG_{\ell,\ell+1}$ minus one, that we denote by $\nc-1$. To build a generating set of $H^2(\hat Z_{\ell,\ell+1})$ we choose on each connected component (except one) of $\MG_{\ell,\ell+1}$ one Greville cell, and the associated piecewise constant basis function $z^2_j$, for $j=1, \ldots, \nc - 1$. The generating set of $H^2(\hat Z_{\ell+1,\ell+1})$ is built in an analogous way.

The dimension of $H^1(\hat Z_{\ell,\ell+1})$ is equal to the number of ``holes'' of $\MG_{\ell,\ell+1}$, $\nh$, that in the case of a planar manifold with boundary is the number of connected components of the boundary $\partial \MG_{\ell,\ell+1}$ minus the number of connected components of $\MG_{\ell,\ell+1}$. To construct a generating set of the cohomology group we first choose a reference boundary on each connected component of $\MG_{\ell,\ell+1}$, and then we pick the remaining connected components of the boundary in such a way that we have a set of boundaries $\Gamma^\MG_j$, for $j = 1, \ldots, \nh$. For each index $j$ we consider the nodal finite element function with degrees of freedom equal to one on $\Gamma^\MG_j$ and zero elsewhere, and then take the function ${\bf z}^1_j$ as its gradient, see Figure~\ref{fig:harmonic} for a graphical explanation. For a discussion on the construction of a basis of harmonic forms see Section~1.4 and Appendix~A.4 in \cite{AV-book}, and references therein.

The generators of the cohomology groups for spline spaces $H^k(\Xhat_{\ell,\ell+1})$ are constructed from the finite element ones, applying the isomorphisms \eqref{eq:cd-iga-fem}, and will be denoted by ${\boldsymbol \zeta}^1_j := \hat{I}^1_h ({\bf z}^1_j)$ and $\zeta^2_j := \hat{I}^2_h(z^2_j)$.
\begin{figure}[t!]
\includegraphics[width=0.32\textwidth]{harmonic_bezier}
\includegraphics[width=0.32\textwidth]{harmonic_greville_vertices}
\includegraphics[width=0.32\textwidth]{harmonic_greville_edges}
\caption{Construction of the harmonic function for $\MG_{0,1}$ corresponding to the hierarchical B\'ezier mesh on the left. In the middle, we choose the degrees of freedom associated to $\Gamma^\MG_2$ to be equal to one and all the others equal to zero. On the right, the gradient of that function expressed in terms of the degrees of freedom of $\hat Z^1_{\ell,\ell+1}$, with coefficients equal to one or minus one depending on the arrow orientation, gives ${\bf z}^1_j$.} \label{fig:harmonic}
\end{figure}

\begin{remark} \label{rem:orthogonal}
The functions ${\bf z}^1_j$ are generators of the cohomology group for finite elements, but are not \emph{harmonic forms}, in the sense that they are not orthogonal to the exact forms. In order to obtain the harmonic forms, one could take the gradients of the functions that solve the problem
\begin{equation*}
\left \{
\begin{array}{rl}
\displaystyle 
\int_{\MG_{\ell,\ell+1}} \grad \phi_j \cdot \grad \psi = 0 & \forall \psi \in \hat Z^0_{\ell,\ell+1}, \\
\phi_j = 1 & \text{\rm  on } \Gamma^\MG_j, \\
\phi_j = 0 & \text{\rm  on } \partial \MG_{\ell,\ell+1} \setminus \Gamma^\MG_j.
\end{array}
\right.
\end{equation*}
However, orthogonality is lost when applying the isomorphism $\hat I_h^1$ to construct the spline functions ${\boldsymbol \zeta}_j^1$.
\end{remark}

\begin{lemma} \label{lemma:curves}
Under Assumptions~\ref{ass:support} and~\ref{ass:overlap}, the following statements hold.
\begin{enumerate}[i)]
\item Given a spline closed form $\psi \in Z^2(\Xhat_{\ell,\ell+1})$ (respectively, $\psi \in Z^2(\Xhat_{\ell+1,\ell+1})$), its equivalence class in $H^2(\Xhat_{\ell,\ell+1})$ (resp. $H^2(\Xhat_{\ell+1,\ell+1})$) is uniquely determined by
\begin{equation*}
\int_{\omega_j} \psi \, dx \quad \text{\rm for } j = 1, \ldots, \nc-1,
\end{equation*}
with $\omega_j \subset \Omega_{\ell+1}$ denoting the connected components of $\Omega_{\ell+1}$.
\item There exists a set of curves $\gamma_j$ in $\Omega_{\ell+1}$, with $j = 1, \ldots, \nh$, such  that given a closed form $\bv \in Z^1(\Xhat_{\ell,\ell+1})$ (respectively $\bv \in Z^1(\Xhat_{\ell+1,\ell+1})$), its equivalence class in $H^1(\Xhat_{\ell,\ell+1})$ (resp. $H^1(\Xhat_{\ell+1,\ell+1})$) is uniquely determined by
\begin{equation*}
\int_{\gamma_j} \bv \cdot d{\bf s} \quad \text{\rm for } j = 1, \ldots, \nh.
\end{equation*}
\end{enumerate}
\end{lemma}
\begin{proof}
Noting that the support of a B-spline function associated to a Greville cell of $\MG_{\ell,\ell+1}$ is contained in a connected component of $\Omega_{\ell+1}$, point i) is an immediate consequence of the definition of the forms $\zeta^2_j$, and the fact that there is a one-to-one correspondence between the connected components of $\MG_{\ell,\ell+1}$ and $\Omega_{\ell+1}$, as stated in Theorem~\ref{th:homology}, and more specifically in Proposition~\ref{prop:cc}. It is then clear that $\int_{\omega_j} \zeta^2_i$ form a non-singular diagonal matrix.

Point ii) requires a more technical proof, which is detailed in Appendix~\ref{sec:appendixb}.
\end{proof}


\begin{lemma} \label{lemma:projectors}
If Assumptions~\ref{ass:support} and~\ref{ass:overlap} hold, then it is possible to define a set of cochain projectors $\hat \Pi^k: \Xhat^k_{\ell+1,\ell+1} \rightarrow \Xhat^k_{\ell,\ell+1}$. That is, for every $\phi^k \in \Xhat^k_{\ell,\ell+1}$ it holds $\hat \Pi^k(\phi^k) = \phi^k$, and the following diagram commutes:
\begin{equation*}
\begin{CD}
0 @>>> \Xhat^0_{\ell+1,\ell+1} @>\grad>> \Xhat^1_{\ell+1,\ell+1} @>\curls>> \Xhat^2_{\ell+1,\ell+1} @>>> \mathbb{R} @>>> 0 \\
@. @V\hat \Pi^0VV @V\hat \Pi^1VV @V\hat \Pi^2VV  \\
0 @>>> \Xhat^0_{\ell,\ell+1} @>\grad>> \Xhat^1_{\ell,\ell+1} @>\curls>> \Xhat^2_{\ell,\ell+1} @>>> \mathbb{R} @>>> 0.
\end{CD}
\end{equation*}
\end{lemma}
\begin{proof}
The construction of these commutative projectors is inspired by \cite{DB05}. We recall that we are always considering spaces with homogeneous boundary conditions.

Given $q \in \Xhat^0_{\ell+1,\ell+1}$, we define $\hat \Pi^0 q \in \Xhat^0_{\ell,\ell+1}$ as the unique solution to
\begin{align*}
(\grad \hat \Pi^0 q, \grad \phi) = (\grad q, \grad \phi) \quad \forall \phi \in \Xhat^0_{\ell,\ell+1}.
\end{align*}

Given $\bv \in \Xhat^1_{\ell+1,\ell+1}$, we define $\hat \Pi^1 \bv \in \Xhat^1_{\ell,\ell+1}$ as the unique solution to 
\begin{align*}
(\curls \hat \Pi^1 \bv, \curls \bw) = (\curls \bv, \curls \bw) &\quad \forall \bw \in \Xhat^1_{\ell,\ell+1}, \\
(\hat \Pi^1 \bv, \grad \phi) = (\bv, \grad \phi) & \quad \forall \phi \in \Xhat^0_{\ell,\ell+1}, \\
\int_{\gamma_j} \hat \Pi^1 \bv \cdot d{\bf s} = \int_{\gamma_j} \bv \cdot d{\bf s} & \quad \text{ for } j = 1, \ldots, \nh,
\end{align*}
where the curves $\gamma_j$ are defined as in Lemma~\ref{lemma:curves}.

Given $\psi \in \Xhat^2_{\ell+1,\ell+1}$ we define $\hat \Pi^2 \psi \in \Xhat^2_{\ell,\ell+1}$ as the unique solution to 
\begin{align*}
(\hat \Pi^2 \psi, \curls \bw) = (\psi, \curls \bw) &\quad \forall \bw \in \Xhat^1_{\ell,\ell+1}, \\
\int_{\omega_j} \hat \Pi^2 \psi \, dx = \int_{\omega_j} \psi \, dx &\quad \text{ for } j = 1, \ldots, \nc,
\end{align*}
where $\omega_j \subset \Omega_{\ell+1}$ are the connected components of $\Omega_{\ell+1}$.

The correct definition of the projectors is a consequence of Lemma~\ref{lemma:curves}, and the fact that we are working with spaces with boundary conditions. The commutativity of the diagram comes trivially from the definition of the projectors.
\end{proof}

\subsubsection{Final Part of the Proof: The Main Result}

We can finally prove the main result of this section.
\begin{proof}[Proof of Theorem~\ref{th:local}]
The theorem is proved by an induction argument. The case of $\ell = 0$ corresponds to standard tensor-product B-splines, and the result holds from \cite{BRSV11}. Assuming that the sequence is exact for $\ell$, and using Theorem~\ref{th:exact}, in order to prove the exactness for $\ell+1$ we have to show that the inclusion $j: \Xhat_{\ell,{\ell+1}} \longrightarrow \Xhat_{\ell+1,{\ell+1}}$ induces an isomorphism between the cohomology groups $H^k(\Xhat_{\ell,{\ell+1}})$ and $H^k(\Xhat_{\ell+1,{\ell+1}})$.

From Corollary~\ref{corol:cohomology} we have $H^k(\Xhat_{\ell,{\ell+1}}) \cong H^k(\Xhat_{\ell+1,{\ell+1}})$, and since the spaces are finite-dimensional, it is enough to prove that $j^*:H^k(\Xhat^k_{\ell,\ell+1}) \rightarrow H^k(\Xhat^k_{\ell+1,\ell+1})$ is injective. This is proved using the cochain projectors in Lemma~\ref{lemma:projectors}. Since $\hat \Pi^k \circ j = {\rm Id}$, we have that $(\hat \Pi^k \circ j)^* = (\hat \Pi^k)^* \circ j^* = {\rm Id}^*$, which is the identity in cohomology. As a consequence $j^*$ is injective (and ($\hat \Pi^k)^*$ is surjective), which ends the proof.
\end{proof}

\begin{remark}
The exactness of the sequence might be also proved using the characterization of hierarchical B-splines in terms of piecewise polynomials of \cite{Mokris2014}, invoking the same arguments already used for T-splines in \cite{BSV14} and for LR-splines in \cite{Johannessen15}.
\end{remark}


==> paper_1/header.tex <==
%%%%%%%%%%%%
% Packages to include
%%%%%%%%%%%%

\usepackage[left=1.00in,top=1.00in,right=1.00in,bottom=1.00in]{geometry}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amscd}
\usepackage[pdftex]{graphicx}
\usepackage{color}
\usepackage{enumerate}
\usepackage{subfigure}
\usepackage[titletoc,title]{appendix}
%\usepackage{authblk}

%%%%%%%%%%
% Path for figures
%%%%%%%%%%

\graphicspath{{./}{figures/}{Figures/}}

%%%%%%%%%%%%%%
% New theorem constructs
%%%%%%%%%%%%%%

\newtheorem{definition}{Definition}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{example}{Example}
\newtheorem{assumption}{Assumption}

%%%%%%%%%%
% New commands
%%%%%%%%%%

\DeclareMathOperator{\Ima}{Im}

\newcommand{\curl}{{\bf curl}\,}
\newcommand{\rot}{{\bf rot}\,}
\newcommand{\curls}{{\rm curl}\,}
\def\div{{\rm div}}
\newcommand{\grad}{{\bf grad}\,}

\newcommand{\supp}{\mathrm{supp}}

\newcommand{\Rd}{\color{red}}
\newcommand{\Bd}{\color{blue}}

\newcommand{\bA}{{\bf A}}
\newcommand{\ba}{{\bf a}}
\newcommand{\bp}{{\bf p}}
\newcommand{\bv}{{\bf v}}
\newcommand{\bw}{{\bf w}}

\newcommand{\M}{{\cal M}}
%\newcommand{\MG}{{\cal M}^G}
\newcommand{\MG}{{\cal G}}

\newcommand{\Xhath}[1]{\,\hspace{-1pt}\widehat{X}^{#1}_h\hspace{-1pt}\,}
\newcommand{\Xhathb}[1]{\,\hspace{-1pt}\widehat{X}^{#1}_{h,0}\hspace{-1pt}\,}
\newcommand{\Zhath}[1]{\,\hspace{-1pt}\widehat{Z}^{#1}_h\hspace{-1pt}\,}
\newcommand{\Zhathb}[1]{\,\hspace{-1pt}\widehat{Z}^{#1}_{h,0}\hspace{-1pt}\,}
\newcommand{\ZhatIh}[1]{\,\hspace{-1pt}\widehat{Z}^{#1}_{I,h}\hspace{-1pt}\,}
\newcommand{\XhatIh}[1]{\,\hspace{-1pt}\widehat{X}^{#1}_{I,h}\hspace{-1pt}\,}
\newcommand{\Xhatlh}[1]{\,\hspace{-1pt}\widehat{X}^{#1}_{\ell,h}\hspace{-1pt}\,}
\newcommand{\XhatOm}[2]{\,\hspace{-1pt}\widehat{X}^{#1}_{\Omega_{#2}}\hspace{-1pt}\,}
\newcommand{\ZhatOm}[2]{\,\hspace{-1pt}\widehat{Z}^{#1}_{\Omega_{#2}}\hspace{-1pt}\,}
\newcommand{\What}{\hat W}
\newcommand{\Xhat}{\hat X}


\newcommand{\curlhat}{\,\hspace{-1pt}{\widehat{\bf curl}}\hspace{-1pt}\,}
\newcommand{\divhat}{\,\hspace{-1pt}{\widehat{\textup{div}}}\hspace{-1pt}\,}
\newcommand{\gradhat}{\,\hspace{-1pt}{\widehat{\bf grad}}\hspace{-1pt}\,}

%\newcommand{\Xhatzeroh}{\,\hspace{-1pt}\widehat{X}^0_h\hspace{-1pt}\,}
%\newcommand{\Xhatoneh}{\,\hspace{-1pt}\widehat{X}^1_h\hspace{-1pt}\,}
%\newcommand{\Xhattwoh}{\,\hspace{-1pt}\widehat{X}^2_h\hspace{-1pt}\,}

%\newcommand{\Zhatzeroh}{\,\hspace{-1pt}\widehat{Z}^0_h\hspace{-1pt}\,}
%\newcommand{\Zhatoneh}{\,\hspace{-1pt}\widehat{Z}^1_h\hspace{-1pt}\,}
%\newcommand{\Zhattwoh}{\,\hspace{-1pt}\widehat{Z}^2_h\hspace{-1pt}\,}

%\newcommand{\Ihatzeroh}{\,\hspace{-1pt}\widehat{I}^0_h\hspace{-1pt}\,}
%\newcommand{\Ihatoneh}{\,\hspace{-1pt}\widehat{I}^1_h\hspace{-1pt}\,}
%\newcommand{\Ihattwoh}{\,\hspace{-1pt}\widehat{I}^2_h\hspace{-1pt}\,}

%\newcommand{\XhatzeroIh}{\,\hspace{-1pt}\widehat{X}^0_{I,h}\hspace{-1pt}\,}
%\newcommand{\XhatoneIh}{\,\hspace{-1pt}\widehat{X}^1_{I,h}\hspace{-1pt}\,}
%\newcommand{\XhattwoIh}{\,\hspace{-1pt}\widehat{X}^2_{I,h}\hspace{-1pt}\,}
%\newcommand{\XhatiIh}{\,\hspace{-1pt}\widehat{X}^i_{I,h}\hspace{-1pt}\,}

%\newcommand{\ZhatzeroIh}{\,\hspace{-1pt}\widehat{Z}^0_{I,h}\hspace{-1pt}\,}
%\newcommand{\ZhatoneIh}{\,\hspace{-1pt}\widehat{Z}^1_{I,h}\hspace{-1pt}\,}
%\newcommand{\ZhattwoIh}{\,\hspace{-1pt}\widehat{Z}^2_{I,h}\hspace{-1pt}\,}

%\newcommand{\IhatzeroIh}{\,\hspace{-1pt}\widehat{I}^0_{I,h}\hspace{-1pt}\,}
%\newcommand{\IhatoneIh}{\,\hspace{-1pt}\widehat{I}^1_{I,h}\hspace{-1pt}\,}
%\newcommand{\IhattwoIh}{\,\hspace{-1pt}\widehat{I}^2_{I,h}\hspace{-1pt}\,}

\newcommand{\XhatzerocIh}{\,\hspace{-1pt}\widehat{X}^{0,c}_{I,h}\hspace{-1pt}\,}
%\newcommand{\XhatonecIh}{\,\hspace{-1pt}\widehat{X}^{1,c}_{I,h}\hspace{-1pt}\,}
\newcommand{\XhattwocIh}{\,\hspace{-1pt}\widehat{X}^{2,c}_{I,h}\hspace{-1pt}\,}
%\newcommand{\XhaticIh}{\,\hspace{-1pt}\widehat{X}^{i,c}_{I,h}\hspace{-1pt}\,}

\let\hat\widehat
\let\tilde\widetilde

\newcommand{\nh}{n_{holes}}
\newcommand{\nc}{n_{comp}}

\newcommand{\hole}{\eta}


==> paper_1/hierarchicalcomplex.tex <==
In this section, we finally present the hierarchical B-spline complex of isogeometric discrete differential forms.  We start with a short introduction of hierarchical B-splines, where we follow the construction in \cite{Kraft} and \cite{Vuong_giannelli_juttler_simeon}, and we present an auxiliary lemma that will be useful for further study of the hierarchical B-spline complex. We then introduce a simple definition of the hierarchical B-spline complex, and we provide a counterexample showing that the complex is not always exact.  We next introduce the concept of Greville subgrids which will prove useful for the analysis of exactness in Section~\ref{sec:exactness}. We end the section with an explanation on how to construct the complex in the physical domain as well as for multi-patch domains.

For the sake of simplicity, from now on we only use spaces with homogeneous boundary conditions. The zero subindex corresponding to these spaces is removed to alleviate notation. For ease of reading, a given level of the multi-level mesh associated with a hierarchical B-spline basis is indicated by the subindex $\ell$, while the position in the complex for $k$-forms is indicated by the superindex $k$. %We will also often refer to hierarchical B-splines as simply hierarchical splines.



\subsection{Hierarchical B-splines} \label{sec:HB-splines}

Recall that the parametric domain is given by $\hat \Omega = (0,1)^n$. Let us assume that we have a sequence of tensor-product spline spaces of 0-forms
\begin{equation}\label{eq:subspaces}
\Xhat_{0,h} \subset \Xhat_{1,h} \subset \ldots \subset \Xhat_{N,h}.
\end{equation}
More precisely, for each {\bf\emph{level}} $\ell = 0, \ldots, N$, the $n$-variate tensor product spline space $\Xhat_{\ell,h} \subset H^1(\hat \Omega)$ is defined as the tensor product of univariate spline spaces $S_{p_{j,\ell}}(\Xi_{j,\ell})$, each of degree $p_{j,\ell}$ and built using a knot vector $\Xi_{j,\ell}$.  That is, $\Xhat_{\ell,h} = \otimes_{j=1}^n S_{p_{j,\ell}}(\Xi_{j,\ell})$. We denote the set of B-spline basis functions for each level by ${\cal B}_\ell$, and we denote by $\M_\ell$ the corresponding B\'ezier mesh, that is, the Cartesian grid generated by the knot vectors without repetitions. 
Let moreover
\begin{equation}\label{eq:subdomains}
\hat \Omega = \Omega_0 \supset \Omega_1 \supset \ldots \supset \Omega_{N} \supset \Omega_{N+1} = \emptyset
\end{equation}
denote a sequence of nested subdomains, where we assume that (the closure of) each subdomain $\Omega_\ell$ is (the closure of) a union of elements of $\M_{\ell-1}$ for $\ell = 1, \ldots, N$. This is the same condition as the {\bf \emph{strong condition}} in \cite{Vuong_giannelli_juttler_simeon}.  With the above notation, \textbf{\textit{hierarchical B-splines}} are defined in a recursive manner as follows.

\begin{definition} \label{def:hierarchical}
We define the space of hierarchical splines $\What_N = {\rm span} \{{\cal H}_N\}$, with ${\cal H}_N$ the hierarchical basis constructed with the following recursive algorithm \cite{Kraft}:
\begin{enumerate}
\item Initialization: ${\cal H}_0 = {\cal B}_0$.
\item Recursively construct ${\cal H}_{\ell+1}$ from ${\cal H}_{\ell}$ by setting
\begin{equation*}
{\cal H}_{\ell+1} = {\cal H}_{\ell+1,c} \cup {\cal H}_{\ell+1,f}, \text{ for } \ell = 0, \ldots N-1,
\end{equation*}
with 
\begin{equation*}
\begin{array}{l}
{\cal H}_{\ell+1,c} = \{\beta \in {\cal H}_{\ell} : \supp(\beta) \not \subset \Omega_{\ell+1}\}, \\
{\cal H}_{\ell+1,f} = \{\beta \in {\cal B}_{\ell+1} : \supp(\beta) \subset \Omega_{\ell+1}\}.
\end{array}
\end{equation*}
%\item ${\cal H} = {\cal H}_{N}$.
\end{enumerate}
\end{definition}
\noindent That is, at step $\ell$ of the recursive algorithm we add the basis functions of level $\ell+1$ completely supported in $\Omega_{\ell+1}$ to the basis and remove the functions of previous levels completely supported in $\Omega_{\ell+1}$ from the basis. B-spline basis functions which are included in ${\cal H}_N$ are referred to as \textbf{\textit{active}} basis functions, and in particular, ${\cal H}_N \cap {\cal B}_\ell$ is the set of active basis functions of level $\ell$, for an integer $0 \leq \ell \leq N$.

Associated with the space of hierarchical splines $\What_N$ is a \textit{\textbf{hierarchical B\'{e}zier mesh}}
\begin{equation}
\mathcal{M}_\mathcal{H} := \bigcup_{\ell=0}^N \{Q \in {\cal M}_\ell \, \text{ such that } \, Q \subset \Omega_\ell \, \text{ and } \, Q \not \subset \Omega_{\ell+1} \}.
\end{equation}
The elements of the hierarchical B\'{e}zier mesh are precisely those included in a formation and assembly routine for isogeometric analysis \cite{Hennig16, Garau16}. An example of a two-dimensional hierarchical B\'ezier mesh, for a simple configuration with only two levels, is depicted in Figure~\ref{fig:hierarchical_bezier}. We have identified the Greville points (see Subsection~\ref{sec:geometric_interpretation}) associated with the active basis functions for both levels in Figure~\ref{fig:0forms_two_levels} assuming the basis functions are maximally continuous and of degree $p_1 = p_2 = 2$.

\begin{figure}
\centerline{\includegraphics[width=0.4\textwidth, trim = 11cm 2cm 11cm 2cm, clip]{Figures/hmsh_2levels_bezier.pdf}}
\caption{Example of a hierarchical B\'ezier mesh with two levels.}
\label{fig:hierarchical_bezier}
\end{figure}

\begin{figure}
\centerline{\includegraphics[width=0.4\textwidth, trim = 11cm 2cm 11cm 1cm, clip]{Figures/hmsh_2levels_0forms_level1.pdf}
\includegraphics[width=0.4\textwidth, trim = 11cm 2cm 11cm 1cm, clip]{Figures/hmsh_2levels_0forms_level2.pdf}}
\caption{Greville points associated with the active basis functions for levels $\ell = 0$ (left) and $\ell = 1$ (right) in the hierarchical B\'ezier mesh depicted in Figure~\ref{fig:hierarchical_bezier} assuming the basis functions are maximally continuous and of degree $p_1 = p_2 = 2$.}
\label{fig:0forms_two_levels}
\end{figure}

It is useful to define, for $0 \le \ell \le \ell' \le N$, the set of basis functions of level $\ell$ with support contained in $\Omega_{\ell'}$, that is 
\begin{equation} \label{eq:B_lk}
{\cal B}_{\ell,\Omega_{\ell'}} \equiv {\cal B}_{\ell,\ell'} := \{ \beta \in {\cal B}_\ell : \supp (\beta) \subset \Omega_{\ell'} \}.
\end{equation}
Notice that, in Definition \ref{def:hierarchical}, we have ${\cal H}_{\ell+1,f} = {\cal B}_{\ell+1, {\ell+1}}$. We will also make use of the following auxiliary spaces, which are closely related to the recursive construction of the hierarchical spline space.
\begin{definition} \label{def:X_ell}
For $0 \le \ell \le \ell' \le N$, we define the spaces:
\begin{align*}
& \What_\ell := {\rm span} \{ {\cal H}_\ell \}, \\
& \Xhat_{\ell,\Omega_{\ell'}} \equiv \Xhat_{\ell,\ell'} := {\rm span} \{ {\cal B}_{\ell,\ell'} \} = \{ \beta \in \hat X_{\ell,h} : \supp (\beta) \subset \Omega_{\ell'} \},
\end{align*}
where the equality holds thanks to the local linear independence of B-splines.
\end{definition}
\noindent Note that we are using the $\Xhat$ notation for spaces spanned by basis functions of one single level, and we are using $\What$ for spaces spanned by functions of multiple levels. In particular, in the previous definition, the space $\What_\ell$ represents the space of hierarchical splines when applying the recursive algorithm up to level $\ell$. The set of auxiliary spaces denoted with the $\Xhat$ notation is helpful to represent the spaces spanned by the basis functions that have to be added ($\Xhat_{\ell+1,{\ell+1}}$) and removed ($\Xhat_{\ell,{\ell+1}}$) at each level in the recursive algorithm, as stated in the following lemma.

\begin{lemma} \label{lemma:cupcap}
For $0 \le \ell \le N-1$ it holds that
\begin{enumerate}[i)]
\item $\What_{\ell+1} = \What_{\ell} + \Xhat_{\ell+1,{\ell+1}} := \{u = v + w: v \in \What_\ell, \, w \in \Xhat_{\ell, {\ell+1}} \}$.
\item $\What_\ell \cap \Xhat_{\ell+1, {\ell+1}} = \Xhat_{\ell, {\ell+1}}$.
\end{enumerate}
\end{lemma}
\begin{proof}
To prove the result, we show that inclusions in both directions hold. The first inclusion in i), that is, $\What_{\ell+1} \subset \What_{\ell} + \Xhat_{\ell+1,{\ell+1}}$, follows from Definitions~\ref{def:hierarchical} and~\ref{def:X_ell} since ${\cal H}_{\ell+1} = {\cal H}_{\ell+1,c} \cup {\cal H}_{\ell+1,f} \subset {\cal H}_\ell \cup {\cal H}_{\ell+1,f}$ and $\Xhat_{\ell+1,{\ell+1}} = {\rm span}\{{\cal H}_{\ell+1,f}\}$. For the second inclusion, it is obvious that $\Xhat_{\ell+1,{\ell+1}} \subset \What_{\ell+1}$, and $\What_\ell \subset \What_{\ell+1}$ is a consequence of their definition and the nestedness provided by~\eqref{eq:subspaces}.

For the first inclusion in ii), we have that $u \in \What_\ell = {\rm span}\{{\cal H}_\ell\} \subset {\rm span\{\cal B}_\ell\}$, and moreover $u \in \Xhat_{\ell+1,{\ell+1}}$ implies that $\supp (u) \subset \Omega_{\ell+1}$, which along with the local linear independence of \mbox{B-splines} yields $u \in \Xhat_{\ell, {\ell+1}}$. For the second inclusion we first use the nestedness of the subdomains given by~\eqref{eq:subdomains} and then the result from i) to obtain $\Xhat_{\ell,{\ell+1}} \subset \Xhat_{\ell,\ell} \subset \What_\ell$. Then, the nestedness of the spline spaces~\eqref{eq:subspaces}, together with the local linear independence of B-splines, immediately gives $\Xhat_{\ell, {\ell+1}} \subset \Xhat_{\ell+1, {\ell+1}}$, which completes the proof.
\end{proof}

\subsection{The Hierarchical B-spline Complex}
The construction of the hierarchical B-spline complex is based on a simple idea: given a multi-level mesh, construct a sequence of hierarchical B-splines of mixed degree, using for each level the B-spline complex in Section~\ref{sec:spline-complex}. We will see, however, that this construction does not, in general, yield an exact complex of hierarchical B-splines.  As was done for the tensor-product B-spline complex, we first define the hierarchical B-spline complex in the parametric domain before mapping it onto the physical domain.

Assume we are given a sequence of nested tensor-product spline spaces
\begin{equation*}
\Xhat_{0,h} \subset \Xhat_{1,h} \subset \ldots \subset \Xhat_{N,h},
\end{equation*}
as in~\eqref{eq:subspaces} and a sequence of nested subdomains as in~\eqref{eq:subdomains}. For each level $\ell = 0, \ldots, N$, we select $\Xhatlh{0} = \Xhat_{\ell,h}$ as the discrete space of 0-forms, and we construct a discrete de Rham complex using tensor-product splines of mixed degree as explained in Section~\ref{sec:spline-complex}. This forms a complex $(\Xhatlh{},d)$ for each level:
\begin{equation} \label{eq:spline_complex}
\begin{CD}
\Xhatlh{0} @>d^0>> \Xhatlh{1} @>d^1>> \ldots @>d^{n-1}>> \Xhatlh{n} .
\end{CD}
\end{equation}
Moreover, with each space of the sequence, $\Xhatlh{k}$, we associate the same set of basis functions introduced in Section~\ref{sec:spline-complex}, and we denote this set of basis functions by ${\cal B}^k_\ell$. Recall that we can define isomorphisms from our B-spline complex to the low-order finite element complex defined on the Greville grid using these bases.

Now, for each $k =0, \ldots, n$, we can construct the hierarchical B-splines bases ${\cal H}^k_N$ and the corresponding hierarchical spline spaces $\What^k_N = {\rm span} \{ {\cal H}^k_N \}$ following the same procedure as in Definition~\ref{def:hierarchical}.  In practice, for spaces of vector-valued splines, the hierarchical B-spline basis can be determined using the recursive algorithm for each component. Adopting the notation introduced in Section \ref{sec:derham} for Hilbert complexes, the \textbf{\textit{hierarchical B-spline complex}} is then simply $\left(\What_N,d\right)$.  As an example, let us recall consider a maximally continuous hierarchical B-spline complex with $p_1 = p_2 = 3$ defined on the hierarchical B\'ezier mesh depicted in Figure~\ref{fig:hierarchical_bezier}.  The Greville nodes associated with active basis functions for $0$-forms are displayed in Figure~\ref{fig:0forms_two_levels}.  All 0-form basis functions are biquadratic, that is, of degree $(2,2)$.  The Greville edges associated with active 1-form basis functions are displayed in Figure~\ref{fig:1forms_two_levels}, where the horizontal arrows correspond to rightward oriented basis functions of degree $(1,2)$ and the vertical arrows to upward oriented basis functions of degree $(2,1)$.  The Greville cells associated with active 2-form basis functions are displayed in Figure~\ref{fig:2forms_two_levels}.  All 2-form basis functions are bilinear, that is, of degree $(1,1)$.

As in \eqref{eq:B_lk}, it will be useful to define, for $0 \le \ell \le \ell' \le N$ and $0 \le k \le n$, the set of basis functions of level $\ell$ that are completely contained in $\Omega_{\ell'}$, that is
\begin{equation} \label{eq:Bik}
{\cal B}^k_{\ell,\Omega_{\ell'}} \equiv {\cal B}^k_{\ell,\ell'} := \{ \beta^k \in {\cal B}^k_\ell : \supp (\beta^k) \subset \Omega_{\ell'} \}.
\end{equation}
Moreover, we can also apply Definition~\ref{def:X_ell} for each $k$ to define
\begin{align}
& \What^k_\ell := {\rm span}\{{\cal H}^k_\ell\}, \\
& \Xhat^k_{\ell,\Omega_{\ell'}} \equiv \Xhat^k_{\ell,\ell'} := {\rm span} \{{\cal B}^k_{\ell,\ell'}\} =  \{ \beta^k \in \Xhatlh{k}  : \supp (\beta^k) \subset \Omega_{\ell'} \},
\end{align}
and the results of Lemma~\ref{lemma:cupcap} also hold. These spaces also form spline complexes, as proved in the next lemma.

\begin{figure}
\centerline{\includegraphics[width=0.4\textwidth, trim = 11cm 2cm 11cm 1cm, clip]{Figures/hmsh_2levels_1forms_level1.pdf}
\includegraphics[width=0.4\textwidth, trim = 11cm 2cm 11cm 1cm, clip]{Figures/hmsh_2levels_1forms_level2.pdf}}
\caption{Greville edges associated with the active 1-form basis functions for levels $\ell = 0$ (left) and $\ell = 1$ (right) in the hierarchical B\'ezier mesh depicted in Figure~\ref{fig:hierarchical_bezier} assuming the 0-form basis functions are maximally continuous and of degree $p_1 = p_2 = 2$.}
\label{fig:1forms_two_levels}
\end{figure}

\begin{figure}[t!]
\centerline{\includegraphics[width=0.4\textwidth, trim = 11cm 2cm 11cm 1cm, clip]{Figures/hmsh_2levels_2forms_level1.pdf}
\includegraphics[width=0.4\textwidth, trim = 11cm 2cm 11cm 1cm, clip]{Figures/hmsh_2levels_2forms_level2.pdf}}
\caption{Greville faces associated with the active 2-form basis functions for levels $\ell = 0$ (left) and $\ell = 1$ (right) in the hierarchical B\'ezier mesh depicted in Figure~\ref{fig:hierarchical_bezier} assuming the 0-form basis functions are maximally continuous and of degree $p_1 = p_2 = 2$.}
\label{fig:2forms_two_levels}
\end{figure}

\begin{lemma}\label{lemma:subcomplex}
For $0 \le \ell \le \ell' \le N$, $(\Xhat_{\ell,\ell'},d)$ and $(\What_\ell,d)$ are Hilbert complexes, not necessarily exact.
\end{lemma}
\begin{proof}
The result for $\Xhat^k_{\ell,\ell'}$ is trivial, because clearly $d^k(\Xhat^k_{\ell,\ell'}) \subset \Xhat^{k+1}_{\ell,\ell'}$ and $(\Xhat_{\ell,\ell'},d)$ is a subcomplex of $(\Xhat_{\ell,h},d)$. For $\What^k_\ell$, since the spaces are contained in $\Xhatlh{k}$, the differential operators $d^k$ are well defined, and to prove the result we proceed by induction. The result is true for $\ell =0$, since $\What^k_0 = \hat X^k_{0,h}$ are the tensor-product spline spaces in Section~\ref{sec:spline-complex}. Assuming that $(\What_\ell,d)$ forms a Hilbert complex, the result holds for $(\What_{\ell+1},d)$, because $\What^k_{\ell+1} = \What^k_{\ell} + \Xhat^k_{\ell+1,{\ell+1}}$ by Lemma~\ref{lemma:cupcap}, and it is immediate to see that $d^k (\What^k_{\ell} + \Xhat^k_{\ell+1,{\ell+1}}) \subset (\What^{k+1}_{\ell} + \Xhat^{k+1}_{\ell+1,{\ell+1}})$.
% and {\Rd Lemma~\ref{lemma:cupcap_derham}}, because $\What^i_{\ell+1} = \What^i_{\ell} \cup \What^i_{\ell+1,\Omega_{\ell+1}}$.
\end{proof}


%\subsection{A Counterexample of the Exactness}
The result of Lemma~\ref{lemma:subcomplex} for $\ell = N$ guarantees that the hierarchical spline spaces $\What^k_N$ form a Hilbert complex, but in general the complex {\bf \emph{may not be exact}}. Actually, it is relatively easy to find counterexamples where the hierarchical spline spaces do not form an exact sequence. For instance, in the two-dimensional case a necessary (but not sufficient) condition for exactness is
\begin{equation*}
\dim (\What^0_N) + \dim (\What^2_N) = \dim (\What^1_N) + 1.
\end{equation*}
We can see that the condition is not fulfilled for the maximally continuous hierarchical B-spline complex with $p_1 = p_2 = 3$ defined on the hierarchical B\'{e}zier mesh depicted in Figure~\ref{fig:2x2}. In this case, a simple computation gives that the dimensions of the hierarchical spaces with boundary conditions are $\dim (\What^0_N) = 147$, $\dim (\What^1_N) = 328$, $\dim(\What^2_N) = 181$, which violates the previous condition.

\begin{figure}[t]
\centerline{\includegraphics[width=0.45\textwidth]{refined_2x2}}
\caption{A hierarchical B\'{e}zier mesh for which the sequence is not exact for $p_1 = p_2 = 3$.}
\label{fig:2x2}
\end{figure}

Exactness of the hierarchical B-spline complex is crucial for the correct behavior of discretization schemes based on the complex, as we will see later in the examples of Section~\ref{sec:stability}. In Section~\ref{sec:exactness}, we develop conditions guaranteeing exactness of the complex based on an analysis of the spaces $\Xhat^k_{\ell,\ell}$ and $\Xhat^k_{\ell,\ell+1}$ appearing in the construction of the hierarchical B-spline complex. In this analysis, we invoke the concept of a Greville subgrid which we now describe in detail.

\begin{remark}
In the two-dimensional setting, a \textbf{rotated hierarchical B-spline complex} may easily be constructed by rotating the orientation of the discrete 1-forms by $\pi/2$ in parametric space, just as was the case for tensor-product B-splines.
\end{remark}

\subsection{The Spline Complex Restricted to a Submesh and the Greville Subgrid}\label{sec:submesh}
Consider a particular level $\ell$, and consider a subdomain $\Omega_{\ell'}$ with $0 \le \ell \le \ell' \le N-1$. From the strong condition in Section~\ref{sec:HB-splines}, we know that $\Omega_{\ell'}$ is a union of elements in $\M_\ell$ for $\ell' \in \{\ell,\ell+1\}$. %We recall that we defined ${\cal B}^k_{\ell, \ell'}$ in \eqref{eq:Bik} as the basis of tensor product $k$-forms completely contained in $\Omega_{\ell'}$, and $\Xhat^k_{\ell,\ell'}$ is the space they span. 
As we already proved in Lemma~\ref{lemma:subcomplex}, the spaces $\Xhat^k_{\ell,\ell'}$ form the complex $(\Xhat_{\ell,\ell'},d)$, but the sequence they form is not necessarily exact.

Employing the geometrical entities in the Greville grid $\MG_\ell$ associated with the basis functions in ${\cal B}^k_{\ell,\ell'}$, we build a {\bf \emph{Greville subgrid}} that we denote by $\MG_{\ell,\ell'} \subset \MG_\ell$. With some abuse of notation, we will also denote by $\MG_{\ell,\ell'}$ (the interior of the closure of) the union of the cells in $\MG_{\ell,\ell'}$. In Figure~\ref{fig:submeshes} we have included, for the same spaces of tensor-product B-splines depicted in Figure~\ref{fig:meshes}, an example of a subdomain $\Omega_{\ell'}$ and the corresponding Greville subgrid. We notice that, in general, the subdomain defined by $\MG_{\ell,\ell'}$ is different from $\Omega_{\ell'}$, and in fact it will depend on the degree of the spline space. We also notice that, since the support of the B-spline basis functions is reduced with the degree, the basis functions associated to the entities on the boundary of $\MG_{\ell,\ell'}$ do not belong to ${\cal B}^k_{\ell,\ell'}$.

\begin{figure}[tp]
\begin{subfigure}[The subdomain $\Omega_{\ell'}$ as a B\'ezier submesh of $\M_\ell$]{
\centering
\includegraphics[width=3.0in]{Bezier_submesh.pdf}
\label{fig:subbezier}
}
\end{subfigure}
\begin{subfigure}[The corresponding Greville subgrid $\MG_{\ell,\ell'}$]{
\includegraphics[width=3.0in]{Greville_submesh.pdf}
\label{fig:subgreville}
}
\end{subfigure}
\caption{Construction of the Greville subgrid $\MG_{\ell,\ell'}$. Considering the same degrees and knot vectors as in Figure~\ref{fig:meshes} to represent $\M_\ell$ and $\MG_\ell$, we choose the subdomain  $\Omega_{\ell'} = (1/6,5/6) \times (1/5,4/5)$ in (a). The Greville subgrid $\MG_{\ell,\ell'}$ is formed by the darkened elements in (b), while the geometric entities corresponding to basis functions in ${\cal B}^k_{\ell,\ell'}$ are marked by blue dots (0-forms), red arrows (1-forms) and green squares (2-forms).}
\label{fig:submeshes}
\end{figure}

Finally, for each level $\ell$, we can define isomorphisms as in the diagram \eqref{eq:cd-iga-fem} that relate the B-spline complex to the low-order finite element complex defined on the Greville grid. Considering the subdomain $\Omega_{\ell'}$, the same isomorphisms relate the spline subspaces $\Xhat^k_{\ell,\ell'}$ to the spaces of the finite element complex defined on the Greville subgrid, which we henceforth denote by $\hat{Z}^k_{\ell,\ell'}$, and a commutative diagram can also be defined for these subspaces.

\begin{remark}
Since we are assuming homogeneous boundary conditions on $\partial \Omega$, the finite element spaces $\hat{Z}^k_{\ell,\ell'}$ have homogeneous boundary conditions on $\partial \MG_{\ell,\ell'}$. Removing this assumption would cause the finite element spaces to have homogeneous boundary conditions on $\partial \MG_{\ell,\ell'} \setminus (\partial \MG_{\ell,\ell'} \cap \partial \hat \Omega)$. The results of the paper can be easily applied to this case, but writing it in detail would only add more complexity without giving more insight.
\end{remark}

\subsection{Extension to the Physical Domain and Multi-patch Geometries}

The hierarchical B-spline complex in the physical domain is built in exactly the same manner as the B-spline complex. Namely, assuming that we have a parametrization ${\bf F}: \hat \Omega \rightarrow \Omega$, we simply use the pullback operators defined in Subsection \ref{subsec:pullback}, yielding:
\begin{equation*}
W_\ell^k\left(\Omega\right) := \left\{ \omega \in X^k\left(\Omega\right) : \iota^k(\omega) \in \What^k_\ell \right\}
\end{equation*}
for all integers $0 \leq k \leq n$ and $0 \leq \ell \leq N$.

To define hierarchical differential forms in a multi-patch domain, one must take into account the presence of non-conforming meshes between patches \cite{Scott2014222}. This can be easily done following the approach used in \cite{Buchegger2016159} for 0-forms. We start by defining a multi-patch B-spline complex for each level, exactly as in Section~\ref{sec:multipatch}. Then, we apply the hierarchical algorithm of Definition~\ref{def:hierarchical} to the multi-patch spaces of the complex, taking into account that the supports of interface functions overlap two or more patches. 
%With this procedure, the check of the support and the orientation assignment for each basis function can be done at the tensor-product level.  JOHN: I found this possibly confusing for the reader.
We show an example of the construction for a multi-patch, maximally continuous hierarchical B-spline complex with $p_1 = p_2 = 2$ defined on the hierarchical B\'{e}zier mesh in Figure~\ref{fig:multipatch}, where the thick line represents the interface between both interfaces. The set of active basis functions for 0-forms is represented in the Greville grid in Figure~\ref{fig:multi_0forms}, for levels 0 and 1. We note the presence of an active basis function at level 0 on the interface that would not appear on the left patch when considering the patches separately. This is due to the fact that the basis function is supported on both patches. Similarly, some functions of level 1 on the interface are not active but would be active on the left patch if we considered the patches separately. A similar behavior is also encountered for the 1-forms depicted in Figure~\ref{fig:multi_1forms}.

\begin{figure}[t]
\centerline{\includegraphics[width=0.6\textwidth, trim=5cm 4cm 4cm 3cm, clip]{multipatch_bezier}}
\caption{A hierarchical B\'{e}zier mesh for a simple multi-patch geometry with $p_1 = p_2 = 2$.}\label{fig:multipatch}
\end{figure}

\begin{figure}[t]
\begin{subfigure}[Active basis functions of level 0]{
\includegraphics[width=0.49\textwidth, trim=5cm 4cm 4cm 3cm, clip]{multipatch_0forms_level1}
\label{fig:multi_0forms_1lev}
}
\end{subfigure}
\begin{subfigure}[Active basis functions of level 1]{
\includegraphics[width=0.49\textwidth, trim=5cm 4cm 4cm 3cm, clip]{multipatch_0forms_level2}
\label{fig:multi_0forms_2lev}
}
\end{subfigure}
\caption{Geometric entities in the Greville grids associated with active basis functions for 0-forms corresponding to the multi-patch example in Figure~\ref{fig:multipatch}.}
\label{fig:multi_0forms}
\end{figure}

\begin{figure}[h!]
\begin{subfigure}[Active basis functions of level $\ell = 0$]{
\includegraphics[width=0.49\textwidth, trim=5cm 4cm 4cm 3cm, clip]{multipatch_1forms_level1}
\label{fig:multi_1forms_1lev}
}
\end{subfigure}
\begin{subfigure}[Active basis functions of level $\ell = 1$]{
\includegraphics[width=0.49\textwidth, trim=5cm 4cm 4cm 3cm, clip]{multipatch_1forms_level2}
\label{fig:multi_1forms_2lev}
}
\end{subfigure}
\caption{Geometric entities in the Greville grids associated with active basis functions for 1-forms corresponding to the multi-patch example in Figure~\ref{fig:multipatch}.}
\label{fig:multi_1forms}
\end{figure}

%% \subsection{The Spline Complex Restricted to a Submesh}\label{sec:submesh}
%% For the construction of a de Rham complex with hierarchical splines, we need to define suitable spline complexes in the subdomains $\Omega_\ell$. We recall that we assume (the closure of) each subdomain $\Omega_\ell$ to be (the closure of) the union of the union of B\'ezier elements in $\M$. {\Rd We will denote by $\M_{\Omega_\ell}$ the {\bf \emph{B\'ezier submesh}}, that is, the restriction of the B\'ezier mesh $\M$ to the subdomain~$\Omega_\ell$.}

%% We now construct the B-spline complexes restricted to the subdomain $\Omega_\ell$. Let us first define, in an analogous way to \eqref{eq:B_lk}
%%  the set of basis functions
%% \begin{equation} %\label{eq:Bik}
%% {\cal B}^k_{\Omega_\ell} := \{\beta \in {\cal B}^k : \supp (\beta^k) \subset \Omega_\ell \},
%% \end{equation}
%% and the space spanned by them
%% \begin{equation*}
%% \XhatOm{k}{\ell} := {\rm span} ({\cal B}^k_{\Omega_\ell}) = \{ u \in \Xhath{k} : \supp (u) \subset \Omega_\ell \},
%% \end{equation*}
%% where the equality holds thanks to the local linear independence of B-splines. It is easily shown that $d^k (\XhatOm{k}{\ell}) \subset \XhatOm{k+1}{\ell}$, so we have the following complex:
%% \begin{equation*}
%% \begin{CD}
%% \XhatOm{0}{\ell} @>d^0>> \XhatOm{1}{\ell} @>d^1>> \ldots @>d^{n-1}>> \XhatOm{n}{\ell}.
%% \end{CD}
%% \end{equation*}
%% However, the complex is {\bf \emph{not}} necessarily {\bf \emph{exact}}. {\Rd REDUCED COHOMOLOGY}

%% Selecting for the basis functions in ${\cal B}^k_{\Omega_\ell}$ their associated geometrical entities in the Greville grid $\MG$, we build a {\bf \emph{Greville subgrid}} $\MG_{\Omega_\ell} \equiv \MG_{\ell} \subset \MG$. With some abuse of notation, we will also denote by $\MG_{\ell}$ (the interior of the closure of) the union of the cells in $\MG_{\ell}$. In Figure~\ref{fig:submeshes} we have included an example of a B\'ezier submesh, and the corresponding Greville subgrid when considering the same spaces of B-splines of Figure~\ref{fig:meshes}. We notice that, in general, the subdomain defined by $\MG_{\ell}$ is different from $\Omega_\ell$, and in fact it will depend on the degree of the spline space. We also notice that, since the support of the spline basis functions is reduced with the degree, the basis functions associated to the entities on the boundary of $\MG_{\ell}$ do not belong to ${\cal B}^k_{\Omega_\ell}$.
%% \begin{figure}[tp]
%% \begin{subfigure}[A B\'ezier submesh]{
%% \centering
%% \includegraphics[width=3.0in]{Bezier_submesh.pdf}
%% }
%% \end{subfigure}
%% \begin{subfigure}[The corresponding Greville subgrid]{
%% \includegraphics[width=3.0in]{Greville_submesh.pdf}
%% }
%% \end{subfigure}
%% \caption{B-spline submeshes associated with polynomial degrees $p_1 = 2$ and $p_2 = 2$, knot vectors $\Xi_1 = [0,0,0,1/6,2/6,3/6,4/6,5/6,1,1,1]$ and $\Xi_2 = [0,0,0,1/5,2/5,3/5,4/5,1,1,1]$, and the subdomain $\Omega_\ell = (1/6,5/6) \times (1/5,4/5)$. The Greville subgrid $\MG_\ell$ is formed by the darkened elements in (b), while the the functions in ${\cal B}^k_{\Omega_\ell}$ are marked by blue dots (0-forms), red arrows (1-forms) and green squares (2-forms).}
%% \label{fig:submeshes}
%% \end{figure}

%% We can restrict the isomorphisms $\hat I^k_h$ to the subspaces $\XhatOm{k}{\ell}$, and define the finite element spaces $\ZhatOm{k}{\ell} := \hat I^k_h (\XhatOm{k}{\ell})$. The isomorphisms also relate the topological structure of the spline subspaces $\XhatOm{k}{\ell}$ to that of the finite element spaces $\ZhatOm{k}{\ell}$, and we have the following commutative diagram:
%% {\Rd IS THIS NECESSARY?}
%% \begin{equation} \label{eq:subcd-iga-fem}
%% \begin{CD}
%% %\mathbb{R} @>>> 
%% \XhatOm{0}{\ell} @>d^0>> \XhatOm{1}{\ell} @>d^1>> \ldots @>d^{n-1}>> \XhatOm{n}{\ell} \\
%% @V\hat I^0_hVV @V\hat I^1_hVV @. @V\hat I^n_hVV \\
%% %\mathbb{R} @>>> 
%% \ZhatOm{0}{\ell} @>d^0>> \ZhatOm{1}{\ell} @>d^1>> \ldots @>d^{n-1}>> \ZhatOm{n}{\ell}.
%% \end{CD}
%% \end{equation}
%% Notice that, since we are assuming homogeneous boundary conditions on $\partial \Omega$, the spaces $\ZhatOm{k}{\ell}$ are in fact the lowest-order finite element spaces defined in the Greville subgrids, with homogenous boundary conditions on $\partial \MG_{\ell}$. Working on spaces without boundary conditions would cause the finite-element spaces $\ZhatOm{k}{\ell}$ to have homogeneous boundary conditions on $\partial \MG_{\ell} \setminus (\partial \MG_{\ell} \cap \partial \hat \Omega)$, that is, on the boundaries of the subgrid $\MG_{\ell}$ that do not belong to the boundary of the domain. We have preferred to work with spaces with boundary conditions to avoid precising the boundary of each subdomain, but the results work also without boundary conditions with minor changes.






%% Finally, we can also define suitable projectors $\hat \Pi^k_{\Omega_\ell} \equiv \hat \Pi^k_\ell$ to obtain a commutative diagram similar to \eqref{eq:cd-iga-pi} (or \eqref{eq:cd-iga-pi}) for the spaces of the subcomplex. In practice, the projectors $\hat \Pi^k$ in \eqref{eq:cd-iga-pi} are defined from a dual basis, see \cite{BRSV11}, thus it is enough to restrict the definition to the dual functionals associated to the basis functions in ${\cal B}^k_\ell$ to obtain $\hat \Pi^k_\ell$. By doing so we obtain the commutative diagram {\Rd BOUNDARY CONDITIONS}

%% {\Rd REMOVE THE PROJECTORS, IF NOT NEEDED}
%% \begin{equation} \label{eq:subcd-iga-pi}
%% \begin{CD}
%% \Xhat^0(\Omega_\ell) @>d^0>> \Xhat^1(\Omega_\ell) @>d^1>> \ldots @>d^{n-1}>> \Xhat^n(\Omega_\ell) \\
%% @V\hat \Pi_\ell^0 VV @V\hat \Pi_\ell^1 VV @. @V\hat \Pi_\ell^n VV\\
%% \XhatOm{0}{\ell} @>d^0>> \XhatOm{1}{\ell} @>d^1>> \ldots @>d^{n-1}>> \XhatOm{n}{\ell} .
%% \end{CD}
%% \end{equation}
%% It is worth to note that, although the projectors are local and stable and the diagram commutes, the subspaces $\XhatOm{k}{\ell}$ do not guarantee optimal approximation properties in $\Omega_\ell$. Indeed, since the spaces $\XhatOm{k}{\ell}$ only contain the functions of $\Xhath{k}$ that are completely contained in $\Omega_\ell$, they do not reproduce global polynomials in $\Omega_\ell$, because this requires functions that are not completely supported in the subdomain.

%% After introducing all the machinery, we are now in a position to define the spline complex with hierarchical B-splines.

%% \subsection{The Hierarchical Spline Complex in the Parametric Domain}
%% The construction of the hierarchical spline complex is based on a simple idea: given a multi-level mesh, construct a sequence of hierarchical splines of mixed degree, using for each level the de Rham complex of tensor product B-splines in Section~\ref{sec:spline-complex}. We will see, however, that in general this construction does not give an exact complex of hierarchical splines.

%% Assume we are given a sequence of nested spline spaces
%% \begin{equation*}
%% \Xhat_{0,h} \subset \Xhat_{1,h} \subset \ldots \subset \Xhat_{N,h},
%% \end{equation*}
%% as in~\eqref{eq:subspaces}, and a sequence of nested subdomains as in~\eqref{eq:subdomains}. For each level $\ell = 0, \ldots, N$ we select $\Xhatlh{0} = \Xhat_{\ell,h}$, and construct a discrete de Rham complex using tensor-product splines of mixed degree, as explained in Section~\ref{sec:spline-complex}. This forms a complex $(\Xhatlh{},d)$ for each level:
%% \begin{equation} \label{eq:spline_complex}
%% \begin{CD}
%% \Xhatlh{0} @>d^0>> \Xhatlh{1} @>d^1>> \ldots @>d^{n-1}>> \Xhatlh{n} .
%% \end{CD}
%% \end{equation}
%% Moreover, for each space of the sequence we use the same set of basis functions explained in Section~\ref{sec:spline-complex}, and denote it by ${\cal B}^k_\ell$. We recall that using these bases we can define isomorphisms from our spline complex to the low-order finite element complex defined on the Greville grid.

%% Now, for each $k =0, \ldots, n$ we can construct the hierarchical spline bases ${\cal H}^k_N$ and the corresponding hierarchical spline space $\What^k_N = {\rm span} \{ {\cal H}^k_N \}$ following the same procedure as in Definition~\ref{def:hierarchical}. {\Rd In practice, for spaces of vector-valued splines, the hierarchical spline space can be computed using the recursive algorithm for each component}.

%% As in \eqref{eq:B_lk} and \eqref{eq:Bik}, it will be useful to define for $0 \le \ell \le \ell' \le N$, and for $0 \le k \le n$ the set of basis functions of level $\ell$ that are completely contained in $\Omega_{\ell'}$, that is
%% \begin{equation*}
%% {\cal B}^k_{\ell,\Omega_{\ell'}} \equiv {\cal B}^k_{\ell,\ell'} := \{ \beta^k \in {\cal B}^k_\ell : \supp (\beta^k) \subset \Omega_{\ell'} \}.
%% \end{equation*}
%% Moreover, we can also apply Definition~\ref{def:X_ell} for each $k$ to define
%% \begin{align}
%% & \What^k_\ell := {\rm span}\{{\cal H}^k_\ell\}, \\
%% & \Xhat^k_{\ell,\Omega_{\ell'}} \equiv \Xhat^k_{\ell,\ell'} := {\rm span} \{{\cal B}^k_{\ell,\ell'}\} =  \{ u^k \in \Xhatlh{k}  : \supp (u^k) \subset \Omega_{\ell'} \},
%% \end{align}
%% and the results of Lemma~\ref{lemma:cupcap} also hold. These spaces also form spline complexes, as it is proved in the next lemma.

%% \begin{lemma}
%% For $0 \le \ell \le \ell' \le N$, $(\Xhat_{\ell,\ell'},d)$ and $(\What_\ell,d)$ are two de Rham sequences, not necessarily exact.
%% \end{lemma}
%% \begin{proof}
%% The result for $\Xhat^k_{\ell,\ell'}$ holds from Section~\ref{sec:submesh}. For $\What^k_\ell$, since the spaces are contained in $\Xhatlh{k}$, the differential operators $d^k$ are well defined, and to prove the result we proceed by induction. The result is true for $\ell =0$, since $\What^k_0 = \hat X^k_{0,h}$ are the tensor-product spline spaces in Section~\ref{sec:spline-complex}. Assuming that $(\What_\ell,d)$ forms a de Rham sequence, the result holds for $(\What_{\ell+1},d)$, because by Lemma~\ref{lemma:cupcap} $\What^k_{\ell+1} = \What^k_{\ell} + \Xhat^k_{\ell+1,{\ell+1}}$, and it is immediate to see that $d^k (\What^k_{\ell} + \Xhat^k_{\ell+1,{\ell+1}}) \subset (\What^{k+1}_{\ell} + \Xhat^{k+1}_{\ell+1,{\ell+1}})$.
%% % and {\Rd Lemma~\ref{lemma:cupcap_derham}}, because $\What^i_{\ell+1} = \What^i_{\ell} \cup \What^i_{\ell+1,\Omega_{\ell+1}}$.
%% \end{proof}

%% In particular, for $\ell = N$ the lemma guarantees that the hierarchical spline spaces $\What^i_N$ form a de Rham complex, but the complex {\bf \emph{may not be exact}}.{\Rd REDUCED COHOMOLOGY} Actually, it is relatively easy to find counterexamples where the hierarchical spline spaces do not form an exact sequence. For instance, in the two-dimensional case a necessary (but not sufficient) condition for exactness is
%% \begin{equation*}
%% \dim (\What^0_N) + \dim (\What^2_N) = \dim (\What^1_N) + 1.
%% \end{equation*}
%% We can see that the condition is not fulfilled in the example of Figure~\ref{fig:2x2} for degree $p=3$ and maximum continuity. In this case, a simple computation gives that the dimension of the hierarchical spaces with boundary conditions is $\dim (\What^0_N) = 147$, $\dim (\What^1_N) = 328$, $\dim(\What^2_N) = 181$, which violates the previous condition.

%% \begin{figure}[ht]
%% \centerline{\includegraphics[width=0.45\textwidth]{refined_2x2}}
%% \caption{A hierarchical mesh for which the sequence is not exact, for $p=3$.}
%% \label{fig:2x2}
%% \end{figure}

%% The exactness of the sequence is crucial for the correct behavior of discretization schemes based on this discrete complex. {\Rd REWRITE For instance, if the spaces of the complex are to be used for the solution of mixed problems, working with a non-exact sequence may deteriorate the inf-sup stability constant at each refinement step}. Losing the exactness of the sequence may also lead to spurious solutions, as we will see in the examples of Section~\ref{sec:tests} for the solution of Maxwell eigenvalue problem.

%% In the next sections we provide conditions to guarantee that the hierarchical spline spaces form an exact de Rham complex.

%% \subsection{The Hierarchical Spline Complex in the Physical Domain}
%% The hierarchical spline complex in the physical domain is built in exactly the same manner as the B-spline complex.  Namely, we simply use the pullback operators defined in Subsection \ref{subsec:pullback}, yielding:
%% \begin{equation*}
%% W_\ell^k := \left\{ \omega : \iota^k(\omega) \in \Xhath{k} \right\}
%% \end{equation*}
%% for all integers $0 \leq k \leq n$ and $0 \leq \ell \leq N$.

%% \subsection{Extension to Multi-patch Geometries}
%% {\color{blue} \textbf{Remarks (John):} This is not the worst ever, but it may be pretty confusing for the new reader.  Though at this point, I am not sure I care so much about the new reader =).}\\

%% {\Rd I DON'T LIKE THIS SECTION, BUT IT IS A STARTING POINT}

%% {\Rd WE SHOULD DISCUSS ABOUT THE FIGURES.}

%% Most geometries of scientific and engineering interest cannot be represented as the image of the unit domain. For complex geometries we invoke the multi-patch concept. We assume that there exist $n_p$ smooth parametrizations of the form
%% \[
%% {\bf F}^{(j)} : (0,1)^n \rightarrow \Omega^{(j)} \subset \mathbb{R}^n, \quad j = 1, \ldots, n_p,
%% \]
%% such that the patches $\Omega^{(j)}$ do not overlap, then the domain is defined as the union of the $n_p$ patches
%% \[
%% \overline \Omega = \bigcup_{j=1}^{n_p} \overline {\Omega^{(j)}}.
%% \]
%% The construction of multi-patch spaces for tensor-product B-splines and conforming meshes is standard: assuming that the meshes of two adjacent patches are conforming on the interface, that is, the restriction of the parametrization and the knot vectors on the interface are the same, then $C^0$ functions for 0-forms are constructed as an equivalence of basis functions from the adjacent patches, see \cite[Section~3.5]{IGA-book}, and \cite[Section~3.2]{BBSV-acta} for the assumptions on the interface. Under the same assumptions, differential forms for B-splines on multi-patch domains can be also defined \cite[Section~5.4]{BBSV-acta}. Denoting by $(X_h^{(j)},d)$ the B-spline complex in the patch $\Omega^{(j)}$, the multi-patch spaces are given by 
%% \begin{equation} \label{eq:spline_complex_multipatch}
%% X^k_h = \{ u \in X^k : u|_{\Omega^{(j)}} \in X_h^{k,(j)} \},
%% \end{equation}
%% while in practice the basis functions are again constructed as an equivalence of basis functions between adjacent patches, plus an {\bf \emph{orientation}} for the functions associated to edges and faces of the Greville grid. The orientation of these functions can be directly associated to the entities of the Greville grid, and it works exactly as in the finite element case.

%% To define hierarchical differential forms in a multi-patch domain, one must take into account the presence of non-conforming meshes between patches \cite{Scott2014222}. This can be easily done following the approach used in \cite{Buchegger2016159} for 0-forms: we start defining a multi-patch spline complex for each level, using only tensor-product B-splines on each patch as in \eqref{eq:spline_complex_multipatch}; then we apply the hierarchical algorithm of Definition~\ref{def:hierarchical} to the multi-patch spaces of the complex, taking into account that the support of interface functions overlaps two or more patches. With this procedure, the check of the support and the orientation assignment can be done at the tensor-product level. We show an example of the construction for the mesh in Figure~\ref{fig:multipatch}, where the thick line represents the interface between both interfaces. The set of active basis functions for 0-forms is given in Figure~\ref{fig:multi_0forms}, for levels zero and one. We note the presence at level zero of an active basis function on the interface, that would not appear on the left patch when considering the patches separately. Similarly, some functions of level one on the interface are not active, but would be active on the left patch if we considered the patches separately. A similar behavior is also encountered for the 1-forms of Figure~\ref{fig:multi_1forms}.

%% \begin{figure}
%% \centerline{\includegraphics[width=0.8\textwidth, trim=5cm 4cm 4cm 3cm, clip]{multipatch_bezier}}
%% \caption{B\'ezier mesh for a simple multi-patch geometry}\label{fig:multipatch}
%% \end{figure}

%% \begin{figure}[ht]
%% \begin{subfigure}[Active basis functions of level 0]{
%% \includegraphics[width=0.49\textwidth, trim=5cm 4cm 4cm 3cm, clip]{multipatch_0forms_level1}
%% \label{fig:multi_0forms_1lev}
%% }
%% \end{subfigure}
%% \begin{subfigure}[Active basis functions of level 1]{
%% \includegraphics[width=0.49\textwidth, trim=5cm 4cm 4cm 3cm, clip]{multipatch_0forms_level2}
%% \label{fig:multi_0forms_2lev}
%% }
%% \end{subfigure}
%% \caption{Active basis functions for 0-forms, corresponding to the multi-patch example in Figure~\ref{fig:multipatch}}
%% \label{fig:multi_0forms}
%% \end{figure}

%% \begin{figure}[ht]
%% \begin{subfigure}[Active basis functions of level 0]{
%% \includegraphics[width=0.49\textwidth, trim=5cm 4cm 4cm 3cm, clip]{multipatch_1forms_level1}
%% \label{fig:multi_1forms_1lev}
%% }
%% \end{subfigure}
%% \begin{subfigure}[Active basis functions of level 1]{
%% \includegraphics[width=0.49\textwidth, trim=5cm 4cm 4cm 3cm, clip]{multipatch_1forms_level2}
%% \label{fig:multi_1forms_2lev}
%% }
%% \end{subfigure}
%% \caption{Active basis functions for 1-forms, corresponding to the multi-patch example in Figure~\ref{fig:multipatch}}
%% \label{fig:multi_1forms}
%% \end{figure}



==> paper_1/introduction.tex <==
Many systems of partial differential equations exhibit important underlying geometric structure, often in the form of topological constraints, conservation or balance laws, symmetries, or invariants. For a large collection of these systems, the underlying geometric structure is best expressed in the language of exterior calculus of differential forms. For instance, the primary quantities of interest in electromagnetics, namely potential fields, electric fields, magnetic fields, and current densities, may be described as differential 0, 1, 2, and 3-forms, respectively, and the symmetry and invariance properties of Maxwell's equations are directly embedded in the classical de Rham complex of differential forms \cite{BOS88}.  Consequently, there has been significant research in recent years dedicated to the development of numerical methods based on discrete analogues of exterior calculus, including discrete exterior calculus \cite{DEC-arxiv,Hirani-darcy,Hirani} and finite element exterior calculus \cite{AFW06,AFW-2}.

Isogeometric discrete differential forms were recently introduced to extend finite element exterior calculus to the emerging framework of isogeometric analysis \cite{BRSV11,Buffa_Sangalli_Vazquez}.  Isogeometric discrete differential forms are constructed via an exact sequence of spline spaces of mixed degree, and they can be understood as generalizations of nodal, edge, face, and volume finite elements to splines of high regularity.  Isogeometric discrete differential forms were first constructed based on tensor-product B-splines, though generalizations based on analysis-suitable T-splines \cite{BSV14} and LR B-splines \cite{Johannessen15} have also been proposed.  It was shown in \cite{BRSV11} that isogeometric discrete differential forms based on tensor-product B-splines conform to a commutative de Rham diagram in conjunction with specially defined projection operators, thus they are a suitable candidate for use in computational electromagnetics.  Indeed, isogeometric discrete differential forms have been applied to the stable and convergent discretization of Maxwell's equations \cite{BRSV11,Corno20161}, and they have also been used in the development of divergence-conforming discretization methods for incompressible fluid flow \cite{Buffa_deFalco_Sangalli,Evans12,EvHu12,EvHu12-2,EvHu12-3,Van17}.  In these works, it is demonstrated that isogeometric discrete differential forms are more accurate on a per degree of freedom basis than classical finite element methods for electromagnetic scattering and incompressible fluid flow.

In this paper, we extend the definition of isogeometric discrete differential forms to the setting of hierarchical B-splines.  As opposed to tensor-product B-splines, hierarchical B-splines allow for local refinement of a B-spline space through the select addition of basis functions belonging to a hierarchy of nested B-spline spaces \cite{Grinspun02,Kraft,Vuong_giannelli_juttler_simeon}.  Therefore, they may be employed in an adaptive isogeometric solution framework in conjunction with suitable error estimators and refinement strategies \cite{Kuru14,Buffa16-1,Buffa16-2,BGi17}.  Hierarchical B-splines have been successfully applied to problems arising in fluid mechanics \cite{Dettmer16}, structural mechanics \cite{Schillinger12}, and fluid-structure interaction \cite{Kadapa16}, though they have not yet been applied to the stable approximation of electromagnetic scattering or the divergence-conforming approximation of incompressible fluid flow.  These latter applications require the use of hierarchical B-spline spaces comprising a discrete de Rham complex, inspiring the current work.

There are many challenges associated with extending isogeometric discrete differential forms to hierarchical B-splines, including the specification of conditions guaranteeing exactness and stability of the hierarchical B-spline complex of isogeometric discrete differential forms.  In this paper, we not only define isogeometric discrete differential forms based on hierarchical B-splines, but we also derive a sufficient and necessary condition guaranteeing exactness of the hierarchical B-spline complex for arbitrary spatial dimension.  Moreover, we derive a set of local, easy-to-compute, and sufficient exactness conditions for the two-dimensional setting, and we demonstrate through numerical example that these conditions also yield stable approximations of both the Maxwell eigenvalue problem and the Stokes problem.  Though the focus of this paper is on hierarchical B-splines, the theory presented in this paper also applies to other spaces of discrete differential forms with hierarchical structure including hierarchical T-splines \cite{Evans15} and wavelets \cite{Cohen01}.

An outline of the paper is as follows.  In Section~\ref{sec:derham}, we discuss mathematical preliminaries, including mathematical notation as well as the definition of the de Rham complex of differential forms.  In Section~\ref{sec:splinecomplex}, we present the B-spline complex of isogeometric discrete differential forms, and we discuss exactness and stability properties exhibited by the B-spline complex.  In Section~\ref{sec:hierarchicalcomplex}, we introduce the hierarchical B-spline complex of isogeometric discrete differential forms.  In Section~\ref{sec:exactness}, we examine the cohomological structure of the hierarchical B-spline complex, and we establish a set of conditions guaranteeing exactness of the complex.  In Section~\ref{sec:stability}, we examine the stability properties of the hierarchical B-spline complex in the context of the Maxwell eigenvalue problem and the Stokes problem.  In Section~\ref{sec:tests}, we apply the hierarchical B-spline complex to the numerical solution of canonical electromagnetics and creeping flow problems of interest.  Finally, in Section~\ref{Sec:conclusion}, we draw conclusions.


==> paper_1/numericalresults.tex <==
% \textcolor{black}{All this section has to be checked.}

% \textcolor{black}{Increase the fontsize of the figures.}

% \textcolor{black}{Use exterior derivative also for the the Galerkin formulation. Write the two formulations separately. Use spaces with boundary conditions. The same for Maxwell.}

% \textcolor{black}{The geometry is planar, use a planar view. In the figure, the geometry looks $C^0$. Give the knot vector and control points.}
In the following the analysis from the previous section is numerically tested on selected elliptic problems, furthermore the important case of eigenvalue approximation is studied numerically to consolidate the more general structure preserving aim of the proposed method. Time dependent problems will be studied in a subsequent companion contribution, for which the present study provides a necessary foundation.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/harmonic_deformation.eps}\qquad
    \includegraphics[width=0.45\textwidth]{figures/nurbs_eighth_ring.eps}
    \caption{\magentamod{Reparametrization of the unit square via the map in \eqref{eq:harmonic_map} with $a=0.3$ and the one-eighth ring geometry $\Omega = [1,2]\times[0,\pi/4]$ in polar coordinates $(r,\varphi)$, used for both the boundary value and eigenvalue test problem studied.}}\label{fig:reparam}
\end{figure}

\subsection{Elliptic boundary value problem} \label{sec:elliptic_numerical}
As a first test we show how the various approaches to construct a discrete Hodge operator work for a problem in which only one Hodge--star operator, namely $\star^1_\gamma$, is needed. The discretization of the static problem \eqref{eq:continuousproblem} \textcolor{black}{with $k=0$ fits the requirements, since taking $\gamma=1$ and $\beta=0$ gives us the standard Poisson problem}.
%In the usual IGA setting we write the problem in weak form and, given an $f\in L^2$, we seek $u\in X_h^0$ such that:
% \begin{equation}
%     \langle \nabla u,\nabla v \rangle = \langle f, v \rangle, \;\;\;\forall v \in X_{0,h}^0,\label{eq:galerkin}
% \end{equation}
% \begin{equation}
%      -d^{n-1}\star_h^1 d^0 u  = \star_h^0\left(\Pi_{L^2}^{X_h^0}(f)\right),\label{eq:hodge_f}
% \end{equation}
% \noindent where we use the same symbol for vector proxies and differential forms for the sake of readability. It is understood that there is always an isomorphism between the two spaces.
As a convergence test we choose the domain to be the usual unit square $\Omega = \hat{\Omega} := (0,1)^n$, but in the more interesting case in which the interior of the physical domain has been displaced by means of the map
\begin{equation}
x_i = u_i + \frac{a}{2}\, \textcolor{black}{\Pi_{j=1}^{n} \sin (2\pi(u_j-1/2))} , \; \text{ for } i \in \{ 1, 2, \dots , n\},\label{eq:harmonic_map}
\end{equation}
%\begin{align}\label{eq:harmonic_map}
%    & x = u + \frac{a}{2}\, sin (2\pi(u-1/2)) sin(2\pi(v-1/2))),\\
%    & y = v + \frac{a}{2}\, sin (2\pi(u-1/2)) sin(2\pi(v-1/2))),
%\end{align}
\noindent inspired by \cite{jain_construction_2020}, where $u_i$ are the parametric coordinates while $x_i$ are the physical ones on the mapped domain. The parameter $a$, with $0<a<1$, regulates the peak deformation in the mesh with respect to a Cartesian--orthogonal one, and we set $a = 0.3$. The effect of the above is to obtain a nontrivial map of $\hat{\Omega}$ to itself, shown \magentamod{on the left in Fig.~\ref{fig:reparam}}. In this way, we can evaluate how faithfully a non-polynomial perturbation of the metric is approximated by the Hodge--star operator on a test for which a well-known closed form solution is still easily computable.
For starting polynomial degrees $p=3,4,5$ in the primal sequence and \magentamod{$p-1$ continuity} we show performance of the standard Galerkin IGA, as implemented in \cite{Vazquez_2016aa}, and discrete Hodge--star $\star_h^1$ obtained either by \textcolor{black}{the global operator \eqref{eq:def_hodge_discrete1} (labeled $1^{st}$ in the plots), by the global $L^2$--projection onto the target space \eqref{eq:def_hodge_discrete2} (labeled $2^{nd}$ in the plots)}, or by the quasi-interpolant based on local projections discussed in Section~\ref{sec:dsplinecomplex} (labeled $3^{rd}$).
We show convergence rates in the ${H\Lambda^0(\Omega)}$ norm %(or equivalently, the usual $H^1$ norm) 
in Fig.~\ref{fig:h1_error_noK} %with specific attention dedicated to the cases of lower regularity of basis functions for the case of $p=5$ in Fig.~\ref{fig:h1_error_lowreg}.
where asymptotic rates confirm the theoretical results of Section~\ref{sec:erroranalysis}.
\magentamod{The values obtained for the errors are also tabulated in Table \ref{tab:h1_error_table1} for reproducibility of convergence rate.}
Specifically, the first global operator converges as fast as the standard IGA Galerkin approach, as expected from the result in Theorem~\ref{thm:first-hodge}. The standard Galerkin IGA approach can be shown in fact to be algebraically derivable from the first approach, even though they are not computationally equivalent.
The convergence rate of the second operator %depends on the regularity of splines, and achieves better rates when lower regularity is enforced.
and of the local operator usually have one order of convergence less and confirm the analysis in Theorem~\ref{thm:error_bound}.

%%%%%%%%%%%%%%%%% H1 norm error %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t!]
    \centering 
    \begin{tikzpicture}[]
    %/*
\pgfplotsset{
    width=0.36\textwidth, 
    height=0.36\textwidth, 
    ymin=10^-7.5,ymax=200,xmin=8e-3,xmax=0.15, 
    ylabel near ticks,
    tick label style={font=\footnotesize},
    % legend style={font=\scriptsize, }, 
    label style={font=\footnotesize},
    every x tick scale label/.style={at={(1,0)},anchor=north,yshift=-5pt,inner sep=0pt},
%     scaled y ticks = false,
%     width=\fwidth*0.35,
%     height=\fheight,
%     axis on top,
%     xticklabel style={text width=2em,align=center},
%     xticklabels={\empty},
%     xmin=-5,xmax=5,
%     ymin=-5,ymax=5,
%     xminorticks=true,
%     yminorticks=true,
%     ylabel shift={-1.5em},
%     ylabel style={align=center}
}
%     
        \begin{groupplot}[ 
            group style={
            group size=3 by 1,
            % vertical sep=25pt,
            horizontal sep=30pt
            },
        ]
        %-----------
        % Plot [1, 1]
        %-----------
            \nextgroupplot[ymode=log,xmode=log,title={$p=3,\;C^2$},ylabel={$H\Lambda^0$ error},xlabel={$h$},
            legend style={at={($(0,0)+(1cm,1cm)$)},legend columns=4,fill=none,draw=black,anchor=center,align=center},
            legend to name=fred]
            \addplot [blue, mark=triangle*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_mappedsquare_p3r2_global.csv};
            \addplot [red, mark=*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_mappedsquare_p3r2_l2.csv};
            \addplot [green, mark=square*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_mappedsquare_p3r2_llm.csv};
            \addplot [magenta, mark=diamond*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_mappedsquare_p3r2_standard_iga.csv};
            % \node[] at (axis cs:10^-1.6, 10)   (a) {$p=3,\;C^2$};
            \draw (axis cs:0.024,2^2*10^-1.9)--(axis cs:0.012,10^-1.9)--(axis cs:0.012,2^2*10^-1.9) node[pos=0.05,anchor=north] {}--cyclenode[pos=0.0,anchor=west] {};
            \draw (axis cs:0.025,10^-4.5)--(axis cs:0.0125,10^-4.5)--(axis cs:0.025,2^3*10^-4.5) node[pos=0.05,anchor=north] {}--cyclenode[pos=0.0,anchor=west] {};
            \node[] at (axis cs:0.01,10^-1.8)   (c) {$2$};
            \node[] at (axis cs:0.03, 10^-4.0)   (c) {$3$};
            \node[] at (axis cs:0.02,10^-0.8)   (c) {$1$};
            \node[] at (axis cs:0.02,10^-5.0)   (c) {$1$};
            \addlegendentry{1$^{\text{st}}$};    
            \addlegendentry{2$^{\text{nd}}$};    
            \addlegendentry{3$^{\text{rd}}$};   
            \addlegendentry{IGA}; 
            \coordinate (c1) at (rel axis cs:0,1);
        %-----------
        % Plot [1, 2]
        %-----------
            \nextgroupplot[ymode=log,xmode=log,title={$p=4,\;C^3$},xlabel={$h$}]
            \addplot [blue, mark=triangle*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_mappedsquare_p4r3_global.csv};
            \addplot [red, mark=*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_mappedsquare_p4r3_l2.csv};
            \addplot [green, mark=square*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_mappedsquare_p4r3_llm.csv};
            \addplot [magenta, mark=diamond*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_mappedsquare_p4r3_standard_iga.csv};
            % \node[] at (axis cs:10^-1.6, 10)   (a) {$p=4,\;C^3$};
            \draw (axis cs:0.024,2^3*10^-3)--(axis cs:0.012,10^-3)--(axis cs:0.012,2^3*10^-3) node[pos=0.05,anchor=north] {}--cyclenode[pos=0.0,anchor=west] {};
            \node[] at (axis cs:0.01,10^-2.5)   (c) {$3$};
            \draw (axis cs:0.025,10^-5.5)--(axis cs:0.0125,10^-5.5)--(axis cs:0.025,2^4*10^-5.5) node[pos=-0.05,anchor=north] {}--cyclenode[pos=1.0,anchor=west] {};
            \node[] at (axis cs:0.03, 0.9*10^-5.5+0.1*2^4*10^-5.5)   (b) {$4$};
            \node[] at (axis cs:0.02,10^-1.5)   (c) {$1$};
            \node[] at (axis cs:0.02,10^-6.0)   (c) {$1$};
        %-----------
        % Plot [1, 3]
        %-----------
            \nextgroupplot[ymode=log,xmode=log,title={$p=5,\;C^4$},xlabel={$h$}]
            \addplot [blue, mark=triangle*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_mappedsquare_p5r4_global.csv};
            \addplot [red, mark=*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_mappedsquare_p5r4_l2.csv};
            \addplot [green, mark=square*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_mappedsquare_p5r4_llm.csv};
            \addplot [magenta, mark=diamond*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_mappedsquare_p5r4_standard_iga.csv};
            % \node[] at (axis cs:10^-1.6, 10)   (a) {$p=5,\;C^4$};
            \draw (axis cs:0.0125,2^4*10^-3.7)--(axis cs:0.0125,10^-3.7)--(axis cs:0.025,2^4*10^-3.7) node[pos=-0.05,anchor=north] {}--cyclenode[pos=1.0,anchor=west] {};
            \draw (axis cs:0.03,10^-6.3)--(axis cs:0.015,10^-6.3)--(axis cs:0.03,2^5 * 10^-6.3) node[pos=-0.05,anchor=north] {}--cyclenode[pos=1.0,anchor=west] {};
            \node[] at (axis cs:0.01, 10^-3.0)   (b) {$4$};
            \node[] at (axis cs:0.035, 0.95*10^-6.0+0.05*2^5*10^-6.0)   (c) {$5$};
            \node[] at (axis cs:0.02,10^-1.8)   (c) {$1$};
            \node[] at (axis cs:0.02,10^-7.0)   (c) {$1$};
            % (Relative) Coordinate at top of the second plot
            \coordinate (c2) at (rel axis cs:1,1);
        \end{groupplot}
        \coordinate (c3) at ($(c1)!.5!(c2)$);
        \node[below] at (c3 |- current bounding box.south)
        {\pgfplotslegendfromname{fred}};
    \end{tikzpicture} 
    \caption{Elliptic source problem for the parametric domain, with the nontrivial map of (\ref{eq:harmonic_map}): a comparison of the error in the $H\Lambda^0(\Omega)$ norm (or $H^1$ norm) for the three choices of discrete Hodge operators.}%\textcolor{black}{FOR ALL FIGURES: in the reference triangle, the length should be in the proper place, next to the side of length $k$ (the vertical side). You can also consider writing the two lengths, $1$ (horizontal) and $k$ (vertical), as in the CMAME paper.}}
    \label{fig:h1_error_noK}
\end{figure}

\begin{table}\scriptsize
    \centering
\begin{tabular}{lccc}
     & \multicolumn{3}{c}{$p=3,\; C^2$} \\
    \cmidrule(lr){2-4}
    $\star_h$ choice  & $h=0.05$   & $h=0.025$ & $h=0.0125$    \\\midrule
    1$^{\text{st}}$  & \num[round-precision=3,round-mode=figures]{0.025311} & \num[round-precision=3,round-mode=figures]{0.0019756} & \num[round-precision=3,round-mode=figures]{0.00021078} \\
    2$^{\text{nd}}$ & \num[round-precision=3,round-mode=figures]{0.16429} & \num[round-precision=3,round-mode=figures]{0.021151} & \num[round-precision=3,round-mode=figures]{0.003267} \\
    3$^{\text{nd}}$ & \num[round-precision=3,round-mode=figures]{0.090346} & \num[round-precision=3,round-mode=figures]{0.017625} & \num[round-precision=3,round-mode=figures]{0.0040793} \\
    IGA  & \num[round-precision=3,round-mode=figures]{0.024755} & \num[round-precision=3,round-mode=figures]{0.0019579} & \num[round-precision=3,round-mode=figures]{0.00021004} \\\toprule
    & \multicolumn{3}{c}{$p=4,\; C^3$}\\
    \cmidrule(lr){2-4}
    $\star_h$ choice & $h=0.05$   & $h=0.025$ & $h=0.0125$  \\\midrule
    1$^{\text{st}}$  & \num[round-precision=3,round-mode=figures]{0.0066309} & \num[round-precision=3,round-mode=figures]{0.00019995} & \num[round-precision=3,round-mode=figures]{9.8496e-06} \\
    2$^{\text{nd}}$ & \num[round-precision=3,round-mode=figures]{0.012494} & \num[round-precision=3,round-mode=figures]{0.00058874} & \num[round-precision=3,round-mode=figures]{2.5853e-05}\\
    3$^{\text{nd}}$  & \num[round-precision=3,round-mode=figures]{0.03654} & \num[round-precision=3,round-mode=figures]{0.0019885} & \num[round-precision=3,round-mode=figures]{0.0001148} \\
    IGA  & \num[round-precision=3,round-mode=figures]{0.006577} & \num[round-precision=3,round-mode=figures]{0.00019968} & \num[round-precision=3,round-mode=figures]{9.8464e-06}\\\toprule
    & \multicolumn{3}{c}{$p=5,\; C^4$}\\
    \cmidrule(lr){2-4}
    $\star_h$ choice  & $h=0.05$   & $h=0.025$ & $h=0.0125$ \\\midrule
    1$^{\text{st}}$    & \num[round-precision=3,round-mode=figures]{0.0023772} & \num[round-precision=3,round-mode=figures]{2.5016e-05} & \num[round-precision=3,round-mode=figures]{5.3954e-07} \\
    2$^{\text{nd}}$  & \num[round-precision=3,round-mode=figures]{0.0024953} & \num[round-precision=3,round-mode=figures]{7.2662e-05} & \num[round-precision=3,round-mode=figures]{3.365e-06} \\
    3$^{\text{nd}}$    & \num[round-precision=3,round-mode=figures]{0.02376} & \num[round-precision=3,round-mode=figures]{0.0010841} & \num[round-precision=3,round-mode=figures]{5.8109e-05} \\
    IGA & \num[round-precision=3,round-mode=figures]{0.0023637} & \num[round-precision=3,round-mode=figures]{2.494e-05} & \num[round-precision=3,round-mode=figures]{5.3898e-07} \\\toprule
\end{tabular}
    \caption{Values for errors displayed in Fig.~\ref{fig:h1_error_noK}, $H\Lambda^0$ error, $\Omega$ as in Fig.~\ref{fig:reparam} (left).} \label{tab:h1_error_table1}
\end{table}

%\textcolor{black}{COMMENT: are you using $\hat \Omega$ or the mapped domain? Say it explicitly.} 
Another interesting case in which a high order geometric method is desired is the case in which material parameters involved in the constitutive equations are not piecewise constants but instead smooth functions, This setting, in which we instead use the parametric domain $\Omega = \hat \Omega$ \magentamod{defined with the identity mapping}, is particularly relevant in the wave propagation simulations, for instance in designing non reflective boundary conditions via perfectly matched layers~\cite{collino_optimizing_1998}.
We choose as an example the material parameter 
\begin{equation}\label{eq:smoothgamma}
\gamma = 1 + e^{-\frac{(x-1/2)^2 + (y-1/2)^2}{20^2}},
\end{equation} 
and perform a new convergence test by means of a manufactured solution on the unit square with homogeneous boundary conditions. This second test differs from the first one since the material parameter acts as a weight in the projection but is not involved in the pullbacks of differential forms, differently from manipulating the geometry of the domain. \textcolor{black}{To compute the integrals we use the same quadrature rules as in the previous test, which are Gauss-Legendre rules with $(p+1)^2$ quadrature points per element. 
The convergence results in Fig.~\ref{fig:h1_error_smooth_coeff} confirm that we maintain the convergence rates of the previous case, in which we only manipulated the geometry, without adding more quadrature points.}
\magentamod{Again, numerical values obtained for the errors are also tabulated in Table \ref{tab:h1_error_table2}.} %Low order methods fail to construct accurate discrete Hodge--star operators in this case even in the case of mesh cells which involve only affine maps from a reference cell.} %ARE YOU SURE OF THIS? I mean, how bad is the approximation with low order methods, if we consider a piecewise constant approximation of the material?}

The condition number of the resulting system matrices for the test problem is studied in Fig.~\ref{fig:conditioning_and_sparsity_laplace}, left panel, \textcolor{black}{for the practically very relevant case of splines of degree $p=3$ and maximum smoothness for the $X^0$ space}.
When dealing with a square and invertible matrix $\mathbf{A}$, the condition number $\kappa(\mathbf{A})$ is defined in terms of the 2-norm of $\mathbf{A}$ as follows: %\textcolor{black}{COMMENT: the definition was not correct, and the spectral radius and the 2-norm are not the same in general.}
$\kappa(\mathbf{A}) = {\Vert\mathbf{A}\Vert_2} {\Vert\mathbf{A^{-1}}\Vert_2}$.
%\noindent \textcolor{black}{THIS SENTENCE CAN BE REMOVED, RIGHT? HOW ARE YOU COMPUTING THE CONDITION NUMBER?} but the definition is easily extended to the case of non-symmetric ones.
In our examples $\kappa$ is computed for the matrix discretising the composition of exterior derivatives (pre-- and post--) with the $\star_h^1$ operator, \textcolor{black}{ that is, the matrix on the left-hand side of \eqref{eq:problem_matrix} with $\beta = 0$}. \textcolor{black}{The new approach in general yields the same asymptotic growth in condition number under mesh refinement as standard IGA, albeit degraded by a constant factor.} Furthermore, we remark that the system matrices \textcolor{black}{in \eqref{eq:problem_matrix}} are not in general symmetric and require an appropriate solving strategy (e.g. GMRES). \textcolor{black}{While this can be fixed for the two global operators by multiplying by the matrix $\tilde{\mathbf{K}}^k_{n-k}$ (which is equivalent to multiply by a test function, as we did for the analysis in Section~\ref{sec:erroranalysis}), the problem remains for the local operator based on quasi-interpolants. This is an important issue} when one aims to use the new machinery to evolve hyperbolic systems of equations in time, and it begs for further theoretical study.

% and a comparison is shown for all approaches, again in Fig.~\ref{fig:conditioning_and_sparsity_laplace}.
The sparsity achieved in the final system matrix is also reported in Fig.~\ref{fig:conditioning_and_sparsity_laplace} on the right panel, \textcolor{black}{where we plot the number of nonzeros again for degree $p=3$ and maximum continuity of the spline spaces}. The local projector yields sparser system matrices than the global operators, as expected, and even sparser than the standard IGA approach by a factor which is not dependent on $h$.

%Unfortunately, in general, the local operator gives higher errors. In the case of lowest possible smoothness of $X_h^0$, i.e. $C^1$ 0--forms, the local projector becomes a conventional L$^2$ projection operator, since the support of basis functions is restricted to one knot--mesh element.

%%%%%%%%%%%%%%%%% L2 norm error %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \newpage
% \begin{figure}[h]
%     \centering
%     \begin{tikzpicture}[]
%         \begin{loglogaxis}[width=0.36\columnwidth, height=0.36\columnwidth, ylabel={L$^2$ error},xlabel={$h$}, 
%             ymin=10^-9.5,ymax=10,xmin=0.005,xmax=0.5,ylabel near ticks,tick label style={font=\footnotesize},  legend style={font=\scriptsize, }, label style={font=\footnotesize},every x tick scale label/.style={at={(1,0)},anchor=north,yshift=-5pt,inner sep=0pt},legend pos= south east]
%         \addplot [blue, mark=triangle*, mark options={solid}] table [x index=0, y index=1, col sep=comma] {figures/laplace_results_mappedsquare_p3r2_global.csv};
%         \addplot [red, mark=*, mark options={solid}] table [x index=0, y index=1, col sep=comma] {figures/laplace_results_mappedsquare_p3r2_l2.csv};
%         \addplot [green, mark=square*, mark options={solid}] table [x index=0, y index=1, col sep=comma] {figures/laplace_results_mappedsquare_p3r2_llm.csv};
%         \addplot [magenta, mark=diamond*, mark options={solid}] table [x index=0, y index=1, col sep=comma] {figures/laplace_results_mappedsquare_p3r2_standard_iga.csv};
%         \node[] at (axis cs:10^-1.6, 1)   (a) {$p=3,\;C^2$};
%         \draw (axis cs:0.025,10^-4.0)--(axis cs:0.0125,10^-4.0)--(axis cs:0.025,2^2*10^-4.0) node[pos=0.5,anchor=north] {}--cyclenode[pos=1.0,anchor=west] {};
%         \draw (axis cs:0.025,10^-6.5)--(axis cs:0.0125,10^-6.5)--(axis cs:0.025,2^4*10^-6.5) node[pos=0.05,anchor=north] {}--cyclenode[pos=0.0,anchor=west] {};
%         \node[] at (axis cs:0.33*0.0125+0.67*0.025, 0.67*10^-4.0+0.33*2^2*10^-4.0)   (b) {$2$};
%         \node[] at (axis cs:0.33*0.0125+0.67*0.025, 0.9*10^-6.5+0.1*2^4*10^-6.5)   (c) {$4$};
%         \legend{1$^{\text{st}}$ \\2$^{\text{nd}}$ \\3$^{\text{rd}}$ \\IGA\\}
%         \end{loglogaxis}
%     \end{tikzpicture}
%     \begin{tikzpicture}[]
%         \begin{loglogaxis}[width=0.36\columnwidth, height=0.36\columnwidth, xlabel={$h$}, 
%             ymin=10^-9.5,ymax=10,xmin=0.005,xmax=0.5,ylabel near ticks,tick label style={font=\footnotesize},  legend style={font=\scriptsize, }, label style={font=\footnotesize},every x tick scale label/.style={at={(1,0)},anchor=north,yshift=-5pt,inner sep=0pt},legend pos= south east]
%         \addplot [blue, mark=triangle*, mark options={solid}] table [x index=0, y index=1, col sep=comma] {figures/laplace_results_mappedsquare_p4r3_global.csv};
%         \addplot [red, mark=*, mark options={solid}] table [x index=0, y index=1, col sep=comma] {figures/laplace_results_mappedsquare_p4r3_l2.csv};
%         \addplot [green, mark=square*, mark options={solid}] table [x index=0, y index=1, col sep=comma] {figures/laplace_results_mappedsquare_p4r3_llm.csv};
%         \addplot [magenta, mark=diamond*, mark options={solid}] table [x index=0, y index=1, col sep=comma] {figures/laplace_results_mappedsquare_p4r3_standard_iga.csv};
%         \node[] at (axis cs:10^-1.6, 1)   (a) {$p=4,\;C^3$};
%         \draw (axis cs:0.025,10^-5.5)--(axis cs:0.0125,10^-5.5)--(axis cs:0.025,2^4*10^-5.5) node[pos=-0.05,anchor=north] {}--cyclenode[pos=1.0,anchor=west] {};
%         \draw (axis cs:0.03,10^-7.5)--(axis cs:0.015,10^-7.5)--(axis cs:0.03,2^5 * 10^-7.5) node[pos=-0.05,anchor=north] {}--cyclenode[pos=1.0,anchor=west] {};
%         \node[] at (axis cs:0.33*0.0125+0.67*0.025, 0.9*10^-5.5+0.1*2^4*10^-5.5)   (b) {$4$};
%         \node[] at (axis cs:0.33*0.015+0.67*0.03, 0.95*10^-7.5+0.05*2^5*10^-7.5)   (c) {$5$};
%         \legend{1$^{\text{st}}$ \\2$^{\text{nd}}$ \\3$^{\text{rd}}$ \\IGA\\}
%         \end{loglogaxis}
%     \end{tikzpicture}
%     \begin{tikzpicture}[]
%         \begin{loglogaxis}[width=0.36\columnwidth, height=0.36\columnwidth, xlabel={$h$}, 
%             ymin=10^-9.5,ymax=10,xmin=0.005,xmax=0.5,ylabel near ticks,tick label style={font=\footnotesize},  legend style={font=\scriptsize, }, label style={font=\footnotesize},every x tick scale label/.style={at={(1,0)},anchor=north,yshift=-5pt,inner sep=0pt},legend pos= south east]
%         \addplot [blue, mark=triangle*, mark options={solid}] table [x index=0, y index=1, col sep=comma] {figures/laplace_results_mappedsquare_p5r4_global.csv};
%         \addplot [red, mark=*, mark options={solid}] table [x index=0, y index=1, col sep=comma] {figures/laplace_results_mappedsquare_p5r4_l2.csv};
%         \addplot [green, mark=square*, mark options={solid}] table [x index=0, y index=1, col sep=comma] {figures/laplace_results_mappedsquare_p5r4_llm.csv};
%         \addplot [magenta, mark=diamond*, mark options={solid}] table [x index=0, y index=1, col sep=comma] {figures/laplace_results_mappedsquare_p5r4_standard_iga.csv};
%         \node[] at (axis cs:10^-1.6, 1)   (a) {$p=5,\;C^4$};
%         \draw (axis cs:0.025,10^-5.7)--(axis cs:0.0125,10^-5.7)--(axis cs:0.025,2^4*10^-5.7) node[pos=-0.05,anchor=north] {}--cyclenode[pos=1.0,anchor=west] {};
%         \draw (axis cs:0.03,10^-8.5)--(axis cs:0.015,10^-8.5)--(axis cs:0.03,2^6 * 10^-8.5) node[pos=-0.05,anchor=north] {}--cyclenode[pos=1.0,anchor=west] {};
%         \node[] at (axis cs:0.33*0.0125+0.67*0.025, 0.95*10^-5.7+0.05*2^4*10^-5.7)   (b) {$4$};
%         \node[] at (axis cs:0.33*0.015+0.67*0.03, 0.95*10^-8.5+0.05*2^6*10^-8.5)   (c) {$6$};
%         \legend{1$^{\text{st}}$ \\2$^{\text{nd}}$ \\3$^{\text{rd}}$ \\IGA\\}
%         \end{loglogaxis}
%     \end{tikzpicture}
% \caption{Poisson problem: error in the $L^2$ norm in the case of the parametric domain, with the nontrivial map of (\ref{eq:harmonic_map}) for the three choices of discrete Hodge operators proposed in the paper.}
%     \label{fig:l2_error_noK}
% \end{figure}

%%%%%%%%%%%%%%%%% H1 norm error smooth eps %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t!]
    \centering 
    \begin{tikzpicture}[]
    %/*
        \pgfplotsset{
            width=0.36\textwidth, 
            height=0.36\textwidth, 
            ymin=10^-7.5,ymax=5*10^0,xmin=8e-3,xmax=0.15, 
            ylabel near ticks,
            tick label style={font=\footnotesize},
            % legend style={font=\scriptsize, }, 
            label style={font=\footnotesize},
            every x tick scale label/.style={at={(1,0)},anchor=north,yshift=-5pt,inner sep=0pt},
        %     scaled y ticks = false,
        %     width=\fwidth*0.35,
        %     height=\fheight,
        %     axis on top,
        %     xticklabel style={text width=2em,align=center},
        %     xticklabels={\empty},
        %     xmin=-5,xmax=5,
        %     ymin=-5,ymax=5,
        %     xminorticks=true,
        %     yminorticks=true,
        %     ylabel shift={-1.5em},
        %     ylabel style={align=center}
        }
%     
        \begin{groupplot}[ 
            group style={
            group size=3 by 1,
            % vertical sep=25pt,
            horizontal sep=30pt
            },
        ]
        %-----------
        % Plot [1, 1]
        %-----------
            \nextgroupplot[ymode=log,xmode=log,title={$p=2,\;C^1$},ylabel={$H\Lambda^0$ error},xlabel={$h$},
            legend style={at={($(0,0)+(1cm,1cm)$)},legend columns=4,fill=none,draw=black,anchor=center,align=center},
            legend to name=barney]
            \addplot [blue, mark=triangle*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_square_highreg_smoothgamma_p2r1_global.csv};
            \addplot [red, mark=*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_square_highreg_smoothgamma_p2r1_l2.csv};
            \addplot [green, mark=square*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_square_highreg_smoothgamma_p2r1_llm.csv};
            \addplot [magenta, mark=diamond*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_square_highreg_smoothgamma_p2r1_standard_iga.csv};
            % \node[] at (axis cs:10^-1.6, 10)   (a) {$p=2,\;C^1$};
            \draw (axis cs:0.012,0.5*10^-0.4)--(axis cs:0.024,10^-0.4)--(axis cs:0.012,10^-0.4) node[pos=0.05,anchor=north] {}--cyclenode[pos=0.0,anchor=west] {};
            \node[] at (axis cs:0.01, 10^-0.5)   (c) {$1$};
            \draw (axis cs:0.024,2^2*10^-3.4)--(axis cs:0.024,10^-3.4)--(axis cs:0.012,10^-3.4) node[pos=0.05,anchor=north] {}--cyclenode[pos=0.0,anchor=west] {};
            \node[] at (axis cs:0.03, 10^-3.2)   (c) {$2$};
            \node[] at (axis cs:0.02,10^-0.0125)   (c) {$1$};
            \node[] at (axis cs:0.02,10^-4.0)   (c) {$1$};
            \addlegendentry{1$^{\text{st}}$};    
            \addlegendentry{2$^{\text{nd}}$};    
            \addlegendentry{3$^{\text{rd}}$};   
            \addlegendentry{IGA}; 
            \coordinate (c1) at (rel axis cs:0,1);
        %-----------
        % Plot [1, 2]
        %-----------
            \nextgroupplot[ymode=log,xmode=log,title={$p=3,\;C^2$},xlabel={$h$}]
            \addplot [blue, mark=triangle*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_square_highreg_smoothgamma_p3r2_global.csv};
            \addplot [red, mark=*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_square_highreg_smoothgamma_p3r2_l2.csv};
            \addplot [green, mark=square*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_square_highreg_smoothgamma_p3r2_llm.csv};
            \addplot [magenta, mark=diamond*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_square_highreg_smoothgamma_p3r2_standard_iga.csv};
            % \node[] at (axis cs:10^-1.6, 10)   (a) {$p=3,\;C^2$};
            \draw (axis cs:0.024,2^2*10^-2.4)--(axis cs:0.012,10^-2.4)--(axis cs:0.012,2^2*10^-2.4) node[pos=0.05,anchor=north] {}--cyclenode[pos=0.0,anchor=west] {};
            \draw (axis cs:0.025,10^-5.0)--(axis cs:0.0125,10^-5.0)--(axis cs:0.025,2^3*10^-5.0) node[pos=0.05,anchor=north] {}--cyclenode[pos=0.0,anchor=west] {};
            \node[] at (axis cs:0.01, 10^-2.2)   (c) {$2$};
            \node[] at (axis cs:0.03, 10^-4.5)   (c) {$3$};
            \node[] at (axis cs:0.02,10^-1.2)   (c) {$1$};
            \node[] at (axis cs:0.02,10^-5.5)   (c) {$1$};
        %-----------
        % Plot [1, 3]
        %-----------
            \nextgroupplot[ymode=log,xmode=log,title={$p=4,\;C^3$},xlabel={$h$}]
            \addplot [blue, mark=triangle*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_square_highreg_smoothgamma_p4r3_global.csv};
            \addplot [red, mark=*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_square_highreg_smoothgamma_p4r3_l2.csv};
            \addplot [green, mark=square*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_square_highreg_smoothgamma_p4r3_llm.csv};
            \addplot [magenta, mark=diamond*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_square_highreg_smoothgamma_p4r3_standard_iga.csv};
            % \node[] at (axis cs:10^-1.6, 10)   (a) {$p=4,\;C^3$};
            \draw (axis cs:0.024,2^3*10^-3.4)--(axis cs:0.012,10^-3.4)--(axis cs:0.012,2^3*10^-3.4) node[pos=0.05,anchor=north] {}--cyclenode[pos=0.0,anchor=west] {};
            \node[] at (axis cs:0.01,10^-3.0)   (c) {$3$};
            \draw (axis cs:0.025,10^-6.4)--(axis cs:0.0125,10^-6.4)--(axis cs:0.025,2^4*10^-6.4) node[pos=-0.05,anchor=north] {}--cyclenode[pos=1.0,anchor=west] {};
            \node[] at (axis cs:0.03,10^-6.0)   (b) {$4$};
            \node[] at (axis cs:0.02,10^-2.0)   (c) {$1$};
            \node[] at (axis cs:0.02,10^-7.0)   (c) {$1$};
            % (Relative) Coordinate at top of the second plot
            \coordinate (c2) at (rel axis cs:1,1);
        \end{groupplot}
        \coordinate (c3) at ($(c1)!.5!(c2)$);
        \node[below] at (c3 |- current bounding box.south)
        {\pgfplotslegendfromname{barney}};
    \end{tikzpicture} 
    \caption{Static problem in the case of the parametric domain, with the smooth perturbation of the material parameter $\gamma$ introduced in \eqref{eq:smoothgamma}: a comparison of the error in the $H\Lambda^0(\Omega)$ norm (or $H^1$ norm) for various polynomial degrees for the three choices of discrete Hodge operators.}
    \label{fig:h1_error_smooth_coeff}
\end{figure}

% \begin{figure}[t!]
%     \centering 
%     \begin{tikzpicture}[]
%     \begin{loglogaxis}[width=0.36\columnwidth, height=0.36\columnwidth, ylabel={H$^1$ error},xlabel={$h$}, 
%     ymin=3e-10,ymax=5e1,xmin=8e-3,xmax=0.5, ylabel near ticks,tick label style={font=\footnotesize},  legend style={font=\scriptsize, }, label style={font=\footnotesize},every x tick scale label/.style={at={(1,0)},anchor=north,yshift=-5pt,inner sep=0pt},legend pos= south east]
%     \addplot [blue, mark=triangle*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_square_highreg_smoothgamma_p2r1_global.csv};
%     \addplot [red, mark=*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_square_highreg_smoothgamma_p2r1_l2.csv};
%     \addplot [green, mark=square*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_square_highreg_smoothgamma_p2r1_llm.csv};
%     \addplot [magenta, mark=diamond*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_square_highreg_smoothgamma_p2r1_standard_iga.csv};
%     \node[] at (axis cs:10^-1.6, 10)   (a) {$p=2,\;C^1$};
%     \draw (axis cs:0.012,0.5*10^-0.4)--(axis cs:0.024,10^-0.4)--(axis cs:0.012,10^-0.4) node[pos=0.05,anchor=north] {}--cyclenode[pos=0.0,anchor=west] {};
%     \node[] at (axis cs:0.01, 10^-0.5)   (c) {$1$};
%     \draw (axis cs:0.024,2^2*10^-3.4)--(axis cs:0.024,10^-3.4)--(axis cs:0.012,10^-3.4) node[pos=0.05,anchor=north] {}--cyclenode[pos=0.0,anchor=west] {};
%     \node[] at (axis cs:0.67*0.012+0.33*0.024, 10^-4.5)   (c) {$2$};
%     % \draw (axis cs:0.025,10^-5.0)--(axis cs:0.0125,10^-5.0)--(axis cs:0.025,2^3*10^-5.0) node[pos=0.05,anchor=north] {}--cyclenode[pos=0.0,anchor=west] {};
%     % \node[] at (axis cs:0.67*0.012+0.33*0.024, 10^-4.5)   (c) {$2$};
%     % \node[] at (axis cs:0.33*0.0125+0.67*0.025, 0.9*10^-5.9+0.1*2^3*10^-5.9)   (c) {$3$};
%     \legend{1$^{\text{st}}$ \\2$^{\text{nd}}$ \\3$^{\text{rd}}$ \\IGA\\}
%     \end{loglogaxis}
%     \end{tikzpicture}
%     \begin{tikzpicture}[]
%     \begin{loglogaxis}[width=0.36\columnwidth, height=0.36\columnwidth, xlabel={$h$}, 
%     ymin=3e-10,ymax=5e1,xmin=8e-3,xmax=0.5, ylabel near ticks,tick label style={font=\footnotesize},  legend style={font=\scriptsize, }, label style={font=\footnotesize},every x tick scale label/.style={at={(1,0)},anchor=north,yshift=-5pt,inner sep=0pt},legend pos= south east]
%     \addplot [blue, mark=triangle*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_square_highreg_smoothgamma_p3r2_global.csv};
%     \addplot [red, mark=*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_square_highreg_smoothgamma_p3r2_l2.csv};
%     \addplot [green, mark=square*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_square_highreg_smoothgamma_p3r2_llm.csv};
%     \addplot [magenta, mark=diamond*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_square_highreg_smoothgamma_p3r2_standard_iga.csv};
%     \node[] at (axis cs:10^-1.6, 10)   (a) {$p=3,\;C^2$};
%     \draw (axis cs:0.024,2^2*10^-2.4)--(axis cs:0.012,10^-2.4)--(axis cs:0.012,2^2*10^-2.4) node[pos=0.05,anchor=north] {}--cyclenode[pos=0.0,anchor=west] {};
%     \draw (axis cs:0.025,10^-5.0)--(axis cs:0.0125,10^-5.0)--(axis cs:0.025,2^3*10^-5.0) node[pos=0.05,anchor=north] {}--cyclenode[pos=0.0,anchor=west] {};
%     \node[] at (axis cs:0.67*0.012+0.33*0.024, 0.9*10^-1.0+0.1*2^3*10^-1.0)   (c) {$2$};
%     \node[] at (axis cs:0.33*0.0125+0.67*0.025, 0.9*10^-5.9+0.1*2^3*10^-5.9)   (c) {$3$};
%     \legend{1$^{\text{st}}$ \\2$^{\text{nd}}$ \\3$^{\text{rd}}$ \\IGA\\}
%     \end{loglogaxis}
%     \end{tikzpicture}
%     \begin{tikzpicture}[]
%     \begin{loglogaxis}[width=0.36\columnwidth, height=0.36\columnwidth, xlabel={$h$}, 
%     ymin=3e-10,ymax=5e1,xmin=8e-3,xmax=0.5, ylabel near ticks,tick label style={font=\footnotesize},  legend style={font=\scriptsize, }, label style={font=\footnotesize},every x tick scale label/.style={at={(1,0)},anchor=north,yshift=-5pt,inner sep=0pt},legend pos= south east]
%     \addplot [blue, mark=triangle*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_square_highreg_smoothgamma_p4r3_global.csv};
%     \addplot [red, mark=*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_square_highreg_smoothgamma_p4r3_l2.csv};
%     \addplot [green, mark=square*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_square_highreg_smoothgamma_p4r3_llm.csv};
%     \addplot [magenta, mark=diamond*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_square_highreg_smoothgamma_p4r3_standard_iga.csv};
%     \node[] at (axis cs:10^-1.6, 10)   (a) {$p=4,\;C^3$};
%     \draw (axis cs:0.024,2^3*10^-3.4)--(axis cs:0.012,10^-3.4)--(axis cs:0.012,2^3*10^-3.4) node[pos=0.05,anchor=north] {}--cyclenode[pos=0.0,anchor=west] {};
%     \node[] at (axis cs:0.67*0.012+0.33*0.024, 0.9*10^-1.5+0.1*2^3*10^-6.0)   (c) {$3$};
%     \draw (axis cs:0.025,10^-6.8)--(axis cs:0.0125,10^-6.8)--(axis cs:0.025,2^4*10^-6.8) node[pos=-0.05,anchor=north] {}--cyclenode[pos=1.0,anchor=west] {};
%     \node[] at (axis cs:0.33*0.0125+0.67*0.025, 0.9*10^-6.8+0.1*2^4*10^-6.8)   (b) {$4$};
%     \legend{1$^{\text{st}}$ \\2$^{\text{nd}}$ \\3$^{\text{rd}}$ \\IGA\\}
%     \end{loglogaxis}
%     \end{tikzpicture}
%     % \begin{tikzpicture}[]
%     % \begin{loglogaxis}[width=0.36\columnwidth, height=0.36\columnwidth, xlabel={$h$}, 
%     % ymin=10^-9.5,ymax=200,xmin=0.005,xmax=0.5, ylabel near ticks,tick label style={font=\footnotesize}, legend style={font=\scriptsize, }, label style={font=\footnotesize},every x tick scale label/.style={at={(1,0)},anchor=north,yshift=-5pt,inner sep=0pt},legend pos= south east]
%     % \addplot [blue, mark=triangle*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_square_highreg_smoothgamma_p5r4_global.csv};
%     % \addplot [red, mark=*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_square_highreg_smoothgamma_p5r4_l2.csv};
%     % \addplot [green, mark=square*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_square_highreg_smoothgamma_p5r4_llm.csv};
%     % \addplot [magenta, mark=diamond*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/laplace_results_square_highreg_smoothgamma_p5r4_standard_iga.csv};
%     % \node[] at (axis cs:10^-1.6, 10)   (a) {$p=5,\;C^4$};
%     % \draw (axis cs:0.0125,2^4*10^-3.7)--(axis cs:0.0125,10^-3.7)--(axis cs:0.025,2^4*10^-3.7) node[pos=-0.05,anchor=north] {}--cyclenode[pos=1.0,anchor=west] {};
%     % \draw (axis cs:0.03,10^-7.0)--(axis cs:0.015,10^-7.0)--(axis cs:0.03,2^5 * 10^-7.0) node[pos=-0.05,anchor=north] {}--cyclenode[pos=1.0,anchor=west] {};
%     % \node[] at (axis cs:0.33*0.0125+0.67*0.025, 0.95*10^-3.7+0.05*2^4*10^-3.7)   (b) {$4$};
%     % \node[] at (axis cs:0.33*0.015+0.67*0.03, 0.95*10^-7.0+0.05*2^5*10^-7.0)   (c) {$5$};
%     % \legend{1$^{\text{st}}$ \\2$^{\text{nd}}$ \\3$^{\text{rd}}$ \\IGA\\}
%     % \end{loglogaxis}
%     % \end{tikzpicture} 
%     \caption{Static problem: a comparison of the error in the $H\Lambda^0(\Omega)$ norm (or $H^1$ norm) for higher polynomial degrees in the case of the parametric domain, with the smooth perturbation of the material parameter $\gamma$ introduced in \eqref{eq:smoothgamma} for the three choices of discrete Hodge operators proposed in the paper. \textcolor{black}{There is a lot of space below the curves. Can we put a single legend above the three figures (groupplot)?} }
%     \label{fig:h1_error_smooth_coeff}
% \end{figure}

% p3 c2 mappedsquare
% [0.710680080312178 & 0.0253109118775127 & 0.00197555523592769 & 0.000210782814890373;
% 1.16670708560291 & 0.164292316880371 & 0.0211512160198395 & 0.00326699248332802;
% 0.856659563622199 & 0.0903460430149194 & 0.0176249316266017 & 0.00407929028265476;
% 0.690733331319589 & 0.0247549325914696 & 0.00195785128195846 & 0.000210042242548923]

% p4 c3 mappedsquare
% [0.279255900489102,
% 0.00663090868052165,
% 0.000199950950925885,
% 9.84958156534983e-06;
% 0.381356279478068,
% 0.012494238483791,
% 0.00058873852855726,
% 2.58528026753669e-05;
% 0.530462463813219,
% 0.0365400626335323,
% 0.00198850796135789,
% 0.000114797460710365;
% 0.271094043651844,
% 0.00657704304334999,
% 0.000199677660365391,
% 9.8464158284513e-06]


\begin{table}[ht]\scriptsize
    \centering
    \begin{tabular}{lccc}
         &  \multicolumn{3}{c}{$p=2,\; C^1$}\\
        \cmidrule(lr){2-4}
        $\star_h$ choice & $h=0.05$   & $h=0.025$ & $h=0.0125$    \\\midrule
        1$^{\text{st}}$  & \num[round-precision=3,round-mode=figures]{0.050758} & \num[round-precision=3,round-mode=figures]{0.012758} & \num[round-precision=3,round-mode=figures]{0.0031942}\\
        2$^{\text{nd}}$  & \num[round-precision=3,round-mode=figures]{0.33895} & \num[round-precision=3,round-mode=figures]{0.15902} & \num[round-precision=3,round-mode=figures]{0.062892}\\
        3$^{\text{nd}}$ & \num[round-precision=3,round-mode=figures]{0.10908} & \num[round-precision=3,round-mode=figures]{0.13384} & \num[round-precision=3,round-mode=figures]{0.016405} \\
        IGA   & \num[round-precision=3,round-mode=figures]{0.019147} & \num[round-precision=3,round-mode=figures]{0.0046027} & \num[round-precision=3,round-mode=figures]{0.001139} \\\toprule
        & \multicolumn{3}{c}{$p=3,\; C^2$}\\
         \cmidrule(lr){2-4}
        $\star_h$ choice &   $h=0.05$  & $h=0.025$ & $h=0.0125$   \\\midrule
        1$^{\text{st}}$  & \num[round-precision=3,round-mode=figures]{0.0020163} & \num[round-precision=3,round-mode=figures]{0.00022275} & \num[round-precision=3,round-mode=figures]{2.7011e-05} \\
        2$^{\text{nd}}$  & \num[round-precision=3,round-mode=figures]{0.022192} & \num[round-precision=3,round-mode=figures]{0.003549} & \num[round-precision=3,round-mode=figures]{0.00060305}\\
        3$^{\text{nd}}$  & \num[round-precision=3,round-mode=figures]{0.016764} & \num[round-precision=3,round-mode=figures]{0.0042108} & \num[round-precision=3,round-mode=figures]{0.0010568}\\
        IGA   & \num[round-precision=3,round-mode=figures]{0.0019748} & \num[round-precision=3,round-mode=figures]{0.00022102} & \num[round-precision=3,round-mode=figures]{2.6929e-05}\\\toprule
         & \multicolumn{3}{c}{$p=4,\; C^3$}\\
         \cmidrule(lr){2-4}
        $\star_h$ choice & $h=0.05$  & $h=0.025$ & $h=0.0125$   \\\midrule
        1$^{\text{st}}$  & \num[round-precision=3,round-mode=figures]{0.00029198} & \num[round-precision=3,round-mode=figures]{1.452e-05} & \num[round-precision=3,round-mode=figures]{8.5337e-07} \\
        2$^{\text{nd}}$  & \num[round-precision=3,round-mode=figures]{0.0013368} & \num[round-precision=3,round-mode=figures]{7.7106e-05} & \num[round-precision=3,round-mode=figures]{6.9449e-06} \\
        3$^{\text{nd}}$ & \num[round-precision=3,round-mode=figures]{0.0022657} & \num[round-precision=3,round-mode=figures]{0.00014972} & \num[round-precision=3,round-mode=figures]{9.6642e-06} \\
        IGA & \num[round-precision=3,round-mode=figures]{0.00029149} & \num[round-precision=3,round-mode=figures]{1.4515e-05} & \num[round-precision=3,round-mode=figures]{8.5328e-07} \\\toprule
    \end{tabular}
    \caption{Values for errors displayed in Fig.~\ref{fig:h1_error_smooth_coeff}, $H\Lambda^0$ error, $\Omega=(0,1)^2$, $\gamma$ given by \eqref{eq:smoothgamma}.}
    \label{tab:h1_error_table2}
\end{table}

\normalsize

% & \num[round-precision=3,round-mode=figures]{0.025311} & \num[round-precision=3,round-mode=figures]{0.0019756} & \num[round-precision=3,round-mode=figures]{0.00021078} & \num[round-precision=3,round-mode=figures]{0.050758} & \num[round-precision=3,round-mode=figures]{0.012758} & \num[round-precision=3,round-mode=figures]{0.0031942}
% & \num[round-precision=3,round-mode=figures]{0.16429} & \num[round-precision=3,round-mode=figures]{0.021151} & \num[round-precision=3,round-mode=figures]{0.003267} & \num[round-precision=3,round-mode=figures]{0.33895} & \num[round-precision=3,round-mode=figures]{0.15902} & \num[round-precision=3,round-mode=figures]{0.062892}
% & \num[round-precision=3,round-mode=figures]{0.090346} & \num[round-precision=3,round-mode=figures]{0.017625} & \num[round-precision=3,round-mode=figures]{0.0040793} & \num[round-precision=3,round-mode=figures]{0.10908} & \num[round-precision=3,round-mode=figures]{0.13384} & \num[round-precision=3,round-mode=figures]{0.016405}
% & \num[round-precision=3,round-mode=figures]{0.024755} & \num[round-precision=3,round-mode=figures]{0.0019579} & \num[round-precision=3,round-mode=figures]{0.00021004} & \num[round-precision=3,round-mode=figures]{0.019147} & \num[round-precision=3,round-mode=figures]{0.0046027} & \num[round-precision=3,round-mode=figures]{0.001139}

%%%%%%%%%%%%%%%%% conditioning and sparsity %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t!]
    \centering
    \begin{tikzpicture}[]
        \begin{loglogaxis}[width=0.45\columnwidth, height=0.45\columnwidth, ylabel={$\kappa$},xlabel={$h$},xmin=10^-2.0, ylabel near ticks,tick label style={font=\footnotesize},  legend style={font=\scriptsize, }, label style={font=\footnotesize},every x tick scale label/.style={at={(1,0)},anchor=north,yshift=-5pt,inner sep=0pt},legend pos= north east]
        \addplot [blue, mark=triangle*, mark options={solid}] table [x index=0, y index=3, col sep=comma] {figures/laplace_results_mappedsquare_p4r3_global.csv};
        \addplot [red, mark=*, mark options={solid}] table [x index=0, y index=3, col sep=comma] {figures/laplace_results_mappedsquare_p4r3_l2.csv};
        \addplot [green, mark=square*, mark options={solid}] table [x index=0, y index=3, col sep=comma] {figures/laplace_results_mappedsquare_p4r3_llm.csv};
        \addplot [magenta, mark=diamond*, mark options={solid}] table [x index=0, y index=3, col sep=comma] {figures/laplace_results_mappedsquare_p3r2_standard_iga.csv};
        \node[] at (axis cs:10^-1.6, 1)   (a) {$p=3,\;C^2$};
        \draw (axis cs:0.02,10^2.5)--(axis cs:0.04,10^2.5)--(axis cs:0.02,2^2.5*10^2.5) node[pos=0.05,anchor=north] {}--cyclenode[pos=0.0,anchor=west] {};
        \node[] at (axis cs:0.015, 10^3.0)   (c) {$2.5$};
        \node[] at (axis cs:0.03,10^2.2)   (c) {$1$};
        %\draw (axis cs:10^-1.8,10^-4.5)--(axis cs:10^-1.6,10^-4.5/10^0.1)--(axis cs:10^-1.6,10^-4.5) node[pos=0.5,anchor=west] {\footnotesize$2$}--cyclenode[pos=0.5,anchor=north] {\footnotesize$1$};
        \legend{1$^{\text{st}}$ \\2$^{\text{nd}}$ \\3$^{\text{rd}}$ \\IGA\\}
        \end{loglogaxis}
    \end{tikzpicture}
    \begin{tikzpicture}[]
        \begin{loglogaxis}[width=0.45\columnwidth, height=0.45\columnwidth, ylabel={Number of nonzeros},xlabel={$h$}, xmin=10^-2.0, ylabel near ticks,tick label style={font=\footnotesize}, legend style={font=\scriptsize, }, label style={font=\footnotesize},every x tick scale label/.style={at={(1,0)},anchor=north,yshift=-5pt,inner sep=0pt},legend pos= north east]
        \addplot [blue, mark=triangle*, mark options={solid}] table [x index=0, y index=4, col sep=comma] {figures/laplace_results_mappedsquare_p3r2_global.csv};
        \addplot [red, mark=*, mark options={solid}] table [x index=0, y index=4, col sep=comma] {figures/laplace_results_mappedsquare_p3r2_l2.csv};
        \addplot [green, mark=square*, mark options={solid}] table [x index=0, y index=4, col sep=comma] {figures/laplace_results_mappedsquare_p3r2_llm.csv};
        \addplot [magenta, mark=diamond*, mark options={solid}] table [x index=0, y index=4, col sep=comma] {figures/laplace_results_mappedsquare_p3r2_standard_iga.csv};
        \node[] at (axis cs:10^-1.6, 10^-0.5)   (a) {$p=3,\;C^2$};
        \draw (axis cs:0.02,10^4.0)--(axis cs:0.04,10^4.0)--(axis cs:0.02,2^2.0*10^4.0) node[pos=0.05,anchor=north] {}--cyclenode[pos=0.0,anchor=west] {};
        \node[] at (axis cs:0.018, 10^4.2)   (c) {$2$};
        \node[] at (axis cs:0.03,10^3.8)   (c) {$1$};
        \legend{1$^{\text{st}}$ \\2$^{\text{nd}}$ \\3$^{\text{rd}}$ \\IGA\\}
        \end{loglogaxis}
    \end{tikzpicture} 
    \caption{Elliptic source problem for the parametric domain, with the nontrivial map of (\ref{eq:harmonic_map}): a comparison of condition number and sparsity degrade for the case of $h$ refinement for $p=3$ and $C^2$ splines in the first space of the primal sequence.}
    \label{fig:conditioning_and_sparsity_laplace}
\end{figure}
% \begin{figure}[!t]
%     \centering
% \includegraphics[width=0.45\textwidth]{figures/laplace_results_mappedsquare_noK_p2r1_l2.eps}
% \includegraphics[width=0.45\textwidth]{figures/laplace_results_mappedsquare_noK_p3r2_l2.eps}
% \includegraphics[width=0.475\textwidth]{figures/laplace_results_mappedsquare_p4r3_l2.eps}
% \includegraphics[width=0.45\textwidth]{figures/laplace_results_mappedsquare_noK_p5r4_l2.eps}
% \caption{Poisson problem: error in the $L^2$ norm in the case of the parametric domain, with the nontrivial map of (\ref{eq:harmonic_map}).}
% \label{fig:l2_error_noK}
% \end{figure}

% \begin{figure}[!t]
% \centering
% \includegraphics[width=0.45\textwidth]{figures/laplace_results_mappedsquare_noK_p2r1_h1.eps}
% \includegraphics[width=0.45\textwidth]{figures/laplace_results_mappedsquare_noK_p3r2_h1.eps}
% \includegraphics[width=0.45\textwidth]{figures/laplace_results_mappedsquare_noK_p4r3_h1.eps}
% \includegraphics[width=0.45\textwidth]{figures/laplace_results_mappedsquare_noK_p5r4_h1.eps}
% \caption{Poisson problem: error in the $H^1$ norm in the case of the parametric domain, with the nontrivial map of (\ref{eq:harmonic_map}).}
% \label{fig:h1_error_noK}
% \end{figure}

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/laplace_results_mappedsquare_p2r1_h1.eps}
%     \includegraphics[width=0.45\textwidth]{figures/laplace_results_mappedsquare_p3r2_h1.eps}
%     \includegraphics[width=0.45\textwidth]{figures/laplace_results_mappedsquare_p4r3_h1.eps}
%     \includegraphics[width=0.45\textwidth]{figures/laplace_results_mappedsquare_p5r4_h1.eps}
%     \caption{Poisson problem: error in the $H^1$ norm in the case of the parametric domain, with the nontrivial map of (\ref{eq:harmonic_map}).}
%     \label{fig:h1_error_K}
% \end{figure}

% \begin{figure}[!t]
% \centering
% \includegraphics[width=0.45\textwidth]{figures/laplace_results_mappedsquare_noK_p2r1_condnum.eps}
% \includegraphics[width=0.45\textwidth]{figures/laplace_results_mappedsquare_noK_p3r2_condnum.eps}
% \includegraphics[width=0.45\textwidth]{figures/laplace_results_mappedsquare_noK_p4r3_condnum.eps}
% \includegraphics[width=0.45\textwidth]{figures/laplace_results_mappedsquare_noK_p5r4_condnum.eps}
% \caption{Poisson problem: condition number of the system matrix in the case of the parametric domain, with the trivial map.}
% \label{fig:condnum_noK}
% \end{figure}

% \begin{figure}[!t]
% \centering
% \includegraphics[width=0.45\textwidth]{figures/laplace_results_mappedsquare_p2r1_condnum.eps}
% \includegraphics[width=0.45\textwidth]{figures/laplace_results_mappedsquare_p3r2_condnum.eps}
% \includegraphics[width=0.45\textwidth]{figures/laplace_results_mappedsquare_p4r3_condnum.eps}
% \includegraphics[width=0.45\textwidth]{figures/laplace_results_mappedsquare_p5r4_condnum.eps}
% \caption{Condition number of the system matrix in the case of the parametric domain, with the nontrivial map of (\ref{eq:harmonic_map}).}
% \label{fig:condnum_K}
% \end{figure}

% \begin{figure}[!t]
% \centering
% \includegraphics[width=0.45\textwidth]{figures/laplace_results_mappedsquare_noK_p2r1_sparsity.eps}
% \includegraphics[width=0.45\textwidth]{figures/laplace_results_mappedsquare_noK_p3r2_sparsity.eps}
% \includegraphics[width=0.45\textwidth]{figures/laplace_results_mappedsquare_noK_p4r3_sparsity.eps}
% \includegraphics[width=0.45\textwidth]{figures/laplace_results_mappedsquare_noK_p5r4_sparsity.eps}
% \caption{Poisson problem: number of non-zeros in the system matrix in the case of the parametric domain, with the trivial map.}
% \label{fig:sparsity_noK}
% \end{figure}

\subsection{Second order eigenvalue problem}

In the case of the eigenvalue problem \eqref{eq:evp_with_forms} \textcolor{black}{we are particularly interested in Maxwell eigenvalue problem, for which we set $k=1$ and the material parameters $\gamma = \beta = 1$. The} most important property we want to investigate in the proposed approach is its spectral accuracy. This test is fundamental in a twofold sense: firstly, the absence of numerical spurious eigenfunctions in the kernel of the exterior derivative operators is a key feature of structure preserving methods, secondly the optimal $2p$ convergence rate in eigenvalue errors is sought to confirm that the approach is indeed a high-order one. 

% 1,2,2.00000000000069,2.00000000174406,2.00001698469034,2.99999999994896
% 2,2,2.00000000000091,2.00000000174416,2.0000169846908,2.0000000000017
% 3,2,2.00000000000202,2.00000000174481,2.00001698469135,2.00000000000171
% 4,3,3.00000000000165,3.00000000174426,3.00001698469063,3.33333333333219
% 5,3,3.00000000000222,3.00000000174438,3.000016984691,3.00000000000168
% 6,5,5.00000000038169,5.00000009494528,5.00021765945886,5.39999999999899
% 7,5,5.00000000038169,5.0000000949453,5.00021765945952,5.00000000038181
% 8,5,5.00000000038181,5.00000009494548,5.00021765945957,5.00000000038182
% 9,5,5.00000000038186,5.0000000949456,5.00021765945979,5.00000000038183
% 10,5,5.00000000038198,5.00000009494564,5.00021765945991,5.00000000038183
% 11,5,5.00000000038244,5.00000009494572,5.00021765946033,5.00000000038183
% 12,6,6.00000000031816,6.00000007941195,6.00018421366449,6.16666666634847
% 13,6,6.0000000003183,6.00000007941199,6.00018421366468,6.00000000031846
% 14,6,6.00000000031834,6.00000007941202,6.00018421366474,6.00000000031848
% 15,6,6.00000000031844,6.00000007941203,6.00018421366483,6.00000000031848
% 16,6,6.00000000031851,6.00000007941207,6.00018421366486,6.00000000031849
% 17,6,6.00000000031892,6.0000000794121,6.00018421366491,6.00000000031849
% 18,8,8.00000000047665,8.00000011824564,8.00026782815136,8.24999999976113
% 19,8,8.00000000047673,8.00000011824581,8.00026782815184,8.00000000047686
% 20,8,8.00000000047679,8.00000011824584,8.00026782815236,8.00000000047687

\begin{figure}[t!]
    \centering 
    \begin{tikzpicture}[]
            \begin{axis}[width=0.45\columnwidth, height=0.45\columnwidth, ylabel={},xlabel={Eigenvalue index}, 
                ymin=0,ymax=110,xmin=0,xmax=21, ylabel={$\tau$}, ylabel near ticks,tick label style={font=\footnotesize},  legend style={font=\scriptsize, }, label style={font=\footnotesize},every x tick scale label/.style={at={(1,0)},anchor=north,yshift=-5pt,inner sep=0pt},legend pos= south east]
            % \addplot [blue, only marks, mark=square*, %mark options={solid}
            % ] table [x index=0, y index=2, col sep=comma] {figures/maxwell_results_eighthring_p3r2_refinement1.csv};
            \addplot [red, only marks, mark=diamond*, %mark options={solid}
            ] table [x index=0, y index=2, col sep=comma] {figures/maxwell_results_eighthring_reference_p4r3_refinement1.csv};
            \addplot [green, only marks, mark=x, %mark options={solid}
            ] table [x index=0, y index=3, col sep=comma] {figures/maxwell_results_eighthring_reference_p4r3_refinement1.csv};
            \addplot [black, only marks, mark=square, mark options={}
            ] table [x index=0, y index=4, col sep=comma] {figures/maxwell_results_eighthring_reference_p4r3_refinement1.csv};
            % \node[] at (axis cs:5,5)  (a) {$p=3,\;C^2$};
            \node[] at (axis cs:10,99)   (b) {$1/8$ of a ring};
            \legend{2$^{\text{nd}}$ \\3$^{\text{rd}}$ \\Reference\\}
            \end{axis}
    \end{tikzpicture}
    \begin{tikzpicture}[]
            \begin{axis}[width=0.45\columnwidth, height=0.45\columnwidth, ylabel={$\tau/\pi^2$},xlabel={Eigenvalue index}, 
                ymin=0,ymax=9,xmin=0,xmax=21, ylabel near ticks,tick label style={font=\footnotesize},  legend style={font=\scriptsize, }, label style={font=\footnotesize},every x tick scale label/.style={at={(1,0)},anchor=north,yshift=-5pt,inner sep=0pt},legend pos= south east]
            % \addplot [blue, only marks, mark=square*, %mark options={solid}
            % ] table [x index=0, y index=2, col sep=comma] {figures/maxwell_results_cube_p4r3_refinement3.csv};
            \addplot [red, only marks, mark=diamond*, %mark options={solid}
            ] table [x index=0, y index=3, col sep=comma] {figures/maxwell_results_cube_p4r3_refinement1.csv};
            \addplot [green, only marks, mark=x, %mark options={solid}
            ] table [x index=0, y index=4, col sep=comma] {figures/maxwell_results_cube_p4r3_refinement1.csv};
            \addplot [black, only marks, mark=square, mark options={}
            ] table [x index=0, y index=1, col sep=comma] {figures/maxwell_results_cube_p4r3_refinement1.csv};
            % \node[] at (axis cs:5,14)  (a) {$p=4,\;C^3$};
            \node[] at (axis cs:10,8)   (b) {Unit cube};
            \legend{2$^{\text{nd}}$ \\3$^{\text{rd}}$ \\Reference\\}
            \end{axis}
    \end{tikzpicture}
    \caption{Spectral fidelity: comparison of the computed eigenvalues for the second and third discrete Hodge operators with reference eigenvalues for one eighth of a ring, and for a deformation of the unit cube. \redmod{All results with $p=4$ and maximal continuity B-splines. The mesh for the $1/8$ ring consists of $20\times 20= 400$ elements. The one for the cube includes $20\times20\times 20 =8000$ elements.}}
%all approaches are shown to behave correctly in approximating the spectrum of the second order differential operator in \eqref{eq:evp_with_forms}, for general deformations of an $n$-dimenisional cube.}
    \label{fig:ev_correctness}
\end{figure}

The first property is easily proved for the first proposed global discrete Hodge--star operator, through its algebraic equivalence with a standard Galerkin formulation. Furthermore, it is also reasonably expected to hold for the second kind of operator (being it equivalent to an $L^2$ projection) combining insight from~\cite{BRSV11} on the existence of projectors commuting with the De-Rham sequence operators and results in~\cite{Buffa_2020aa} concerning the stable $L^2$ pairing of univariate spline spaces of degree $(p,p-2)$. 
The fact that spectral correctness is observed in the case of the third proposed operator is instead considerably less trivial and deserves further attention, since the proposed local projector does not commute with differential operators in the sequence.
A full proof of this statement goes beyond the scope of the present article. % and will be aimed at in future work.
Nevertheless, we show that this property is numerically corroborated in Fig.~\ref{fig:ev_correctness} both in two dimensions, \magentamod{for the case of the domain on the right of Fig.~\ref{fig:reparam}}, and in three dimensions for the usual unit cube, albeit with the nontrivial map already used for the square in the problem of Section~\ref{sec:elliptic_numerical}, with the same value of $a=0.3$. \textcolor{black}{In the first case the reference eigenvalues are computed by a Galerkin method in a very fine mesh, while in the second case the exact eigenvalues are known.} 
\magentamod{The convergence rate in eigenvalue errors, computed for the second eigenvalue in the case of the eighth of a ring cavity and for the twentieth eigenvalue in the case of the cube and shown in Fig.~\ref{fig:ev_error_8th_ring} (with values also reported in Table \ref{tab:ev_error_ring_table}) and Fig.~\ref{fig:ev_error} (with values also reported in Table \ref{tab:ev_error_table})}, respectively, are again the optimal ones for the approach which is algebraically equivalent to the standard Galerkin IGA one. %\textcolor{black}{REMOVE? which suggests this kind of Hodge--star as a starting point for the study of hyperbolic problems}. 
The other two suggested projectors instead lose orders of convergence upon $h-$refinement. Since we perform $L^2$ projections into spaces of splines with mixed degree between $p-1$ and $p-2$ the $2^\text{nd}$ operator actually exhibits the \textcolor{black}{expected convergence rate deriving from Theorem~\ref{thm:error_bound}}, i.e. $h^{2(p-1)}$. The local operator instead loses more (and the behaviour gets more evident for increasing polynomial degrees) as a result of the combination of loss of symmetry of the system matrix and the filtering of tails of some basis functions in the local projection operator. The high order nature of the method is still preserved, yet future work is needed to optimize it for eigenvalue solvers.
%\textcolor{black}{REFER to the figures of convergence. Make sure that you refer to the three figures in the correct order in the text.}

% We seek a pair $\left(\boldsymbol{u}(\boldsymbol{x}),\lambda \right)$ in $\mathrm{X}_1 \times \mathbb{R}$ such that:
% \begin{align}
%     & \left( \mu^{-1}\nabla\times\boldsymbol{u}, \nabla\times\boldsymbol{w}\right) = \lambda\left( \varepsilon \boldsymbol{u},\boldsymbol{w} \right), & \forall \boldsymbol{w}\in\mathrm{X}_1,\label{eq:galerkin_evp}\\
%     & d^{n-2}\star_h^2 d^1 \boldsymbol{u} = \lambda \star_h^1 \boldsymbol{u}, & \; \label{eq:hodge_maxwell}
% \end{align}

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.48\textwidth]{figures/maxwell_results_mappedsquare_p4r3_ev.eps}
%     \includegraphics[width=0.48\textwidth]{figures/maxwell_results_mappedsquare_p5r4_ev.eps}
%     \caption{Maxwell eigenvalue problem: error in the 20th eigenvalue.}
%     \label{fig:ev_error_maxwell}
% \end{figure}



%%%%%%%%%%%%%%%%% EV error maxwell %%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t!]
    \centering 
    \begin{tikzpicture}[]
    \begin{loglogaxis}[width=0.45\columnwidth, height=0.45\columnwidth, ylabel={Eigenvalue error},xlabel={$h$}, title={$p=3,\;C^2$},
    ymin=10^-10,ymax=10^-1,xmin=0.01,xmax=0.5, ylabel near ticks,tick label style={font=\footnotesize},  legend style={font=\scriptsize, }, label style={font=\footnotesize},every x tick scale label/.style={at={(1,0)},anchor=north,yshift=-5pt,inner sep=0pt},legend pos= south east]
    \addplot [blue, mark=triangle*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/maxwell_results_eighthring_href_p3r2_global.csv};
    \addplot [red, mark=*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/maxwell_results_eighthring_href_p3r2_l2.csv};
    \addplot [green, mark=square*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/maxwell_results_eighthring_href_p3r2_llm.csv};
    \addplot [magenta, mark=diamond*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/maxwell_results_eighthring_href_p3r2_standard_iga.csv};
    % \node[] at (axis cs:0.1,10^-1)   (a) {$p=3,\;C^2$};
    \draw (axis cs:0.05,2^4*10^-3.2)--(axis cs:0.05,10^-3.2)--(axis cs:0.1,2^4*10^-3.2) node[pos=-0.05,anchor=north] {}--cyclenode[pos=1.0,anchor=west] {};
    \draw (axis cs:0.02,2^6 * 10^-9.0)--(axis cs:0.02,10^-9.0)--(axis cs:0.04,2^6 * 10^-9.0) node[pos=-0.05,anchor=north] {}--cyclenode[pos=1.0,anchor=west] {};
%    \draw (axis cs:0.05,2^8 * 10^-11.7)--(axis cs:0.05,10^-11.7)--(axis cs:0.1,2^8 * 10^-11.7) node[pos=-0.05,anchor=north] {}--cyclenode[pos=1.0,anchor=west] {};
    \node[] at (axis cs:0.04, 10^-2.5)   (b) {$4$};
    \node[] at (axis cs:0.015, 0.9*10^-9.0+0.1*2^6*10^-9.0)   (c) {$6$};
    \node[] at (axis cs:0.07, 10^-1.5)   (b) {$1$};
    \node[] at (axis cs:0.03, 10^-6.8)   (c) {$1$};
%    \node[] at (axis cs:0.035, 0.9*10^-12.0+0.1*2^8*10^-12.0)   (c) {$8$};
    \legend{1$^{\text{st}}$ \\2$^{\text{nd}}$ \\3$^{\text{rd}}$ \\IGA\\}
    \end{loglogaxis}
    \end{tikzpicture}
    \begin{tikzpicture}[]
    \begin{loglogaxis}[width=0.45\columnwidth, height=0.45\columnwidth, ylabel={},xlabel={$h$}, title={$p=3,\;C^1$},
    ymin=10^-10,ymax=10^-1,xmin=0.01,xmax=0.5, ylabel near ticks,tick label style={font=\footnotesize},  legend style={font=\scriptsize, }, label style={font=\footnotesize},every x tick scale label/.style={at={(1,0)},anchor=north,yshift=-5pt,inner sep=0pt},legend pos= south east]
    \addplot [blue, mark=triangle*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/maxwell_results_eighthring_href_p3r1_global.csv};
    \addplot [red, mark=*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/maxwell_results_eighthring_href_p3r1_l2.csv};
    \addplot [green, mark=square*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/maxwell_results_eighthring_href_p3r1_llm.csv};
    \addplot [magenta, mark=diamond*, mark options={solid}] table [x index=0, y index=2, col sep=comma] {figures/maxwell_results_eighthring_href_p3r1_standard_iga.csv};
    % \node[] at (axis cs:0.1,10^-1)   (a) {$p=3,\;C^1$};
    \draw (axis cs:0.06,2^4*10^-3.7)--(axis cs:0.06,10^-3.7)--(axis cs:0.12,2^4*10^-3.7) node[pos=-0.05,anchor=north] {}--cyclenode[pos=1.0,anchor=west] {};
    \draw (axis cs:0.02,2^6 * 10^-9.0)--(axis cs:0.02,10^-9.0)--(axis cs:0.04,2^6 * 10^-9.0) node[pos=-0.05,anchor=north] {}--cyclenode[pos=1.0,anchor=west] {};
    %\draw (axis cs:0.3,10^-12.0)--(axis cs:0.15,10^-12.0)--(axis cs:0.3,2^10 * 10^-12.0) node[pos=-0.05,anchor=north] {}--cyclenode[pos=1.0,anchor=west] {};
    \node[] at (axis cs:0.05, 0.95*10^-3.2+0.05*2^4*10^-3.2)   (b) {$4$};
    \node[] at (axis cs:0.015, 0.9*10^-9.0+0.1*2^6*10^-9.0)   (c) {$6$};
    \node[] at (axis cs:0.08, 10^-2.0)   (b) {$1$};
    \node[] at (axis cs:0.03, 10^-6.8)   (c) {$1$};
   % \node[] at (axis cs:0.45, 0.5*10^-14.0+0.5*2^10*10^-14.0)   (c) {$10$};
    \legend{1$^{\text{st}}$ \\2$^{\text{nd}}$ \\3$^{\text{rd}}$ \\IGA\\}
    \end{loglogaxis}
    \end{tikzpicture}
    \caption{Eigenvalue problem: convergence in the second eigenvalue error for the various choices of projectors for the eighth ring in two dimensions. The case of starting degree $p=3$ both with $C^2$ and $C^1$ continuous spline spaces.}
    \label{fig:ev_error_8th_ring}
\end{figure}

%%%%%%%%%%%%%%%%% EV error maxwell %%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t!]
    \centering 
    \begin{tikzpicture}[]
            \begin{loglogaxis}[width=0.45\columnwidth, title={$p=4,\;C^3$}, height=0.45\columnwidth, ylabel={Eigenvalue error},xlabel={$h$}, 
                ymin=10^-12.2,ymax=10^-0.2,xmin=0.02,xmax=2, ylabel near ticks,tick label style={font=\footnotesize},  legend style={font=\scriptsize, }, label style={font=\footnotesize},every x tick scale label/.style={at={(1,0)},anchor=north,yshift=-5pt,inner sep=0pt},legend pos= south east]
            \addplot [blue, mark=triangle*, mark options={solid}] table [x index=0, y index=20, col sep=comma] {figures/maxwell_results_cube_p4r3_global.csv};
            \addplot [red, mark=*, mark options={solid}] table [x index=0, y index=20, col sep=comma] {figures/maxwell_results_cube_p4r3_l2.csv};
            \addplot [green, mark=square*, mark options={solid}] table [x index=0, y index=20, col sep=comma] {figures/maxwell_results_cube_p4r3_llm.csv};
            \addplot [magenta, mark=diamond*, mark options={solid}] table [x index=0, y index=20, col sep=comma] {figures/maxwell_results_cube_p4r3_standard_iga.csv};
            % \node[] at (axis cs:10^-1,10^-0.5)   (a) {$p=4,\;C^3$};
            \draw (axis cs:0.05,2^4*10^-3.7)--(axis cs:0.05,10^-3.7)--(axis cs:0.1,2^4*10^-3.7) node[pos=-0.05,anchor=north] {}--cyclenode[pos=1.0,anchor=west] {};
            \draw (axis cs:0.05,2^6 * 10^-7.0)--(axis cs:0.05,10^-7.0)--(axis cs:0.1,2^6 * 10^-7.0) node[pos=-0.05,anchor=north] {}--cyclenode[pos=1.0,anchor=west] {};
            \draw (axis cs:0.2,10^-8.7)--(axis cs:0.1,10^-8.7)--(axis cs:0.2,2^8 * 10^-8.7) node[pos=-0.05,anchor=north] {}--cyclenode[pos=1.0,anchor=west] {};
            \node[] at (axis cs:0.04, 0.95*10^-3.0+0.05*2^4*10^-3.0)   (b) {$4$};
            \node[] at (axis cs:0.04, 0.9*10^-7.0+0.1*2^6*10^-7.0)   (c) {$6$};
            \node[] at (axis cs:0.25, 0.9*10^-9.0+0.1*2^8*10^-9.0)   (c) {$8$};
            \node[] at (axis cs:0.07, 10^-2.0)   (b) {$1$};
            \node[] at (axis cs:0.07, 10^-4.5)   (c) {$1$};
            \node[] at (axis cs:0.15, 10^-9.5)   (c) {$1$};
            % \node[] at (axis cs:0.05,10^-2.5)   (c) {$1$};
            % \node[] at (axis cs:0.05,10^-5.5)   (c) {$1$};
            % \node[] at (axis cs:0.05,10^-.5)   (c) {$1$};
            \legend{1$^{\text{st}}$ \\2$^{\text{nd}}$ \\3$^{\text{rd}}$ \\IGA\\}
            \end{loglogaxis}
        \end{tikzpicture}
        \begin{tikzpicture}[]
                \begin{loglogaxis}[width=0.45\columnwidth, title={$p=5,\;C^4$}, height=0.45\columnwidth, ylabel={},xlabel={$h$}, 
                    ymin=10^-12.2,ymax=10^-0.2,xmin=0.02,xmax=2, ylabel near ticks,tick label style={font=\footnotesize},  legend style={font=\scriptsize, }, label style={font=\footnotesize},every x tick scale label/.style={at={(1,0)},anchor=north,yshift=-5pt,inner sep=0pt},legend pos= south east]
                \addplot [blue, mark=triangle*, mark options={solid}] table [x index=0, y index=20, col sep=comma] {figures/maxwell_results_cube_p5r4_global.csv};
                \addplot [red, mark=*, mark options={solid}] table [x index=0, y index=20, col sep=comma] {figures/maxwell_results_cube_p5r4_l2.csv};
                \addplot [green, mark=square*, mark options={solid}] table [x index=0, y index=20, col sep=comma] {figures/maxwell_results_cube_p5r4_llm.csv};
                \addplot [magenta, mark=diamond*, mark options={solid}] table [x index=0, y index=20, col sep=comma] {figures/maxwell_results_mappedcube_p5r4_standard_iga.csv};
                % \node[] at (axis cs:10^-1,10^-0.5)   (a) {$p=5,\;C^4$};
                \draw (axis cs:0.05,2^4*10^-3.7)--(axis cs:0.05,10^-3.7)--(axis cs:0.1,2^4*10^-3.7) node[pos=-0.05,anchor=north] {}--cyclenode[pos=1.0,anchor=west] {};
                \draw (axis cs:0.08,2^8 * 10^-7.5)--(axis cs:0.08,10^-7.5)--(axis cs:0.16,2^8 * 10^-7.5) node[pos=-0.05,anchor=north] {}--cyclenode[pos=1.0,anchor=west] {};
                \draw (axis cs:0.16,10^-11.0)--(axis cs:0.08,10^-11.0)--(axis cs:0.16,2^10 * 10^-11.0) node[pos=-0.05,anchor=north] {}--cyclenode[pos=1.0,anchor=west] {};
                \node[] at (axis cs:0.04, 0.95*10^-3.2+0.05*2^4*10^-3.2)   (b) {$4$};
                \node[] at (axis cs:0.06, 0.9*10^-7.0+0.1*2^6*10^-7.0)   (c) {$8$};
                \node[] at (axis cs:0.2, 10^-10.0)   (c) {$10$};
                \node[] at (axis cs:0.07, 10^-2.0)   (b) {$1$};
                \node[] at (axis cs:0.12, 10^-4.5)   (c) {$1$};
                \node[] at (axis cs:0.12, 10^-11.5)   (c) {$1$};
                \legend{1$^{\text{st}}$ \\2$^{\text{nd}}$ \\3$^{\text{rd}}$ \\IGA\\}
                \end{loglogaxis}
            \end{tikzpicture}
    \caption{Eigenvalue problem: convergence in the twentieth eigenvalue error for the various choices of projectors for the unit cube in three dimensions. The case of starting degrees $p=4$, $p=5$ with maximum continuity of spline spaces.}
    \label{fig:ev_error}
\end{figure}


\begin{table}\scriptsize
    \centering
    \begin{tabular}{lccc}
         & \multicolumn{3}{c}{$p=3,\; C^2$} \\
        \cmidrule(lr){2-4}
        $\star_h$ choice & $h=0.1$   & $h=0.05$ & $h=0.025$ \\\midrule
        1$^{\text{st}}$ & \num[round-precision=3,round-mode=figures]{2.4823e-06} & \num[round-precision=3,round-mode=figures]{3.3299e-08} & \num[round-precision=3,round-mode=figures]{4.9932e-10} \\
        2$^{\text{nd}}$  & \num[round-precision=3,round-mode=figures]{0.00022543} & \num[round-precision=3,round-mode=figures]{1.3303e-05} & \num[round-precision=3,round-mode=figures]{8.1822e-07} \\
        3$^{\text{nd}}$  & \num[round-precision=3,round-mode=figures]{0.0016065} & \num[round-precision=3,round-mode=figures]{0.00011474} & \num[round-precision=3,round-mode=figures]{7.5516e-06} \\
        IGA & \num[round-precision=3,round-mode=figures]{2.4823e-06} & \num[round-precision=3,round-mode=figures]{3.3299e-08} & \num[round-precision=3,round-mode=figures]{4.9901e-10} \\\toprule
         & \multicolumn{3}{c}{$p=3,\; C^1$}\\
        \cmidrule(lr){2-4}
        $\star_h$ choice & $h=0.1$   & $h=0.05$ & $h=0.025$ \\\midrule
        1$^{\text{st}}$ & \num[round-precision=3,round-mode=figures]{1.7561e-06} & \num[round-precision=3,round-mode=figures]{3.0375e-08} & \num[round-precision=3,round-mode=figures]{4.8695e-10} \\
        2$^{\text{nd}}$ & \num[round-precision=3,round-mode=figures]{0.00020374} & \num[round-precision=3,round-mode=figures]{1.2946e-05} & \num[round-precision=3,round-mode=figures]{8.1252e-07} \\
        3$^{\text{nd}}$ & \num[round-precision=3,round-mode=figures]{0.00019181} & \num[round-precision=3,round-mode=figures]{1.118e-05} & \num[round-precision=3,round-mode=figures]{6.4952e-07}\\
        IGA  & \num[round-precision=3,round-mode=figures]{1.7561e-06} & \num[round-precision=3,round-mode=figures]{3.0375e-08} & \num[round-precision=3,round-mode=figures]{4.8753e-10} \\\toprule
    \end{tabular}
        \caption{Eigenvalue errors displayed in Fig.~\ref{fig:ev_error_8th_ring}, for the eighth of a ring as in Fig.~\ref{fig:reparam} (right).}
        \label{tab:ev_error_ring_table}
\end{table}

\begin{table}\scriptsize
    \centering
    \begin{tabular}{lccc}
        & \multicolumn{3}{c}{$p=4,\; C^3$}\\
        \cmidrule(lr){2-4}
        $\star_h$ choice & $h=0.1$   & $h=0.05$ & $h=0.025$ \\\midrule
        1$^{\text{st}}$ & \num[round-precision=3,round-mode=figures]{5.2216e-05} & \num[round-precision=3,round-mode=figures]{1.4952e-07} & \num[round-precision=3,round-mode=figures]{4.7673e-10} \\
        2$^{\text{nd}}$  & \num[round-precision=3,round-mode=figures]{0.00087635} & \num[round-precision=3,round-mode=figures]{8.4195e-06} & \num[round-precision=3,round-mode=figures]{1.1825e-07} \\
        3$^{\text{nd}}$  & \num[round-precision=3,round-mode=figures]{0.054706} & \num[round-precision=3,round-mode=figures]{0.0041133} & \num[round-precision=3,round-mode=figures]{0.00026783} \\
        IGA & \num[round-precision=3,round-mode=figures]{5.2216e-05} & \num[round-precision=3,round-mode=figures]{1.4952e-07} & \num[round-precision=3,round-mode=figures]{4.7686e-10} \\\toprule
         & \multicolumn{3}{c}{$p=5,\; C^4$}\\
        \cmidrule(lr){2-4}
        $\star_h$ choice & $h=0.1$   & $h=0.05$ & $h=0.025$ \\\midrule
        1$^{\text{st}}$  & \num[round-precision=3,round-mode=figures]{1.0562e-05} & \num[round-precision=3,round-mode=figures]{3.3832e-09} & \num[round-precision=3,round-mode=figures]{1.8761e-12}\\
        2$^{\text{nd}}$ & \num[round-precision=3,round-mode=figures]{0.00011429} & \num[round-precision=3,round-mode=figures]{1.8729e-07} & \num[round-precision=3,round-mode=figures]{5.3067e-10} \\
        3$^{\text{nd}}$ & \num[round-precision=3,round-mode=figures]{0.037563} & \num[round-precision=3,round-mode=figures]{0.0029882} & \num[round-precision=3,round-mode=figures]{0.00014765} \\
        IGA & \num[round-precision=3,round-mode=figures]{1.0562e-05} & \num[round-precision=3,round-mode=figures]{3.3832e-09} & \num[round-precision=3,round-mode=figures]{2.1829e-12} \\\toprule
    \end{tabular}
        \caption{Eigenvalue errors displayed in Fig.~\ref{fig:ev_error}, for $\Omega=(0,1)^3$ using \eqref{eq:harmonic_map} with $a=0.3$.}
        \label{tab:ev_error_table}
\end{table}

\normalsize

% & \num[round-precision=3,round-mode=figures]{2.4823e-06} & \num[round-precision=3,round-mode=figures]{3.3299e-08} & \num[round-precision=3,round-mode=figures]{4.9932e-10} & \num[round-precision=3,round-mode=figures]{5.2216e-05} & \num[round-precision=3,round-mode=figures]{1.4952e-07} & \num[round-precision=3,round-mode=figures]{4.7673e-10}
% & \num[round-precision=3,round-mode=figures]{0.00022543} & \num[round-precision=3,round-mode=figures]{1.3303e-05} & \num[round-precision=3,round-mode=figures]{8.1822e-07} & \num[round-precision=3,round-mode=figures]{0.00087635} & \num[round-precision=3,round-mode=figures]{8.4195e-06} & \num[round-precision=3,round-mode=figures]{1.1825e-07}
% & \num[round-precision=3,round-mode=figures]{0.0016065} & \num[round-precision=3,round-mode=figures]{0.00011474} & \num[round-precision=3,round-mode=figures]{7.5516e-06} & \num[round-precision=3,round-mode=figures]{0.054706} & \num[round-precision=3,round-mode=figures]{0.0041133} & \num[round-precision=3,round-mode=figures]{0.00026783}
% & \num[round-precision=3,round-mode=figures]{2.4823e-06} & \num[round-precision=3,round-mode=figures]{3.3299e-08} & \num[round-precision=3,round-mode=figures]{4.9901e-10} & \num[round-precision=3,round-mode=figures]{5.2216e-05} & \num[round-precision=3,round-mode=figures]{1.4952e-07} & \num[round-precision=3,round-mode=figures]{4.7686e-10}

% & \num[round-precision=3,round-mode=figures]{1.7561e-06} & \num[round-precision=3,round-mode=figures]{3.0375e-08} & \num[round-precision=3,round-mode=figures]{4.8695e-10} & \num[round-precision=3,round-mode=figures]{1.0562e-05} & \num[round-precision=3,round-mode=figures]{3.3832e-09} & \num[round-precision=3,round-mode=figures]{1.8761e-12}
% & \num[round-precision=3,round-mode=figures]{0.00020374} & \num[round-precision=3,round-mode=figures]{1.2946e-05} & \num[round-precision=3,round-mode=figures]{8.1252e-07} & \num[round-precision=3,round-mode=figures]{0.00011429} & \num[round-precision=3,round-mode=figures]{1.8729e-07} & \num[round-precision=3,round-mode=figures]{5.3067e-10}
% & \num[round-precision=3,round-mode=figures]{0.00019181} & \num[round-precision=3,round-mode=figures]{1.118e-05} & \num[round-precision=3,round-mode=figures]{6.4952e-07} & \num[round-precision=3,round-mode=figures]{0.037563} & \num[round-precision=3,round-mode=figures]{0.0029882} & \num[round-precision=3,round-mode=figures]{0.00014765}
% & \num[round-precision=3,round-mode=figures]{1.7561e-06} & \num[round-precision=3,round-mode=figures]{3.0375e-08} & \num[round-precision=3,round-mode=figures]{4.8753e-10} & \num[round-precision=3,round-mode=figures]{1.0562e-05} & \num[round-precision=3,round-mode=figures]{3.3832e-09} & \num[round-precision=3,round-mode=figures]{2.1829e-12}


==> paper_1/siamart_190516/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{An Example Article}{D. Doe, P. T. Frank, and J. E. Smith}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{An Example Article\thanks{Submitted to the editors DATE.
\funding{This work was funded by the Fog Research Institute under contract no.~FRI-454.}}}

% Authors: full names plus addresses.
\author{Dianne Doe\thanks{Imagination Corp., Chicago, IL 
  (\email{ddoe@imag.com}, \url{http://www.imag.com/\string~ddoe/}).}
\and Paul T. Frank\thanks{Department of Applied Mathematics, Fictional University, Boise, ID 
  (\email{ptfrank@fictional.edu}, \email{jesmith@fictional.edu}).}
\and Jane E. Smith\footnotemark[3]}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> paper_1/splinecomplex.tex <==
%\noindent {\color{blue} \textbf{Assigned Author(s):} Vazquez and Evans}\\

%\noindent {\color{blue} \textbf{Synopsis:} Provide background on previous work on B-spline complexes of isogeometric discrete differential forms.  The aim is to introduce not only the flavor of isogeometric discrete differential forms, but also introduce notions such as Greville grids which we will later exploit in our discussion of hierarchical spline complexes.  This will also require introducing the notion of a spline complex restricted to a submesh.  We should also make mention of T-spline complexes.}

In this section, we present the tensor-product B-spline complex of isogeometric discrete differential forms, which we refer to henceforth as simply the B-spline complex, extending the construction in \cite{BRSV11} to arbitrary dimension.  This complex is built using the tensor-product nature of multivariate B-splines as its name implies.  To fix notation, we first present univariate B-splines and multivariate B-splines before introducing the B-spline complex in both the parametric and physical domain.  We then discuss exactness and stability properties exhibited by the B-spline complex, and we finish with a geometric interpretation of the complex.

\subsection{Univariate B-splines} \label{sec:univariate}
To begin, let us briefly recall the definition of {\bf \em{univariate B-splines}}, and we refer the reader to \cite{deBoor} for further details.  Let $p$ denote the polynomial degree of the univariate B-splines, and let $m$ denote the number of B-spline basis functions in the space.  To define the B-spline basis functions, we first introduce a {\bf \em{($p$-)open knot vector}} $\Xi = \{\xi_{1}, \ldots , \xi_{m+p+1} \}$, where
\begin{equation*}
0 = \xi_{1} = \ldots = \xi_{p+1} < \xi_{p+2} \le \ldots \le \xi_m < \xi_{m+1} = \ldots = \xi_{m+p+1} = 1.
\end{equation*}
Using the well known Cox-de Boor formula, we can then define B-spline basis functions $\left\{B_{i,p}\right\}_{i=1}^m$.  We denote by $S_p(\Xi)$ the space they span, which is the space of piecewise polynomials of degree $p$, with the number of continuous derivatives at each knot $\xi_i$ given by $p-r_i$, where $r_i$ is the multiplicity of the knot.

We can actually define the $i^{\textup{th}}$ B-spline basis function $B_{i,p}$ as the unique B-spline basis function defined from the Cox-de Boor algorithm and the local knot vector $\{\xi_i, \ldots, \xi_{i+p+1}\}$, and its {\bf \emph{support}} is given by the interval $(\xi_i,\xi_{i+p+1})$. We remark that the support of functions will be always taken as an open set\footnote{This is the standard choice in the literature for hierarchical B-splines.} throughout the paper. From the internal knots of the local knot vector, we associate to each basis function a {\bf \emph{Greville site}} \cite[Chapter~9]{deBoor}:
\begin{equation} \label{eq:greville-point}
\gamma_i = \frac{\xi_{i+1} + \ldots + \xi_{i+p}}{p}.
\end{equation}
We will make heavy use of Greville sites in our later mathematical analysis.

Assuming the multiplicity of each of the internal knots is less or equal to $p$ (i.e., the B-spline functions are at least continuous), the derivative of a B-spline belonging to the space  $S_{p}(\Xi)$ is a B-spline belonging to the space $S_{p-1}(\Xi')$, where $\Xi' = \{\xi_2, \ldots, \xi_{m+p}\}$ is defined from $\Xi$ by removing the first and last repeated knots. We define the normalized basis functions $D_{i,p-1} = \frac{p}{\xi_{i+p} - \xi_i}B_{i,p-1}$, also called {\bf \em{Curry-Schoenberg B-splines}}, and note the following formula holds:
\begin{equation*}
B'_{i,p}(\zeta) = D_{i,p-1}(\zeta) - D_{i+1,p-1}(\zeta)
\end{equation*}
for $i = 1, \ldots, m$, where we are considering the convention that $D_{1,p-1}(\zeta) = D_{m+1,p-1}(\zeta) = 0$ for any $\zeta \in (0,1)$.  Analogous to before, the support of the $i^{\textup{th}}$ Curry-Schoenberg B-spline $D_{i,p}$ is $(\xi_i, \ldots, \xi_{i+p})$, and we can uniquely define the Curry-Schoenberg B-splines from their local knot vectors.

\subsection{Multivariate Tensor-Product B-splines}

{\bf \em{Multivariate tensor-product B-splines}}, or simply multivariate B-splines, are constructed from a tensor-product of univariate B-splines.  Namely, given a vector of polynomial degrees ${\bf p} = (p_1, \ldots, p_n)$ and a set of open knot vectors ${\boldsymbol \Xi} = \left\{ \Xi_q \right\}_{q=1}^n$, we define the multivariate B-spline basis as
\[
{\cal B}_{\bf p}(\boldsymbol \Xi) := \{ B_{\bf i,p}({\boldsymbol \zeta}) = B_{i_1,p_1}(\zeta_1) \ldots B_{i_n,p_n}(\zeta_n) \} \; \textup{ for ${\boldsymbol \zeta} \in (0,1)^n$},
\]
and the corresponding space they span as
\begin{equation*}
S_{\bf p}(\boldsymbol \Xi) \equiv S_{p_1,\ldots,p_n}(\Xi_1,\ldots,\Xi_n) = \otimes^n_{q=1} S_{p_q}\left(\Xi_q\right) = {\rm span} ({\cal B}_{\bf p}(\boldsymbol \Xi)),
\end{equation*}
where we have introduced the shorthand $S_{\bf p}(\boldsymbol \Xi)$ for ease of notation. %The Greville sites can also be generalized to the multivariate setting by simple Cartesian product.

For the definition of the B-spline complex, it is convenient to define an alternate set of multivariate B-splines as the product of a suitable choice of standard B-splines and Curry-Schoenberg B-splines. To do so we first introduce, for a given multi-index $\boldsymbol \alpha = \left(\alpha_1,\alpha_2,\ldots,\alpha_k\right)$, the notation
\begin{equation*}
\tilde{p}_q \equiv \tilde{p}_q(\boldsymbol \alpha) = \left\{
\begin{array}{cl}
p_q - 1 & \textup{ if } q = \alpha_j \textup{ for some } j \in \left\{1, \ldots, k \right\}, \\
p_q & \textup{ otherwise, }
\end{array} \right.
\end{equation*}
and
\begin{equation*}
\tilde{\Xi}_q \equiv \tilde{\Xi}_q(\boldsymbol \alpha) = \left\{
\begin{array}{cl}
\Xi'_q & \textup{ if } q = \alpha_j \textup{ for some } j \in \left\{1, \ldots, k \right\}, \\
\Xi_q & \textup{ otherwise. }
\end{array} \right.
\end{equation*}
With this notation, we define
\[
{\cal B}_{\bf p}(\boldsymbol \Xi; \boldsymbol \alpha) := \{\tilde B_{\bf i,\tilde p}({\boldsymbol \zeta}) = \tilde{B}_{i_1,\tilde p_1}(\zeta_1) \ldots \tilde{B}_{i_n,\tilde p_n}(\zeta_n) \} \; \textup{ for ${\boldsymbol \zeta} \in (0,1)^n$},
\]
where
\[
\tilde B_{i_q,\tilde p_q} \equiv \tilde B_{i_q,\tilde p_q}(\boldsymbol \alpha) := 
\left \{
\begin{array}{cl}
D_{i_q,p_q-1} & \textup{ if } q = \alpha_j \textup{ for some } j \in \left\{1, \ldots, k \right\}, \\
B_{i_q,p_q} & \textup{ otherwise, }
\end{array}
\right.
\]
and we denote the space these basis functions span by
\begin{equation*}
S_{\bf p}(\boldsymbol \Xi;\boldsymbol \alpha) = \otimes^n_{q=1} S_{\tilde{p}_q}\left(\tilde{\Xi}_q\right) = {\rm span}({\cal B}_{\bf p}(\boldsymbol \Xi; \boldsymbol \alpha)). 
\end{equation*}
Note that in constructing the multivariate spline space $S_{\bf p}(\boldsymbol \Xi;\boldsymbol \alpha)$, we have reduced the polynomial degree and continuity in each of the directions indicated by the multi-index $\boldsymbol \alpha$. In these directions, standard univariate B-splines are replaced by Curry-Schoenberg B-splines in order to construct multivariate basis functions.

%% \begin{equation*}
%% S_{\bf p}(\boldsymbol \Xi;\boldsymbol \alpha) \equiv S_{p_1,\ldots,p_n}(\Xi_1,\ldots,\Xi_n; \boldsymbol \alpha) = \otimes^n_{i=1} S_{\tilde{p}_i(\alpha)}\left(\tilde{\Xi}_i(\alpha)\right), 
%% \end{equation*}
%% where
%% \begin{equation*}
%% \tilde{p}_i(\alpha) = \left\{
%% \begin{array}{cc}
%% p_i - 1 & \textup{ if } i = \alpha_j \textup{ for some } j \in \left\{1, \ldots, k \right\}, \\
%% p_i & \textup{ otherwise, }
%% \end{array} \right.
%% \end{equation*}
%% and
%% \begin{equation*}
%% \tilde{\Xi}_i(\alpha) = \left\{
%% \begin{array}{cc}
%% \Xi'_i & \textup{ if } i = \alpha_j \textup{ for some } j \in \left\{1, \ldots, k \right\}, \\
%% \Xi_i & \textup{ otherwise, }
%% \end{array} \right.
%% \end{equation*}
%% where again we have introduced the shorthand $S_p(\Xi;\alpha)$ for ease of notation.  Note that in constructing the multivariate B-spline space $S_p(\Xi;\alpha)$, we have reduced the polynomial degree and continuity in each of the directions indicated by the multi-index $\alpha$.  Consequently, each of the basis functions for $S_p(\Xi;\alpha)$ is built from a tensor product of a suitable choice of standard B-spline basis functions $B_{i_j,p_j}$, and Curry-Schoenberg B-splines $D_{i_j,p_j-1}$. See \cite[Section~4]{BSV14} or \cite{Ratnani} for more details.

\subsection{The B-spline Complex}\label{sec:spline-complex}
We are now in a position to define the {\bf \em{B-spline complex of isogeometric discrete differential forms}}.  We first define this complex in the parametric domain before mapping it onto the physical domain.  To begin, let us assume that we are given a set of polynomial degrees $\left\{p_q\right\}_{q=1}^n$ and open knot vectors $\left\{ \Xi_q \right\}_{q=1}^n$, and let us further assume that multiplicity of the internal knots of $\Xi_q$ is never greater than $p_q$ for $q = 1, \ldots, n$.  This implies that the functions in $S_{\bf p}(\boldsymbol \Xi)$ are continuous and hence $S_{\bf p}(\boldsymbol \Xi) \subset H^1(\hat \Omega)$.  Then, we define the tensor-product spline space of isogeometric discrete differential $0$-forms as $\Xhath{0} := S_{\bf p}(\boldsymbol \Xi)$, and denote the corresponding basis by ${\cal B}^0 := {\cal B}_{\bf p}(\boldsymbol \Xi)$. For $k>0$, we define the basis of B-splines differential $k$-forms as
\begin{equation*}
{\cal B}^k = \bigcup_{\boldsymbol \alpha \in {\cal I}_k} \left\{ \tilde B_{\bf i, \tilde p} d\hat{x}_{\alpha_1} \wedge \ldots \wedge d\hat{x}_{\alpha_k} : \, \tilde B_{\bf i, \tilde p} \in {\cal B}_{\bf p}(\boldsymbol \Xi;\boldsymbol \alpha) \right\},
\end{equation*}
and we denote the space they span, which we call the tensor-product spline space of isogeometric discrete differential $k$-forms, by
\begin{equation*}
\Xhath{k} = \left\{ \hat{\omega}^h = \sum_{\boldsymbol \alpha \in \mathcal{I}_k} \hat{\omega}^h_{\boldsymbol \alpha} d\hat{x}_{\alpha_1} \wedge \ldots \wedge d\hat{x}_{\alpha_k} : \, \hat{\omega}^h_{\boldsymbol \alpha} \in S_{\bf p}(\boldsymbol \Xi;\boldsymbol \alpha), \hspace{5pt} \forall \boldsymbol \alpha \in \mathcal{I}_k \right\} = {\rm span}({\cal B}^k).
\end{equation*}
%\begin{equation*}
%\Xhath{k} = \left\{ \hat{\omega}^h = \sum_{\alpha \in \mathcal{I}_k} \hat{\omega}^h_\alpha d\hat{x}_{\alpha_1} \wedge \ldots \wedge d\hat{x}_{\alpha_k} : \hat{\omega}^h_{\alpha} \in S_p(\Xi;\alpha), \hspace{5pt} \forall \alpha \in \mathcal{I}_k \right\}.
%\end{equation*}
Then, it is easily shown that the above spaces comprise a discrete de Rham complex of the form:
\begin{equation} \label{eq:cd-iga-tp}
\begin{CD}
0 @>>> \mathbb{R} @>\subset>> \Xhath{0} @>d^0>> \Xhath{1} @>d^1>> \ldots @>d^{n-1}>> \Xhath{n} @>>> 0,
\end{CD}
\end{equation}
which we call the B-spline complex.

As in the infinite-dimensional setting, the meaning of the B-spline complex is most evident in the two- and three-dimensional settings, since the exterior derivatives coincide with differential operators of calculus via scalar or vector proxy fields.  In the two-dimensional case, we find that:
\begin{align}
\Xhath{0} &= S_{\bf p}(\boldsymbol \Xi) = S_{p_1,p_2}(\Xi_1,\Xi_2) \nonumber \\
\Xhath{1} &= S_{\bf p}\left(\boldsymbol \Xi; 1\right) \times S_{\bf p}\left(\boldsymbol \Xi; 2\right) = S_{p_1-1,p_2}(\Xi'_1,\Xi_2) \times S_{p_1,p_2-1}(\Xi_1,\Xi'_2) \nonumber \\
\Xhath{2} &= S_{\bf p}\left(\boldsymbol \Xi; (1, 2) \right) = S_{p_1-1,p_2-1}(\Xi'_1,\Xi'_2), \nonumber
\end{align}
and in the three-dimensional case, we find that:
\begin{align}
\Xhath{0} &= S_{\bf p}(\boldsymbol \Xi) \nonumber \\
&= S_{p_1,p_2,p_3}(\Xi_1,\Xi_2,\Xi_3) \nonumber \\
\Xhath{1} &= S_{\bf p}\left(\boldsymbol \Xi; 1\right) \times S_{\bf p}\left(\boldsymbol \Xi; 2\right) \times S_{\bf p}\left(\boldsymbol \Xi; 3\right) \nonumber \\
&= S_{p_1-1,p_2,p_3}(\Xi'_1,\Xi_2,\Xi_3) \times S_{p_1,p_2-1,p_3}(\Xi_1,\Xi'_2,\Xi_3) \times S_{p_1,p_2,p_3-1}(\Xi_1,\Xi_2,\Xi'_3) \nonumber \\
\Xhath{2} &= S_{\bf p}\left(\boldsymbol \Xi; (2,3)\right) \times S_{\bf p}\left(\boldsymbol \Xi; (1,3)\right) \times S_{\bf p}\left(\boldsymbol \Xi; (1,2)\right) \nonumber \\
&= S_{p_1,p_2-1,p_3-1}(\Xi_1,\Xi'_2,\Xi'_3) \times S_{p_1-1,p_2,p_3-1}(\Xi'_1,\Xi_2,\Xi'_3) \times S_{p_1-1,p_2-1,p_3}(\Xi'_1,\Xi'_2,\Xi_3) \nonumber \\
\Xhath{3} &= S_{\bf p}\left(\boldsymbol \Xi; (1, 2, 3) \right) \nonumber \\
&= S_{p_1-1,p_2-1,p_3-1}(\Xi'_1,\Xi'_2,\Xi'_3). \nonumber
\end{align}
Note that when all of the polynomial degrees are equal to one, the above spaces collapse onto the spaces of the {\bf \em{lowest-order finite element complex}}.  For instance, in the three-dimensional case, the discrete $0$-forms become continuous piecewise trilinear finite elements, the discrete $1$-forms 
become lowest-order edge N\'{e}d\'{e}lec finite elements, the discrete $2$-forms become lowest-order face N\'{e}d\'{e}lec finite elements, and the discrete $3$-forms become discontinuous piecewise constant finite elements.  Later, we will exploit a relationship between the B-spline complex and the lowest-order finite element complex to develop a geometric interpretation of the B-spline complex.

Throughout this paper, we will work with spaces subject to vanishing boundary conditions.  With this in mind, we define $\Xhathb{k} = \Xhath{k} \cap \Xhat^k_0$ to be the tensor-product spline space of isogeometric discrete differential $k$-forms subject to vanishing boundary conditions for all integers $k \geq 0$, and it can again be easily shown that these spaces comprise a discrete de Rham complex of the form:
\begin{equation} \label{eq:cd-iga-tp-bc}
\begin{CD}
0 @>>> \Xhathb{0} @>d^0>> \Xhathb{1} @>d^1>> \ldots @>d^{n-1}>> \Xhathb{n} @>\int>> \mathbb{R} @>>> 0.
\end{CD}
\end{equation}
Now that we have defined B-spline complexes with and without vanishing boundary conditions, it remains to define the corresponding B-spline complexes in the physical domain.  This is simply done using the pullback operators defined in Subsection \ref{subsec:pullback}.  Specifically, we define
\begin{equation*}
X_h^k\left(\Omega\right) := \left\{ \omega : \iota^k(\omega) \in \Xhath{k} \right\},
\end{equation*}
and
\begin{equation*}
X_{h,0}^k\left(\Omega\right) := \left\{ \omega : \iota^k(\omega) \in \Xhathb{k} \right\}
\end{equation*}
for all integers $k \geq 0$.  Using the definition of the pullback operators, it is easily shown that the above spaces comprise discrete de Rham complexes in the physical domain.

In the two-dimensional setting, a \textbf{\textit{rotated B-spline complex}} may easily be constructed by rotating the orientation of the discrete 1-forms by $\pi/2$ in parametric space and employing appropriate push-forward operators to map the rotated complex to the physical domain.  The rotated B-spline complex is ideally suited for the design of divergence-conforming discretizations for incompressible fluid flow.  See \cite{Evans12,EvHu12,EvHu12-2,EvHu12-3} for more details.

\subsection{Exactness and Stability of the B-spline Complex}

We have the following result regarding the exactness and stability of the B-spline complexes introduced in the preceding section.  The result was proven in three dimensions in \cite{BRSV11}, though the method of proof extends naturally to an arbitrary number of spatial dimensions.

\begin{proposition}
\label{proposition:commuting_parametric}
There exist $L^2$-stable projection operators $\Pi^k: X^k\left(\Omega\right) \rightarrow X^k_h\left(\Omega\right)$ and $\Pi^k_0 : X^k_0\left(\Omega\right) \rightarrow X^k_{h,0}\left(\Omega\right)$ for $k = 0, \ldots, n$ such that both
\begin{equation}
\begin{CD}
0 @>>> \mathbb{R} @>\subset>> X^0\left(\Omega\right) @>d^0>> X^1\left(\Omega\right) @>d^1>> \ldots @>d^{n-1}>> X^n\left(\Omega\right) @>>> 0 \\
& & & & @V \Pi^0 VV @V \Pi^1 VV & & @V \Pi^n VV \\
0 @>>> \mathbb{R} @>\subset>> X^0_h\left(\Omega\right) @>d^0>> X^1_h\left(\Omega\right) @>d^1>> \ldots @>d^{n-1}>> X^n_h\left(\Omega\right) @>>> 0
\end{CD}
\end{equation}
and
\begin{equation}
\begin{CD}
0 @>>> X_0^0\left(\Omega\right) @>d^0>> X_0^1\left(\Omega\right) @>d^1>> \ldots @>d^{n-1}>> X_0^n\left(\Omega\right) @>\int>> \mathbb{R} @>>> 0 \\
& & @V \Pi^0_0 VV @V \Pi^1_0 VV & & @V \Pi^n_0 VV & &\\
0 @>>> X^0_{h,0}\left(\Omega\right) @>d^0>> X^1_{h,0}\left(\Omega\right) @>d^1>> \ldots @>d^{n-1}>> X^n_{h,0}\left(\Omega\right) @>\int>> \mathbb{R} @>>> 0
\end{CD}
\end{equation}
commute. Furthermore, the continuity constants associated with the commutative projection operators only depend on the polynomial degrees of the B-spline discretization, the shape regularity of the B\'{e}zier mesh, and the parametric mapping.
\end{proposition}

The above result has two very important consequences regarding the B-spline complex.  First of all, the result states that the B-spline complex has the same cohomological structure as the de Rham complex.  Notably, when the domain $\Omega$ is contractible, the extended B-spline complexes, defined in a similar manner as the extended de Rham complexes, are exact.  Second of all, the existence of a set of commutative projection operators ensures that a discretization of the Maxwell eigenproblem using the B-spline complex is stable and convergent, and it also ensures that a discretization of the Stokes problem using the B-spline complex is inf-sup stable.

\subsection{Geometric Interpretation of the B-spline Complex} \label{sec:geometric_interpretation}

Now that we have properly defined the B-spline complex and examined its topological properties, we are ready to present a geometric interpretation of the complex.  This will prove especially useful when defining and analyzing the hierarchical B-spline complex.  To proceed forward, we need to establish the notion of a {\bf \emph{Greville grid}}.  We define the Greville grid in the parametric domain, but the Greville grid may also be defined in the physical domain using pushforward operators.

Recall from our previous discussion that we associate to each univariate B-spline basis function a Greville site.  Since multivariate B-splines are built from a tensor-product of univariate B-splines, we can associate to each basis function in $\Xhath{0}$ a {\bf \emph{Greville point}} defined as the Cartesian product of univariate Greville sites.  By connecting the Greville points, we obtain a Cartesian grid which we refer to as the Greville grid and we denote by $\MG$.  The Greville grid is a convenient means of visualizing the degrees of freedom of the B-spline complex, and we can in fact associate the basis functions of the spaces of the B-spline complex to the geometrical entities of the Greville grid as explained in \cite{BSV14}. By construction, the basis functions in $\Xhath{0}$ are uniquely identified with the {\bf \emph{vertices}} of the Greville grid $\MG$. Similarly, the basis functions of $\Xhath{1}$ and $\Xhath{2}$ are uniquely identified with the {\bf \emph{edges}} and the {\bf \emph{faces}} of $\MG$, respectively, while the basis functions of $\Xhath{3}$ are uniquely identified by the {\bf \emph{cells}} of $\MG$ in the three-dimensional setting. The matrices representing the differential operators $\{d^k\}_{k=0}^n$ between the spaces of the B-spline complex in terms of their respective basis functions are precisely the {\bf \emph{incidence matrices}} of the Greville grid.

Using tools from finite element exterior calculus, we can establish a more formal identification between the B-spline complex and the Greville grid.  In this direction, let us define $\{\Zhath{k}\}_{k=0}^n$ to be spaces of the {\bf \emph{lowest-order finite element complex}} defined on the Greville grid $\MG$.  The degrees of freedom for the spaces $\Zhath{0}$, $\Zhath{1}$, and $\Zhath{2}$ are associated to the vertices, the edges, and the faces of $\MG$, respectively, while the degrees of freedom of $\Zhath{3}$ are associated to the cells of $\MG$ in the three-dimensional setting. Exploiting the structure of the Greville grid, it was shown in \cite{BSV14} (see also \cite[Section~5]{BBSV-acta}) that we can define isomorphisms $\hat I^k_h: \Xhath{k} \longrightarrow \Zhath{k}$ that commute with the differential operators, that is,
\begin{equation*}
\hat I^{k+1}_h d^k = d^k \hat I^{k}_h, \text{ for } k = 0, \ldots, n-1,
\end{equation*}
and as a consequence we have the following de Rham commutative diagram:
\begin{equation} \label{eq:cd-iga-fem}
\begin{CD}
\Xhath{0} @>d^0>> \Xhath{1} @>d^1>> \ldots @>d^{n-1}>> \Xhath{n} \\
@V\hat I^0_hVV @V\hat I^1_hVV @. @V\hat I^n_hVV\\
\Zhath{0} @>d^0>> \Zhath{1} @>d^1>> \ldots @>d^{n-1}>> \Zhath{n}.
\end{CD}
\end{equation}
This indicates that the topological structure of the B-spline complex is identical to that of the finite element complex.  Moreover, as the cohomological structure of the finite element complex is tightly linked to the Greville grid, so is the cohomological structure of the B-spline complex.  We will exploit this property later when analyzing the hierarchical B-spline complex.

As was mentioned earlier, we will frequently work with spline spaces with vanishing boundary conditions in this work.  It is a straight-forward exercise to build a lowest-order finite element complex which commutes with such a B-spline complex using the Greville grid, so we do not discuss details herein for the sake of brevity.  We simply remark that we use the zero subindex (e.g., $\Zhathb{k}$) to identify spaces with vanishing boundary conditions.

We will need one more geometric concept in our later mathematical analysis.  Namely, we will need the concept of a {\bf \emph{B\'ezier mesh}}.  The B\'ezier mesh is simply the Cartesian grid generated by the knot vectors of multivariate B-splines, neglecting knot repetitions, and we denote this mesh by $\M$.  Note that the B\'ezier mesh and Greville grid only align in the setting when $p_1 = p_2 = \ldots = p_n = 1$.

To ground the concepts of B\'ezier mesh and Greville grid in an example, consider a two-dimensional B-spline complex with polynomial degrees $p_1 = 2$ and $p_2 = 2$ and knot vectors $\Xi_1 = \{0,0,0,1/6,2/6,3/6,4/6,5/6,1,1,1 \}$ and $\Xi_2 = \{ 0,0,0,1/5,2/5,3/5,4/5,1,1,1 \}$.  The B\'ezier and Greville grids for this particular example are displayed in Figure~\ref{fig:meshes}.  Note that as $p_1 \neq 1$ and $p_2 \neq 1$, the B\'ezier and Greville grids do not align as expected.  The finite element spaces $\Zhath{0}, \Zhath{1}$ and $\Zhath{2}$ are the spaces of {\bf \emph{bilinear nodal elements}}, {\bf \emph{lowest-order edge elements}}, and {\bf \emph{piecewise constant elements}}, respectively, defined on the Greville grid $\MG$ with degrees of freedom associated with the vertices, edges, and cells of the grid.
%Defining $\Xhath{0} = S_{p,p}(\Xi_1,\Xi_2)$, the space of splines of degree $p$, the spline complex takes the form
%\begin{equation*}
%\begin{CD}
%0 @>>> \mathbb{R} @>\subset>>\Xhath{0} @>\hat \grad>> \Xhath{1} @>\hat \curl>> \Xhath{2} @>>> 0 ,
%\end{CD}
%\end{equation*}
%where, with obvious notation, the space of 1-forms is the space of vector-valued splines of mixed degree $\Xhath{1}= (S_{p-1,p}(\Xi'_1,\Xi_2), S_{p,p-1}(\Xi_1,\Xi'_2))$, and the space of 2-forms is $\Xhath{2} = S_{p-1,p-1}(\Xi_1',\Xi_2')$. The knot vectors $\Xi_1'$ and $\Xi'_2$ are simply defined by removing from $\Xi_1$ and $\Xi_2$ the first and last knots. 
\begin{figure}[tp]
\begin{subfigure}[B\'ezier mesh]{
\centering
\includegraphics[width=3in]{Bezier.pdf}
}
\end{subfigure}
\begin{subfigure}[Greville grid]{
\centering
\includegraphics[width=3in]{Greville.pdf}
}
\end{subfigure}
\caption{B-spline meshes associated with polynomial degrees $p_1 = 2$ and $p_2 = 2$ and knot vectors $\Xi_1 = [0,0,0,1/6,2/6,3/6,4/6,5/6,1,1,1]$ and $\Xi_2 = [0,0,0,1/5,2/5,3/5,4/5,1,1,1]$.}
\label{fig:meshes}
\end{figure}

\subsection{Extension to Multi-Patch Geometries} \label{sec:multipatch}
Most geometries of scientific and engineering interest cannot be represented as the image of the unit domain.  Instead, the {\bf \emph{multi-patch concept}} must be invoked.  In this direction, we assume that there exist $n_p$ (corresponding to the number of patches) sufficiently smooth parametric mappings $\textbf{F}^j : \hat \Omega = \left(0,1\right)^n \rightarrow \mathbb{R}^n$ such that the subdomains 
$$\Omega^j = \textbf{F}^j(\widehat{\Omega}), \hspace{3pt} j = 1,\ldots,n_p$$ 
are non-overlapping and
\begin{equation}
\overline{\Omega} = \cup_{j=1}^{n_p} \overline{\Omega^j}. \nonumber
\end{equation}
We refer to each subdomain $\Omega^j$ (and its pre-image) as a {\bf \emph{patch}}.  For a visual depiction of a multi-patch construction in $\mathbb{R}^2$, see Figure \ref{fig:stokes_multipatch}.  We build B-spline complexes over each patch $\Omega^j, \hspace{3pt} j = 1,\ldots,n_p$ in the same manner as described in previous subsections, and we denote the tensor-product spline spaces for these complexes as $\left\{ X^k_h(\Omega^j) \right\}_{k=1}^n$.

\begin{figure}[tp]
\centering
\includegraphics[width=4.50in]{Figures/multipatch.pdf} 
\caption[Multi-patch construction]{Example multi-patch construction in $\mathbb{R}^2$.}
\label{fig:stokes_multipatch}
\end{figure}

To proceed further, we must make some assumptions.  First of all, we assume that if two disjoint patches $\Omega^{j_1}$ and $\Omega^{j_2}$ have the property that $\partial \Omega^{j_1} \cap \partial \Omega^{j_2} \neq \emptyset$, then this intersection consists strictly of $k$-faces with $k < n$ (e.g., vertices, edges, and faces in the three-dimensional setting).  More succinctly, two patches cannot intersect along an isolated portion of a $k$-face.  Second, we assume that if two patches $\Omega^{j_1}$ and $\Omega^{j_2}$ share a $k$-face, the B-spline meshes associated with the patches are identical along that $k$-face.  This guarantees our mesh is conforming.  Finally, we assume that the mappings $\left\{ \textbf{F}^j \right\}_{j=1}^{n_p}$ are compatible in the following sense: if two patches $\Omega^{j_1}$ and $\Omega^{j_2}$ share a $k$-face, then $\textbf{F}^{j_1}$ and $\textbf{F}^{j_2}$ parametrize that $k$-face identically up to changes in orientation.  The above three assumptions automatically hold if we employ a conforming NURBS multi-patch construction.  See, for example, \cite[Chapter~2]{IGA-book}.

With the above assumptions in mind, the spaces of the de Rham complex over the multi-patch geometry are simply defined as
\begin{equation} \label{eq:spline_complex_multipatch}
X^k_h = \left\{ \omega \in X^k(\Omega) : \omega|_{\Omega^j} \in X^k_h\left(\Omega^j\right),  \textup{ for } j = 1, \ldots, n_p \right\} \nonumber
\end{equation}
for $k = 1, \ldots, n$.  Basis functions for these spaces are easily constructed from their patch-wise counterparts.  For discrete 0-forms, we equivalence the coefficients of any basis functions whose traces are nonzero and equal in magnitude along shared hyper-faces between patches.  For discrete $k$-forms with $0 < k < n$, we use a similar procedure to equivalence basis functions between adjacent patches except that we must take into account the {\bf \textit{orientation}} of the basis functions.  The orientations are directly associated to the entities of the Greville grid as described in the preceding subsection.  For example, the orientations of discrete $2$-forms are associated with the faces of the Greville grid (and, in particular, the normal vectors to said faces) in the three-dimensional setting.  Thus, along the intersection between adjacent patches, we (i) equivalence the coefficients of any basis functions whose normal components are nonzero and equal in magnitude and direction and (ii) set the coefficient of one to minus the coefficient of another for any basis functions whose normal components are nonzero, equal in magnitude, and opposite in direction.  This is in direct analogy with finite element differential forms.  Finally, discrete $n$-forms are piecewise discontinuous and hence we do not need to equivalence basis functions between adjacent patches.  For more details on the construction of the B-spline complex in the multi-patch setting, the reader is referred to \cite[Section~5.4]{BBSV-acta}.\\

%\noindent {\color{blue} \textbf{Remarks (John):} Rafa, do you think we need a picture here?  I feel like we can simply point the reader to other work, especially as we have pictures for the hierarchical setting.}

%we need to establish a bit more notation.  Namely, let ${\cal B}^k$ denote the set of basis functions for the spline space $\Xhath{k}$.  Recall that the basis functions are standard tensor-product B-splines for $k = 0$, built from univariate B-spline basis functions $B_{i_j,p_j}$.  For $k > 0$, the basis functions are built as the tensor-product of standard B-spline basis functions $B_{i_j,p_j}$ and Curry-Schoenberg B-splines $D_{i_j,p_j}$.

%Let us recall that our goal is to create structure preserving discretizations of the complex $(\Xhat,d)$ presented in the introduction, using hierarchical splines. Before presenting the construction of the complex for hierarchical splines, we recall here some of the results that already exist for the tensor product case, which are mainly from \cite{BRSV11} and \cite{BSV14}.

%Let the space of tensor product splines $\Xhath{0} = \otimes_{j=1}^n S_{p_j}(\Xi_j)$, constructed from the univariate spaces of degree $p_j \ge 1$, with $p_j$-open knot vectors $\Xi_j$. We assume that the multiplicity of the internal knots of $\Xi_j$ is never greater than $p_j$, which implies that the functions in $\Xhath{0}$ are continuous, hence $\Xhath{0} \subset \Xhat^0 = H^1(\hat \Omega)$. As for hierarchical splines, we will denote by $\M$ the {\bf \emph{B\'ezier mesh}}, that is, the Cartesian grid generated by the knot vectors.

%Following the procedure explained in \cite[Section~4]{BSV14} we can construct a {\bf \emph{discrete de Rham complex}} of {\bf \emph{isogeometric differential forms}} $(\Xhath{},d)$, and a set of \emph{local and stable projectors} $\hat \Pi^i$ such that they satisfy the commutative diagram:
%{\Rd REMOVE THE PROJECTORS, IF NOT NEEDED}
%\begin{equation} \label{eq:cd-iga-pi}
%\begin{CD}
%\Xhat^0 @>d^0>> \Xhat^1 @>d^1>> \ldots @>d^{n-1}>> \Xhat^n, \\
%@.  @V\hat \Pi^0VV @V\hat \Pi^1VV @. @V\hat \Pi^nVV  \\
%\Xhath{0} @>d^0>> \Xhath{1} @>d^1>> \ldots @>d^{n-1}>> \Xhath{n},
%\end{CD}
%\end{equation}
%where each discrete space $\Xhath{i}$, or each component of the space, is defined by tensor product, taking suitable combinations of univariate spline spaces $S_{p_j}(\Xi_j)$ and $S_{p_j-1}(\Xi_j')$. Examples~\ref{ex:2d} and~\ref{ex:3d} below give more details about how to build the spaces.

%We will denote by ${\cal B}^i$ the basis for the spline space $\Xhath{i}$. For $i=0$, the basis functions are the standard tensor product B-splines, built from the univariate B-splines $B_{k_j,p_j}$. For $i>0$, the basis functions are built as the tensor product of a suitable choice of standard B-splines $B_{k_j,p_j}$, and the normalized B-splines $D_{k_j,p_j-1}$. See \cite[Section~4]{BSV14} or \cite{Ratnani} for the details.

%To each basis function in ${\cal B}^0$ we associate its corresponding {\bf \emph{Greville site}}, which are defined considering in each coordinate the univariate Greville sites in \eqref{eq:greville-point}. By connecting the Greville sites we obtain a Cartesian grid, that will be called {\bf \emph{Greville grid}}, and denoted by $\MG$. We remark that, in general, the Greville grid and the B\'ezier mesh do not overlap, as is shown in Example~\ref{ex:2d} and in Figure~\ref{fig:meshes}.

%{\Rd CHANGE NOTATION for $\hat Z$? similar to closed forms $Z$} Let us now define $\Zhath{i}$ to be spaces of the {\bf \emph{lowest-order finite element complex}} defined on the Greville grid $\MG$. The degrees of freedom for the spaces $\Zhath{0}$, $\Zhath{1}$, $\Zhath{2}$ are associated to the vertices, the edges and the faces of $\MG$, respectively, while in the three-dimensional case the degrees of freedom of $\Zhath{3}$ are associated to the volumes of $\MG$. Exploiting the structure of the Greville grid, it was shown in \cite{BSV14} (see also \cite[Sect.~5]{BBSV-acta}) that we can define isomorphisms $\hat I^i_h: \Xhath{i} \longrightarrow \Zhath{i}$ that commute with the differential operators, that is,
%\begin{equation*}
%\hat I^i_h d^i = d^i \hat I^{i+1}_h, \text{ for } i = 0, \ldots, n-1,
%\end{equation*}
%and as a consequence we have the following de Rham commutative diagram:
%\begin{equation} \label{eq:cd-iga-fem}
%\begin{CD}
%\Xhath{0} @>d^0>> \Xhath{1} @>d^1>> \ldots @>d^{n-1}>> \Xhath{n} \\
%@V\hat I^0_hVV @V\hat I^1_hVV @. @V\hat I^n_hVV\\
%\Zhath{0} @>d^0>> \Zhath{1} @>d^1>> \ldots @>d^{n-1}>> \Zhath{n}.
%\end{CD}
%\end{equation}
%This indicates that the topological structure of the spline spaces $\Xhath{i}$ is identical to that of the finite element spaces $\Zhath{i}$.
%
%Finally, it is important to note that we can also define spline spaces with vanishing boundary conditions, and also suitable projectors into these spaces. In this case the complex takes the form:
%{\Rd REMOVE THE PROJECTORS, IF NOT NEEDED}
%\begin{equation}\label{eq:cd-iga-pi0}
%\begin{CD}
%\Xhat_0^0 @>d^0>> \Xhat_0^1 @>d^1>> \ldots @>d^{n-1}>> \Xhat_0^n, \\
%@V\hat \Pi_0^0VV @V\hat \Pi_0^1VV @. @V\hat \Pi_0^nVV  \\
%\Xhathb{0} @>d^0>> \Xhathb{1} @>d^1>> \ldots @>d^{n-1}>> \Xhathb{n},
%\end{CD}
%\end{equation}
%and a commutative diagram analogous to \eqref{eq:cd-iga-fem} is also valid, considering the finite element spaces with boundary conditions defined on the Greville grid.
%
%In the following we will always work with spaces with homogeneous boundary conditions. This will allow a uniform treatment of the boundary of the domain and the boundary of the nested subdomains that define the hierarchical spaces, as we will see in Section~\ref{sec:submesh}. In order to alleviate notation, from now on \emph{we will drop the zero subindex} for spaces with boundary conditions.


%\begin{example}\label{ex:2d}
%Let us consider the two-dimensional case with $p_1 = p_2 = p=2$, and let the knot vectors $\Xi_1 = \{0,0,0,1/6,2/6,3/6,4/6,5/6,1,1,1 \}$ and $\Xi_2 = \{ 0,0,0,1/5,2/5,3/5,4/5,1,1,1 \}$. Defining $\Xhath{0} = S_{p,p}(\Xi_1,\Xi_2)$, the space of splines of degree $p$, the spline complex takes the form
%\begin{equation*}
%\begin{CD}
%0 @>>> \mathbb{R} @>\subset>>\Xhath{0} @>\hat \grad>> \Xhath{1} @>\hat \curl>> \Xhath{2} @>>> 0 ,
%\end{CD}
%\end{equation*}
%where, with obvious notation, the space of 1-forms is the space of vector-valued splines of mixed degree $\Xhath{1}= (S_{p-1,p}(\Xi'_1,\Xi_2), S_{p,p-1}(\Xi_1,\Xi'_2))$, and the space of 2-forms is $\Xhath{2} = S_{p-1,p-1}(\Xi_1',\Xi_2')$. The knot vectors $\Xi_1'$ and $\Xi'_2$ are simply defined by removing from $\Xi_1$ and $\Xi_2$ the first and last knots. The B\'ezier and Greville grids for this particular example are given in Figure~\ref{fig:meshes}. The finite element spaces $\Zhath{0}, \Zhath{1}$ and $\Zhath{2}$ are the spaces of {\bf \emph{nodal elements}} $Q^1$, low order {\bf \emph{edge elements}} and {\bf \emph{piecewise constant elements}}, respectively, defined on the grid $\MG$.
%\end{example}

%\begin{example}\label{ex:3d}
%Using the same notation for spline spaces, in the three-dimensional case for degrees $p_1, p_2$ and $p_3$, and open knot vectors $\Xi_1, \Xi_2$ and $\Xi_3$, the spaces of the complex are given by
%\begin{align*}
%& \Xhath{0} = S_{p_1,p_2,p_3}(\Xi_1, \Xi_2, \Xi_3),\\
%& \Xhath{1} = (S_{p_1-1,p_2,p_3}(\Xi'_1, \Xi_2, \Xi_3), S_{p_1,p_2-1,p_3}(\Xi_1, \Xi'_2, \Xi_3), S_{p_1,p_2,p_3-1}(\Xi_1, \Xi_2, \Xi'_3)), \\
%& \Xhath{2} = (S_{p_1,p_2-1,p_3-1}(\Xi_1, \Xi'_2, \Xi'_3), S_{p_1-1,p_2,p_3-1}(\Xi'_1, \Xi_2, \Xi'_3), S_{p_1-1,p_2-1,p_3}(\Xi'_1, \Xi'_2, \Xi_3)), \\
%& \Xhath{3} = S_{p_1-1,p_2-1,p_3-1}(\Xi'_1, \Xi'_2, \Xi'_3).
%\end{align*}
%which form the following exact sequence:
%\begin{equation*}
%\begin{CD}
%0 @>>> \mathbb{R} @>\subset>> \Xhath{0} @>\hat \grad>> \Xhath{1} @>\hat \curl>> \Xhath{2} @>\hat \div>> \Xhath{3} @>>> 0.
%\end{CD}
%\end{equation*}
%\end{example}



==> paper_1/stability.tex <==
In this section, we examine the stability properties of the hierarchical B-spline complex with specific reference to the Maxwell eigenproblem and the Stokes problem.  For these applications, stability is typically proven based on the construction of a set of local, stable and commutative projectors from the continuous de Rham complex to the discrete subcomplex. In the B-spline case, such projectors can be easily built exploiting the tensor-product structure of B-splines \cite{BRSV11}. The construction in the case of hierarchical B-splines is more subtle and is the subject of future work.

Due to the current lack of a complete theory based on commutative projectors, we have chosen to numerically study the stability of isogeometric discrete differential forms as applied to the Maxwell eigenproblem and the Stokes problem.  Not too unexpectedly, the numerical results show that exactness by itself is not sufficient to obtain a spurious free solution of Maxwell eigenproblem (see \cite{CFR01}), nor to obtain an inf-sup stable scheme for Stokes.  Instead, the numerical results suggest that Assumption~\ref{ass:support} is a necessary condition for stability for the considered applications.  However, our numerical results also suggest that Assumptions~\ref{ass:support} and~\ref{ass:overlap} together, plus a suitable grading of the mesh, are sufficient to obtain a stable scheme for both the Maxwell eigenproblem and the Stokes problem.

\subsection{Numerical Assessment of Spectral Correctness}

In our first group of stability tests, we consider the Maxwell eigenvalue problem.  In variational form, the problem consists of finding the eigenpair $({\bf u}_h, \lambda_h) \in W^1_N \times \mathbb{R}$, with $\lambda_h \ne 0$, such that 
\begin{equation}
(\curls {\bf u}_h, \curls {\bf v}_h) = \lambda_h ({\bf u}_h, {\bf v}_h) \quad \forall {\bf v}_h \in W^1_N, \label{eq:maxwell}
\end{equation}
where $(\cdot,\cdot)$ is the $L^2$-inner product defined over $\Omega$ and $W^1_N$ is the space of 1-forms, or curl conforming splines, in the hierarchical B-spline complex. In order to assess how the hierarchical B\'{e}zier mesh configuration affects the exactness of the complex, we also solve the mixed problems \cite{Boffi07}
\begin{equation} \label{eq:mf1}
\left \{
\begin{array}{rl}
(\curls {\bf u}_h, \curls {\bf v}_h) + (\grad p_h, {\bf v}_h) = \lambda_h ({\bf u}_h, {\bf v}_h) & \forall {\bf v}_h \in W^1_N, \\
(\grad q_h, {\bf u}_h) = 0 & \forall q_h \in W^0_N,
\end{array}
\right.
\end{equation}
and
\begin{equation} \label{eq:mf2}
\left \{
\begin{array}{rl}
({\bf u}_h, {\bf v}_h) + (\curls {\bf v}_h, \phi_h) = 0 & \forall {\bf v}_h \in W^1_N, \\
(\curls {\bf u}_h, \psi_h) = -\lambda_h (\phi_h, \psi_h) & \forall \psi_h \in W^2_N / \mathbb{R},
\end{array}
\right.
\end{equation}
which involve the other spaces of the sequence. For simplicity, the computations are conducted in the square domain $\Omega = (0,\pi)^2$ using the homogeneous Dirichlet condition ${\bf u}_h \times {\bf n}= 0$. In all the computations, the degree is taken equal to four in the first space of the discrete complex, which means that 1-forms are discretized with hierarchical splines of mixed degree three and four.

We have performed numerical tests for several hierarchical B\'{e}zier meshes, displayed in Figure~\ref{fig:meshes-maxwell1}, to assess the influence of Assumptions~\ref{ass:support} and~\ref{ass:overlap} on the eigenproblem discretization and also to see how the mesh configuration affects the exactness. The first mesh, in Figure~\ref{fig:mesh_3lines} does not satisfy any of the two assumptions for the chosen degree, and it does not satisfy the condition for exactness described in Section~\ref{sec:nec-suff}. The second mesh in Figure~\ref{fig:mesh_3lines_bulge} is a variation of the previous one, and it does not satisfy any of the assumptions but satisfies the exactness condition. The third through sixth meshes, in Figures~\ref{fig:mesh_p4_1x1}-\ref{fig:mesh_p4_4x4}, are refined along the diagonal, with a configuration inspired by Figures~\ref{fig:remove-add-1x1}--\ref{fig:assumptions-1-2}. They all satisfy Assumption~\ref{ass:support}, but only the last one satisfies Assumption~\ref{ass:overlap}. It can be easily checked that, among these last four meshes, only the ones in Figure~\ref{fig:mesh_p4_1x1} and Figure~\ref{fig:mesh_p4_4x4} satisfy the exactness condition. The properties satisfied by the six meshes, for the chosen degree, are summarized in Table~\ref{tab:maxwell-prop1}.

\begin{figure}[htp]
\begin{center}
\begin{subfigure}[]
{\includegraphics[width = 0.45\textwidth, trim=1cm 1cm 1cm 0cm, clip]{new_meshes/mesh_horizontal_p4_3lines}\label{fig:mesh_3lines}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.45\textwidth, trim=1cm 1cm 1cm 0cm, clip]{new_meshes/mesh_horizontal_p4_3lines_with_bulge}\label{fig:mesh_3lines_bulge}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.45\textwidth, trim=1cm 1cm 1cm 0cm, clip]{new_meshes/mesh_p4_1x1}\label{fig:mesh_p4_1x1}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.45\textwidth, trim=1cm 1cm 1cm 0cm, clip]{new_meshes/mesh_p4_2x2}\label{fig:mesh_p4_2x2}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.45\textwidth, trim=1cm 1cm 1cm 0cm, clip]{new_meshes/mesh_p4_3x3}\label{fig:mesh_p4_3x3}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.45\textwidth, trim=1cm 1cm 1cm 0cm, clip]{new_meshes/mesh_p4_4x4}\label{fig:mesh_p4_4x4}}
\end{subfigure}
\end{center}
\caption{The six different hierarchical B\'{e}zier mesh configurations used in the Maxwell eigenproblem tests.  Maximally continuous B-splines with $p_1 = p_2 = 4$ were employed in the tests.} \label{fig:meshes-maxwell1}
\end{figure}

\begin{table}
\caption{Properties satisfied by the six meshes tested for the Maxwell eigenproblem.} \label{tab:maxwell-prop1}
\centering
\begin{tabular}{|c||c|c|c|c|c|c|}
\hline
Mesh & Fig.~\ref{fig:mesh_3lines} & Fig.~\ref{fig:mesh_3lines_bulge} & Fig~\ref{fig:mesh_p4_1x1} & Fig.~\ref{fig:mesh_p4_2x2} & Fig.~\ref{fig:mesh_p4_3x3} & Fig.~\ref{fig:mesh_p4_4x4} \\
\hline
Assumption~\ref{ass:support} & No & No & Yes & Yes & Yes & Yes\\
Assumption~\ref{ass:overlap} & No & No & No & No & No & Yes \\
Exact sequence & No & Yes & Yes & No & No & Yes \\
\hline
No. of zeros in \eqref{eq:mf1} & 0 & 0 & 0 & 4 & 6 & 0 \\
No. of zeros in \eqref{eq:mf2} & 1 & 0 & 0 & 0 & 0 & 0 \\
Spurious free & No & No & Yes & No & Yes & Yes \\
\hline
\end{tabular}
\end{table}

%% , all the tests are performed in meshes that satisfy the condition of Section~\ref{sec:nec-suff}, and that are chosen to assess the influence of Assumptions~\ref{ass:support} and~\ref{ass:overlap} in the discretization. The first mesh, in Figure~\ref{fig:mesh_bulge}, does not satisfy any of the two assumptions for the chosen degree. The second and third mesh, in Figures~\ref{fig:mesh_min} and~\ref{fig:mesh_minmin} are refined along the diagonal with a configuration inspired by Figure~\ref{fig:remove-add-1x1}, and satisfy Assumption~\ref{ass:support} but not Assumption~\ref{ass:overlap}. The fourth mesh is also refined along the diagonal, and satisfies both assumptions. The properties satisfied by these meshes, for the chosen degree, is summarized in Table~\ref{tab:maxwell-prop}.

%% \begin{figure}[ht]
%% \begin{center}
%% \begin{subfigure}[]
%% {\includegraphics[width = 0.35\textwidth, trim=9cm 0cm 9cm 0cm, clip]{mesh_twocellLine_with_bulge.png}\label{fig:mesh_bulge}}
%% \end{subfigure}
%% \begin{subfigure}[]
%% {\includegraphics[width = 0.35\textwidth, trim=9cm 0cm 9cm 0cm, clip]{mesh_minimum_overlap.png}\label{fig:mesh_min}}
%% \end{subfigure}
%% \begin{subfigure}[]
%% {\includegraphics[width = 0.35\textwidth, trim=9cm 0cm 9cm 0cm, clip]{mesh_minmin_overlap.png}\label{fig:mesh_minmin}}
%% \end{subfigure}
%% \begin{subfigure}[]
%% {\includegraphics[width = 0.35\textwidth, trim=9cm 0cm 9cm 0cm, clip]{mesh_maximum_overlap.png}\label{fig:mesh_max} }
%% \end{subfigure}
%% \end{center}
%% \caption{Four different mesh configurations used in the numerical tests} \label{fig:meshes-maxwell}
%% \end{figure}

%% \begin{table}
%% \centering
%% \begin{tabular}{|c||c|c|c|c|}
%% \hline
%% Mesh & Fig.~\ref{fig:mesh_bulge} & Fig~\ref{fig:mesh_min} & Fig.~\ref{fig:mesh_minmin} & Fig.~\ref{fig:mesh_max} \\
%% \hline
%% Exact sequence & Yes & Yes & Yes & Yes \\
%% Assumption~\ref{ass:support} & No & Yes & Yes & Yes \\
%% Assumption~\ref{ass:overlap} & No & No & No & Yes \\
%% Spurious free & No & No & No & Yes \\
%% \hline
%% \end{tabular}
%% \caption{Properties satisfied by the four meshes tested in Maxwell eigenproblem} \label{tab:maxwell-prop}
%% \end{table}

In Figure~\ref{fig:spectrum}, we plot the first 50 eigenvalues computed using each of the six mesh configurations and compare them with the exact ones, including the multiplicity of each eigenvalue. In the results corresponding to the first mesh, which does not satisfy Assumption~\ref{ass:support}, spurious eigenvalues appear all along the spectrum in Figure~\ref{fig:spectrum_3lines}, and from the number of zeros in the solution of the mixed formulations~\eqref{eq:mf1} and~\eqref{eq:mf2}, reported in Table~\ref{tab:maxwell-prop1}, we see that exactness is lost in the second part of the sequence (that is, $\curls W^1_N \neq W^2_N / \mathbb{R}$). The exactness issue is fixed in the second mesh, but it also presents spurious eigenvalues in Figure~\ref{fig:spectrum_3lines_bulge}. This suggests that {\bf \emph{Assumption~\ref{ass:support} is a necessary condition}} to obtain a spurious-free discrete scheme.

For last four meshes, the lack of exactness in the meshes of Figures~\ref{fig:mesh_p4_2x2} and~\ref{fig:mesh_p4_3x3} only affects the first part of the sequence, since the zero eigenvalue appears in the solution of the mixed variational problem \eqref{eq:mf1}. The results of Figure~\ref{fig:spectrum} show that the mesh in Figure~\ref{fig:mesh_p4_2x2} presents spurious eigenvalues at positions $28^{\rm th}$, $31^{\rm st}$, $35^{\rm th}$ and $40^{\rm th}$. An analysis of the associated eigenfunctions, as the one represented in Figure~\ref{fig:eigenfunction}, suggests that spurious results are related to regions where Assumption~\ref{ass:overlap} fails. Surprisingly, the mesh in Figure~\ref{fig:mesh_p4_3x3} does not seem to present spurious eigenvalues, despite the lack of exactness. Finally, the meshes in Figures~~\ref{fig:mesh_p4_1x1} and~\ref{fig:mesh_p4_4x4} yield exact sequences and the corresponding results are spurious-free.

We have conducted a number of additional tests, and in each of these, we found that hierarchical B\'{e}zier meshes satisfying both Assumptions~\ref{ass:support} and~\ref{ass:overlap} yield spurious-free approximations for the Maxwell eigenproblem.  This suggests that {\bf \emph{Assumptions~\ref{ass:support} and~\ref{ass:overlap} are sufficient conditions}} to obtain a spurious-free discrete scheme.

\begin{figure}[htp]
\begin{subfigure}[]
{\includegraphics[width = 0.49\textwidth]{new_meshes/spectrum_horizontal_p4_3lines}\label{fig:spectrum_3lines}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.49\textwidth]{new_meshes/spectrum_horizontal_p4_3lines_with_bulge}\label{fig:spectrum_3lines_bulge}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.49\textwidth]{new_meshes/spectrum_p4_1x1}\label{fig:spectrum_p4_1x1}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.49\textwidth]{new_meshes/spectrum_p4_2x2}\label{fig:spectrum_p4_2x2}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.49\textwidth]{new_meshes/spectrum_p4_3x3}\label{fig:spectrum_p4_3x3}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.49\textwidth]{new_meshes/spectrum_p4_4x4}\label{fig:spectrum_p4_4x4}}
\end{subfigure}
\caption{Comparison of the exact and computed eigenvalues for the six meshes depicted in Figure~\ref{fig:meshes-maxwell1}.} \label{fig:spectrum}
\end{figure}

\begin{figure}[ht]
\centerline{\includegraphics[width=0.5\textwidth]{new_meshes/28th-eigenfunction-2x2}}
\caption{Magnitude of the first spurious eigenfunction for the mesh depicted in Figure~\ref{fig:mesh_p4_2x2}.}\label{fig:eigenfunction}
\end{figure}



%% In Figure~\ref{fig:spectrum} we compare the first eigenvalues computed in the four mesh configurations with the exact ones. In the first mesh, which fails to satisfy Assumption~\ref{ass:support}, spurious eigenvalues appear all along the spectrum in Figure~\ref{fig:spectrum_bulge}, and in fact the spurious results correspond to the solution of the eigenvalue problem (with Dirichlet condition) in the refined subregion where the assumption is violated, that is, where new functions are added without removing any coarse one.

%% \begin{figure}[ht]
%% \begin{subfigure}[]
%% {\includegraphics[width = 0.49\textwidth]{spectrum_TwoLineWithBulge.pdf}\label{fig:spectrum_bulge}}
%% \end{subfigure}
%% \begin{subfigure}[]
%% {\includegraphics[width = 0.49\textwidth]{spectrum_min_overlap.pdf}\label{fig:spectrum_min}}
%% \end{subfigure}
%% \begin{subfigure}[]
%% {\includegraphics[width = 0.49\textwidth]{spectrum_minmin_overlap.pdf}\label{fig:spectrum_minmin}}
%% \end{subfigure}
%% \begin{subfigure}[]
%% {\includegraphics[width = 0.49\textwidth]{spectrum_max_overlap.pdf} \label{fig:spectrum_max}}
%% \end{subfigure}
%% \caption{Comparison of the exact and computed eigenvalues, in the four meshes of Figure~\ref{fig:meshes-maxwell}} \label{fig:spectrum}
%% \end{figure}

%% In the second mesh the solution presents spurious eigenvalues at the $29^{\rm th}$ and $30^{\rm th}$ position in Figure~\ref{fig:spectrum_min}. The plot of the first spurious eigenfunction, in Figure~\ref{fig:eigenfunction}, makes clear that this bad behavior is caused by the violation of Assumption~\ref{ass:overlap}, because the magnitude of the function is greater in the regions where the assumption does not hold. Further refinement of the mesh without correcting this wrong configuration, as in Figure~\ref{fig:mesh_minmin}, does not lead to better results, and in fact the spurious eigenvalues appear earlier in the spectrum ($14^{\rm th}$ and $19^{\rm th}$ position in Figure~\ref{fig:spectrum_minmin}).

%% \begin{figure}[ht]
%% \centerline{\includegraphics[width=0.5\textwidth]{29th-eigenf-minimum-overlap-magnitude.png}}
%% \caption{Magnitude of the first spurious eigenfunction in the mesh of Figure~\ref{fig:mesh_min}}\label{fig:eigenfunction}
%% \end{figure}

%% Finally, the mesh in Figure~\ref{fig:mesh_max}, which satisfies both Assumption~\ref{ass:support} and Assumption~\ref{ass:overlap}, is the only one that presents a solution that is free of spurious modes, as seen in Figure~\ref{fig:spectrum_max}. These results, and several other tests not presented in this paper, suggest that the two assumptions are required to obtain a spurious free discretization.

\subsection{Numerical Assessment of Inf-Sup Stability}
Our second group of tests regards the inf-sup stability of a Stokes flow discretization based on the hierarchical B-spline complex. The variational formulation of the problem is to find a velocity ${\bf u}_h \in \textbf{V}_h$ and a pressure $p_h \in Q_h$ such that

\begin{equation*}
\left \{
\begin{array}{ll}
2 \nu ({\bf grad}^s\, {\bf u}_h, {\bf grad}^s {\bf v}_h) - c({\bf u}_h, {\bf v}_h) - (p_h, \div \, {\bf v}_h) = ({\bf f}, {\bf v}_h) - L({\bf v}_h) & \forall {\bf v}_h \in \textbf{V}_h, \\
(q_h, \div \, {\bf u}_h) = 0 & \forall q_h \in Q_h, \label{eq:stokes}
\end{array}
\right.
\end{equation*}
where ${\bf grad}^s$ is the symmetric part of the gradient, $\nu$ is a constant viscosity, ${\bf f}$ is a given source term, and the terms $c({\bf u}_h, {\bf v}_h)$ and $L({\bf v}_h)$ come from the weak imposition of tangential Dirichlet boundary conditions using Nitsche's method.  In particular:
\begin{equation*}
\begin{array}{l}
\displaystyle c({\bf u}_h, {\bf v}_h) = \int_{\Gamma_D} 2 \nu \left ((({\bf grad}^s {\bf u}_h) {\bf n}) \cdot {\bf v}_h + (({\bf grad}^s {\bf v}_h) {\bf n}) \cdot {\bf u}_h - \frac{C_{pen}}{h_F} {\bf u}_h \cdot {\bf v}_h \right), \\
\displaystyle L({\bf v}_h) = \int_{\Gamma_D} 2 \nu \left( (({\bf grad}^s {\bf v}_h){\bf n}) \cdot {\bf u}_{B} - \frac{C_{pen}}{h_F} {\bf v}_h \cdot {\bf u}_{B} \right),
\end{array}
\end{equation*}
where ${\bf u}_B$ is the imposed velocity along the Dirichlet boundary $\Gamma_D$, $h_F$ is the element size in the normal direction, and $C_{pen}$ is a sufficiently large penalization constant, see \cite{EvHu12} for details.  For the calculations shown here, $C_{pen} = 5 \max_{1 \leq i \leq n} p_i$.

In order to guarantee stability of the discretization scheme, the discrete spaces $V_h$ and $Q_h$ must satisfy the {\bf \emph{inf-sup}} stability condition
%\begin{equation*}
%\inf_{\substack{q_h \in Q_h \\ q_h \ne 0}} \sup_{\substack{ {\bf v}_h \in V_h \\ {\bf v}_h \ne 0}} \frac{(q_h, \div \, {\bf v}_h)}{\|{\bf v}_h\|_{H^1} \|q_h\|_{L^2} } \ge \beta,
%\end{equation*}
\begin{equation} \label{eq:inf-sup}
\inf_{q_h \in Q_h \setminus\{0\}} \sup_{{\bf v}_h \in \textbf{V}_h\setminus\{0\}} \frac{(q_h, \div \, {\bf v}_h)}{\|{\bf v}_h\|_{\textbf{V}_h} \|q_h\|_{L^2(\Omega)} } \ge \beta > 0,
\end{equation}
where $\beta$ is a positive constant independent of the mesh size and the number of levels and $\|\cdot \|_{\textbf{V}_h}$ is a suitable discrete norm.  Following \cite{EvHu12}, we choose:
\begin{equation}
\| \textbf{v}_h \|_{\textbf{V}_h} := \left( \| {\bf grad}^s \textbf{v}_h \|_{L^2(\Omega)}^2 + \| h^{1/2}_F \left( {\bf grad}^s \textbf{v}_h \right) {\bf n} \|^2_{L^2(\Gamma_D)} + \| \left(C_{pen}/h_F\right)^{1/2} \textbf{v}_h \|^2_{L^2(\Gamma_D)} \right)^{1/2}.
\end{equation}
We are also interested in discretization spaces that provide a pointwise divergence-free solution. A sufficient condition to satisfy the incompressibility constraint is that the divergence of $\textbf{V}_h$ is contained in $Q_h$, that is,
\begin{equation} \label{eq:equality}
\{ \div \, {\bf v}_h, {\bf v}_h \in \textbf{V}_h \} \subseteq Q_h,
\end{equation}
but this condition is in conflict with \eqref{eq:inf-sup} unless the two spaces in \eqref{eq:equality} are equal.

\begin{figure}[t]
\centering
\begin{subfigure}[]
{\includegraphics[width = 0.4\textwidth, trim=1cm 1cm 1cm 0cm, clip]{mesh_p3_1x1}\label{fig:mesh_min_stokes}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.4\textwidth, trim=1cm 1cm 1cm 0cm, clip]{mesh_p3_2x2}\label{fig:mesh_med_stokes}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.4\textwidth, trim=1cm 1cm 1cm 0cm, clip]{mesh_p3_3x3}\label{fig:mesh_max_stokes} }
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.4\textwidth, trim=1cm 1cm 1cm 0cm, clip]{mesh_p3_with_bulge}\label{fig:mesh_bulge_stokes}}
\end{subfigure}
\caption{The four different two-level hierarchical B\'{e}zier mesh configurations used in the Stokes inf-sup tests.  Maximally continuous B-splines with $p_1 = p_2 = 3$ were employed in the tests.} \label{fig:meshes-stokes}
\end{figure}

\begin{table}[t!]
\caption{Properties satisfied by the four two-level meshes considered for the Stokes inf-sup tests.} \label{tab:stokes_meshes}
\centering
\begin{tabular}{|c||c|c|c|c|}
\hline
& $1\times 1$ overlap & $2\times 2$ overlap & $3\times 3$ overlap & Bulge \\
Mesh & Fig.~\ref{fig:mesh_min_stokes} & Fig.~\ref{fig:mesh_med_stokes} & Fig.~\ref{fig:mesh_max_stokes} & Fig.~\ref{fig:mesh_bulge_stokes} \\
\hline
Assumption~\ref{ass:support} & Yes & Yes & Yes & No \\
Assumption~\ref{ass:overlap} & No & No & Yes & No \\
Exact sequence & Yes & No & Yes & Yes \\
\hline
Inf-sup stable (two levels) & Yes & Yes & Yes & No \\
Inf-sup stable (multilevel) & No & Yes & Yes & No \\
\hline
\end{tabular}
\end{table}

\begin{table}[t!]
\caption{Results of the Stokes inf-sup tests with the two-level meshes.} \label{tab:2levels}
\centering
\begin{tabular}{|c||c|c|c|c|c|}
\hline
Level 0 size & Uniform & $1\times 1$ overlap & $2\times 2$ overlap & $3\times 3$ overlap & Bulge \\
\hline
1/10 & 0.40996 & 0.40963 & 0.40963 & 0.40963 & 0.04818 \\
1/22 & 0.40957 & 0.40943 & 0.40943 & 0.40943 & 0.02046 \\
1/40 & 0.40943 & 0.40934 & 0.40934 & 0.40934 & 0.01098 \\
\hline
\end{tabular}
\end{table}

\begin{figure}[t!]
\begin{center}
\begin{subfigure}[]
{\includegraphics[width = 0.4\textwidth, trim=1cm 1cm 1cm 0cm, clip]{new_meshes/mesh_p3_1x1_4levels}\label{fig:min_4levels}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.4\textwidth, trim=1cm 1cm 1cm 0cm, clip]{new_meshes/mesh_p3_2x2_4levels}\label{fig:med_4levels}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.4\textwidth, trim=1cm 1cm 1cm 0cm, clip]{new_meshes/mesh_p3_3x3_4levels}\label{fig:max_4levels}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.4\textwidth, trim=1cm 1cm 1cm 0cm, clip]{new_meshes/mesh_p3_maxmin_4levels}\label{fig:maxmin_4levels}}
\end{subfigure}
\end{center}
\caption{The four different multilevel hierarchical B\'{e}zier mesh configurations, with four levels, used in the Stokes inf-sup tests.  Maximally continuous B-splines with $p_1 = p_2 = 3$ were employed in the tests.} \label{fig:meshes-stokes2}
\end{figure}

\begin{table}[t!]
\caption{Results of the Stokes inf-sup tests with the multilevel meshes.} \label{tab:multilevel}
\centering
\begin{tabular}{|c||c|c|c|c|}
\hline
& $1\times 1$ overlap & $2\times 2$ overlap & $3\times 3$ overlap & Graded ($1\times 1$) overlap\\
Levels& Fig.~\ref{fig:min_4levels} & Fig.~\ref{fig:med_4levels} & Fig.~\ref{fig:max_4levels} & Fig.~\ref{fig:maxmin_4levels} \\
\hline
1 & 0.40996 & 0.40996 & 0.40996 & 0.40996 \\
2 & 0.40963 & 0.40963 & 0.40963 & 0.40963 \\
3 & 0.29883 & 0.40945 & 0.40945 & 0.40944 \\
4 & 0.22467 & 0.40935 & 0.40935 & 0.40935 \\
5 & 0.17209 & 0.40929 & 0.40929 & 0.40916 \\
6 & 0.14519 & 0.40926 & 0.40926 & 0.40926 \\
\hline
\end{tabular}
\end{table}

In \cite{Buffa_deFalco_Sangalli} and \cite{EvHu12} a discretization scheme based on spline differential forms was proposed that is both divergence-free and stable. The key point is to choose the space of divergence-conforming splines (i.e., 1-forms in the rotated hierarchical B-spline complex in the two-dimensional setting and 2-forms in the standard hierarchical B-spline complex in the three-dimensional setting) as the velocity space $\textbf{V}_h$ and the spline space of $n$-forms as the pressure space $Q_h$.  When Dirichlet boundary conditions are enforced along the entire boundary, we set $\textbf{V}_h = W^2_N$ and $Q_h = W^3_N/\mathbb{R}$ in the three-dimensional setting.  Provided the velocity space $\textbf{V}_h$ satisfies $\textbf{V}_h \subset \left(H^1(\Omega)\right)^n$, the exactness of the tensor-product B-spline complex as well as associated commutative projectors guarantee that both \eqref{eq:inf-sup} and \eqref{eq:equality} are satisfied in the case of tensor-product B-splines (see \cite{EvHu12} for details). For hierarchical B-splines, the condition \eqref{eq:equality} is satisfied by construction, but since a set of commutative projectors is not available to prove \eqref{eq:inf-sup}, we have instead numerically computed the inf-sup constant through the solution of a discrete eigenvalue problem (see \cite{inf-sup-test}) for several mesh configurations to understand whether the resulting discretization scheme is stable or not. All the examples consider quadratic splines for pressure approximation and mixed quadratic-cubic splines for the velocity approximation.

The first set of tests regards hierarchical B\'{e}zier meshes with only two levels, and the value of the constant is compared also with the one obtained for tensor-product spaces with one single level. We have considered four different kind of refinements, similar to those already tested in Maxwell eigenproblem. For the first three, displayed in Figures~\ref{fig:mesh_min_stokes}-\ref{fig:mesh_max_stokes}, we refine several regions of $4\times4$ elements along the diagonal with different levels of overlaps between them. The fourth mesh, displayed in Figure~\ref{fig:mesh_bulge_stokes}, gives an exact sequence, but it does not satisfy Assumption~\ref{ass:support}. The properties satisfied by each of the four meshes are summarized in Table~\ref{tab:stokes_meshes}.

The results of the inf-sup test are reported in Table~\ref{tab:2levels}. All the diagonal refinements show a good behavior, even if the $2\times2$ overlap does not satisfy the exactness condition (see Figure~\ref{fig:remove-add-2x2}). In fact, we have seen in the previous tests for the Maxwell eigenproblem that the lack of exactness in this latter case only affects the ``left part'' of the diagram. On the contrary, the refinement in Figure~\ref{fig:mesh_bulge_stokes}, which does not satisfy Assumption~\ref{ass:support}, gives a discrete scheme that becomes unstable with increasing levels of mesh resolution. This suggests that {\bf \emph{Assumption~\ref{ass:support} is a necessary condition}} for inf-sup stability.

To understand whether the inf-sup constant depends on the number of levels present in the hierarchical B-spline complex, we have considered spline spaces with multiple levels in a second set of tests. We consider meshes with refinement along the diagonal as before but with an increasing number of levels.  See Figure~\ref{fig:min_4levels}-\ref{fig:max_4levels} for the resulting hierarchical B\'{e}zier meshes with four levels of refinement. The results obtained for the inf-sup constant are summarized in Table~\ref{tab:multilevel}. In this case, the discrete scheme remains stable for the $2\times 2$ and the $3 \times 3$ overlap, while the stability deteriorates for the $1\times 1$ overlap. This loss of stability is caused by the presence of adjacent elements corresponding to non-consecutive levels, and the issue can be avoided with a better grading of the mesh (see, e.g., \cite{Scott2014222}) which can be obtained using the $m$-admissible meshes defined in \cite{Buffa16-1}. To show this, we have repeated the inf-sup test for hierarchical B\'{e}zier meshes similar in appearance to Figure~\ref{fig:maxmin_4levels} where only the finest level is like in the $1\times 1$ overlap, thus avoiding non-graded meshes. The results in Table~\ref{tab:multilevel} show that in this case the scheme is stable with increasing levels of mesh resolution. It is worth to note that the loss of stability on non-graded meshes does not appear when using the generalization of Taylor-Hood elements with hierarchical splines \cite{Bressan-Juttler}, but in that case the incompressibility condition is not fulfilled exactly.  We have conducted a number of additional tests, and all of these suggest that {\bf \emph{Assumptions~\ref{ass:support} and~\ref{ass:overlap}, together with a suitable grading of the mesh, are sufficient conditions}} for inf-sup stability.  However, as demonstrated above for diagonal refinements with $2\times 2$ overlap, Assumption~\ref{ass:overlap} is not necessary for inf-sup stability.  Further study is required to develop necessary and sufficient conditions for inf-sup stability.

==> stability.tex <==
In this section, we examine the stability properties of the hierarchical B-spline complex with specific reference to the Maxwell eigenproblem and the Stokes problem.  For these applications, stability is typically proven based on the construction of a set of local, stable and commutative projectors from the continuous de Rham complex to the discrete subcomplex. In the B-spline case, such projectors can be easily built exploiting the tensor-product structure of B-splines \cite{BRSV11}. The construction in the case of hierarchical B-splines is more subtle and is the subject of future work.

Due to the current lack of a complete theory based on commutative projectors, we have chosen to numerically study the stability of isogeometric discrete differential forms as applied to the Maxwell eigenproblem and the Stokes problem.  Not too unexpectedly, the numerical results show that exactness by itself is not sufficient to obtain a spurious free solution of Maxwell eigenproblem (see \cite{CFR01}), nor to obtain an inf-sup stable scheme for Stokes.  Instead, the numerical results suggest that Assumption~\ref{ass:support} is a necessary condition for stability for the considered applications.  However, our numerical results also suggest that Assumptions~\ref{ass:support} and~\ref{ass:overlap} together, plus a suitable grading of the mesh, are sufficient to obtain a stable scheme for both the Maxwell eigenproblem and the Stokes problem.

\subsection{Numerical Assessment of Spectral Correctness}

In our first group of stability tests, we consider the Maxwell eigenvalue problem.  In variational form, the problem consists of finding the eigenpair $({\bf u}_h, \lambda_h) \in W^1_N \times \mathbb{R}$, with $\lambda_h \ne 0$, such that 
\begin{equation}
(\curls {\bf u}_h, \curls {\bf v}_h) = \lambda_h ({\bf u}_h, {\bf v}_h) \quad \forall {\bf v}_h \in W^1_N, \label{eq:maxwell}
\end{equation}
where $(\cdot,\cdot)$ is the $L^2$-inner product defined over $\Omega$ and $W^1_N$ is the space of 1-forms, or curl conforming splines, in the hierarchical B-spline complex. In order to assess how the hierarchical B\'{e}zier mesh configuration affects the exactness of the complex, we also solve the mixed problems \cite{Boffi07}
\begin{equation} \label{eq:mf1}
\left \{
\begin{array}{rl}
(\curls {\bf u}_h, \curls {\bf v}_h) + (\grad p_h, {\bf v}_h) = \lambda_h ({\bf u}_h, {\bf v}_h) & \forall {\bf v}_h \in W^1_N, \\
(\grad q_h, {\bf u}_h) = 0 & \forall q_h \in W^0_N,
\end{array}
\right.
\end{equation}
and
\begin{equation} \label{eq:mf2}
\left \{
\begin{array}{rl}
({\bf u}_h, {\bf v}_h) + (\curls {\bf v}_h, \phi_h) = 0 & \forall {\bf v}_h \in W^1_N, \\
(\curls {\bf u}_h, \psi_h) = -\lambda_h (\phi_h, \psi_h) & \forall \psi_h \in W^2_N / \mathbb{R},
\end{array}
\right.
\end{equation}
which involve the other spaces of the sequence. For simplicity, the computations are conducted in the square domain $\Omega = (0,\pi)^2$ using the homogeneous Dirichlet condition ${\bf u}_h \times {\bf n}= 0$. In all the computations, the degree is taken equal to four in the first space of the discrete complex, which means that 1-forms are discretized with hierarchical splines of mixed degree three and four.

We have performed numerical tests for several hierarchical B\'{e}zier meshes, displayed in Figure~\ref{fig:meshes-maxwell1}, to assess the influence of Assumptions~\ref{ass:support} and~\ref{ass:overlap} on the eigenproblem discretization and also to see how the mesh configuration affects the exactness. The first mesh, in Figure~\ref{fig:mesh_3lines} does not satisfy any of the two assumptions for the chosen degree, and it does not satisfy the condition for exactness described in Section~\ref{sec:nec-suff}. The second mesh in Figure~\ref{fig:mesh_3lines_bulge} is a variation of the previous one, and it does not satisfy any of the assumptions but satisfies the exactness condition. The third through sixth meshes, in Figures~\ref{fig:mesh_p4_1x1}-\ref{fig:mesh_p4_4x4}, are refined along the diagonal, with a configuration inspired by Figures~\ref{fig:remove-add-1x1}--\ref{fig:assumptions-1-2}. They all satisfy Assumption~\ref{ass:support}, but only the last one satisfies Assumption~\ref{ass:overlap}. It can be easily checked that, among these last four meshes, only the ones in Figure~\ref{fig:mesh_p4_1x1} and Figure~\ref{fig:mesh_p4_4x4} satisfy the exactness condition. The properties satisfied by the six meshes, for the chosen degree, are summarized in Table~\ref{tab:maxwell-prop1}.

\begin{figure}[htp]
\begin{center}
\begin{subfigure}[]
{\includegraphics[width = 0.45\textwidth, trim=1cm 1cm 1cm 0cm, clip]{new_meshes/mesh_horizontal_p4_3lines}\label{fig:mesh_3lines}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.45\textwidth, trim=1cm 1cm 1cm 0cm, clip]{new_meshes/mesh_horizontal_p4_3lines_with_bulge}\label{fig:mesh_3lines_bulge}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.45\textwidth, trim=1cm 1cm 1cm 0cm, clip]{new_meshes/mesh_p4_1x1}\label{fig:mesh_p4_1x1}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.45\textwidth, trim=1cm 1cm 1cm 0cm, clip]{new_meshes/mesh_p4_2x2}\label{fig:mesh_p4_2x2}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.45\textwidth, trim=1cm 1cm 1cm 0cm, clip]{new_meshes/mesh_p4_3x3}\label{fig:mesh_p4_3x3}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.45\textwidth, trim=1cm 1cm 1cm 0cm, clip]{new_meshes/mesh_p4_4x4}\label{fig:mesh_p4_4x4}}
\end{subfigure}
\end{center}
\caption{The six different hierarchical B\'{e}zier mesh configurations used in the Maxwell eigenproblem tests.  Maximally continuous B-splines with $p_1 = p_2 = 4$ were employed in the tests.} \label{fig:meshes-maxwell1}
\end{figure}

\begin{table}
\caption{Properties satisfied by the six meshes tested for the Maxwell eigenproblem.} \label{tab:maxwell-prop1}
\centering
\begin{tabular}{|c||c|c|c|c|c|c|}
\hline
Mesh & Fig.~\ref{fig:mesh_3lines} & Fig.~\ref{fig:mesh_3lines_bulge} & Fig~\ref{fig:mesh_p4_1x1} & Fig.~\ref{fig:mesh_p4_2x2} & Fig.~\ref{fig:mesh_p4_3x3} & Fig.~\ref{fig:mesh_p4_4x4} \\
\hline
Assumption~\ref{ass:support} & No & No & Yes & Yes & Yes & Yes\\
Assumption~\ref{ass:overlap} & No & No & No & No & No & Yes \\
Exact sequence & No & Yes & Yes & No & No & Yes \\
\hline
No. of zeros in \eqref{eq:mf1} & 0 & 0 & 0 & 4 & 6 & 0 \\
No. of zeros in \eqref{eq:mf2} & 1 & 0 & 0 & 0 & 0 & 0 \\
Spurious free & No & No & Yes & No & Yes & Yes \\
\hline
\end{tabular}
\end{table}

%% , all the tests are performed in meshes that satisfy the condition of Section~\ref{sec:nec-suff}, and that are chosen to assess the influence of Assumptions~\ref{ass:support} and~\ref{ass:overlap} in the discretization. The first mesh, in Figure~\ref{fig:mesh_bulge}, does not satisfy any of the two assumptions for the chosen degree. The second and third mesh, in Figures~\ref{fig:mesh_min} and~\ref{fig:mesh_minmin} are refined along the diagonal with a configuration inspired by Figure~\ref{fig:remove-add-1x1}, and satisfy Assumption~\ref{ass:support} but not Assumption~\ref{ass:overlap}. The fourth mesh is also refined along the diagonal, and satisfies both assumptions. The properties satisfied by these meshes, for the chosen degree, is summarized in Table~\ref{tab:maxwell-prop}.

%% \begin{figure}[ht]
%% \begin{center}
%% \begin{subfigure}[]
%% {\includegraphics[width = 0.35\textwidth, trim=9cm 0cm 9cm 0cm, clip]{mesh_twocellLine_with_bulge.png}\label{fig:mesh_bulge}}
%% \end{subfigure}
%% \begin{subfigure}[]
%% {\includegraphics[width = 0.35\textwidth, trim=9cm 0cm 9cm 0cm, clip]{mesh_minimum_overlap.png}\label{fig:mesh_min}}
%% \end{subfigure}
%% \begin{subfigure}[]
%% {\includegraphics[width = 0.35\textwidth, trim=9cm 0cm 9cm 0cm, clip]{mesh_minmin_overlap.png}\label{fig:mesh_minmin}}
%% \end{subfigure}
%% \begin{subfigure}[]
%% {\includegraphics[width = 0.35\textwidth, trim=9cm 0cm 9cm 0cm, clip]{mesh_maximum_overlap.png}\label{fig:mesh_max} }
%% \end{subfigure}
%% \end{center}
%% \caption{Four different mesh configurations used in the numerical tests} \label{fig:meshes-maxwell}
%% \end{figure}

%% \begin{table}
%% \centering
%% \begin{tabular}{|c||c|c|c|c|}
%% \hline
%% Mesh & Fig.~\ref{fig:mesh_bulge} & Fig~\ref{fig:mesh_min} & Fig.~\ref{fig:mesh_minmin} & Fig.~\ref{fig:mesh_max} \\
%% \hline
%% Exact sequence & Yes & Yes & Yes & Yes \\
%% Assumption~\ref{ass:support} & No & Yes & Yes & Yes \\
%% Assumption~\ref{ass:overlap} & No & No & No & Yes \\
%% Spurious free & No & No & No & Yes \\
%% \hline
%% \end{tabular}
%% \caption{Properties satisfied by the four meshes tested in Maxwell eigenproblem} \label{tab:maxwell-prop}
%% \end{table}

In Figure~\ref{fig:spectrum}, we plot the first 50 eigenvalues computed using each of the six mesh configurations and compare them with the exact ones, including the multiplicity of each eigenvalue. In the results corresponding to the first mesh, which does not satisfy Assumption~\ref{ass:support}, spurious eigenvalues appear all along the spectrum in Figure~\ref{fig:spectrum_3lines}, and from the number of zeros in the solution of the mixed formulations~\eqref{eq:mf1} and~\eqref{eq:mf2}, reported in Table~\ref{tab:maxwell-prop1}, we see that exactness is lost in the second part of the sequence (that is, $\curls W^1_N \neq W^2_N / \mathbb{R}$). The exactness issue is fixed in the second mesh, but it also presents spurious eigenvalues in Figure~\ref{fig:spectrum_3lines_bulge}. This suggests that {\bf \emph{Assumption~\ref{ass:support} is a necessary condition}} to obtain a spurious-free discrete scheme.

For last four meshes, the lack of exactness in the meshes of Figures~\ref{fig:mesh_p4_2x2} and~\ref{fig:mesh_p4_3x3} only affects the first part of the sequence, since the zero eigenvalue appears in the solution of the mixed variational problem \eqref{eq:mf1}. The results of Figure~\ref{fig:spectrum} show that the mesh in Figure~\ref{fig:mesh_p4_2x2} presents spurious eigenvalues at positions $28^{\rm th}$, $31^{\rm st}$, $35^{\rm th}$ and $40^{\rm th}$. An analysis of the associated eigenfunctions, as the one represented in Figure~\ref{fig:eigenfunction}, suggests that spurious results are related to regions where Assumption~\ref{ass:overlap} fails. Surprisingly, the mesh in Figure~\ref{fig:mesh_p4_3x3} does not seem to present spurious eigenvalues, despite the lack of exactness. Finally, the meshes in Figures~~\ref{fig:mesh_p4_1x1} and~\ref{fig:mesh_p4_4x4} yield exact sequences and the corresponding results are spurious-free.

We have conducted a number of additional tests, and in each of these, we found that hierarchical B\'{e}zier meshes satisfying both Assumptions~\ref{ass:support} and~\ref{ass:overlap} yield spurious-free approximations for the Maxwell eigenproblem.  This suggests that {\bf \emph{Assumptions~\ref{ass:support} and~\ref{ass:overlap} are sufficient conditions}} to obtain a spurious-free discrete scheme.

\begin{figure}[htp]
\begin{subfigure}[]
{\includegraphics[width = 0.49\textwidth]{new_meshes/spectrum_horizontal_p4_3lines}\label{fig:spectrum_3lines}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.49\textwidth]{new_meshes/spectrum_horizontal_p4_3lines_with_bulge}\label{fig:spectrum_3lines_bulge}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.49\textwidth]{new_meshes/spectrum_p4_1x1}\label{fig:spectrum_p4_1x1}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.49\textwidth]{new_meshes/spectrum_p4_2x2}\label{fig:spectrum_p4_2x2}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.49\textwidth]{new_meshes/spectrum_p4_3x3}\label{fig:spectrum_p4_3x3}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.49\textwidth]{new_meshes/spectrum_p4_4x4}\label{fig:spectrum_p4_4x4}}
\end{subfigure}
\caption{Comparison of the exact and computed eigenvalues for the six meshes depicted in Figure~\ref{fig:meshes-maxwell1}.} \label{fig:spectrum}
\end{figure}

\begin{figure}[ht]
\centerline{\includegraphics[width=0.5\textwidth]{new_meshes/28th-eigenfunction-2x2}}
\caption{Magnitude of the first spurious eigenfunction for the mesh depicted in Figure~\ref{fig:mesh_p4_2x2}.}\label{fig:eigenfunction}
\end{figure}



%% In Figure~\ref{fig:spectrum} we compare the first eigenvalues computed in the four mesh configurations with the exact ones. In the first mesh, which fails to satisfy Assumption~\ref{ass:support}, spurious eigenvalues appear all along the spectrum in Figure~\ref{fig:spectrum_bulge}, and in fact the spurious results correspond to the solution of the eigenvalue problem (with Dirichlet condition) in the refined subregion where the assumption is violated, that is, where new functions are added without removing any coarse one.

%% \begin{figure}[ht]
%% \begin{subfigure}[]
%% {\includegraphics[width = 0.49\textwidth]{spectrum_TwoLineWithBulge.pdf}\label{fig:spectrum_bulge}}
%% \end{subfigure}
%% \begin{subfigure}[]
%% {\includegraphics[width = 0.49\textwidth]{spectrum_min_overlap.pdf}\label{fig:spectrum_min}}
%% \end{subfigure}
%% \begin{subfigure}[]
%% {\includegraphics[width = 0.49\textwidth]{spectrum_minmin_overlap.pdf}\label{fig:spectrum_minmin}}
%% \end{subfigure}
%% \begin{subfigure}[]
%% {\includegraphics[width = 0.49\textwidth]{spectrum_max_overlap.pdf} \label{fig:spectrum_max}}
%% \end{subfigure}
%% \caption{Comparison of the exact and computed eigenvalues, in the four meshes of Figure~\ref{fig:meshes-maxwell}} \label{fig:spectrum}
%% \end{figure}

%% In the second mesh the solution presents spurious eigenvalues at the $29^{\rm th}$ and $30^{\rm th}$ position in Figure~\ref{fig:spectrum_min}. The plot of the first spurious eigenfunction, in Figure~\ref{fig:eigenfunction}, makes clear that this bad behavior is caused by the violation of Assumption~\ref{ass:overlap}, because the magnitude of the function is greater in the regions where the assumption does not hold. Further refinement of the mesh without correcting this wrong configuration, as in Figure~\ref{fig:mesh_minmin}, does not lead to better results, and in fact the spurious eigenvalues appear earlier in the spectrum ($14^{\rm th}$ and $19^{\rm th}$ position in Figure~\ref{fig:spectrum_minmin}).

%% \begin{figure}[ht]
%% \centerline{\includegraphics[width=0.5\textwidth]{29th-eigenf-minimum-overlap-magnitude.png}}
%% \caption{Magnitude of the first spurious eigenfunction in the mesh of Figure~\ref{fig:mesh_min}}\label{fig:eigenfunction}
%% \end{figure}

%% Finally, the mesh in Figure~\ref{fig:mesh_max}, which satisfies both Assumption~\ref{ass:support} and Assumption~\ref{ass:overlap}, is the only one that presents a solution that is free of spurious modes, as seen in Figure~\ref{fig:spectrum_max}. These results, and several other tests not presented in this paper, suggest that the two assumptions are required to obtain a spurious free discretization.

\subsection{Numerical Assessment of Inf-Sup Stability}
Our second group of tests regards the inf-sup stability of a Stokes flow discretization based on the hierarchical B-spline complex. The variational formulation of the problem is to find a velocity ${\bf u}_h \in \textbf{V}_h$ and a pressure $p_h \in Q_h$ such that

\begin{equation*}
\left \{
\begin{array}{ll}
2 \nu ({\bf grad}^s\, {\bf u}_h, {\bf grad}^s {\bf v}_h) - c({\bf u}_h, {\bf v}_h) - (p_h, \div \, {\bf v}_h) = ({\bf f}, {\bf v}_h) - L({\bf v}_h) & \forall {\bf v}_h \in \textbf{V}_h, \\
(q_h, \div \, {\bf u}_h) = 0 & \forall q_h \in Q_h, \label{eq:stokes}
\end{array}
\right.
\end{equation*}
where ${\bf grad}^s$ is the symmetric part of the gradient, $\nu$ is a constant viscosity, ${\bf f}$ is a given source term, and the terms $c({\bf u}_h, {\bf v}_h)$ and $L({\bf v}_h)$ come from the weak imposition of tangential Dirichlet boundary conditions using Nitsche's method.  In particular:
\begin{equation*}
\begin{array}{l}
\displaystyle c({\bf u}_h, {\bf v}_h) = \int_{\Gamma_D} 2 \nu \left ((({\bf grad}^s {\bf u}_h) {\bf n}) \cdot {\bf v}_h + (({\bf grad}^s {\bf v}_h) {\bf n}) \cdot {\bf u}_h - \frac{C_{pen}}{h_F} {\bf u}_h \cdot {\bf v}_h \right), \\
\displaystyle L({\bf v}_h) = \int_{\Gamma_D} 2 \nu \left( (({\bf grad}^s {\bf v}_h){\bf n}) \cdot {\bf u}_{B} - \frac{C_{pen}}{h_F} {\bf v}_h \cdot {\bf u}_{B} \right),
\end{array}
\end{equation*}
where ${\bf u}_B$ is the imposed velocity along the Dirichlet boundary $\Gamma_D$, $h_F$ is the element size in the normal direction, and $C_{pen}$ is a sufficiently large penalization constant, see \cite{EvHu12} for details.  For the calculations shown here, $C_{pen} = 5 \max_{1 \leq i \leq n} p_i$.

In order to guarantee stability of the discretization scheme, the discrete spaces $V_h$ and $Q_h$ must satisfy the {\bf \emph{inf-sup}} stability condition
%\begin{equation*}
%\inf_{\substack{q_h \in Q_h \\ q_h \ne 0}} \sup_{\substack{ {\bf v}_h \in V_h \\ {\bf v}_h \ne 0}} \frac{(q_h, \div \, {\bf v}_h)}{\|{\bf v}_h\|_{H^1} \|q_h\|_{L^2} } \ge \beta,
%\end{equation*}
\begin{equation} \label{eq:inf-sup}
\inf_{q_h \in Q_h \setminus\{0\}} \sup_{{\bf v}_h \in \textbf{V}_h\setminus\{0\}} \frac{(q_h, \div \, {\bf v}_h)}{\|{\bf v}_h\|_{\textbf{V}_h} \|q_h\|_{L^2(\Omega)} } \ge \beta > 0,
\end{equation}
where $\beta$ is a positive constant independent of the mesh size and the number of levels and $\|\cdot \|_{\textbf{V}_h}$ is a suitable discrete norm.  Following \cite{EvHu12}, we choose:
\begin{equation}
\| \textbf{v}_h \|_{\textbf{V}_h} := \left( \| {\bf grad}^s \textbf{v}_h \|_{L^2(\Omega)}^2 + \| h^{1/2}_F \left( {\bf grad}^s \textbf{v}_h \right) {\bf n} \|^2_{L^2(\Gamma_D)} + \| \left(C_{pen}/h_F\right)^{1/2} \textbf{v}_h \|^2_{L^2(\Gamma_D)} \right)^{1/2}.
\end{equation}
We are also interested in discretization spaces that provide a pointwise divergence-free solution. A sufficient condition to satisfy the incompressibility constraint is that the divergence of $\textbf{V}_h$ is contained in $Q_h$, that is,
\begin{equation} \label{eq:equality}
\{ \div \, {\bf v}_h, {\bf v}_h \in \textbf{V}_h \} \subseteq Q_h,
\end{equation}
but this condition is in conflict with \eqref{eq:inf-sup} unless the two spaces in \eqref{eq:equality} are equal.

\begin{figure}[t]
\centering
\begin{subfigure}[]
{\includegraphics[width = 0.4\textwidth, trim=1cm 1cm 1cm 0cm, clip]{mesh_p3_1x1}\label{fig:mesh_min_stokes}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.4\textwidth, trim=1cm 1cm 1cm 0cm, clip]{mesh_p3_2x2}\label{fig:mesh_med_stokes}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.4\textwidth, trim=1cm 1cm 1cm 0cm, clip]{mesh_p3_3x3}\label{fig:mesh_max_stokes} }
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.4\textwidth, trim=1cm 1cm 1cm 0cm, clip]{mesh_p3_with_bulge}\label{fig:mesh_bulge_stokes}}
\end{subfigure}
\caption{The four different two-level hierarchical B\'{e}zier mesh configurations used in the Stokes inf-sup tests.  Maximally continuous B-splines with $p_1 = p_2 = 3$ were employed in the tests.} \label{fig:meshes-stokes}
\end{figure}

\begin{table}[t!]
\caption{Properties satisfied by the four two-level meshes considered for the Stokes inf-sup tests.} \label{tab:stokes_meshes}
\centering
\begin{tabular}{|c||c|c|c|c|}
\hline
& $1\times 1$ overlap & $2\times 2$ overlap & $3\times 3$ overlap & Bulge \\
Mesh & Fig.~\ref{fig:mesh_min_stokes} & Fig.~\ref{fig:mesh_med_stokes} & Fig.~\ref{fig:mesh_max_stokes} & Fig.~\ref{fig:mesh_bulge_stokes} \\
\hline
Assumption~\ref{ass:support} & Yes & Yes & Yes & No \\
Assumption~\ref{ass:overlap} & No & No & Yes & No \\
Exact sequence & Yes & No & Yes & Yes \\
\hline
Inf-sup stable (two levels) & Yes & Yes & Yes & No \\
Inf-sup stable (multilevel) & No & Yes & Yes & No \\
\hline
\end{tabular}
\end{table}

\begin{table}[t!]
\caption{Results of the Stokes inf-sup tests with the two-level meshes.} \label{tab:2levels}
\centering
\begin{tabular}{|c||c|c|c|c|c|}
\hline
Level 0 size & Uniform & $1\times 1$ overlap & $2\times 2$ overlap & $3\times 3$ overlap & Bulge \\
\hline
1/10 & 0.40996 & 0.40963 & 0.40963 & 0.40963 & 0.04818 \\
1/22 & 0.40957 & 0.40943 & 0.40943 & 0.40943 & 0.02046 \\
1/40 & 0.40943 & 0.40934 & 0.40934 & 0.40934 & 0.01098 \\
\hline
\end{tabular}
\end{table}

\begin{figure}[t!]
\begin{center}
\begin{subfigure}[]
{\includegraphics[width = 0.4\textwidth, trim=1cm 1cm 1cm 0cm, clip]{new_meshes/mesh_p3_1x1_4levels}\label{fig:min_4levels}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.4\textwidth, trim=1cm 1cm 1cm 0cm, clip]{new_meshes/mesh_p3_2x2_4levels}\label{fig:med_4levels}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.4\textwidth, trim=1cm 1cm 1cm 0cm, clip]{new_meshes/mesh_p3_3x3_4levels}\label{fig:max_4levels}}
\end{subfigure}
\begin{subfigure}[]
{\includegraphics[width = 0.4\textwidth, trim=1cm 1cm 1cm 0cm, clip]{new_meshes/mesh_p3_maxmin_4levels}\label{fig:maxmin_4levels}}
\end{subfigure}
\end{center}
\caption{The four different multilevel hierarchical B\'{e}zier mesh configurations, with four levels, used in the Stokes inf-sup tests.  Maximally continuous B-splines with $p_1 = p_2 = 3$ were employed in the tests.} \label{fig:meshes-stokes2}
\end{figure}

\begin{table}[t!]
\caption{Results of the Stokes inf-sup tests with the multilevel meshes.} \label{tab:multilevel}
\centering
\begin{tabular}{|c||c|c|c|c|}
\hline
& $1\times 1$ overlap & $2\times 2$ overlap & $3\times 3$ overlap & Graded ($1\times 1$) overlap\\
Levels& Fig.~\ref{fig:min_4levels} & Fig.~\ref{fig:med_4levels} & Fig.~\ref{fig:max_4levels} & Fig.~\ref{fig:maxmin_4levels} \\
\hline
1 & 0.40996 & 0.40996 & 0.40996 & 0.40996 \\
2 & 0.40963 & 0.40963 & 0.40963 & 0.40963 \\
3 & 0.29883 & 0.40945 & 0.40945 & 0.40944 \\
4 & 0.22467 & 0.40935 & 0.40935 & 0.40935 \\
5 & 0.17209 & 0.40929 & 0.40929 & 0.40916 \\
6 & 0.14519 & 0.40926 & 0.40926 & 0.40926 \\
\hline
\end{tabular}
\end{table}

In \cite{Buffa_deFalco_Sangalli} and \cite{EvHu12} a discretization scheme based on spline differential forms was proposed that is both divergence-free and stable. The key point is to choose the space of divergence-conforming splines (i.e., 1-forms in the rotated hierarchical B-spline complex in the two-dimensional setting and 2-forms in the standard hierarchical B-spline complex in the three-dimensional setting) as the velocity space $\textbf{V}_h$ and the spline space of $n$-forms as the pressure space $Q_h$.  When Dirichlet boundary conditions are enforced along the entire boundary, we set $\textbf{V}_h = W^2_N$ and $Q_h = W^3_N/\mathbb{R}$ in the three-dimensional setting.  Provided the velocity space $\textbf{V}_h$ satisfies $\textbf{V}_h \subset \left(H^1(\Omega)\right)^n$, the exactness of the tensor-product B-spline complex as well as associated commutative projectors guarantee that both \eqref{eq:inf-sup} and \eqref{eq:equality} are satisfied in the case of tensor-product B-splines (see \cite{EvHu12} for details). For hierarchical B-splines, the condition \eqref{eq:equality} is satisfied by construction, but since a set of commutative projectors is not available to prove \eqref{eq:inf-sup}, we have instead numerically computed the inf-sup constant through the solution of a discrete eigenvalue problem (see \cite{inf-sup-test}) for several mesh configurations to understand whether the resulting discretization scheme is stable or not. All the examples consider quadratic splines for pressure approximation and mixed quadratic-cubic splines for the velocity approximation.

The first set of tests regards hierarchical B\'{e}zier meshes with only two levels, and the value of the constant is compared also with the one obtained for tensor-product spaces with one single level. We have considered four different kind of refinements, similar to those already tested in Maxwell eigenproblem. For the first three, displayed in Figures~\ref{fig:mesh_min_stokes}-\ref{fig:mesh_max_stokes}, we refine several regions of $4\times4$ elements along the diagonal with different levels of overlaps between them. The fourth mesh, displayed in Figure~\ref{fig:mesh_bulge_stokes}, gives an exact sequence, but it does not satisfy Assumption~\ref{ass:support}. The properties satisfied by each of the four meshes are summarized in Table~\ref{tab:stokes_meshes}.

The results of the inf-sup test are reported in Table~\ref{tab:2levels}. All the diagonal refinements show a good behavior, even if the $2\times2$ overlap does not satisfy the exactness condition (see Figure~\ref{fig:remove-add-2x2}). In fact, we have seen in the previous tests for the Maxwell eigenproblem that the lack of exactness in this latter case only affects the ``left part'' of the diagram. On the contrary, the refinement in Figure~\ref{fig:mesh_bulge_stokes}, which does not satisfy Assumption~\ref{ass:support}, gives a discrete scheme that becomes unstable with increasing levels of mesh resolution. This suggests that {\bf \emph{Assumption~\ref{ass:support} is a necessary condition}} for inf-sup stability.

To understand whether the inf-sup constant depends on the number of levels present in the hierarchical B-spline complex, we have considered spline spaces with multiple levels in a second set of tests. We consider meshes with refinement along the diagonal as before but with an increasing number of levels.  See Figure~\ref{fig:min_4levels}-\ref{fig:max_4levels} for the resulting hierarchical B\'{e}zier meshes with four levels of refinement. The results obtained for the inf-sup constant are summarized in Table~\ref{tab:multilevel}. In this case, the discrete scheme remains stable for the $2\times 2$ and the $3 \times 3$ overlap, while the stability deteriorates for the $1\times 1$ overlap. This loss of stability is caused by the presence of adjacent elements corresponding to non-consecutive levels, and the issue can be avoided with a better grading of the mesh (see, e.g., \cite{Scott2014222}) which can be obtained using the $m$-admissible meshes defined in \cite{Buffa16-1}. To show this, we have repeated the inf-sup test for hierarchical B\'{e}zier meshes similar in appearance to Figure~\ref{fig:maxmin_4levels} where only the finest level is like in the $1\times 1$ overlap, thus avoiding non-graded meshes. The results in Table~\ref{tab:multilevel} show that in this case the scheme is stable with increasing levels of mesh resolution. It is worth to note that the loss of stability on non-graded meshes does not appear when using the generalization of Taylor-Hood elements with hierarchical splines \cite{Bressan-Juttler}, but in that case the incompressibility condition is not fulfilled exactly.  We have conducted a number of additional tests, and all of these suggest that {\bf \emph{Assumptions~\ref{ass:support} and~\ref{ass:overlap}, together with a suitable grading of the mesh, are sufficient conditions}} for inf-sup stability.  However, as demonstrated above for diagonal refinements with $2\times 2$ overlap, Assumption~\ref{ass:overlap} is not necessary for inf-sup stability.  Further study is required to develop necessary and sufficient conditions for inf-sup stability.
